Averages of $b$-hadron, $c$-hadron, and $\tau$-lepton properties as of 2023

This paper reports world averages of measurements of $b$-hadron, $c$-hadron, and $\tau$-lepton properties obtained by the Heavy Flavour Averaging Group using results available before October 2023. In rare cases, significant results obtained several months later are also used. For the averaging, common input parameters used in the various analyses are adjusted (rescaled) to common values, and known correlations are taken into account. The averages include branching fractions, lifetimes, neutral meson mixing parameters, CP violation parameters, parameters of semileptonic decays, and Cabibbo-Kobayashi-Maskawa matrix elements.

==> tau/avg-taubr-2023-elab-vadirect.tex <==
\dxQuantDef{alph}{}{}{0.0072973525693 \pm 0.0000000000011}{0.0072973525693}{0.0000000000011}
\dxQuantDef{B_tau_had_fit}{}{}{64.73 \pm 0.11}{64.73}{0.11}
\dxQuantDef{B_tau_had_uni}{}{}{64.80 \pm 0.06}{64.80}{0.06}
\dxQuantDef{B_tau_had_uni_SM}{}{}{64.86 \pm 0.05}{64.86}{0.05}
\dxQuantDef{B_tau_s_fit}{}{}{2.908 \pm 0.048}{2.908}{0.048}
\dxQuantDef{B_tau_s_unitarity}{}{}{0.0298 \pm 0.0010}{0.0298}{0.0010}
\dxQuantDef{B_tau_VA}{}{}{0.6182 \pm 0.0010}{0.6182}{0.0010}
\dxQuantDef{B_tau_VA_fit}{}{}{61.82 \pm 0.10}{61.82}{0.10}
\dxQuantDef{B_tau_VA_unitarity}{}{}{0.6189 \pm 0.0008}{0.6189}{0.0008}
\dxQuantDef{Be_by_tau_life_th}{}{}{(612.61 \pm 0.15)\cdot 10^{-6}}{612.61 \cdot 10^{-6}}{0.15 \cdot 10^{-6}}
\dxQuantDef{Be_fit}{}{}{0.1784 \pm 0.0004}{0.1784}{0.0004}
\dxQuantDef{Be_from_Bmu}{}{}{0.1785 \pm 0.0004}{0.1785}{0.0004}
\dxQuantDef{Be_from_taulife}{}{}{0.17784 \pm 0.00032}{0.17784}{0.00032}
\dxQuantDef{Be_lept}{}{}{17.845 \pm 0.032}{17.845}{0.032}
\dxQuantDef{Be_lept_unc_perc}{}{}{0.180}{0.180}{0}
\dxQuantDef{Be_unitarity}{}{}{0.1791 \pm 0.0010}{0.1791}{0.0010}
\dxQuantDef{Be_univ}{}{}{17.815 \pm 0.023}{17.815}{0.023}
\dxQuantDef{Bmu_by_Be_th}{}{}{0.9725659 \pm 0.0000026}{0.9725659}{0.0000026}
\dxQuantDef{Bmu_by_tau_life_th}{}{}{(595.81 \pm 0.15)\cdot 10^{-6}}{595.81 \cdot 10^{-6}}{0.15 \cdot 10^{-6}}
\dxQuantDef{Bmu_fit}{}{}{0.1736 \pm 0.0004}{0.1736}{0.0004}
\dxQuantDef{Bmu_from_taulife}{}{}{0.17296 \pm 0.00032}{0.17296}{0.00032}
\dxQuantDef{Bmu_unitarity}{}{}{0.1743 \pm 0.0010}{0.1743}{0.0010}
\dxQuantDef{c0}{}{}{0.30 \cdot 10^{9}}{0.30 \cdot 10^{9}}{0}
\dxQuantDef{corr_R_tau_s_R_tau_VA_pc}{}{}{-3.6}{-3.6}{0}
\dxQuantDef{deltaR_su3break}{}{}{0.239 \pm 0.032}{0.239}{0.032}
\dxQuantDef{deltaR_su3break_d2pert}{}{}{9.3 \pm 3.4}{9.3}{3.4}
\dxQuantDef{deltaR_su3break_pheno}{}{}{0.154 \pm 0.004}{0.154}{0.004}
\dxQuantDef{deltaR_su3break_remain}{}{}{0.0034 \pm 0.0028}{0.0034}{0.0028}
\dxQuantDef{dRrad_mu_e_W}{}{}{(1036.82 \pm 0.31)\cdot 10^{-9}}{1036.82 \cdot 10^{-9}}{0.31 \cdot 10^{-9}}
\dxQuantDef{dRrad_mu_gamma}{}{}{-0.004}{-0.004}{0}
\dxQuantDef{dRrad_tau_e_W}{}{}{(293.23 \pm 0.09)\cdot 10^{-6}}{293.23 \cdot 10^{-6}}{0.09 \cdot 10^{-6}}
\dxQuantDef{dRrad_tau_gamma}{}{}{-0.004}{-0.004}{0}
\dxQuantDef{dRrad_tau_K}{}{}{-0.15 \pm 0.57}{-0.15}{0.57}
\dxQuantDef{dRrad_tau_K_by_Kmu2}{}{}{0.97 \pm 0.58}{0.97}{0.58}
\dxQuantDef{dRrad_tau_K_by_tau_pi}{}{}{0.10 \pm 0.80}{0.10}{0.80}
\dxQuantDef{dRrad_tau_K_with_SEW}{}{}{1.76 \pm 0.58}{1.76}{0.58}
\dxQuantDef{dRrad_tau_mu_W}{}{}{(296.34 \pm 0.09)\cdot 10^{-6}}{296.34 \cdot 10^{-6}}{0.09 \cdot 10^{-6}}
\dxQuantDef{dRrad_tau_pi}{}{}{-0.24 \pm 0.56}{-0.24}{0.56}
\dxQuantDef{dRrad_tau_pi_by_pimu2}{}{}{0.18 \pm 0.57}{0.18}{0.57}
\dxQuantDef{dRrad_tau_pi_with_SEW}{}{}{1.67 \pm 0.57}{1.67}{0.57}
\dxQuantDef{f_Kpm}{}{}{155.7 \pm 0.3}{155.7}{0.3}
\dxQuantDef{f_Kpm_by_f_pipm}{}{}{1.1934 \pm 0.0019}{1.1934}{0.0019}
\dxQuantDef{gf}{}{}{(11663787 \pm 6)\cdot 10^{-12}}{11663787 \cdot 10^{-12}}{6 \cdot 10^{-12}}
\dxQuantDef{gmubyge_tau}{}{}{1.0002 \pm 0.0011}{1.0002}{0.0011}
\dxQuantDef{gtaubyge_tau}{}{}{1.0018 \pm 0.0014}{1.0018}{0.0014}
\dxQuantDef{gtaubygemu_tau}{}{}{1.0017 \pm 0.0013}{1.0017}{0.0013}
\dxQuantDef{gtaubygemu_tau_syst_Be_lept_perc}{}{}{0.180}{0.180}{0}
\dxQuantDef{gtaubygemu_tau_syst_tau_life_perc}{}{}{0.181}{0.181}{0}
\dxQuantDef{gtaubygemu_tau_syst_tau_mass_perc}{}{}{0.005}{0.005}{0}
\dxQuantDef{gtaubygemu_tau_unc_perc}{}{}{0.128}{0.128}{0}
\dxQuantDef{gtaubygmu_fit}{}{}{1.0011 \pm 0.0014}{1.0011}{0.0014}
\dxQuantDef{gtaubygmu_K}{}{}{0.986 \pm 0.008}{0.986}{0.008}
\dxQuantDef{gtaubygmu_pi}{}{}{0.996 \pm 0.004}{0.996}{0.004}
\dxQuantDef{gtaubygmu_piK_fit}{}{}{0.9939 \pm 0.0035}{0.9939}{0.0035}
\dxQuantDef{gtaubygmu_tau}{}{}{1.0016 \pm 0.0014}{1.0016}{0.0014}
\dxQuantDef{hbarev}{}{}{0.7 \cdot 10^{-15}}{0.7 \cdot 10^{-15}}{0}
\dxQuantDef{K_life}{}{}{(12380 \pm 20)\cdot 10^{-12}}{12380 \cdot 10^{-12}}{20 \cdot 10^{-12}}
\dxQuantDef{K_mass}{}{}{493.677 \pm 0.016}{493.677}{0.016}
\dxQuantDef{KtoENu}{}{}{(15.82 \pm 0.07)\cdot 10^{-6}}{15.82 \cdot 10^{-6}}{0.07 \cdot 10^{-6}}
\dxQuantDef{KtoMuNu}{}{}{0.6356 \pm 0.0011}{0.6356}{0.0011}
\dxQuantDef{m_s}{}{}{93 \pm 7}{93}{7}
\dxQuantDef{m_W}{}{}{80379 \pm 12}{80379}{12}
\dxQuantDef{mec2mev}{}{}{0.51099895000 \pm 0.00000000015}{0.51099895000}{0.00000000015}
\dxQuantDef{mmuc2mev}{}{}{105.6583755 \pm 0.0000023}{105.6583755}{0.0000023}
\dxQuantDef{mu_life}{}{}{(2196981.1 \pm 2.2)\cdot 10^{-12}}{2196981.1 \cdot 10^{-12}}{2.2 \cdot 10^{-12}}
\dxQuantDef{phspf_mebymmu}{}{}{0.999812949172 \pm 0.000000000008}{0.999812949172}{0.000000000008}
\dxQuantDef{phspf_mebymtau}{}{}{0.99999933841 \pm 0.00000000006}{0.99999933841}{0.00000000006}
\dxQuantDef{phspf_mmubymtau}{}{}{0.9725622 \pm 0.0000026}{0.9725622}{0.0000026}
\dxQuantDef{pi_life}{}{}{(26033 \pm 5)\cdot 10^{-12}}{26033 \cdot 10^{-12}}{5 \cdot 10^{-12}}
\dxQuantDef{pi_mass}{}{}{139.57039 \pm 0.00018}{139.57039}{0.00018}
\dxQuantDef{pitoENu}{}{}{(123.0 \pm 0.4)\cdot 10^{-6}}{123.0 \cdot 10^{-6}}{0.4 \cdot 10^{-6}}
\dxQuantDef{pitoMuNu}{}{}{0.9998770 \pm 0.0000004}{0.9998770}{0.0000004}
\dxQuantDef{R_tau}{}{}{3.634 \pm 0.008}{3.634}{0.008}
\dxQuantDef{R_tau_leptonly}{}{}{3.637 \pm 0.008}{3.637}{0.008}
\dxQuantDef{R_tau_leptuniv}{}{}{3.641 \pm 0.007}{3.641}{0.007}
\dxQuantDef{R_tau_s}{}{}{0.1632 \pm 0.0027}{0.1632}{0.0027}
\dxQuantDef{R_tau_uni}{}{}{3.637 \pm 0.008}{3.637}{0.008}
\dxQuantDef{R_tau_uni_SM}{}{}{3.641 \pm 0.007}{3.641}{0.007}
\dxQuantDef{R_tau_us_by_Vus_sq}{}{}{3.407 \pm 0.022}{3.407}{0.022}
\dxQuantDef{R_tau_VA}{}{}{3.470 \pm 0.008}{3.470}{0.008}
\dxQuantDef{S_EW_R_tau_h}{}{}{1.02350 \pm 0.00030}{1.02350}{0.00030}
\dxQuantDef{S_EW_tau_h}{}{}{1.01910 \pm 0.00030}{1.01910}{0.00030}
\dxQuantDef{S_EW_tau_sub_had}{}{}{0.9967}{0.9967}{0}
\dxQuantDef{S_EW_tau_sub_lep}{}{}{0.9957}{0.9957}{0}
\dxQuantDef{tau_life_unc_perc}{}{}{0.181}{0.181}{0}
\dxQuantDef{tau_mass_unc_perc}{}{}{0.005}{0.005}{0}
\dxQuantDef{Vub}{}{}{0.00382 \pm 0.00020}{0.00382}{0.00020}
\dxQuantDef{Vud}{}{}{0.97384 \pm 0.00026}{0.97384}{0.00026}
\dxQuantDef{Vus_by_Vud_Kl2}{}{}{0.2311 \pm 0.0005}{0.2311}{0.0005}
\dxQuantDef{Vus_by_Vud_tau_K_by_tau_pi}{}{}{0.2289 \pm 0.0019}{0.2289}{0.0019}
\dxQuantDef{Vus_by_Vud_tau_K_by_tau_pi_stat}{}{}{0.0016}{0.0016}{0}
\dxQuantDef{Vus_by_Vud_tau_K_by_tau_pi_syst}{}{}{0.0010}{0.0010}{0}
\dxQuantDef{Vus_by_Vud_tau_Xs}{}{}{0.2243 \pm 0.0022}{0.2243}{0.0022}
\dxQuantDef{Vus_by_Vud_tau_Xs_latt_incl}{}{}{0.2248 \pm 0.0020}{0.2248}{0.0020}
\dxQuantDef{Vus_by_Vud_tau_Xs_latt_incl_stat}{}{}{0.0018}{0.0018}{0}
\dxQuantDef{Vus_by_Vud_tau_Xs_latt_incl_syst}{}{}{0.7 \cdot 10^{-3}}{0.7 \cdot 10^{-3}}{0}
\dxQuantDef{Vus_by_Vud_tau_Xs_latt_incl_unc_perc}{}{}{0.9}{0.9}{0}
\dxQuantDef{Vus_by_Vud_tau_Xs_stat}{}{}{0.0019}{0.0019}{0}
\dxQuantDef{Vus_by_Vud_tau_Xs_syst}{}{}{0.0011}{0.0011}{0}
\dxQuantDef{Vus_by_Vud_tau_Xs_unc_perc}{}{}{1.0}{1.0}{0}
\dxQuantDef{Vus_Kl2}{}{}{0.2250 \pm 0.0005}{0.2250}{0.0005}
\dxQuantDef{Vus_Kl2_mism}{}{}{-0.0022 \pm 0.0013}{-0.0022}{0.0013}
\dxQuantDef{Vus_Kl2_mism_sigma}{}{}{-1.7}{-1.7}{0}
\dxQuantDef{Vus_Kl2_mism_sigma_abs}{}{}{1.7}{1.7}{0}
\dxQuantDef{Vus_Kl3}{}{}{0.2233 \pm 0.0005}{0.2233}{0.0005}
\dxQuantDef{Vus_Kl3_mism}{}{}{-0.0039 \pm 0.0012}{-0.0039}{0.0012}
\dxQuantDef{Vus_Kl3_mism_sigma}{}{}{-3.2}{-3.2}{0}
\dxQuantDef{Vus_Kl3_mism_sigma_abs}{}{}{3.2}{3.2}{0}
\dxQuantDef{Vus_tau}{}{}{0.2208 \pm 0.0014}{0.2208}{0.0014}
\dxQuantDef{Vus_tau_excl}{}{}{0.2225 \pm 0.0017}{0.2225}{0.0017}
\dxQuantDef{Vus_tau_excl_mism}{}{}{-0.0047 \pm 0.0021}{-0.0047}{0.0021}
\dxQuantDef{Vus_tau_excl_mism_sigma}{}{}{-2.3}{-2.3}{0}
\dxQuantDef{Vus_tau_excl_mism_sigma_abs}{}{}{2.3}{2.3}{0}
\dxQuantDef{Vus_tau_excl_stat}{}{}{0.0015}{0.0015}{0}
\dxQuantDef{Vus_tau_excl_syst}{}{}{0.8 \cdot 10^{-3}}{0.8 \cdot 10^{-3}}{0}
\dxQuantDef{Vus_tau_K}{}{}{0.2224 \pm 0.0017}{0.2224}{0.0017}
\dxQuantDef{Vus_tau_K_by_tau_pi}{}{}{0.2229 \pm 0.0019}{0.2229}{0.0019}
\dxQuantDef{Vus_tau_K_by_tau_pi_mism}{}{}{-0.0043 \pm 0.0022}{-0.0043}{0.0022}
\dxQuantDef{Vus_tau_K_by_tau_pi_mism_sigma}{}{}{-2.0}{-2.0}{0}
\dxQuantDef{Vus_tau_K_by_tau_pi_mism_sigma_abs}{}{}{2.0}{2.0}{0}
\dxQuantDef{Vus_tau_K_by_tau_pi_stat}{}{}{0.0016}{0.0016}{0}
\dxQuantDef{Vus_tau_K_by_tau_pi_syst}{}{}{0.0010}{0.0010}{0}
\dxQuantDef{Vus_tau_K_by_tau_pi_unc_perc}{}{}{0.8}{0.8}{0}
\dxQuantDef{Vus_tau_K_by_tau_pi_unc_th_perc}{}{}{0.4}{0.4}{0}
\dxQuantDef{Vus_tau_K_by_tau_pi_unc_th_perc_dRrad_tau_K_by_tau_pi}{}{}{0.4}{0.4}{0}
\dxQuantDef{Vus_tau_K_by_tau_pi_unc_th_perc_f_Kpm_by_f_pipm}{}{}{0.16}{0.16}{0}
\dxQuantDef{Vus_tau_K_mism}{}{}{-0.0048 \pm 0.0021}{-0.0048}{0.0021}
\dxQuantDef{Vus_tau_K_mism_sigma}{}{}{-2.3}{-2.3}{0}
\dxQuantDef{Vus_tau_K_mism_sigma_abs}{}{}{2.3}{2.3}{0}
\dxQuantDef{Vus_tau_K_stat}{}{}{0.0016}{0.0016}{0}
\dxQuantDef{Vus_tau_K_syst}{}{}{0.8 \cdot 10^{-3}}{0.8 \cdot 10^{-3}}{0}
\dxQuantDef{Vus_tau_K_unc_perc}{}{}{0.8}{0.8}{0}
\dxQuantDef{Vus_tau_K_unc_th_perc}{}{}{0.34}{0.34}{0}
\dxQuantDef{Vus_tau_K_unc_th_perc_dRrad_tau_K}{}{}{0.29}{0.29}{0}
\dxQuantDef{Vus_tau_K_unc_th_perc_f_Kpm}{}{}{0.19}{0.19}{0}
\dxQuantDef{Vus_tau_K_unc_th_perc_S_EW_tau_h}{}{}{0.015}{0.015}{0}
\dxQuantDef{Vus_tau_mism}{}{}{-0.0064 \pm 0.0018}{-0.0064}{0.0018}
\dxQuantDef{Vus_tau_mism_sigma}{}{}{-3.6}{-3.6}{0}
\dxQuantDef{Vus_tau_mism_sigma_abs}{}{}{3.6}{3.6}{0}
\dxQuantDef{Vus_tau_stat}{}{}{0.0013}{0.0013}{0}
\dxQuantDef{Vus_tau_syst}{}{}{0.0005}{0.0005}{0}
\dxQuantDef{Vus_tau_Xs}{}{}{0.2184 \pm 0.0021}{0.2184}{0.0021}
\dxQuantDef{Vus_tau_Xs_latt_incl}{}{}{0.2189 \pm 0.0019}{0.2189}{0.0019}
\dxQuantDef{Vus_tau_Xs_latt_incl_mism}{}{}{-0.0083 \pm 0.0022}{-0.0083}{0.0022}
\dxQuantDef{Vus_tau_Xs_latt_incl_mism_sigma}{}{}{-3.7}{-3.7}{0}
\dxQuantDef{Vus_tau_Xs_latt_incl_mism_sigma_abs}{}{}{3.7}{3.7}{0}
\dxQuantDef{Vus_tau_Xs_latt_incl_stat}{}{}{0.0018}{0.0018}{0}
\dxQuantDef{Vus_tau_Xs_latt_incl_syst}{}{}{0.7 \cdot 10^{-3}}{0.7 \cdot 10^{-3}}{0}
\dxQuantDef{Vus_tau_Xs_mism}{}{}{-0.0088 \pm 0.0024}{-0.0088}{0.0024}
\dxQuantDef{Vus_tau_Xs_mism_sigma}{}{}{-3.6}{-3.6}{0}
\dxQuantDef{Vus_tau_Xs_mism_sigma_abs}{}{}{3.6}{3.6}{0}
\dxQuantDef{Vus_tau_Xs_stat}{}{}{0.0018}{0.0018}{0}
\dxQuantDef{Vus_tau_Xs_syst}{}{}{0.0010}{0.0010}{0}
\dxQuantDef{Vus_tau_Xs_unc_exp}{}{}{0.0018}{0.0018}{0}
\dxQuantDef{Vus_tau_Xs_unc_exp_perc}{}{}{0.8}{0.8}{0}
\dxQuantDef{Vus_tau_Xs_unc_perc}{}{}{1.0}{1.0}{0}
\dxQuantDef{Vus_tau_Xs_unc_th}{}{}{0.0010}{0.0010}{0}
\dxQuantDef{Vus_tau_Xs_unc_th_perc}{}{}{0.47}{0.47}{0}
\dxQuantDef{Vus_tau2}{}{}{0.2210 \pm 0.0015}{0.2210}{0.0015}
\dxQuantDef{Vus_tau2_mism}{}{}{-0.0062 \pm 0.0019}{-0.0062}{0.0019}
\dxQuantDef{Vus_tau2_mism_sigma}{}{}{-3.3}{-3.3}{0}
\dxQuantDef{Vus_tau2_mism_sigma_abs}{}{}{3.3}{3.3}{0}
\dxQuantDef{Vus_uni}{}{}{0.2272 \pm 0.0011}{0.2272}{0.0011}
\dxQuantDef{gmubyge_tau_ed}{}{}{1.00024 \pm 0.00114}{1.00024}{0.00114}
\dxQuantDef{gtaubyge_tau_ed}{}{}{1.00185 \pm 0.00140}{1.00185}{0.00140}
\dxQuantDef{gtaubygmu_tau_ed}{}{}{1.00160 \pm 0.00141}{1.00160}{0.00141}
\dxQuantDef{gtaubygemu_tau_ed}{}{}{1.00172 \pm 0.00128}{1.00172}{0.00128}
\dxQuantDef{gtaubygmu_fit_ed}{}{}{1.00106 \pm 0.00138}{1.00106}{0.00138}
\dxQuantDef{gtaubygmu_K_ed}{}{}{0.9856 \pm 0.0075}{0.9856}{0.0075}
\dxQuantDef{gtaubygmu_pi_ed}{}{}{0.9958 \pm 0.0038}{0.9958}{0.0038}
\dxQuantDef{gtaubygmu_piK_fit_ed}{}{}{0.99386 \pm 0.00351}{0.99386}{0.00351}
\dxdef{g_ratios_corr}{%
$\displaystyle\left( \frac{g_\tau}{g_e} \right)_\tau$ &   67\\
$\displaystyle\left( \frac{g_\mu}{g_e} \right)_\tau$ &  -41 &   40\\
$\displaystyle\left( \frac{g_\tau}{g_\mu} \right)_\pi$ &   18 &   19 &    1\\
$\displaystyle\left( \frac{g_\tau}{g_\mu} \right)_K$ &   12 &   12 &   -1 &    7\\
 & $\displaystyle\left( \frac{g_\tau}{g_\mu} \right)_\tau$ & $\displaystyle\left( \frac{g_\tau}{g_e} \right)_\tau$ & $\displaystyle\left( \frac{g_\mu}{g_e} \right)_\tau$ & $\displaystyle\left( \frac{g_\tau}{g_\mu} \right)_\pi$%
}


==> tau/avg-taubr-2023-uc.tex <==
\dxdef{TauBrMeasNum}{171}
\dxdef{TauBrMeasNumAll}{172}
\dxdef{TauBrMeasNumNuisance}{1}
\dxdef{TauBrQuantNum}{136}
\dxdef{TauBrQuantNumAll}{137}
\dxdef{TauBrQuantNumNuisance}{1}
\dxdef{TauBrBaseQuantNum}{47}
\dxdef{TauBrBaseVarNum}{46}
\dxdef{TauBrConstrNum}{91}
\dxdef{TauBrChisq}{138}
\dxdef{TauBrDof}{126}
\dxdef{TauBrChisqProb}{21.3\%}
\dxdef{TauBrChisq_full}{138}
\dxdef{TauBrDof_full}{126}
\dxdef{TauBrChisqProb_full}{21.3\%}
\dxdef{TauBrUnitarityQuantNum}{47}
\dxdef{TauBrPdgQuantNum}{129}
\dxdef{TauBrPdgQuantNumNonRatio}{112}
\dxdef{TauBrPdgQuantNumRatio}{17}
\dxdef{TauBrPdgQuantNumWithMeas}{85}
\dxdef{TauBrPdgQuantNumNonRatioWithMeas}{72}
\dxdef{TauBrPdgQuantNumRatioWithMeas}{13}
\dxdef{TauBrPdgConstrNum}{84}
\dxdef{TauBrNumMeasALEPH}{39}
\dxdef{TauBrNumMeasARGUS}{2}
\dxdef{TauBrNumMeasBaBar}{24}
\dxdef{TauBrNumMeasBelle}{15}
\dxdef{TauBrNumMeasBelle2}{1}
\dxdef{TauBrNumMeasCELLO}{1}
\dxdef{TauBrNumMeasCLEO}{35}
\dxdef{TauBrNumMeasCLEO3}{6}
\dxdef{TauBrNumMeasDELPHI}{14}
\dxdef{TauBrNumMeasHRS}{2}
\dxdef{TauBrNumMeasL3}{11}
\dxdef{TauBrNumMeasOPAL}{19}
\dxdef{TauBrNumMeasTPC}{3}
\dxQuantDef{Gamma1}{\BR_{1}}{\BR(\tau^- \to \text{particle}^- \ge{} 0\, \text{neutrals} \ge{} 0\,  K^0\, \nu_\tau)}{0.8524 \pm 0.0006}{0.8524}{\pm 0.0006}
\dxQuantDef{Gamma2}{\BR_{2}}{\BR(\tau^- \to \text{particle}^- \ge{} 0\, \text{neutrals} \ge{} 0\,  K_L^0\, \nu_\tau)}{0.8458 \pm 0.0006}{0.8458}{\pm 0.0006}
\dxQuantDef{Gamma3}{\BR_{3}}{\BR(\tau^- \to \mu^- \bar{\nu}_\mu \nu_\tau)}{0.17366 \pm 0.00036}{0.17366}{\pm 0.00036}
\dxMeasDef{ALEPH.Gamma3.pub.SCHAEL.05C}{Gamma3}{SCHAEL 05C}{0.17319 \pm 0.00070 \pm 0.00032}{0.17319}{\pm 0.00070}{\pm 0.00032}
\dxMeasDef{DELPHI.Gamma3.pub.ABREU.99X}{Gamma3}{ABREU 99X}{0.17325 \pm 0.00095 \pm 0.00077}{0.17325}{\pm 0.00095}{\pm 0.00077}
\dxMeasDef{L3.Gamma3.pub.ACCIARRI.01F}{Gamma3}{ACCIARRI 01F}{0.17342 \pm 0.00110 \pm 0.00067}{0.17342}{\pm 0.00110}{\pm 0.00067}
\dxMeasDef{OPAL.Gamma3.pub.ABBIENDI.03}{Gamma3}{ABBIENDI 03}{0.17340 \pm 0.00090 \pm 0.00060}{0.17340}{\pm 0.00090}{\pm 0.00060}
\dxQuantDef{Gamma3by5}{\BR_{3 / 5}}{\frac{\BR(\tau^- \to \mu^- \bar{\nu}_\mu \nu_\tau)}{\BR(\tau^- \to e^- \bar{\nu}_e \nu_\tau)}}{0.9730 \pm 0.0022}{0.9730}{\pm 0.0022}
\dxMeasDef{ARGUS.Gamma3by5.pub.ALBRECHT.92D}{Gamma3by5}{ALBRECHT 92D}{0.9970 \pm 0.0350 \pm 0.0400}{0.9970}{\pm 0.0350}{\pm 0.0400}
\dxMeasDef{BaBar.Gamma3by5.pub.AUBERT.10F}{Gamma3by5}{AUBERT 10F}{0.9796 \pm 0.0016 \pm 0.0036}{0.9796}{\pm 0.0016}{\pm 0.0036}
\dxMeasDef{Belle2.Gamma3by5.ADACHI.2024}{Gamma3by5}{Belle2 ADACHI 2024}{0.9675 \pm 0.0007 \pm 0.0036}{0.9675}{\pm 0.0007}{\pm 0.0036}
\dxMeasDef{CLEO.Gamma3by5.pub.ANASTASSOV.97}{Gamma3by5}{ANASTASSOV 97}{0.9777 \pm 0.0063 \pm 0.0087}{0.9777}{\pm 0.0063}{\pm 0.0087}
\dxQuantDef{Gamma5}{\BR_{5}}{\BR(\tau^- \to e^- \bar{\nu}_e \nu_\tau)}{0.1785 \pm 0.0004}{0.1785}{\pm 0.0004}
\dxMeasDef{ALEPH.Gamma5.pub.SCHAEL.05C}{Gamma5}{SCHAEL 05C}{0.1784 \pm 0.0007 \pm 0.0004}{0.1784}{\pm 0.0007}{\pm 0.0004}
\dxMeasDef{CLEO.Gamma5.pub.ANASTASSOV.97}{Gamma5}{ANASTASSOV 97}{0.1776 \pm 0.0006 \pm 0.0017}{0.1776}{\pm 0.0006}{\pm 0.0017}
\dxMeasDef{DELPHI.Gamma5.pub.ABREU.99X}{Gamma5}{ABREU 99X}{0.1788 \pm 0.0011 \pm 0.0011}{0.1788}{\pm 0.0011}{\pm 0.0011}
\dxMeasDef{L3.Gamma5.pub.ACCIARRI.01F}{Gamma5}{ACCIARRI 01F}{0.1781 \pm 0.0010 \pm 0.0008}{0.1781}{\pm 0.0010}{\pm 0.0008}
\dxMeasDef{OPAL.Gamma5.pub.ABBIENDI.99H}{Gamma5}{ABBIENDI 99H}{0.1781 \pm 0.0009 \pm 0.0006}{0.1781}{\pm 0.0009}{\pm 0.0006}
\dxQuantDef{Gamma7}{\BR_{7}}{\BR(\tau^- \to h^- \ge{} 0\,  K_L^0\, \nu_\tau)}{0.1203 \pm 0.0005}{0.1203}{\pm 0.0005}
\dxMeasDef{DELPHI.Gamma7.pub.ABREU.92N}{Gamma7}{ABREU 92N}{0.1240 \pm 0.0070 \pm 0.0070}{0.1240}{\pm 0.0070}{\pm 0.0070}
\dxMeasDef{L3.Gamma7.pub.ACCIARRI.95}{Gamma7}{ACCIARRI 95}{0.1247 \pm 0.0026 \pm 0.0043}{0.1247}{\pm 0.0026}{\pm 0.0043}
\dxMeasDef{OPAL.Gamma7.pub.ALEXANDER.91D}{Gamma7}{ALEXANDER 91D}{0.1210 \pm 0.0070 \pm 0.0050}{0.1210}{\pm 0.0070}{\pm 0.0050}
\dxQuantDef{Gamma8}{\BR_{8}}{\BR(\tau^- \to h^- \nu_\tau)}{0.1151 \pm 0.0005}{0.1151}{\pm 0.0005}
\dxMeasDef{CLEO.Gamma8.pub.ANASTASSOV.97}{Gamma8}{ANASTASSOV 97}{0.1152 \pm 0.0005 \pm 0.0012}{0.1152}{\pm 0.0005}{\pm 0.0012}
\dxMeasDef{DELPHI.Gamma8.pub.ABDALLAH.06A}{Gamma8}{ABDALLAH 06A}{0.1157 \pm 0.0012 \pm 0.0011}{0.1157}{\pm 0.0012}{\pm 0.0011}
\dxMeasDef{OPAL.Gamma8.pub.ACKERSTAFF.98M}{Gamma8}{ACKERSTAFF 98M}{0.1198 \pm 0.0013 \pm 0.0016}{0.1198}{\pm 0.0013}{\pm 0.0016}
\dxQuantDef{Gamma8by5}{\BR_{8 / 5}}{\frac{\BR(\tau^- \to h^- \nu_\tau)}{\BR(\tau^- \to e^- \bar{\nu}_e \nu_\tau)}}{0.6450 \pm 0.0032}{0.6450}{\pm 0.0032}
\dxQuantDef{Gamma9}{\BR_{9}}{\BR(\tau^- \to \pi^- \nu_\tau)}{0.1082 \pm 0.0005}{0.1082}{\pm 0.0005}
\dxMeasDef{ALEPH.Gamma9.pub.SCHAEL.05C}{Gamma9}{SCHAEL 05C}{0.1083 \pm 0.0007 \pm 0.0008}{0.1083}{\pm 0.0007}{\pm 0.0008}
\dxQuantDef{Gamma9by5}{\BR_{9 / 5}}{\frac{\BR(\tau^- \to \pi^- \nu_\tau)}{\BR(\tau^- \to e^- \bar{\nu}_e \nu_\tau)}}{0.6060 \pm 0.0031}{0.6060}{\pm 0.0031}
\dxMeasDef{BaBar.Gamma9by5.pub.AUBERT.10F}{Gamma9by5}{AUBERT 10F}{0.5945 \pm 0.0014 \pm 0.0061}{0.5945}{\pm 0.0014}{\pm 0.0061}
\dxQuantDef{Gamma10}{\BR_{10}}{\BR(\tau^- \to K^- \nu_\tau)}{0.00697 \pm 0.00010}{0.00697}{\pm 0.00010}
\dxMeasDef{ALEPH.Gamma10.pub.BARATE.99K}{Gamma10}{BARATE 99K}{0.00696 \pm 0.00025 \pm 0.00014}{0.00696}{\pm 0.00025}{\pm 0.00014}
\dxMeasDef{CLEO.Gamma10.pub.BATTLE.94}{Gamma10}{BATTLE 94}{0.00660 \pm 0.00070 \pm 0.00090}{0.00660}{\pm 0.00070}{\pm 0.00090}
\dxMeasDef{DELPHI.Gamma10.pub.ABREU.94K}{Gamma10}{ABREU 94K}{0.00850 \pm 0.00180 \pm 0.00000}{0.00850}{\pm 0.00180}{\pm 0.00000}
\dxMeasDef{OPAL.Gamma10.pub.ABBIENDI.01J}{Gamma10}{ABBIENDI 01J}{0.00658 \pm 0.00027 \pm 0.00029}{0.00658}{\pm 0.00027}{\pm 0.00029}
\dxQuantDef{Gamma10by5}{\BR_{10 / 5}}{\frac{\BR(\tau^- \to K^- \nu_\tau)}{\BR(\tau^- \to e^- \bar{\nu}_e \nu_\tau)}}{0.03903 \pm 0.00054}{0.03903}{\pm 0.00054}
\dxMeasDef{BaBar.Gamma10by5.pub.AUBERT.10F}{Gamma10by5}{AUBERT 10F}{0.03882 \pm 0.00032 \pm 0.00057}{0.03882}{\pm 0.00032}{\pm 0.00057}
\dxQuantDef{Gamma10by9}{\BR_{10 / 9}}{\frac{\BR(\tau^- \to K^- \nu_\tau)}{\BR(\tau^- \to \pi^- \nu_\tau)}}{0.0644 \pm 0.0009}{0.0644}{\pm 0.0009}
\dxQuantDef{Gamma11}{\BR_{11}}{\BR(\tau^- \to h^- \ge{} 1\,  \text{neutrals}\, \nu_\tau)}{0.3700 \pm 0.0009}{0.3700}{\pm 0.0009}
\dxQuantDef{Gamma12}{\BR_{12}}{\BR(\tau^- \to h^- \ge{} 1\, \pi^0\, \nu_\tau\;(\text{ex.}K^0))}{0.3650 \pm 0.0009}{0.3650}{\pm 0.0009}
\dxQuantDef{Gamma13}{\BR_{13}}{\BR(\tau^- \to h^- \pi^0 \nu_\tau)}{0.25926 \pm 0.00089}{0.25926}{\pm 0.00089}
\dxMeasDef{Belle.Gamma13.pub.FUJIKAWA.08}{Gamma13}{FUJIKAWA 08}{0.25670 \pm 0.00010 \pm 0.00390}{0.25670}{\pm 0.00010}{\pm 0.00390}
\dxMeasDef{CLEO.Gamma13.pub.ARTUSO.94}{Gamma13}{ARTUSO 94}{0.25870 \pm 0.00120 \pm 0.00420}{0.25870}{\pm 0.00120}{\pm 0.00420}
\dxMeasDef{DELPHI.Gamma13.pub.ABDALLAH.06A}{Gamma13}{ABDALLAH 06A}{0.25740 \pm 0.00201 \pm 0.00138}{0.25740}{\pm 0.00201}{\pm 0.00138}
\dxMeasDef{L3.Gamma13.pub.ACCIARRI.95}{Gamma13}{ACCIARRI 95}{0.25050 \pm 0.00350 \pm 0.00500}{0.25050}{\pm 0.00350}{\pm 0.00500}
\dxMeasDef{OPAL.Gamma13.pub.ACKERSTAFF.98M}{Gamma13}{ACKERSTAFF 98M}{0.25890 \pm 0.00170 \pm 0.00290}{0.25890}{\pm 0.00170}{\pm 0.00290}
\dxQuantDef{Gamma14}{\BR_{14}}{\BR(\tau^- \to \pi^- \pi^0 \nu_\tau)}{0.2549 \pm 0.0009}{0.2549}{\pm 0.0009}
\dxMeasDef{ALEPH.Gamma14.pub.SCHAEL.05C}{Gamma14}{SCHAEL 05C}{0.2547 \pm 0.0010 \pm 0.0008}{0.2547}{\pm 0.0010}{\pm 0.0008}
\dxQuantDef{Gamma16}{\BR_{16}}{\BR(\tau^- \to K^- \pi^0 \nu_\tau)}{0.004328 \pm 0.000148}{0.004328}{\pm 0.000148}
\dxMeasDef{ALEPH.Gamma16.pub.BARATE.99K}{Gamma16}{BARATE 99K}{0.004440 \pm 0.000260 \pm 0.000240}{0.004440}{\pm 0.000260}{\pm 0.000240}
\dxMeasDef{BaBar.Gamma16.pub.AUBERT.07AP}{Gamma16}{AUBERT 07AP}{0.004160 \pm 0.000030 \pm 0.000180}{0.004160}{\pm 0.000030}{\pm 0.000180}
\dxMeasDef{CLEO.Gamma16.pub.BATTLE.94}{Gamma16}{BATTLE 94}{0.005100 \pm 0.001000 \pm 0.000700}{0.005100}{\pm 0.001000}{\pm 0.000700}
\dxMeasDef{OPAL.Gamma16.pub.ABBIENDI.04J}{Gamma16}{ABBIENDI 04J}{0.004710 \pm 0.000590 \pm 0.000230}{0.004710}{\pm 0.000590}{\pm 0.000230}
\dxQuantDef{Gamma17}{\BR_{17}}{\BR(\tau^- \to h^- \ge{} 2\,  \pi^0\, \nu_\tau)}{0.1081 \pm 0.0009}{0.1081}{\pm 0.0009}
\dxMeasDef{OPAL.Gamma17.pub.ACKERSTAFF.98M}{Gamma17}{ACKERSTAFF 98M}{0.0991 \pm 0.0031 \pm 0.0027}{0.0991}{\pm 0.0031}{\pm 0.0027}
\dxQuantDef{Gamma18}{\BR_{18}}{\BR(\tau^- \to h^- 2\pi^0 \nu_\tau)}{0.0948 \pm 0.0010}{0.0948}{\pm 0.0010}
\dxQuantDef{Gamma19}{\BR_{19}}{\BR(\tau^- \to h^- 2\pi^0 \nu_\tau\;(\text{ex.}K^0))}{0.0932 \pm 0.0010}{0.0932}{\pm 0.0010}
\dxMeasDef{DELPHI.Gamma19.pub.ABDALLAH.06A}{Gamma19}{ABDALLAH 06A}{0.0950 \pm 0.0032 \pm 0.0027}{0.0950}{\pm 0.0032}{\pm 0.0027}
\dxMeasDef{L3.Gamma19.pub.ACCIARRI.95}{Gamma19}{ACCIARRI 95}{0.0888 \pm 0.0037 \pm 0.0042}{0.0888}{\pm 0.0037}{\pm 0.0042}
\dxQuantDef{Gamma19by13}{\BR_{19 / 13}}{\frac{\BR(\tau^- \to h^- 2\pi^0 \nu_\tau\;(\text{ex.}K^0))}{\BR(\tau^- \to h^- \pi^0 \nu_\tau)}}{0.360 \pm 0.004}{0.360}{\pm 0.004}
\dxMeasDef{CLEO.Gamma19by13.pub.PROCARIO.93}{Gamma19by13}{PROCARIO 93}{0.342 \pm 0.006 \pm 0.016}{0.342}{\pm 0.006}{\pm 0.016}
\dxQuantDef{Gamma20}{\BR_{20}}{\BR(\tau^- \to \pi^- 2\pi^0 \nu_\tau\;(\text{ex.}K^0))}{0.0926 \pm 0.0010}{0.0926}{\pm 0.0010}
\dxMeasDef{ALEPH.Gamma20.pub.SCHAEL.05C}{Gamma20}{SCHAEL 05C}{0.0924 \pm 0.0009 \pm 0.0009}{0.0924}{\pm 0.0009}{\pm 0.0009}
\dxQuantDef{Gamma23}{\BR_{23}}{\BR(\tau^- \to K^- 2\pi^0 \nu_\tau\;(\text{ex.}K^0))}{0.00065 \pm 0.00022}{0.00065}{\pm 0.00022}
\dxMeasDef{ALEPH.Gamma23.pub.BARATE.99K}{Gamma23}{BARATE 99K}{0.00056 \pm 0.00020 \pm 0.00015}{0.00056}{\pm 0.00020}{\pm 0.00015}
\dxMeasDef{CLEO.Gamma23.pub.BATTLE.94}{Gamma23}{BATTLE 94}{0.00090 \pm 0.00100 \pm 0.00030}{0.00090}{\pm 0.00100}{\pm 0.00030}
\dxQuantDef{Gamma24}{\BR_{24}}{\BR(\tau^- \to h^- \ge{} 3\, \pi^0\, \nu_\tau)}{0.0134 \pm 0.0007}{0.0134}{\pm 0.0007}
\dxQuantDef{Gamma25}{\BR_{25}}{\BR(\tau^- \to h^- \ge{} 3\, \pi^0\, \nu_\tau\;(\text{ex.}K^0))}{0.0126 \pm 0.0007}{0.0126}{\pm 0.0007}
\dxMeasDef{DELPHI.Gamma25.pub.ABDALLAH.06A}{Gamma25}{ABDALLAH 06A}{0.0140 \pm 0.0021 \pm 0.0022}{0.0140}{\pm 0.0021}{\pm 0.0022}
\dxQuantDef{Gamma26}{\BR_{26}}{\BR(\tau^- \to h^- 3\pi^0 \nu_\tau)}{0.0118 \pm 0.0007}{0.0118}{\pm 0.0007}
\dxMeasDef{L3.Gamma26.pub.ACCIARRI.95}{Gamma26}{ACCIARRI 95}{0.0170 \pm 0.0024 \pm 0.0038}{0.0170}{\pm 0.0024}{\pm 0.0038}
\dxQuantDef{Gamma26by13}{\BR_{26 / 13}}{\frac{\BR(\tau^- \to h^- 3\pi^0 \nu_\tau)}{\BR(\tau^- \to h^- \pi^0 \nu_\tau)}}{0.0454 \pm 0.0028}{0.0454}{\pm 0.0028}
\dxMeasDef{CLEO.Gamma26by13.pub.PROCARIO.93}{Gamma26by13}{PROCARIO 93}{0.0440 \pm 0.0030 \pm 0.0050}{0.0440}{\pm 0.0030}{\pm 0.0050}
\dxQuantDef{Gamma27}{\BR_{27}}{\BR(\tau^- \to \pi^- 3\pi^0 \nu_\tau\;(\text{ex.}K^0))}{0.0104 \pm 0.0007}{0.0104}{\pm 0.0007}
\dxMeasDef{ALEPH.Gamma27.pub.SCHAEL.05C}{Gamma27}{SCHAEL 05C}{0.0098 \pm 0.0007 \pm 0.0006}{0.0098}{\pm 0.0007}{\pm 0.0006}
\dxQuantDef{Gamma28}{\BR_{28}}{\BR(\tau^- \to K^- 3\pi^0 \nu_\tau\;(\text{ex.}K^0,\eta))}{(0.48 \pm 0.21)\cdot 10^{-3}}{0.48 \cdot 10^{-3}}{\pm 0.21 \cdot 10^{-3}}
\dxMeasDef{ALEPH.Gamma28.pub.BARATE.99K}{Gamma28}{BARATE 99K}{(0.37 \pm 0.21 \pm 0.11)\cdot 10^{-3}}{0.37 \cdot 10^{-3}}{\pm 0.21 \cdot 10^{-3}}{\pm 0.11 \cdot 10^{-3}}
\dxQuantDef{Gamma29}{\BR_{29}}{\BR(\tau^- \to h^- 4\pi^0 \nu_\tau\;(\text{ex.}K^0))}{0.0016 \pm 0.0004}{0.0016}{\pm 0.0004}
\dxMeasDef{CLEO.Gamma29.pub.PROCARIO.93}{Gamma29}{PROCARIO 93}{0.0016 \pm 0.0005 \pm 0.0005}{0.0016}{\pm 0.0005}{\pm 0.0005}
\dxQuantDef{Gamma30}{\BR_{30}}{\BR(\tau^- \to h^- 4\pi^0 \nu_\tau\;(\text{ex.}K^0,\eta))}{0.00112 \pm 0.00039}{0.00112}{\pm 0.00039}
\dxMeasDef{ALEPH.Gamma30.pub.SCHAEL.05C}{Gamma30}{SCHAEL 05C}{0.00112 \pm 0.00037 \pm 0.00035}{0.00112}{\pm 0.00037}{\pm 0.00035}
\dxQuantDef{Gamma31}{\BR_{31}}{\BR(\tau^- \to K^- \ge{} 0\, \pi^0 \ge{} 0\, K^0 \ge{} 0\, \gamma \nu_\tau)}{0.01552 \pm 0.00029}{0.01552}{\pm 0.00029}
\dxMeasDef{CLEO.Gamma31.pub.BATTLE.94}{Gamma31}{BATTLE 94}{0.01700 \pm 0.00120 \pm 0.00190}{0.01700}{\pm 0.00120}{\pm 0.00190}
\dxMeasDef{DELPHI.Gamma31.pub.ABREU.94K}{Gamma31}{ABREU 94K}{0.01540 \pm 0.00240 \pm 0.00000}{0.01540}{\pm 0.00240}{\pm 0.00000}
\dxMeasDef{OPAL.Gamma31.pub.ABBIENDI.01J}{Gamma31}{ABBIENDI 01J}{0.01528 \pm 0.00039 \pm 0.00040}{0.01528}{\pm 0.00039}{\pm 0.00040}
\dxQuantDef{Gamma32}{\BR_{32}}{\BR(\tau^- \to K^- \ge{} 1\, (\pi^0\,\text{or}\,K^0\,\text{or}\,\gamma) \nu_\tau)}{0.00859 \pm 0.00028}{0.00859}{\pm 0.00028}
\dxQuantDef{Gamma33}{\BR_{33}}{\BR(\tau^- \to K_S^0 (\text{particle}s)^- \nu_\tau)}{0.00943 \pm 0.00028}{0.00943}{\pm 0.00028}
\dxMeasDef{ALEPH.Gamma33.pub.BARATE.98E}{Gamma33}{BARATE 98E}{0.00970 \pm 0.00058 \pm 0.00062}{0.00970}{\pm 0.00058}{\pm 0.00062}
\dxMeasDef{OPAL.Gamma33.pub.AKERS.94G}{Gamma33}{AKERS 94G}{0.00970 \pm 0.00090 \pm 0.00060}{0.00970}{\pm 0.00090}{\pm 0.00060}
\dxQuantDef{Gamma34}{\BR_{34}}{\BR(\tau^- \to h^- \bar{K}^0 \nu_\tau)}{0.00987 \pm 0.00014}{0.00987}{\pm 0.00014}
\dxMeasDef{CLEO.Gamma34.pub.COAN.96}{Gamma34}{COAN 96}{0.00855 \pm 0.00036 \pm 0.00073}{0.00855}{\pm 0.00036}{\pm 0.00073}
\dxQuantDef{Gamma35}{\BR_{35}}{\BR(\tau^- \to \pi^- \bar{K}^0 \nu_\tau)}{0.008384 \pm 0.000138}{0.008384}{\pm 0.000138}
\dxMeasDef{ALEPH.Gamma35.pub.BARATE.99K}{Gamma35}{BARATE 99K}{0.009280 \pm 0.000450 \pm 0.000340}{0.009280}{\pm 0.000450}{\pm 0.000340}
\dxMeasDef{Belle.Gamma35.pub.RYU.14vpc}{Gamma35}{RYU 14vpc}{0.008320 \pm 0.000025 \pm 0.000150}{0.008320}{\pm 0.000025}{\pm 0.000150}
\dxMeasDef{L3.Gamma35.pub.ACCIARRI.95F}{Gamma35}{ACCIARRI 95F}{0.009500 \pm 0.001500 \pm 0.000600}{0.009500}{\pm 0.001500}{\pm 0.000600}
\dxMeasDef{OPAL.Gamma35.pub.ABBIENDI.00C}{Gamma35}{ABBIENDI 00C}{0.009330 \pm 0.000680 \pm 0.000490}{0.009330}{\pm 0.000680}{\pm 0.000490}
\dxQuantDef{Gamma37}{\BR_{37}}{\BR(\tau^- \to K^- K^0 \nu_\tau)}{0.001486 \pm 0.000034}{0.001486}{\pm 0.000034}
\dxMeasDef{ALEPH.Gamma37.pub.BARATE.98E}{Gamma37}{BARATE 98E}{0.001580 \pm 0.000420 \pm 0.000170}{0.001580}{\pm 0.000420}{\pm 0.000170}
\dxMeasDef{ALEPH.Gamma37.pub.BARATE.99K}{Gamma37}{BARATE 99K}{0.001620 \pm 0.000210 \pm 0.000110}{0.001620}{\pm 0.000210}{\pm 0.000110}
\dxMeasDef{BaBar.Gamma37.pub.LEES.18B}{Gamma37}{LEES 18B}{0.001478 \pm 0.000022 \pm 0.000040}{0.001478}{\pm 0.000022}{\pm 0.000040}
\dxMeasDef{Belle.Gamma37.pub.RYU.14vpc}{Gamma37}{RYU 14vpc}{0.001480 \pm 0.000013 \pm 0.000055}{0.001480}{\pm 0.000013}{\pm 0.000055}
\dxMeasDef{CLEO.Gamma37.pub.COAN.96}{Gamma37}{COAN 96}{0.001510 \pm 0.000210 \pm 0.000220}{0.001510}{\pm 0.000210}{\pm 0.000220}
\dxQuantDef{Gamma38}{\BR_{38}}{\BR(\tau^- \to K^- K^0 \ge{} 0\,  \pi^0\, \nu_\tau)}{0.00299 \pm 0.00007}{0.00299}{\pm 0.00007}
\dxMeasDef{OPAL.Gamma38.pub.ABBIENDI.00C}{Gamma38}{ABBIENDI 00C}{0.00330 \pm 0.00055 \pm 0.00039}{0.00330}{\pm 0.00055}{\pm 0.00039}
\dxQuantDef{Gamma39}{\BR_{39}}{\BR(\tau^- \to h^- \bar{K}^0 \pi^0 \nu_\tau)}{0.00532 \pm 0.00013}{0.00532}{\pm 0.00013}
\dxMeasDef{CLEO.Gamma39.pub.COAN.96}{Gamma39}{COAN 96}{0.00562 \pm 0.00050 \pm 0.00048}{0.00562}{\pm 0.00050}{\pm 0.00048}
\dxQuantDef{Gamma40}{\BR_{40}}{\BR(\tau^- \to \pi^- \bar{K}^0 \pi^0 \nu_\tau)}{0.003817 \pm 0.000129}{0.003817}{\pm 0.000129}
\dxMeasDef{ALEPH.Gamma40.pub.BARATE.98E}{Gamma40}{BARATE 98E}{0.002940 \pm 0.000730 \pm 0.000370}{0.002940}{\pm 0.000730}{\pm 0.000370}
\dxMeasDef{ALEPH.Gamma40.pub.BARATE.99K}{Gamma40}{BARATE 99K}{0.003470 \pm 0.000530 \pm 0.000370}{0.003470}{\pm 0.000530}{\pm 0.000370}
\dxMeasDef{Belle.Gamma40.pub.RYU.14vpc}{Gamma40}{RYU 14vpc}{0.003860 \pm 0.000031 \pm 0.000135}{0.003860}{\pm 0.000031}{\pm 0.000135}
\dxMeasDef{L3.Gamma40.pub.ACCIARRI.95F}{Gamma40}{ACCIARRI 95F}{0.004100 \pm 0.001200 \pm 0.000300}{0.004100}{\pm 0.001200}{\pm 0.000300}
\dxQuantDef{Gamma42}{\BR_{42}}{\BR(\tau^- \to K^- K^0 \pi^0 \nu_\tau)}{0.001500 \pm 0.000070}{0.001500}{\pm 0.000070}
\dxMeasDef{ALEPH.Gamma42.pub.BARATE.98E}{Gamma42}{BARATE 98E}{0.001520 \pm 0.000760 \pm 0.000210}{0.001520}{\pm 0.000760}{\pm 0.000210}
\dxMeasDef{ALEPH.Gamma42.pub.BARATE.99K}{Gamma42}{BARATE 99K}{0.001430 \pm 0.000250 \pm 0.000150}{0.001430}{\pm 0.000250}{\pm 0.000150}
\dxMeasDef{Belle.Gamma42.pub.RYU.14vpc}{Gamma42}{RYU 14vpc}{0.001496 \pm 0.000019 \pm 0.000073}{0.001496}{\pm 0.000019}{\pm 0.000073}
\dxMeasDef{CLEO.Gamma42.pub.COAN.96}{Gamma42}{COAN 96}{0.001450 \pm 0.000360 \pm 0.000200}{0.001450}{\pm 0.000360}{\pm 0.000200}
\dxQuantDef{Gamma43}{\BR_{43}}{\BR(\tau^- \to \pi^- \bar{K}^0 \ge{} 1\,  \pi^0\, \nu_\tau)}{0.00408 \pm 0.00025}{0.00408}{\pm 0.00025}
\dxMeasDef{OPAL.Gamma43.pub.ABBIENDI.00C}{Gamma43}{ABBIENDI 00C}{0.00324 \pm 0.00074 \pm 0.00066}{0.00324}{\pm 0.00074}{\pm 0.00066}
\dxQuantDef{Gamma44}{\BR_{44}}{\BR(\tau^- \to \pi^- \bar{K}^0 2\pi^0 \nu_\tau\;(\text{ex.}K^0))}{(0.26 \pm 0.23)\cdot 10^{-3}}{0.26 \cdot 10^{-3}}{\pm 0.23 \cdot 10^{-3}}
\dxMeasDef{ALEPH.Gamma44.pub.BARATE.99R}{Gamma44}{BARATE 99R}{(0.26 \pm 0.24 \pm 0.00)\cdot 10^{-3}}{0.26 \cdot 10^{-3}}{\pm 0.24 \cdot 10^{-3}}{\pm 0.00 \cdot 10^{-3}}
\dxQuantDef{Gamma46}{\BR_{46}}{\BR(\tau^- \to \pi^- K^0 \bar{K}^0 \nu_\tau)}{0.00155 \pm 0.00024}{0.00155}{\pm 0.00024}
\dxQuantDef{Gamma47}{\BR_{47}}{\BR(\tau^- \to \pi^- K_S^0 K_S^0 \nu_\tau)}{(234.9 \pm 6.5)\cdot 10^{-6}}{234.9 \cdot 10^{-6}}{\pm 6.5 \cdot 10^{-6}}
\dxMeasDef{ALEPH.Gamma47.pub.BARATE.98E}{Gamma47}{BARATE 98E}{(260.0 \pm 100.0 \pm 50.0)\cdot 10^{-6}}{260.0 \cdot 10^{-6}}{\pm 100.0 \cdot 10^{-6}}{\pm 50.0 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma47.pub.LEES.12Y}{Gamma47}{LEES 12Y}{(231.0 \pm 4.0 \pm 8.0)\cdot 10^{-6}}{231.0 \cdot 10^{-6}}{\pm 4.0 \cdot 10^{-6}}{\pm 8.0 \cdot 10^{-6}}
\dxMeasDef{Belle.Gamma47.pub.RYU.14vpc}{Gamma47}{RYU 14vpc}{(233.0 \pm 3.3 \pm 9.3)\cdot 10^{-6}}{233.0 \cdot 10^{-6}}{\pm 3.3 \cdot 10^{-6}}{\pm 9.3 \cdot 10^{-6}}
\dxMeasDef{CLEO.Gamma47.pub.COAN.96}{Gamma47}{COAN 96}{(230.0 \pm 50.0 \pm 30.0)\cdot 10^{-6}}{230.0 \cdot 10^{-6}}{\pm 50.0 \cdot 10^{-6}}{\pm 30.0 \cdot 10^{-6}}
\dxQuantDef{Gamma48}{\BR_{48}}{\BR(\tau^- \to \pi^- K_S^0 K_L^0 \nu_\tau)}{0.00108 \pm 0.00024}{0.00108}{\pm 0.00024}
\dxMeasDef{ALEPH.Gamma48.pub.BARATE.98E}{Gamma48}{BARATE 98E}{0.00101 \pm 0.00023 \pm 0.00013}{0.00101}{\pm 0.00023}{\pm 0.00013}
\dxQuantDef{Gamma49}{\BR_{49}}{\BR(\tau^- \to \pi^- \pi^0 K^0 \bar{K}^0 \nu_\tau)}{(0.36 \pm 0.12)\cdot 10^{-3}}{0.36 \cdot 10^{-3}}{\pm 0.12 \cdot 10^{-3}}
\dxQuantDef{Gamma50}{\BR_{50}}{\BR(\tau^- \to \pi^- K_S^0 K_S^0 \pi^0 \nu_\tau)}{(18.2 \pm 2.1)\cdot 10^{-6}}{18.2 \cdot 10^{-6}}{\pm 2.1 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma50.pub.LEES.12Y}{Gamma50}{LEES 12Y}{(16.0 \pm 2.0 \pm 2.2)\cdot 10^{-6}}{16.0 \cdot 10^{-6}}{\pm 2.0 \cdot 10^{-6}}{\pm 2.2 \cdot 10^{-6}}
\dxMeasDef{Belle.Gamma50.pub.RYU.14vpc}{Gamma50}{RYU 14vpc}{(20.0 \pm 2.2 \pm 2.0)\cdot 10^{-6}}{20.0 \cdot 10^{-6}}{\pm 2.2 \cdot 10^{-6}}{\pm 2.0 \cdot 10^{-6}}
\dxQuantDef{Gamma51}{\BR_{51}}{\BR(\tau^- \to \pi^- K_S^0 K_L^0 \pi^0 \nu_\tau)}{(0.32 \pm 0.12)\cdot 10^{-3}}{0.32 \cdot 10^{-3}}{\pm 0.12 \cdot 10^{-3}}
\dxMeasDef{ALEPH.Gamma51.pub.BARATE.98E}{Gamma51}{BARATE 98E}{(0.31 \pm 0.11 \pm 0.05)\cdot 10^{-3}}{0.31 \cdot 10^{-3}}{\pm 0.11 \cdot 10^{-3}}{\pm 0.05 \cdot 10^{-3}}
\dxQuantDef{Gamma53}{\BR_{53}}{\BR(\tau^- \to \bar{K}^0 h^- h^- h^+ \nu_\tau)}{(0.25 \pm 0.20)\cdot 10^{-3}}{0.25 \cdot 10^{-3}}{\pm 0.20 \cdot 10^{-3}}
\dxMeasDef{ALEPH.Gamma53.pub.BARATE.98E}{Gamma53}{BARATE 98E}{(0.23 \pm 0.19 \pm 0.07)\cdot 10^{-3}}{0.23 \cdot 10^{-3}}{\pm 0.19 \cdot 10^{-3}}{\pm 0.07 \cdot 10^{-3}}
\dxQuantDef{Gamma54}{\BR_{54}}{\BR(\tau^- \to h^- h^- h^+ \ge{} 0\, \text{neutrals} \ge{} 0\,  K_L^0\, \nu_\tau)}{0.1520 \pm 0.0006}{0.1520}{\pm 0.0006}
\dxMeasDef{CELLO.Gamma54.pub.BEHREND.89B}{Gamma54}{BEHREND 89B}{0.1500 \pm 0.0040 \pm 0.0030}{0.1500}{\pm 0.0040}{\pm 0.0030}
\dxMeasDef{L3.Gamma54.pub.ADEVA.91F}{Gamma54}{ADEVA 91F}{0.1440 \pm 0.0060 \pm 0.0030}{0.1440}{\pm 0.0060}{\pm 0.0030}
\dxMeasDef{TPC.Gamma54.pub.AIHARA.87B}{Gamma54}{AIHARA 87B}{0.1510 \pm 0.0080 \pm 0.0060}{0.1510}{\pm 0.0080}{\pm 0.0060}
\dxQuantDef{Gamma55}{\BR_{55}}{\BR(\tau^- \to h^- h^- h^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau\;(\text{ex.}K^0))}{0.1455 \pm 0.0006}{0.1455}{\pm 0.0006}
\dxMeasDef{L3.Gamma55.pub.ACHARD.01D}{Gamma55}{ACHARD 01D}{0.1456 \pm 0.0010 \pm 0.0008}{0.1456}{\pm 0.0010}{\pm 0.0008}
\dxMeasDef{OPAL.Gamma55.pub.AKERS.95Y}{Gamma55}{AKERS 95Y}{0.1496 \pm 0.0009 \pm 0.0022}{0.1496}{\pm 0.0009}{\pm 0.0022}
\dxQuantDef{Gamma56}{\BR_{56}}{\BR(\tau^- \to h^- h^- h^+ \nu_\tau)}{0.0980 \pm 0.0005}{0.0980}{\pm 0.0005}
\dxQuantDef{Gamma57}{\BR_{57}}{\BR(\tau^- \to h^- h^- h^+ \nu_\tau\;(\text{ex.}K^0))}{0.0945 \pm 0.0005}{0.0945}{\pm 0.0005}
\dxMeasDef{CLEO.Gamma57.pub.BALEST.95C}{Gamma57}{BALEST 95C}{0.0951 \pm 0.0007 \pm 0.0020}{0.0951}{\pm 0.0007}{\pm 0.0020}
\dxMeasDef{DELPHI.Gamma57.pub.ABDALLAH.06A}{Gamma57}{ABDALLAH 06A}{0.0932 \pm 0.0009 \pm 0.0008}{0.0932}{\pm 0.0009}{\pm 0.0008}
\dxQuantDef{Gamma57by55}{\BR_{57 / 55}}{\frac{\BR(\tau^- \to h^- h^- h^+ \nu_\tau\;(\text{ex.}K^0))}{\BR(\tau^- \to h^- h^- h^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau\;(\text{ex.}K^0))}}{0.6498 \pm 0.0031}{0.6498}{\pm 0.0031}
\dxMeasDef{OPAL.Gamma57by55.pub.AKERS.95Y}{Gamma57by55}{AKERS 95Y}{0.6600 \pm 0.0040 \pm 0.0140}{0.6600}{\pm 0.0040}{\pm 0.0140}
\dxQuantDef{Gamma58}{\BR_{58}}{\BR(\tau^- \to h^- h^- h^+ \nu_\tau\;(\text{ex.}K^0,\omega))}{0.0942 \pm 0.0005}{0.0942}{\pm 0.0005}
\dxQuantDef{Gamma59}{\BR_{59}}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \nu_\tau)}{0.0931 \pm 0.0005}{0.0931}{\pm 0.0005}
\dxQuantDef{Gamma60}{\BR_{60}}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0))}{0.09016 \pm 0.00051}{0.09016}{\pm 0.00051}
\dxMeasDef{BaBar.Gamma60.pub.AUBERT.08}{Gamma60}{AUBERT 08}{0.08830 \pm 0.00010 \pm 0.00130}{0.08830}{\pm 0.00010}{\pm 0.00130}
\dxMeasDef{Belle.Gamma60.pub.LEE.10}{Gamma60}{LEE 10}{0.08420 \pm 0.00000 {}^{+0.00260}_{-0.00250}}{0.08420}{\pm 0.00000}{{}^{+0.00260}_{-0.00250}}
\dxMeasDef{CLEO3.Gamma60.pub.BRIERE.03}{Gamma60}{BRIERE 03}{0.09130 \pm 0.00050 \pm 0.00460}{0.09130}{\pm 0.00050}{\pm 0.00460}
\dxQuantDef{Gamma62}{\BR_{62}}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0,\omega))}{0.0899 \pm 0.0005}{0.0899}{\pm 0.0005}
\dxMeasDef{ALEPH.Gamma62.pub.SCHAEL.05C}{Gamma62}{SCHAEL 05C}{0.0904 \pm 0.0006 \pm 0.0008}{0.0904}{\pm 0.0006}{\pm 0.0008}
\dxQuantDef{Gamma63}{\BR_{63}}{\BR(\tau^- \to h^- h^- h^+ \ge{} 1\,  \text{neutrals}\, \nu_\tau)}{0.0529 \pm 0.0005}{0.0529}{\pm 0.0005}
\dxQuantDef{Gamma64}{\BR_{64}}{\BR(\tau^- \to h^- h^- h^+ \ge{} 1\,  \pi^0\, \nu_\tau\;(\text{ex.}K^0))}{0.0509 \pm 0.0005}{0.0509}{\pm 0.0005}
\dxQuantDef{Gamma65}{\BR_{65}}{\BR(\tau^- \to h^- h^- h^+ \pi^0 \nu_\tau)}{0.0476 \pm 0.0005}{0.0476}{\pm 0.0005}
\dxQuantDef{Gamma66}{\BR_{66}}{\BR(\tau^- \to h^- h^- h^+ \pi^0 \nu_\tau\;(\text{ex.}K^0))}{0.0457 \pm 0.0005}{0.0457}{\pm 0.0005}
\dxMeasDef{CLEO.Gamma66.pub.BALEST.95C}{Gamma66}{BALEST 95C}{0.0423 \pm 0.0006 \pm 0.0022}{0.0423}{\pm 0.0006}{\pm 0.0022}
\dxMeasDef{DELPHI.Gamma66.pub.ABDALLAH.06A}{Gamma66}{ABDALLAH 06A}{0.0454 \pm 0.0011 \pm 0.0010}{0.0454}{\pm 0.0011}{\pm 0.0010}
\dxQuantDef{Gamma67}{\BR_{67}}{\BR(\tau^- \to h^- h^- h^+ \pi^0 \nu_\tau\;(\text{ex.}K^0,\omega))}{0.0279 \pm 0.0007}{0.0279}{\pm 0.0007}
\dxQuantDef{Gamma68}{\BR_{68}}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \pi^0 \nu_\tau)}{0.0462 \pm 0.0005}{0.0462}{\pm 0.0005}
\dxQuantDef{Gamma69}{\BR_{69}}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \pi^0 \nu_\tau\;(\text{ex.}K^0))}{0.0449 \pm 0.0005}{0.0449}{\pm 0.0005}
\dxMeasDef{ALEPH.Gamma69.pub.SCHAEL.05C}{Gamma69}{SCHAEL 05C}{0.0460 \pm 0.0006 \pm 0.0006}{0.0460}{\pm 0.0006}{\pm 0.0006}
\dxMeasDef{CLEO.Gamma69.pub.EDWARDS.00A}{Gamma69}{EDWARDS 00A}{0.0419 \pm 0.0010 \pm 0.0021}{0.0419}{\pm 0.0010}{\pm 0.0021}
\dxQuantDef{Gamma70}{\BR_{70}}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \pi^0 \nu_\tau\;(\text{ex.}K^0,\omega))}{0.0274 \pm 0.0007}{0.0274}{\pm 0.0007}
\dxQuantDef{Gamma74}{\BR_{74}}{\BR(\tau^- \to h^- h^- h^+ \ge{} 2\, \pi^0\, \nu_\tau\;(\text{ex.}K^0))}{0.00517 \pm 0.00031}{0.00517}{\pm 0.00031}
\dxMeasDef{DELPHI.Gamma74.pub.ABDALLAH.06A}{Gamma74}{ABDALLAH 06A}{0.00561 \pm 0.00068 \pm 0.00095}{0.00561}{\pm 0.00068}{\pm 0.00095}
\dxQuantDef{Gamma75}{\BR_{75}}{\BR(\tau^- \to h^- h^- h^+ 2\pi^0 \nu_\tau)}{0.00505 \pm 0.00031}{0.00505}{\pm 0.00031}
\dxQuantDef{Gamma76}{\BR_{76}}{\BR(\tau^- \to h^- h^- h^+ 2\pi^0 \nu_\tau\;(\text{ex.}K^0))}{0.00495 \pm 0.00031}{0.00495}{\pm 0.00031}
\dxMeasDef{ALEPH.Gamma76.pub.SCHAEL.05C}{Gamma76}{SCHAEL 05C}{0.00435 \pm 0.00030 \pm 0.00035}{0.00435}{\pm 0.00030}{\pm 0.00035}
\dxQuantDef{Gamma76by54}{\BR_{76 / 54}}{\frac{\BR(\tau^- \to h^- h^- h^+ 2\pi^0 \nu_\tau\;(\text{ex.}K^0))}{\BR(\tau^- \to h^- h^- h^+ \ge{} 0\, \text{neutrals} \ge{} 0\,  K_L^0\, \nu_\tau)}}{0.0326 \pm 0.0020}{0.0326}{\pm 0.0020}
\dxMeasDef{CLEO.Gamma76by54.pub.BORTOLETTO.93}{Gamma76by54}{BORTOLETTO 93}{0.0340 \pm 0.0020 \pm 0.0030}{0.0340}{\pm 0.0020}{\pm 0.0030}
\dxQuantDef{Gamma77}{\BR_{77}}{\BR(\tau^- \to h^- h^- h^+ 2\pi^0 \nu_\tau\;(\text{ex.}K^0,\omega,\eta))}{0.0010 \pm 0.0004}{0.0010}{\pm 0.0004}
\dxQuantDef{Gamma78}{\BR_{78}}{\BR(\tau^- \to h^- h^- h^+ 3\pi^0 \nu_\tau)}{(213 \pm 30)\cdot 10^{-6}}{213 \cdot 10^{-6}}{\pm 30 \cdot 10^{-6}}
\dxMeasDef{CLEO.Gamma78.pub.ANASTASSOV.01}{Gamma78}{ANASTASSOV 01}{(220 \pm 30 \pm 40)\cdot 10^{-6}}{220 \cdot 10^{-6}}{\pm 30 \cdot 10^{-6}}{\pm 40 \cdot 10^{-6}}
\dxQuantDef{Gamma79}{\BR_{79}}{\BR(\tau^- \to K^- h^- h^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau)}{0.00629 \pm 0.00014}{0.00629}{\pm 0.00014}
\dxQuantDef{Gamma80}{\BR_{80}}{\BR(\tau^- \to K^- \pi^- h^+ \nu_\tau\;(\text{ex.}K^0))}{0.00437 \pm 0.00007}{0.00437}{\pm 0.00007}
\dxQuantDef{Gamma80by60}{\BR_{80 / 60}}{\frac{\BR(\tau^- \to K^- \pi^- h^+ \nu_\tau\;(\text{ex.}K^0))}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0))}}{0.0485 \pm 0.0008}{0.0485}{\pm 0.0008}
\dxMeasDef{CLEO.Gamma80by60.pub.RICHICHI.99}{Gamma80by60}{RICHICHI 99}{0.0544 \pm 0.0021 \pm 0.0053}{0.0544}{\pm 0.0021}{\pm 0.0053}
\dxQuantDef{Gamma81}{\BR_{81}}{\BR(\tau^- \to K^- \pi^- h^+ \pi^0 \nu_\tau\;(\text{ex.}K^0))}{(0.86 \pm 0.12)\cdot 10^{-3}}{0.86 \cdot 10^{-3}}{\pm 0.12 \cdot 10^{-3}}
\dxQuantDef{Gamma81by69}{\BR_{81 / 69}}{\frac{\BR(\tau^- \to K^- \pi^- h^+ \pi^0 \nu_\tau\;(\text{ex.}K^0))}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \pi^0 \nu_\tau\;(\text{ex.}K^0))}}{0.0191 \pm 0.0026}{0.0191}{\pm 0.0026}
\dxMeasDef{CLEO.Gamma81by69.pub.RICHICHI.99}{Gamma81by69}{RICHICHI 99}{0.0261 \pm 0.0045 \pm 0.0042}{0.0261}{\pm 0.0045}{\pm 0.0042}
\dxQuantDef{Gamma82}{\BR_{82}}{\BR(\tau^- \to K^- \pi^- \pi^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau)}{0.00477 \pm 0.00014}{0.00477}{\pm 0.00014}
\dxMeasDef{TPC.Gamma82.pub.BAUER.94}{Gamma82}{BAUER 94}{0.00580 {}^{+0.00150}_{-0.00130} \pm 0.00120}{0.00580}{{}^{+0.00150}_{-0.00130}}{\pm 0.00120}
\dxQuantDef{Gamma83}{\BR_{83}}{\BR(\tau^- \to K^- \pi^- \pi^+ \ge{} 0\,  \pi^0\, \nu_\tau\;(\text{ex.}K^0))}{0.00373 \pm 0.00013}{0.00373}{\pm 0.00013}
\dxQuantDef{Gamma84}{\BR_{84}}{\BR(\tau^- \to K^- \pi^- \pi^+ \nu_\tau)}{0.00345 \pm 0.00007}{0.00345}{\pm 0.00007}
\dxQuantDef{Gamma85}{\BR_{85}}{\BR(\tau^- \to K^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0))}{0.002933 \pm 0.000068}{0.002933}{\pm 0.000068}
\dxMeasDef{ALEPH.Gamma85.pub.BARATE.98}{Gamma85}{BARATE 98}{0.002140 \pm 0.000370 \pm 0.000290}{0.002140}{\pm 0.000370}{\pm 0.000290}
\dxMeasDef{BaBar.Gamma85.pub.AUBERT.08}{Gamma85}{AUBERT 08}{0.002730 \pm 0.000020 \pm 0.000090}{0.002730}{\pm 0.000020}{\pm 0.000090}
\dxMeasDef{Belle.Gamma85.pub.LEE.10}{Gamma85}{LEE 10}{0.003300 \pm 0.000010 {}^{+0.000160}_{-0.000170}}{0.003300}{\pm 0.000010}{{}^{+0.000160}_{-0.000170}}
\dxMeasDef{CLEO3.Gamma85.pub.BRIERE.03}{Gamma85}{BRIERE 03}{0.003840 \pm 0.000140 \pm 0.000380}{0.003840}{\pm 0.000140}{\pm 0.000380}
\dxMeasDef{OPAL.Gamma85.pub.ABBIENDI.04J}{Gamma85}{ABBIENDI 04J}{0.004150 \pm 0.000530 \pm 0.000400}{0.004150}{\pm 0.000530}{\pm 0.000400}
\dxQuantDef{Gamma85by60}{\BR_{85 / 60}}{\frac{\BR(\tau^- \to K^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0))}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0))}}{0.0325 \pm 0.0007}{0.0325}{\pm 0.0007}
\dxQuantDef{Gamma87}{\BR_{87}}{\BR(\tau^- \to K^- \pi^- \pi^+ \pi^0 \nu_\tau)}{0.00131 \pm 0.00012}{0.00131}{\pm 0.00012}
\dxQuantDef{Gamma88}{\BR_{88}}{\BR(\tau^- \to K^- \pi^- \pi^+ \pi^0 \nu_\tau\;(\text{ex.}K^0))}{(0.80 \pm 0.12)\cdot 10^{-3}}{0.80 \cdot 10^{-3}}{\pm 0.12 \cdot 10^{-3}}
\dxMeasDef{ALEPH.Gamma88.pub.BARATE.98}{Gamma88}{BARATE 98}{(0.61 \pm 0.39 \pm 0.18)\cdot 10^{-3}}{0.61 \cdot 10^{-3}}{\pm 0.39 \cdot 10^{-3}}{\pm 0.18 \cdot 10^{-3}}
\dxMeasDef{CLEO3.Gamma88.pub.ARMS.05}{Gamma88}{ARMS 05}{(0.74 \pm 0.08 \pm 0.11)\cdot 10^{-3}}{0.74 \cdot 10^{-3}}{\pm 0.08 \cdot 10^{-3}}{\pm 0.11 \cdot 10^{-3}}
\dxQuantDef{Gamma89}{\BR_{89}}{\BR(\tau^- \to K^- \pi^- \pi^+ \pi^0 \nu_\tau\;(\text{ex.}K^0,\eta))}{(0.76 \pm 0.12)\cdot 10^{-3}}{0.76 \cdot 10^{-3}}{\pm 0.12 \cdot 10^{-3}}
\dxQuantDef{Gamma92}{\BR_{92}}{\BR(\tau^- \to \pi^- K^- K^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau)}{0.001496 \pm 0.000033}{0.001496}{\pm 0.000033}
\dxMeasDef{OPAL.Gamma92.pub.ABBIENDI.00D}{Gamma92}{ABBIENDI 00D}{0.001590 \pm 0.000530 \pm 0.000200}{0.001590}{\pm 0.000530}{\pm 0.000200}
\dxMeasDef{TPC.Gamma92.pub.BAUER.94}{Gamma92}{BAUER 94}{0.001500 {}^{+0.000900}_{-0.000700} \pm 0.000300}{0.001500}{{}^{+0.000900}_{-0.000700}}{\pm 0.000300}
\dxQuantDef{Gamma93}{\BR_{93}}{\BR(\tau^- \to \pi^- K^- K^+ \nu_\tau)}{0.001435 \pm 0.000027}{0.001435}{\pm 0.000027}
\dxMeasDef{ALEPH.Gamma93.pub.BARATE.98}{Gamma93}{BARATE 98}{0.001630 \pm 0.000210 \pm 0.000170}{0.001630}{\pm 0.000210}{\pm 0.000170}
\dxMeasDef{BaBar.Gamma93.pub.AUBERT.08}{Gamma93}{AUBERT 08}{0.001346 \pm 0.000010 \pm 0.000036}{0.001346}{\pm 0.000010}{\pm 0.000036}
\dxMeasDef{Belle.Gamma93.pub.LEE.10}{Gamma93}{LEE 10}{0.001550 \pm 0.000010 {}^{+0.000060}_{-0.000050}}{0.001550}{\pm 0.000010}{{}^{+0.000060}_{-0.000050}}
\dxMeasDef{CLEO3.Gamma93.pub.BRIERE.03}{Gamma93}{BRIERE 03}{0.001550 \pm 0.000060 \pm 0.000090}{0.001550}{\pm 0.000060}{\pm 0.000090}
\dxQuantDef{Gamma93by60}{\BR_{93 / 60}}{\frac{\BR(\tau^- \to \pi^- K^- K^+ \nu_\tau)}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0))}}{0.01592 \pm 0.00030}{0.01592}{\pm 0.00030}
\dxMeasDef{CLEO.Gamma93by60.pub.RICHICHI.99}{Gamma93by60}{RICHICHI 99}{0.01600 \pm 0.00150 \pm 0.00300}{0.01600}{\pm 0.00150}{\pm 0.00300}
\dxQuantDef{Gamma94}{\BR_{94}}{\BR(\tau^- \to \pi^- K^- K^+ \pi^0 \nu_\tau)}{(61 \pm 18)\cdot 10^{-6}}{61 \cdot 10^{-6}}{\pm 18 \cdot 10^{-6}}
\dxMeasDef{ALEPH.Gamma94.pub.BARATE.98}{Gamma94}{BARATE 98}{(750 \pm 290 \pm 150)\cdot 10^{-6}}{750 \cdot 10^{-6}}{\pm 290 \cdot 10^{-6}}{\pm 150 \cdot 10^{-6}}
\dxMeasDef{CLEO3.Gamma94.pub.ARMS.05}{Gamma94}{ARMS 05}{(55 \pm 14 \pm 12)\cdot 10^{-6}}{55 \cdot 10^{-6}}{\pm 14 \cdot 10^{-6}}{\pm 12 \cdot 10^{-6}}
\dxQuantDef{Gamma94by69}{\BR_{94 / 69}}{\frac{\BR(\tau^- \to \pi^- K^- K^+ \pi^0 \nu_\tau)}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \pi^0 \nu_\tau\;(\text{ex.}K^0))}}{0.0014 \pm 0.0004}{0.0014}{\pm 0.0004}
\dxMeasDef{CLEO.Gamma94by69.pub.RICHICHI.99}{Gamma94by69}{RICHICHI 99}{0.0079 \pm 0.0044 \pm 0.0016}{0.0079}{\pm 0.0044}{\pm 0.0016}
\dxQuantDef{Gamma96}{\BR_{96}}{\BR(\tau^- \to K^- K^- K^+ \nu_\tau)}{(21.7 \pm 8.0)\cdot 10^{-6}}{21.7 \cdot 10^{-6}}{\pm 8.0 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma96.pub.AUBERT.08}{Gamma96}{AUBERT 08}{(15.8 \pm 1.3 \pm 1.2)\cdot 10^{-6}}{15.8 \cdot 10^{-6}}{\pm 1.3 \cdot 10^{-6}}{\pm 1.2 \cdot 10^{-6}}
\dxMeasDef{Belle.Gamma96.pub.LEE.10}{Gamma96}{LEE 10}{(32.9 \pm 1.7 {}^{+1.9}_{-2.0})\cdot 10^{-6}}{32.9 \cdot 10^{-6}}{\pm 1.7 \cdot 10^{-6}}{{}^{+1.9}_{-2.0} \cdot 10^{-6}}
\dxQuantDef{Gamma102}{\BR_{102}}{\BR(\tau^- \to 3h^- 2h^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau\;(\text{ex.}K^0))}{0.00099 \pm 0.00004}{0.00099}{\pm 0.00004}
\dxMeasDef{CLEO.Gamma102.pub.GIBAUT.94B}{Gamma102}{GIBAUT 94B}{0.00097 \pm 0.00005 \pm 0.00011}{0.00097}{\pm 0.00005}{\pm 0.00011}
\dxMeasDef{HRS.Gamma102.pub.BYLSMA.87}{Gamma102}{BYLSMA 87}{0.00102 \pm 0.00029 \pm 0.00000}{0.00102}{\pm 0.00029}{\pm 0.00000}
\dxMeasDef{L3.Gamma102.pub.ACHARD.01D}{Gamma102}{ACHARD 01D}{0.00170 \pm 0.00022 \pm 0.00026}{0.00170}{\pm 0.00022}{\pm 0.00026}
\dxQuantDef{Gamma103}{\BR_{103}}{\BR(\tau^- \to 3h^- 2h^+ \nu_\tau\;(\text{ex.}K^0))}{(829 \pm 31)\cdot 10^{-6}}{829 \cdot 10^{-6}}{\pm 31 \cdot 10^{-6}}
\dxMeasDef{ALEPH.Gamma103.pub.SCHAEL.05C}{Gamma103}{SCHAEL 05C}{(720 \pm 90 \pm 120)\cdot 10^{-6}}{720 \cdot 10^{-6}}{\pm 90 \cdot 10^{-6}}{\pm 120 \cdot 10^{-6}}
\dxMeasDef{ARGUS.Gamma103.pub.ALBRECHT.88B}{Gamma103}{ALBRECHT 88B}{(640 \pm 230 \pm 100)\cdot 10^{-6}}{640 \cdot 10^{-6}}{\pm 230 \cdot 10^{-6}}{\pm 100 \cdot 10^{-6}}
\dxMeasDef{CLEO.Gamma103.pub.GIBAUT.94B}{Gamma103}{GIBAUT 94B}{(770 \pm 50 \pm 90)\cdot 10^{-6}}{770 \cdot 10^{-6}}{\pm 50 \cdot 10^{-6}}{\pm 90 \cdot 10^{-6}}
\dxMeasDef{DELPHI.Gamma103.pub.ABDALLAH.06A}{Gamma103}{ABDALLAH 06A}{(970 \pm 150 \pm 50)\cdot 10^{-6}}{970 \cdot 10^{-6}}{\pm 150 \cdot 10^{-6}}{\pm 50 \cdot 10^{-6}}
\dxMeasDef{HRS.Gamma103.pub.BYLSMA.87}{Gamma103}{BYLSMA 87}{(510 \pm 200 \pm 0)\cdot 10^{-6}}{510 \cdot 10^{-6}}{\pm 200 \cdot 10^{-6}}{\pm 0 \cdot 10^{-6}}
\dxMeasDef{OPAL.Gamma103.pub.ACKERSTAFF.99E}{Gamma103}{ACKERSTAFF 99E}{(910 \pm 140 \pm 60)\cdot 10^{-6}}{910 \cdot 10^{-6}}{\pm 140 \cdot 10^{-6}}{\pm 60 \cdot 10^{-6}}
\dxQuantDef{Gamma104}{\BR_{104}}{\BR(\tau^- \to 3h^- 2h^+ \pi^0 \nu_\tau\;(\text{ex.}K^0))}{(165 \pm 11)\cdot 10^{-6}}{165 \cdot 10^{-6}}{\pm 11 \cdot 10^{-6}}
\dxMeasDef{ALEPH.Gamma104.pub.SCHAEL.05C}{Gamma104}{SCHAEL 05C}{(210 \pm 70 \pm 90)\cdot 10^{-6}}{210 \cdot 10^{-6}}{\pm 70 \cdot 10^{-6}}{\pm 90 \cdot 10^{-6}}
\dxMeasDef{CLEO.Gamma104.pub.ANASTASSOV.01}{Gamma104}{ANASTASSOV 01}{(170 \pm 20 \pm 20)\cdot 10^{-6}}{170 \cdot 10^{-6}}{\pm 20 \cdot 10^{-6}}{\pm 20 \cdot 10^{-6}}
\dxMeasDef{DELPHI.Gamma104.pub.ABDALLAH.06A}{Gamma104}{ABDALLAH 06A}{(160 \pm 120 \pm 60)\cdot 10^{-6}}{160 \cdot 10^{-6}}{\pm 120 \cdot 10^{-6}}{\pm 60 \cdot 10^{-6}}
\dxMeasDef{OPAL.Gamma104.pub.ACKERSTAFF.99E}{Gamma104}{ACKERSTAFF 99E}{(270 \pm 180 \pm 90)\cdot 10^{-6}}{270 \cdot 10^{-6}}{\pm 180 \cdot 10^{-6}}{\pm 90 \cdot 10^{-6}}
\dxQuantDef{Gamma106}{\BR_{106}}{\BR(\tau^- \to (5\pi)^- \nu_\tau)}{0.0078 \pm 0.0005}{0.0078}{\pm 0.0005}
\dxQuantDef{Gamma110}{\BR_{110}}{\BR(\tau^- \to X_s^- \nu_\tau)}{0.0292 \pm 0.0004}{0.0292}{\pm 0.0004}
\dxQuantDef{Gamma126}{\BR_{126}}{\BR(\tau^- \to \pi^- \pi^0 \eta \nu_\tau)}{0.001389 \pm 0.000072}{0.001389}{\pm 0.000072}
\dxMeasDef{ALEPH.Gamma126.pub.BUSKULIC.97C}{Gamma126}{BUSKULIC 97C}{0.001800 \pm 0.000400 \pm 0.000200}{0.001800}{\pm 0.000400}{\pm 0.000200}
\dxMeasDef{Belle.Gamma126.pub.INAMI.09}{Gamma126}{INAMI 09}{0.001350 \pm 0.000030 \pm 0.000070}{0.001350}{\pm 0.000030}{\pm 0.000070}
\dxMeasDef{CLEO.Gamma126.pub.ARTUSO.92}{Gamma126}{ARTUSO 92}{0.001700 \pm 0.000200 \pm 0.000200}{0.001700}{\pm 0.000200}{\pm 0.000200}
\dxQuantDef{Gamma128}{\BR_{128}}{\BR(\tau^- \to K^- \eta \nu_\tau)}{(155 \pm 8)\cdot 10^{-6}}{155 \cdot 10^{-6}}{\pm 8 \cdot 10^{-6}}
\dxMeasDef{ALEPH.Gamma128.pub.BUSKULIC.97C}{Gamma128}{BUSKULIC 97C}{(290 {}^{+130}_{-120} \pm 70)\cdot 10^{-6}}{290 \cdot 10^{-6}}{{}^{+130}_{-120} \cdot 10^{-6}}{\pm 70 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E}{Gamma128}{DEL-AMO-SANCHEZ 11E}{(142 \pm 11 \pm 7)\cdot 10^{-6}}{142 \cdot 10^{-6}}{\pm 11 \cdot 10^{-6}}{\pm 7 \cdot 10^{-6}}
\dxMeasDef{Belle.Gamma128.pub.INAMI.09}{Gamma128}{INAMI 09}{(158 \pm 5 \pm 9)\cdot 10^{-6}}{158 \cdot 10^{-6}}{\pm 5 \cdot 10^{-6}}{\pm 9 \cdot 10^{-6}}
\dxMeasDef{CLEO.Gamma128.pub.BARTELT.96}{Gamma128}{BARTELT 96}{(260 \pm 50 \pm 50)\cdot 10^{-6}}{260 \cdot 10^{-6}}{\pm 50 \cdot 10^{-6}}{\pm 50 \cdot 10^{-6}}
\dxQuantDef{Gamma130}{\BR_{130}}{\BR(\tau^- \to K^- \pi^0 \eta \nu_\tau)}{(48 \pm 12)\cdot 10^{-6}}{48 \cdot 10^{-6}}{\pm 12 \cdot 10^{-6}}
\dxMeasDef{Belle.Gamma130.pub.INAMI.09}{Gamma130}{INAMI 09}{(46 \pm 11 \pm 4)\cdot 10^{-6}}{46 \cdot 10^{-6}}{\pm 11 \cdot 10^{-6}}{\pm 4 \cdot 10^{-6}}
\dxMeasDef{CLEO.Gamma130.pub.BISHAI.99}{Gamma130}{BISHAI 99}{(177 \pm 56 \pm 71)\cdot 10^{-6}}{177 \cdot 10^{-6}}{\pm 56 \cdot 10^{-6}}{\pm 71 \cdot 10^{-6}}
\dxQuantDef{Gamma132}{\BR_{132}}{\BR(\tau^- \to \pi^- \bar{K}^0 \eta \nu_\tau)}{(94 \pm 15)\cdot 10^{-6}}{94 \cdot 10^{-6}}{\pm 15 \cdot 10^{-6}}
\dxMeasDef{Belle.Gamma132.pub.INAMI.09}{Gamma132}{INAMI 09}{(88 \pm 14 \pm 6)\cdot 10^{-6}}{88 \cdot 10^{-6}}{\pm 14 \cdot 10^{-6}}{\pm 6 \cdot 10^{-6}}
\dxMeasDef{CLEO.Gamma132.pub.BISHAI.99}{Gamma132}{BISHAI 99}{(220 \pm 70 \pm 22)\cdot 10^{-6}}{220 \cdot 10^{-6}}{\pm 70 \cdot 10^{-6}}{\pm 22 \cdot 10^{-6}}
\dxQuantDef{Gamma136}{\BR_{136}}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \eta \nu_\tau\;(\text{ex.}K^0))}{(220 \pm 13)\cdot 10^{-6}}{220 \cdot 10^{-6}}{\pm 13 \cdot 10^{-6}}
\dxQuantDef{Gamma149}{\BR_{149}}{\BR(\tau^- \to h^- \omega \ge{} 0\,  \text{neutrals}\, \nu_\tau)}{0.0240 \pm 0.0008}{0.0240}{\pm 0.0008}
\dxQuantDef{Gamma150}{\BR_{150}}{\BR(\tau^- \to h^- \omega \nu_\tau)}{0.0199 \pm 0.0006}{0.0199}{\pm 0.0006}
\dxMeasDef{ALEPH.Gamma150.pub.BUSKULIC.97C}{Gamma150}{BUSKULIC 97C}{0.0191 \pm 0.0007 \pm 0.0006}{0.0191}{\pm 0.0007}{\pm 0.0006}
\dxMeasDef{CLEO.Gamma150.pub.BARINGER.87}{Gamma150}{BARINGER 87}{0.0160 \pm 0.0027 \pm 0.0041}{0.0160}{\pm 0.0027}{\pm 0.0041}
\dxQuantDef{Gamma150by66}{\BR_{150 / 66}}{\frac{\BR(\tau^- \to h^- \omega \nu_\tau)}{\BR(\tau^- \to h^- h^- h^+ \pi^0 \nu_\tau\;(\text{ex.}K^0))}}{0.435 \pm 0.014}{0.435}{\pm 0.014}
\dxMeasDef{ALEPH.Gamma150by66.pub.BUSKULIC.96}{Gamma150by66}{BUSKULIC 96}{0.431 \pm 0.033 \pm 0.000}{0.431}{\pm 0.033}{\pm 0.000}
\dxMeasDef{CLEO.Gamma150by66.pub.BALEST.95C}{Gamma150by66}{BALEST 95C}{0.464 \pm 0.016 \pm 0.017}{0.464}{\pm 0.016}{\pm 0.017}
\dxQuantDef{Gamma151}{\BR_{151}}{\BR(\tau^- \to K^- \omega \nu_\tau)}{(0.41 \pm 0.09)\cdot 10^{-3}}{0.41 \cdot 10^{-3}}{\pm 0.09 \cdot 10^{-3}}
\dxMeasDef{CLEO3.Gamma151.pub.ARMS.05}{Gamma151}{ARMS 05}{(0.41 \pm 0.06 \pm 0.07)\cdot 10^{-3}}{0.41 \cdot 10^{-3}}{\pm 0.06 \cdot 10^{-3}}{\pm 0.07 \cdot 10^{-3}}
\dxQuantDef{Gamma152}{\BR_{152}}{\BR(\tau^- \to h^- \pi^0 \omega \nu_\tau)}{0.0041 \pm 0.0004}{0.0041}{\pm 0.0004}
\dxMeasDef{ALEPH.Gamma152.pub.BUSKULIC.97C}{Gamma152}{BUSKULIC 97C}{0.0043 \pm 0.0006 \pm 0.0005}{0.0043}{\pm 0.0006}{\pm 0.0005}
\dxQuantDef{Gamma152by54}{\BR_{152 / 54}}{\frac{\BR(\tau^- \to h^- \omega \pi^0 \nu_\tau)}{\BR(\tau^- \to h^- h^- h^+ \ge{} 0\, \text{neutrals} \ge{} 0\,  K_L^0\, \nu_\tau)}}{0.0269 \pm 0.0028}{0.0269}{\pm 0.0028}
\dxQuantDef{Gamma152by76}{\BR_{152 / 76}}{\frac{\BR(\tau^- \to h^- \omega \pi^0 \nu_\tau)}{\BR(\tau^- \to h^- h^- h^+ 2\pi^0 \nu_\tau\;(\text{ex.}K^0))}}{0.82 \pm 0.08}{0.82}{\pm 0.08}
\dxMeasDef{CLEO.Gamma152by76.pub.BORTOLETTO.93}{Gamma152by76}{BORTOLETTO 93}{0.81 \pm 0.06 \pm 0.06}{0.81}{\pm 0.06}{\pm 0.06}
\dxQuantDef{Gamma167}{\BR_{167}}{\BR(\tau^- \to K^- \phi \nu_\tau)}{(44 \pm 16)\cdot 10^{-6}}{44 \cdot 10^{-6}}{\pm 16 \cdot 10^{-6}}
\dxQuantDef{Gamma168}{\BR_{168}}{\BR(\tau^- \to K^- \phi(K^+ K^-) \nu_\tau)}{(22 \pm 8)\cdot 10^{-6}}{22 \cdot 10^{-6}}{\pm 8 \cdot 10^{-6}}
\dxQuantDef{Gamma169}{\BR_{169}}{\BR(\tau^- \to K^- \phi(K_S^0 K_L^0) \nu_\tau)}{(15 \pm 6)\cdot 10^{-6}}{15 \cdot 10^{-6}}{\pm 6 \cdot 10^{-6}}
\dxQuantDef{Gamma800}{\BR_{800}}{\BR(\tau^- \to \pi^- \omega \nu_\tau)}{0.0195 \pm 0.0006}{0.0195}{\pm 0.0006}
\dxQuantDef{Gamma802}{\BR_{802}}{\BR(\tau^- \to K^- \pi^- \pi^+ \nu_\tau\;(\text{ex.}K^0,\omega))}{0.00293 \pm 0.00007}{0.00293}{\pm 0.00007}
\dxQuantDef{Gamma803}{\BR_{803}}{\BR(\tau^- \to K^- \pi^- \pi^+ \pi^0 \nu_\tau\;(\text{ex.}K^0,\omega,\eta))}{(0.39 \pm 0.14)\cdot 10^{-3}}{0.39 \cdot 10^{-3}}{\pm 0.14 \cdot 10^{-3}}
\dxQuantDef{Gamma804}{\BR_{804}}{\BR(\tau^- \to \pi^- K_L^0 K_L^0 \nu_\tau)}{(235 \pm 6)\cdot 10^{-6}}{235 \cdot 10^{-6}}{\pm 6 \cdot 10^{-6}}
\dxQuantDef{Gamma805}{\BR_{805}}{\BR(\tau^- \to a_1^-(\pi^- \gamma) \nu_\tau)}{(0.40 \pm 0.15)\cdot 10^{-3}}{0.40 \cdot 10^{-3}}{\pm 0.15 \cdot 10^{-3}}
\dxQuantDef{Gamma806}{\BR_{806}}{\BR(\tau^- \to \pi^- K_L^0 K_L^0 \pi^0 \nu_\tau)}{(18.2 \pm 2.1)\cdot 10^{-6}}{18.2 \cdot 10^{-6}}{\pm 2.1 \cdot 10^{-6}}
\dxQuantDef{Gamma810}{\BR_{810}}{\BR(\tau^- \to 2\pi^- \pi^+ 3\pi^0 \nu_\tau\;(\text{ex.}K^0))}{(194 \pm 30)\cdot 10^{-6}}{194 \cdot 10^{-6}}{\pm 30 \cdot 10^{-6}}
\dxQuantDef{Gamma811}{\BR_{811}}{\BR(\tau^- \to \pi^- 2\pi^0 \omega \nu_\tau)}{(72 \pm 16)\cdot 10^{-6}}{72 \cdot 10^{-6}}{\pm 16 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma811.pub.LEES.12X}{Gamma811}{LEES 12X}{(73 \pm 12 \pm 12)\cdot 10^{-6}}{73 \cdot 10^{-6}}{\pm 12 \cdot 10^{-6}}{\pm 12 \cdot 10^{-6}}
\dxQuantDef{Gamma812}{\BR_{812}}{\BR(\tau^- \to 2\pi^- \pi^+ 3\pi^0 \nu_\tau\;(\text{ex.}K^0,\eta,\omega,f_1))}{(14 \pm 27)\cdot 10^{-6}}{14 \cdot 10^{-6}}{\pm 27 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma812.pub.LEES.12X}{Gamma812}{LEES 12X}{(10 \pm 8 \pm 30)\cdot 10^{-6}}{10 \cdot 10^{-6}}{\pm 8 \cdot 10^{-6}}{\pm 30 \cdot 10^{-6}}
\dxQuantDef{Gamma820}{\BR_{820}}{\BR(\tau^- \to 3\pi^- 2\pi^+ \nu_\tau\;(\text{ex.}K^0,\omega))}{(827 \pm 31)\cdot 10^{-6}}{827 \cdot 10^{-6}}{\pm 31 \cdot 10^{-6}}
\dxQuantDef{Gamma821}{\BR_{821}}{\BR(\tau^- \to 3\pi^- 2\pi^+ \nu_\tau\;(\text{ex.}K^0,\omega,f_1))}{(775 \pm 30)\cdot 10^{-6}}{775 \cdot 10^{-6}}{\pm 30 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma821.pub.LEES.12X}{Gamma821}{LEES 12X}{(768 \pm 4 \pm 40)\cdot 10^{-6}}{768 \cdot 10^{-6}}{\pm 4 \cdot 10^{-6}}{\pm 40 \cdot 10^{-6}}
\dxQuantDef{Gamma822}{\BR_{822}}{\BR(\tau^- \to K^- 2\pi^- 2\pi^+ \nu_\tau\;(\text{ex.}K^0))}{(0.6 \pm 1.2)\cdot 10^{-6}}{0.6 \cdot 10^{-6}}{\pm 1.2 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma822.pub.LEES.12X}{Gamma822}{LEES 12X}{(0.6 \pm 0.5 \pm 1.1)\cdot 10^{-6}}{0.6 \cdot 10^{-6}}{\pm 0.5 \cdot 10^{-6}}{\pm 1.1 \cdot 10^{-6}}
\dxQuantDef{Gamma830}{\BR_{830}}{\BR(\tau^- \to 3\pi^- 2\pi^+ \pi^0 \nu_\tau\;(\text{ex.}K^0))}{(164 \pm 11)\cdot 10^{-6}}{164 \cdot 10^{-6}}{\pm 11 \cdot 10^{-6}}
\dxQuantDef{Gamma831}{\BR_{831}}{\BR(\tau^- \to 2\pi^- \pi^+ \omega \nu_\tau\;(\text{ex.}K^0))}{(84 \pm 6)\cdot 10^{-6}}{84 \cdot 10^{-6}}{\pm 6 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma831.pub.LEES.12X}{Gamma831}{LEES 12X}{(84 \pm 4 \pm 6)\cdot 10^{-6}}{84 \cdot 10^{-6}}{\pm 4 \cdot 10^{-6}}{\pm 6 \cdot 10^{-6}}
\dxQuantDef{Gamma832}{\BR_{832}}{\BR(\tau^- \to 3\pi^- 2\pi^+ \pi^0 \nu_\tau\;(\text{ex.}K^0,\eta,\omega,f_1))}{(37.7 \pm 8.7)\cdot 10^{-6}}{37.7 \cdot 10^{-6}}{\pm 8.7 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma832.pub.LEES.12X}{Gamma832}{LEES 12X}{(36.0 \pm 3.0 \pm 9.0)\cdot 10^{-6}}{36.0 \cdot 10^{-6}}{\pm 3.0 \cdot 10^{-6}}{\pm 9.0 \cdot 10^{-6}}
\dxQuantDef{Gamma833}{\BR_{833}}{\BR(\tau^- \to K^- 2\pi^- 2\pi^+ \pi^0 \nu_\tau\;(\text{ex.}K^0))}{(1.1 \pm 0.6)\cdot 10^{-6}}{1.1 \cdot 10^{-6}}{\pm 0.6 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma833.pub.LEES.12X}{Gamma833}{LEES 12X}{(1.1 \pm 0.4 \pm 0.4)\cdot 10^{-6}}{1.1 \cdot 10^{-6}}{\pm 0.4 \cdot 10^{-6}}{\pm 0.4 \cdot 10^{-6}}
\dxQuantDef{Gamma910}{\BR_{910}}{\BR(\tau^- \to 2\pi^- \pi^+ \eta(3\pi^0) \nu_\tau\;(\text{ex.}K^0))}{(72 \pm 4)\cdot 10^{-6}}{72 \cdot 10^{-6}}{\pm 4 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma910.pub.LEES.12X}{Gamma910}{LEES 12X}{(83 \pm 9 \pm 8)\cdot 10^{-6}}{83 \cdot 10^{-6}}{\pm 9 \cdot 10^{-6}}{\pm 8 \cdot 10^{-6}}
\dxQuantDef{Gamma911}{\BR_{911}}{\BR(\tau^- \to \pi^- 2\pi^0 \eta(\pi^+ \pi^- \pi^0) \nu_\tau\;(\text{ex.}K^0))}{(45 \pm 9)\cdot 10^{-6}}{45 \cdot 10^{-6}}{\pm 9 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma911.pub.LEES.12X}{Gamma911}{LEES 12X}{(46 \pm 8 \pm 5)\cdot 10^{-6}}{46 \cdot 10^{-6}}{\pm 8 \cdot 10^{-6}}{\pm 5 \cdot 10^{-6}}
\dxQuantDef{Gamma920}{\BR_{920}}{\BR(\tau^- \to \pi^- f_1(2\pi^- 2\pi^+) \nu_\tau)}{(52.4 \pm 4.4)\cdot 10^{-6}}{52.4 \cdot 10^{-6}}{\pm 4.4 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma920.pub.LEES.12X}{Gamma920}{LEES 12X}{(52.0 \pm 3.1 \pm 3.7)\cdot 10^{-6}}{52.0 \cdot 10^{-6}}{\pm 3.1 \cdot 10^{-6}}{\pm 3.7 \cdot 10^{-6}}
\dxQuantDef{Gamma930}{\BR_{930}}{\BR(\tau^- \to 2\pi^- \pi^+ \eta(\pi^+ \pi^- \pi^0) \nu_\tau\;(\text{ex.}K^0))}{(50.7 \pm 3.0)\cdot 10^{-6}}{50.7 \cdot 10^{-6}}{\pm 3.0 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma930.pub.LEES.12X}{Gamma930}{LEES 12X}{(53.9 \pm 2.7 \pm 4.1)\cdot 10^{-6}}{53.9 \cdot 10^{-6}}{\pm 2.7 \cdot 10^{-6}}{\pm 4.1 \cdot 10^{-6}}
\dxQuantDef{Gamma944}{\BR_{944}}{\BR(\tau^- \to 2\pi^- \pi^+ \eta(\gamma \gamma) \nu_\tau\;(\text{ex.}K^0))}{(86.8 \pm 5.1)\cdot 10^{-6}}{86.8 \cdot 10^{-6}}{\pm 5.1 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma944.pub.LEES.12X}{Gamma944}{LEES 12X}{(82.6 \pm 3.5 \pm 5.1)\cdot 10^{-6}}{82.6 \cdot 10^{-6}}{\pm 3.5 \cdot 10^{-6}}{\pm 5.1 \cdot 10^{-6}}
\dxQuantDef{Gamma945}{\BR_{945}}{\BR(\tau^- \to \pi^- 2\pi^0 \eta \nu_\tau\;(\text{ex.}K^0))}{(0.19 \pm 0.04)\cdot 10^{-3}}{0.19 \cdot 10^{-3}}{\pm 0.04 \cdot 10^{-3}}
\dxQuantDef{GammaAll}{\BR_{\text{all}}}{\BR(\tau^- \to \text{all modes})}{1.0}{1.0}{0}
\dxQuantDef{Gamma980}{\BR_{980}}{\BR(a_1^- \to \pi^- \gamma)}{0.0022 \pm 0.0008}{0.0022}{\pm 0.0008}
\dxMeasDef{ALEPH.Gamma980.pub.SCHAEL.05C}{Gamma980}{SCHAEL 05C}{0.0021 \pm 0.0008 \pm 0.0000}{0.0021}{\pm 0.0008}{\pm 0.0000}
\dxdef{Gamma1-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma1-gn} = \dxuse{Gamma1-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma1}%
}
\dxdef{Gamma2-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma2-gn} = \dxuse{Gamma2-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma2}%
}
\dxdef{Gamma3-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma3-gn} = \dxuse{Gamma3-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma3} \\
\dxuse{ALEPH.Gamma3.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma3.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma3.pub.SCHAEL.05C-pdgref}-cite} \\
\dxuse{DELPHI.Gamma3.pub.ABREU.99X-vu} & \dxuse{\dxuse{DELPHI.Gamma3.pub.ABREU.99X-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma3.pub.ABREU.99X-pdgref}-cite} \\
\dxuse{L3.Gamma3.pub.ACCIARRI.01F-vu} & \dxuse{\dxuse{L3.Gamma3.pub.ACCIARRI.01F-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma3.pub.ACCIARRI.01F-pdgref}-cite} \\
\dxuse{OPAL.Gamma3.pub.ABBIENDI.03-vu} & \dxuse{\dxuse{OPAL.Gamma3.pub.ABBIENDI.03-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma3.pub.ABBIENDI.03-pdgref}-cite}%
}
\dxdef{Gamma3by5-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma3by5-gn} = \dxuse{Gamma3by5-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma3by5} \\
\dxuse{ARGUS.Gamma3by5.pub.ALBRECHT.92D-vu} & \dxuse{\dxuse{ARGUS.Gamma3by5.pub.ALBRECHT.92D-pdgref}-exp} & \dxuse{\dxuse{ARGUS.Gamma3by5.pub.ALBRECHT.92D-pdgref}-cite} \\
\dxuse{BaBar.Gamma3by5.pub.AUBERT.10F-vu} & \dxuse{\dxuse{BaBar.Gamma3by5.pub.AUBERT.10F-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma3by5.pub.AUBERT.10F-pdgref}-cite} \\
\dxuse{Belle2.Gamma3by5.ADACHI.2024-vu} & \dxuse{\dxuse{Belle2.Gamma3by5.ADACHI.2024-pdgref}-exp} & \dxuse{\dxuse{Belle2.Gamma3by5.ADACHI.2024-pdgref}-cite} \\
\dxuse{CLEO.Gamma3by5.pub.ANASTASSOV.97-vu} & \dxuse{\dxuse{CLEO.Gamma3by5.pub.ANASTASSOV.97-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma3by5.pub.ANASTASSOV.97-pdgref}-cite}%
}
\dxdef{Gamma5-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma5-gn} = \dxuse{Gamma5-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma5} \\
\dxuse{ALEPH.Gamma5.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma5.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma5.pub.SCHAEL.05C-pdgref}-cite} \\
\dxuse{CLEO.Gamma5.pub.ANASTASSOV.97-vu} & \dxuse{\dxuse{CLEO.Gamma5.pub.ANASTASSOV.97-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma5.pub.ANASTASSOV.97-pdgref}-cite} \\
\dxuse{DELPHI.Gamma5.pub.ABREU.99X-vu} & \dxuse{\dxuse{DELPHI.Gamma5.pub.ABREU.99X-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma5.pub.ABREU.99X-pdgref}-cite} \\
\dxuse{L3.Gamma5.pub.ACCIARRI.01F-vu} & \dxuse{\dxuse{L3.Gamma5.pub.ACCIARRI.01F-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma5.pub.ACCIARRI.01F-pdgref}-cite} \\
\dxuse{OPAL.Gamma5.pub.ABBIENDI.99H-vu} & \dxuse{\dxuse{OPAL.Gamma5.pub.ABBIENDI.99H-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma5.pub.ABBIENDI.99H-pdgref}-cite}%
}
\dxdef{Gamma7-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma7-gn} = \dxuse{Gamma7-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma7} \\
\dxuse{DELPHI.Gamma7.pub.ABREU.92N-vu} & \dxuse{\dxuse{DELPHI.Gamma7.pub.ABREU.92N-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma7.pub.ABREU.92N-pdgref}-cite} \\
\dxuse{L3.Gamma7.pub.ACCIARRI.95-vu} & \dxuse{\dxuse{L3.Gamma7.pub.ACCIARRI.95-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma7.pub.ACCIARRI.95-pdgref}-cite} \\
\dxuse{OPAL.Gamma7.pub.ALEXANDER.91D-vu} & \dxuse{\dxuse{OPAL.Gamma7.pub.ALEXANDER.91D-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma7.pub.ALEXANDER.91D-pdgref}-cite}%
}
\dxdef{Gamma8-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma8-gn} = \dxuse{Gamma8-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma8} \\
\dxuse{CLEO.Gamma8.pub.ANASTASSOV.97-vu} & \dxuse{\dxuse{CLEO.Gamma8.pub.ANASTASSOV.97-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma8.pub.ANASTASSOV.97-pdgref}-cite} \\
\dxuse{DELPHI.Gamma8.pub.ABDALLAH.06A-vu} & \dxuse{\dxuse{DELPHI.Gamma8.pub.ABDALLAH.06A-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma8.pub.ABDALLAH.06A-pdgref}-cite} \\
\dxuse{OPAL.Gamma8.pub.ACKERSTAFF.98M-vu} & \dxuse{\dxuse{OPAL.Gamma8.pub.ACKERSTAFF.98M-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma8.pub.ACKERSTAFF.98M-pdgref}-cite}%
}
\dxdef{Gamma8by5-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma8by5-gn} = \dxuse{Gamma8by5-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma8by5}%
}
\dxdef{Gamma9-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma9-gn} = \dxuse{Gamma9-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma9} \\
\dxuse{ALEPH.Gamma9.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma9.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma9.pub.SCHAEL.05C-pdgref}-cite}%
}
\dxdef{Gamma9by5-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma9by5-gn} = \dxuse{Gamma9by5-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma9by5} \\
\dxuse{BaBar.Gamma9by5.pub.AUBERT.10F-vu} & \dxuse{\dxuse{BaBar.Gamma9by5.pub.AUBERT.10F-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma9by5.pub.AUBERT.10F-pdgref}-cite}%
}
\dxdef{Gamma10-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma10-gn} = \dxuse{Gamma10-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma10} \\
\dxuse{ALEPH.Gamma10.pub.BARATE.99K-vu} & \dxuse{\dxuse{ALEPH.Gamma10.pub.BARATE.99K-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma10.pub.BARATE.99K-pdgref}-cite} \\
\dxuse{CLEO.Gamma10.pub.BATTLE.94-vu} & \dxuse{\dxuse{CLEO.Gamma10.pub.BATTLE.94-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma10.pub.BATTLE.94-pdgref}-cite} \\
\dxuse{DELPHI.Gamma10.pub.ABREU.94K-vu} & \dxuse{\dxuse{DELPHI.Gamma10.pub.ABREU.94K-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma10.pub.ABREU.94K-pdgref}-cite} \\
\dxuse{OPAL.Gamma10.pub.ABBIENDI.01J-vu} & \dxuse{\dxuse{OPAL.Gamma10.pub.ABBIENDI.01J-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma10.pub.ABBIENDI.01J-pdgref}-cite}%
}
\dxdef{Gamma10by5-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma10by5-gn} = \dxuse{Gamma10by5-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma10by5} \\
\dxuse{BaBar.Gamma10by5.pub.AUBERT.10F-vu} & \dxuse{\dxuse{BaBar.Gamma10by5.pub.AUBERT.10F-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma10by5.pub.AUBERT.10F-pdgref}-cite}%
}
\dxdef{Gamma10by9-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma10by9-gn} = \dxuse{Gamma10by9-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma10by9}%
}
\dxdef{Gamma11-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma11-gn} = \dxuse{Gamma11-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma11}%
}
\dxdef{Gamma12-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma12-gn} = \dxuse{Gamma12-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma12}%
}
\dxdef{Gamma13-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma13-gn} = \dxuse{Gamma13-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma13} \\
\dxuse{Belle.Gamma13.pub.FUJIKAWA.08-vu} & \dxuse{\dxuse{Belle.Gamma13.pub.FUJIKAWA.08-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma13.pub.FUJIKAWA.08-pdgref}-cite} \\
\dxuse{CLEO.Gamma13.pub.ARTUSO.94-vu} & \dxuse{\dxuse{CLEO.Gamma13.pub.ARTUSO.94-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma13.pub.ARTUSO.94-pdgref}-cite} \\
\dxuse{DELPHI.Gamma13.pub.ABDALLAH.06A-vu} & \dxuse{\dxuse{DELPHI.Gamma13.pub.ABDALLAH.06A-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma13.pub.ABDALLAH.06A-pdgref}-cite} \\
\dxuse{L3.Gamma13.pub.ACCIARRI.95-vu} & \dxuse{\dxuse{L3.Gamma13.pub.ACCIARRI.95-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma13.pub.ACCIARRI.95-pdgref}-cite} \\
\dxuse{OPAL.Gamma13.pub.ACKERSTAFF.98M-vu} & \dxuse{\dxuse{OPAL.Gamma13.pub.ACKERSTAFF.98M-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma13.pub.ACKERSTAFF.98M-pdgref}-cite}%
}
\dxdef{Gamma14-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma14-gn} = \dxuse{Gamma14-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma14} \\
\dxuse{ALEPH.Gamma14.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma14.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma14.pub.SCHAEL.05C-pdgref}-cite}%
}
\dxdef{Gamma16-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma16-gn} = \dxuse{Gamma16-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma16} \\
\dxuse{ALEPH.Gamma16.pub.BARATE.99K-vu} & \dxuse{\dxuse{ALEPH.Gamma16.pub.BARATE.99K-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma16.pub.BARATE.99K-pdgref}-cite} \\
\dxuse{BaBar.Gamma16.pub.AUBERT.07AP-vu} & \dxuse{\dxuse{BaBar.Gamma16.pub.AUBERT.07AP-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma16.pub.AUBERT.07AP-pdgref}-cite} \\
\dxuse{CLEO.Gamma16.pub.BATTLE.94-vu} & \dxuse{\dxuse{CLEO.Gamma16.pub.BATTLE.94-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma16.pub.BATTLE.94-pdgref}-cite} \\
\dxuse{OPAL.Gamma16.pub.ABBIENDI.04J-vu} & \dxuse{\dxuse{OPAL.Gamma16.pub.ABBIENDI.04J-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma16.pub.ABBIENDI.04J-pdgref}-cite}%
}
\dxdef{Gamma17-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma17-gn} = \dxuse{Gamma17-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma17} \\
\dxuse{OPAL.Gamma17.pub.ACKERSTAFF.98M-vu} & \dxuse{\dxuse{OPAL.Gamma17.pub.ACKERSTAFF.98M-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma17.pub.ACKERSTAFF.98M-pdgref}-cite}%
}
\dxdef{Gamma18-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma18-gn} = \dxuse{Gamma18-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma18}%
}
\dxdef{Gamma19-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma19-gn} = \dxuse{Gamma19-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma19} \\
\dxuse{DELPHI.Gamma19.pub.ABDALLAH.06A-vu} & \dxuse{\dxuse{DELPHI.Gamma19.pub.ABDALLAH.06A-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma19.pub.ABDALLAH.06A-pdgref}-cite} \\
\dxuse{L3.Gamma19.pub.ACCIARRI.95-vu} & \dxuse{\dxuse{L3.Gamma19.pub.ACCIARRI.95-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma19.pub.ACCIARRI.95-pdgref}-cite}%
}
\dxdef{Gamma19by13-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma19by13-gn} = \dxuse{Gamma19by13-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma19by13} \\
\dxuse{CLEO.Gamma19by13.pub.PROCARIO.93-vu} & \dxuse{\dxuse{CLEO.Gamma19by13.pub.PROCARIO.93-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma19by13.pub.PROCARIO.93-pdgref}-cite}%
}
\dxdef{Gamma20-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma20-gn} = \dxuse{Gamma20-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma20} \\
\dxuse{ALEPH.Gamma20.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma20.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma20.pub.SCHAEL.05C-pdgref}-cite}%
}
\dxdef{Gamma23-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma23-gn} = \dxuse{Gamma23-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma23} \\
\dxuse{ALEPH.Gamma23.pub.BARATE.99K-vu} & \dxuse{\dxuse{ALEPH.Gamma23.pub.BARATE.99K-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma23.pub.BARATE.99K-pdgref}-cite} \\
\dxuse{CLEO.Gamma23.pub.BATTLE.94-vu} & \dxuse{\dxuse{CLEO.Gamma23.pub.BATTLE.94-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma23.pub.BATTLE.94-pdgref}-cite}%
}
\dxdef{Gamma24-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma24-gn} = \dxuse{Gamma24-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma24}%
}
\dxdef{Gamma25-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma25-gn} = \dxuse{Gamma25-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma25} \\
\dxuse{DELPHI.Gamma25.pub.ABDALLAH.06A-vu} & \dxuse{\dxuse{DELPHI.Gamma25.pub.ABDALLAH.06A-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma25.pub.ABDALLAH.06A-pdgref}-cite}%
}
\dxdef{Gamma26-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma26-gn} = \dxuse{Gamma26-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma26} \\
\dxuse{L3.Gamma26.pub.ACCIARRI.95-vu} & \dxuse{\dxuse{L3.Gamma26.pub.ACCIARRI.95-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma26.pub.ACCIARRI.95-pdgref}-cite}%
}
\dxdef{Gamma26by13-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma26by13-gn} = \dxuse{Gamma26by13-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma26by13} \\
\dxuse{CLEO.Gamma26by13.pub.PROCARIO.93-vu} & \dxuse{\dxuse{CLEO.Gamma26by13.pub.PROCARIO.93-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma26by13.pub.PROCARIO.93-pdgref}-cite}%
}
\dxdef{Gamma27-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma27-gn} = \dxuse{Gamma27-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma27} \\
\dxuse{ALEPH.Gamma27.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma27.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma27.pub.SCHAEL.05C-pdgref}-cite}%
}
\dxdef{Gamma28-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma28-gn} = \dxuse{Gamma28-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma28} \\
\dxuse{ALEPH.Gamma28.pub.BARATE.99K-vu} & \dxuse{\dxuse{ALEPH.Gamma28.pub.BARATE.99K-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma28.pub.BARATE.99K-pdgref}-cite}%
}
\dxdef{Gamma29-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma29-gn} = \dxuse{Gamma29-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma29} \\
\dxuse{CLEO.Gamma29.pub.PROCARIO.93-vu} & \dxuse{\dxuse{CLEO.Gamma29.pub.PROCARIO.93-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma29.pub.PROCARIO.93-pdgref}-cite}%
}
\dxdef{Gamma30-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma30-gn} = \dxuse{Gamma30-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma30} \\
\dxuse{ALEPH.Gamma30.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma30.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma30.pub.SCHAEL.05C-pdgref}-cite}%
}
\dxdef{Gamma31-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma31-gn} = \dxuse{Gamma31-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma31} \\
\dxuse{CLEO.Gamma31.pub.BATTLE.94-vu} & \dxuse{\dxuse{CLEO.Gamma31.pub.BATTLE.94-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma31.pub.BATTLE.94-pdgref}-cite} \\
\dxuse{DELPHI.Gamma31.pub.ABREU.94K-vu} & \dxuse{\dxuse{DELPHI.Gamma31.pub.ABREU.94K-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma31.pub.ABREU.94K-pdgref}-cite} \\
\dxuse{OPAL.Gamma31.pub.ABBIENDI.01J-vu} & \dxuse{\dxuse{OPAL.Gamma31.pub.ABBIENDI.01J-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma31.pub.ABBIENDI.01J-pdgref}-cite}%
}
\dxdef{Gamma32-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma32-gn} = \dxuse{Gamma32-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma32}%
}
\dxdef{Gamma33-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma33-gn} = \dxuse{Gamma33-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma33} \\
\dxuse{ALEPH.Gamma33.pub.BARATE.98E-vu} & \dxuse{\dxuse{ALEPH.Gamma33.pub.BARATE.98E-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma33.pub.BARATE.98E-pdgref}-cite} \\
\dxuse{OPAL.Gamma33.pub.AKERS.94G-vu} & \dxuse{\dxuse{OPAL.Gamma33.pub.AKERS.94G-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma33.pub.AKERS.94G-pdgref}-cite}%
}
\dxdef{Gamma34-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma34-gn} = \dxuse{Gamma34-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma34} \\
\dxuse{CLEO.Gamma34.pub.COAN.96-vu} & \dxuse{\dxuse{CLEO.Gamma34.pub.COAN.96-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma34.pub.COAN.96-pdgref}-cite}%
}
\dxdef{Gamma35-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma35-gn} = \dxuse{Gamma35-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma35} \\
\dxuse{ALEPH.Gamma35.pub.BARATE.99K-vu} & \dxuse{\dxuse{ALEPH.Gamma35.pub.BARATE.99K-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma35.pub.BARATE.99K-pdgref}-cite} \\
\dxuse{Belle.Gamma35.pub.RYU.14vpc-vu} & \dxuse{\dxuse{Belle.Gamma35.pub.RYU.14vpc-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma35.pub.RYU.14vpc-pdgref}-cite} \\
\dxuse{L3.Gamma35.pub.ACCIARRI.95F-vu} & \dxuse{\dxuse{L3.Gamma35.pub.ACCIARRI.95F-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma35.pub.ACCIARRI.95F-pdgref}-cite} \\
\dxuse{OPAL.Gamma35.pub.ABBIENDI.00C-vu} & \dxuse{\dxuse{OPAL.Gamma35.pub.ABBIENDI.00C-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma35.pub.ABBIENDI.00C-pdgref}-cite}%
}
\dxdef{Gamma37-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma37-gn} = \dxuse{Gamma37-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma37} \\
\dxuse{ALEPH.Gamma37.pub.BARATE.98E-vu} & \dxuse{\dxuse{ALEPH.Gamma37.pub.BARATE.98E-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma37.pub.BARATE.98E-pdgref}-cite} \\
\dxuse{ALEPH.Gamma37.pub.BARATE.99K-vu} & \dxuse{\dxuse{ALEPH.Gamma37.pub.BARATE.99K-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma37.pub.BARATE.99K-pdgref}-cite} \\
\dxuse{BaBar.Gamma37.pub.LEES.18B-vu} & \dxuse{\dxuse{BaBar.Gamma37.pub.LEES.18B-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma37.pub.LEES.18B-pdgref}-cite} \\
\dxuse{Belle.Gamma37.pub.RYU.14vpc-vu} & \dxuse{\dxuse{Belle.Gamma37.pub.RYU.14vpc-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma37.pub.RYU.14vpc-pdgref}-cite} \\
\dxuse{CLEO.Gamma37.pub.COAN.96-vu} & \dxuse{\dxuse{CLEO.Gamma37.pub.COAN.96-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma37.pub.COAN.96-pdgref}-cite}%
}
\dxdef{Gamma38-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma38-gn} = \dxuse{Gamma38-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma38} \\
\dxuse{OPAL.Gamma38.pub.ABBIENDI.00C-vu} & \dxuse{\dxuse{OPAL.Gamma38.pub.ABBIENDI.00C-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma38.pub.ABBIENDI.00C-pdgref}-cite}%
}
\dxdef{Gamma39-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma39-gn} = \dxuse{Gamma39-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma39} \\
\dxuse{CLEO.Gamma39.pub.COAN.96-vu} & \dxuse{\dxuse{CLEO.Gamma39.pub.COAN.96-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma39.pub.COAN.96-pdgref}-cite}%
}
\dxdef{Gamma40-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma40-gn} = \dxuse{Gamma40-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma40} \\
\dxuse{ALEPH.Gamma40.pub.BARATE.98E-vu} & \dxuse{\dxuse{ALEPH.Gamma40.pub.BARATE.98E-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma40.pub.BARATE.98E-pdgref}-cite} \\
\dxuse{ALEPH.Gamma40.pub.BARATE.99K-vu} & \dxuse{\dxuse{ALEPH.Gamma40.pub.BARATE.99K-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma40.pub.BARATE.99K-pdgref}-cite} \\
\dxuse{Belle.Gamma40.pub.RYU.14vpc-vu} & \dxuse{\dxuse{Belle.Gamma40.pub.RYU.14vpc-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma40.pub.RYU.14vpc-pdgref}-cite} \\
\dxuse{L3.Gamma40.pub.ACCIARRI.95F-vu} & \dxuse{\dxuse{L3.Gamma40.pub.ACCIARRI.95F-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma40.pub.ACCIARRI.95F-pdgref}-cite}%
}
\dxdef{Gamma42-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma42-gn} = \dxuse{Gamma42-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma42} \\
\dxuse{ALEPH.Gamma42.pub.BARATE.98E-vu} & \dxuse{\dxuse{ALEPH.Gamma42.pub.BARATE.98E-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma42.pub.BARATE.98E-pdgref}-cite} \\
\dxuse{ALEPH.Gamma42.pub.BARATE.99K-vu} & \dxuse{\dxuse{ALEPH.Gamma42.pub.BARATE.99K-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma42.pub.BARATE.99K-pdgref}-cite} \\
\dxuse{Belle.Gamma42.pub.RYU.14vpc-vu} & \dxuse{\dxuse{Belle.Gamma42.pub.RYU.14vpc-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma42.pub.RYU.14vpc-pdgref}-cite} \\
\dxuse{CLEO.Gamma42.pub.COAN.96-vu} & \dxuse{\dxuse{CLEO.Gamma42.pub.COAN.96-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma42.pub.COAN.96-pdgref}-cite}%
}
\dxdef{Gamma43-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma43-gn} = \dxuse{Gamma43-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma43} \\
\dxuse{OPAL.Gamma43.pub.ABBIENDI.00C-vu} & \dxuse{\dxuse{OPAL.Gamma43.pub.ABBIENDI.00C-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma43.pub.ABBIENDI.00C-pdgref}-cite}%
}
\dxdef{Gamma44-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma44-gn} = \dxuse{Gamma44-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma44} \\
\dxuse{ALEPH.Gamma44.pub.BARATE.99R-vu} & \dxuse{\dxuse{ALEPH.Gamma44.pub.BARATE.99R-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma44.pub.BARATE.99R-pdgref}-cite}%
}
\dxdef{Gamma46-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma46-gn} = \dxuse{Gamma46-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma46}%
}
\dxdef{Gamma47-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma47-gn} = \dxuse{Gamma47-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma47} \\
\dxuse{ALEPH.Gamma47.pub.BARATE.98E-vu} & \dxuse{\dxuse{ALEPH.Gamma47.pub.BARATE.98E-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma47.pub.BARATE.98E-pdgref}-cite} \\
\dxuse{BaBar.Gamma47.pub.LEES.12Y-vu} & \dxuse{\dxuse{BaBar.Gamma47.pub.LEES.12Y-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma47.pub.LEES.12Y-pdgref}-cite} \\
\dxuse{Belle.Gamma47.pub.RYU.14vpc-vu} & \dxuse{\dxuse{Belle.Gamma47.pub.RYU.14vpc-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma47.pub.RYU.14vpc-pdgref}-cite} \\
\dxuse{CLEO.Gamma47.pub.COAN.96-vu} & \dxuse{\dxuse{CLEO.Gamma47.pub.COAN.96-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma47.pub.COAN.96-pdgref}-cite}%
}
\dxdef{Gamma48-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma48-gn} = \dxuse{Gamma48-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma48} \\
\dxuse{ALEPH.Gamma48.pub.BARATE.98E-vu} & \dxuse{\dxuse{ALEPH.Gamma48.pub.BARATE.98E-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma48.pub.BARATE.98E-pdgref}-cite}%
}
\dxdef{Gamma49-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma49-gn} = \dxuse{Gamma49-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma49}%
}
\dxdef{Gamma50-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma50-gn} = \dxuse{Gamma50-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma50} \\
\dxuse{BaBar.Gamma50.pub.LEES.12Y-vu} & \dxuse{\dxuse{BaBar.Gamma50.pub.LEES.12Y-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma50.pub.LEES.12Y-pdgref}-cite} \\
\dxuse{Belle.Gamma50.pub.RYU.14vpc-vu} & \dxuse{\dxuse{Belle.Gamma50.pub.RYU.14vpc-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma50.pub.RYU.14vpc-pdgref}-cite}%
}
\dxdef{Gamma51-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma51-gn} = \dxuse{Gamma51-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma51} \\
\dxuse{ALEPH.Gamma51.pub.BARATE.98E-vu} & \dxuse{\dxuse{ALEPH.Gamma51.pub.BARATE.98E-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma51.pub.BARATE.98E-pdgref}-cite}%
}
\dxdef{Gamma53-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma53-gn} = \dxuse{Gamma53-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma53} \\
\dxuse{ALEPH.Gamma53.pub.BARATE.98E-vu} & \dxuse{\dxuse{ALEPH.Gamma53.pub.BARATE.98E-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma53.pub.BARATE.98E-pdgref}-cite}%
}
\dxdef{Gamma54-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma54-gn} = \dxuse{Gamma54-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma54} \\
\dxuse{CELLO.Gamma54.pub.BEHREND.89B-vu} & \dxuse{\dxuse{CELLO.Gamma54.pub.BEHREND.89B-pdgref}-exp} & \dxuse{\dxuse{CELLO.Gamma54.pub.BEHREND.89B-pdgref}-cite} \\
\dxuse{L3.Gamma54.pub.ADEVA.91F-vu} & \dxuse{\dxuse{L3.Gamma54.pub.ADEVA.91F-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma54.pub.ADEVA.91F-pdgref}-cite} \\
\dxuse{TPC.Gamma54.pub.AIHARA.87B-vu} & \dxuse{\dxuse{TPC.Gamma54.pub.AIHARA.87B-pdgref}-exp} & \dxuse{\dxuse{TPC.Gamma54.pub.AIHARA.87B-pdgref}-cite}%
}
\dxdef{Gamma55-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma55-gn} = \dxuse{Gamma55-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma55} \\
\dxuse{L3.Gamma55.pub.ACHARD.01D-vu} & \dxuse{\dxuse{L3.Gamma55.pub.ACHARD.01D-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma55.pub.ACHARD.01D-pdgref}-cite} \\
\dxuse{OPAL.Gamma55.pub.AKERS.95Y-vu} & \dxuse{\dxuse{OPAL.Gamma55.pub.AKERS.95Y-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma55.pub.AKERS.95Y-pdgref}-cite}%
}
\dxdef{Gamma56-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma56-gn} = \dxuse{Gamma56-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma56}%
}
\dxdef{Gamma57-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma57-gn} = \dxuse{Gamma57-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma57} \\
\dxuse{CLEO.Gamma57.pub.BALEST.95C-vu} & \dxuse{\dxuse{CLEO.Gamma57.pub.BALEST.95C-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma57.pub.BALEST.95C-pdgref}-cite} \\
\dxuse{DELPHI.Gamma57.pub.ABDALLAH.06A-vu} & \dxuse{\dxuse{DELPHI.Gamma57.pub.ABDALLAH.06A-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma57.pub.ABDALLAH.06A-pdgref}-cite}%
}
\dxdef{Gamma57by55-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma57by55-gn} = \dxuse{Gamma57by55-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma57by55} \\
\dxuse{OPAL.Gamma57by55.pub.AKERS.95Y-vu} & \dxuse{\dxuse{OPAL.Gamma57by55.pub.AKERS.95Y-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma57by55.pub.AKERS.95Y-pdgref}-cite}%
}
\dxdef{Gamma58-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma58-gn} = \dxuse{Gamma58-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma58}%
}
\dxdef{Gamma59-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma59-gn} = \dxuse{Gamma59-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma59}%
}
\dxdef{Gamma60-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma60-gn} = \dxuse{Gamma60-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma60} \\
\dxuse{BaBar.Gamma60.pub.AUBERT.08-vu} & \dxuse{\dxuse{BaBar.Gamma60.pub.AUBERT.08-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma60.pub.AUBERT.08-pdgref}-cite} \\
\dxuse{Belle.Gamma60.pub.LEE.10-vu} & \dxuse{\dxuse{Belle.Gamma60.pub.LEE.10-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma60.pub.LEE.10-pdgref}-cite} \\
\dxuse{CLEO3.Gamma60.pub.BRIERE.03-vu} & \dxuse{\dxuse{CLEO3.Gamma60.pub.BRIERE.03-pdgref}-exp} & \dxuse{\dxuse{CLEO3.Gamma60.pub.BRIERE.03-pdgref}-cite}%
}
\dxdef{Gamma62-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma62-gn} = \dxuse{Gamma62-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma62} \\
\dxuse{ALEPH.Gamma62.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma62.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma62.pub.SCHAEL.05C-pdgref}-cite}%
}
\dxdef{Gamma63-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma63-gn} = \dxuse{Gamma63-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma63}%
}
\dxdef{Gamma64-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma64-gn} = \dxuse{Gamma64-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma64}%
}
\dxdef{Gamma65-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma65-gn} = \dxuse{Gamma65-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma65}%
}
\dxdef{Gamma66-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma66-gn} = \dxuse{Gamma66-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma66} \\
\dxuse{CLEO.Gamma66.pub.BALEST.95C-vu} & \dxuse{\dxuse{CLEO.Gamma66.pub.BALEST.95C-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma66.pub.BALEST.95C-pdgref}-cite} \\
\dxuse{DELPHI.Gamma66.pub.ABDALLAH.06A-vu} & \dxuse{\dxuse{DELPHI.Gamma66.pub.ABDALLAH.06A-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma66.pub.ABDALLAH.06A-pdgref}-cite}%
}
\dxdef{Gamma67-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma67-gn} = \dxuse{Gamma67-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma67}%
}
\dxdef{Gamma68-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma68-gn} = \dxuse{Gamma68-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma68}%
}
\dxdef{Gamma69-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma69-gn} = \dxuse{Gamma69-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma69} \\
\dxuse{ALEPH.Gamma69.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma69.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma69.pub.SCHAEL.05C-pdgref}-cite} \\
\dxuse{CLEO.Gamma69.pub.EDWARDS.00A-vu} & \dxuse{\dxuse{CLEO.Gamma69.pub.EDWARDS.00A-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma69.pub.EDWARDS.00A-pdgref}-cite}%
}
\dxdef{Gamma70-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma70-gn} = \dxuse{Gamma70-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma70}%
}
\dxdef{Gamma74-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma74-gn} = \dxuse{Gamma74-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma74} \\
\dxuse{DELPHI.Gamma74.pub.ABDALLAH.06A-vu} & \dxuse{\dxuse{DELPHI.Gamma74.pub.ABDALLAH.06A-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma74.pub.ABDALLAH.06A-pdgref}-cite}%
}
\dxdef{Gamma75-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma75-gn} = \dxuse{Gamma75-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma75}%
}
\dxdef{Gamma76-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma76-gn} = \dxuse{Gamma76-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma76} \\
\dxuse{ALEPH.Gamma76.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma76.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma76.pub.SCHAEL.05C-pdgref}-cite}%
}
\dxdef{Gamma76by54-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma76by54-gn} = \dxuse{Gamma76by54-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma76by54} \\
\dxuse{CLEO.Gamma76by54.pub.BORTOLETTO.93-vu} & \dxuse{\dxuse{CLEO.Gamma76by54.pub.BORTOLETTO.93-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma76by54.pub.BORTOLETTO.93-pdgref}-cite}%
}
\dxdef{Gamma77-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma77-gn} = \dxuse{Gamma77-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma77}%
}
\dxdef{Gamma78-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma78-gn} = \dxuse{Gamma78-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma78} \\
\dxuse{CLEO.Gamma78.pub.ANASTASSOV.01-vu} & \dxuse{\dxuse{CLEO.Gamma78.pub.ANASTASSOV.01-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma78.pub.ANASTASSOV.01-pdgref}-cite}%
}
\dxdef{Gamma79-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma79-gn} = \dxuse{Gamma79-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma79}%
}
\dxdef{Gamma80-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma80-gn} = \dxuse{Gamma80-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma80}%
}
\dxdef{Gamma80by60-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma80by60-gn} = \dxuse{Gamma80by60-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma80by60} \\
\dxuse{CLEO.Gamma80by60.pub.RICHICHI.99-vu} & \dxuse{\dxuse{CLEO.Gamma80by60.pub.RICHICHI.99-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma80by60.pub.RICHICHI.99-pdgref}-cite}%
}
\dxdef{Gamma81-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma81-gn} = \dxuse{Gamma81-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma81}%
}
\dxdef{Gamma81by69-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma81by69-gn} = \dxuse{Gamma81by69-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma81by69} \\
\dxuse{CLEO.Gamma81by69.pub.RICHICHI.99-vu} & \dxuse{\dxuse{CLEO.Gamma81by69.pub.RICHICHI.99-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma81by69.pub.RICHICHI.99-pdgref}-cite}%
}
\dxdef{Gamma82-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma82-gn} = \dxuse{Gamma82-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma82} \\
\dxuse{TPC.Gamma82.pub.BAUER.94-vu} & \dxuse{\dxuse{TPC.Gamma82.pub.BAUER.94-pdgref}-exp} & \dxuse{\dxuse{TPC.Gamma82.pub.BAUER.94-pdgref}-cite}%
}
\dxdef{Gamma83-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma83-gn} = \dxuse{Gamma83-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma83}%
}
\dxdef{Gamma84-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma84-gn} = \dxuse{Gamma84-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma84}%
}
\dxdef{Gamma85-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma85-gn} = \dxuse{Gamma85-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma85} \\
\dxuse{ALEPH.Gamma85.pub.BARATE.98-vu} & \dxuse{\dxuse{ALEPH.Gamma85.pub.BARATE.98-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma85.pub.BARATE.98-pdgref}-cite} \\
\dxuse{BaBar.Gamma85.pub.AUBERT.08-vu} & \dxuse{\dxuse{BaBar.Gamma85.pub.AUBERT.08-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma85.pub.AUBERT.08-pdgref}-cite} \\
\dxuse{Belle.Gamma85.pub.LEE.10-vu} & \dxuse{\dxuse{Belle.Gamma85.pub.LEE.10-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma85.pub.LEE.10-pdgref}-cite} \\
\dxuse{CLEO3.Gamma85.pub.BRIERE.03-vu} & \dxuse{\dxuse{CLEO3.Gamma85.pub.BRIERE.03-pdgref}-exp} & \dxuse{\dxuse{CLEO3.Gamma85.pub.BRIERE.03-pdgref}-cite} \\
\dxuse{OPAL.Gamma85.pub.ABBIENDI.04J-vu} & \dxuse{\dxuse{OPAL.Gamma85.pub.ABBIENDI.04J-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma85.pub.ABBIENDI.04J-pdgref}-cite}%
}
\dxdef{Gamma85by60-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma85by60-gn} = \dxuse{Gamma85by60-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma85by60}%
}
\dxdef{Gamma87-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma87-gn} = \dxuse{Gamma87-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma87}%
}
\dxdef{Gamma88-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma88-gn} = \dxuse{Gamma88-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma88} \\
\dxuse{ALEPH.Gamma88.pub.BARATE.98-vu} & \dxuse{\dxuse{ALEPH.Gamma88.pub.BARATE.98-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma88.pub.BARATE.98-pdgref}-cite} \\
\dxuse{CLEO3.Gamma88.pub.ARMS.05-vu} & \dxuse{\dxuse{CLEO3.Gamma88.pub.ARMS.05-pdgref}-exp} & \dxuse{\dxuse{CLEO3.Gamma88.pub.ARMS.05-pdgref}-cite}%
}
\dxdef{Gamma89-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma89-gn} = \dxuse{Gamma89-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma89}%
}
\dxdef{Gamma92-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma92-gn} = \dxuse{Gamma92-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma92} \\
\dxuse{OPAL.Gamma92.pub.ABBIENDI.00D-vu} & \dxuse{\dxuse{OPAL.Gamma92.pub.ABBIENDI.00D-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma92.pub.ABBIENDI.00D-pdgref}-cite} \\
\dxuse{TPC.Gamma92.pub.BAUER.94-vu} & \dxuse{\dxuse{TPC.Gamma92.pub.BAUER.94-pdgref}-exp} & \dxuse{\dxuse{TPC.Gamma92.pub.BAUER.94-pdgref}-cite}%
}
\dxdef{Gamma93-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma93-gn} = \dxuse{Gamma93-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma93} \\
\dxuse{ALEPH.Gamma93.pub.BARATE.98-vu} & \dxuse{\dxuse{ALEPH.Gamma93.pub.BARATE.98-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma93.pub.BARATE.98-pdgref}-cite} \\
\dxuse{BaBar.Gamma93.pub.AUBERT.08-vu} & \dxuse{\dxuse{BaBar.Gamma93.pub.AUBERT.08-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma93.pub.AUBERT.08-pdgref}-cite} \\
\dxuse{Belle.Gamma93.pub.LEE.10-vu} & \dxuse{\dxuse{Belle.Gamma93.pub.LEE.10-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma93.pub.LEE.10-pdgref}-cite} \\
\dxuse{CLEO3.Gamma93.pub.BRIERE.03-vu} & \dxuse{\dxuse{CLEO3.Gamma93.pub.BRIERE.03-pdgref}-exp} & \dxuse{\dxuse{CLEO3.Gamma93.pub.BRIERE.03-pdgref}-cite}%
}
\dxdef{Gamma93by60-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma93by60-gn} = \dxuse{Gamma93by60-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma93by60} \\
\dxuse{CLEO.Gamma93by60.pub.RICHICHI.99-vu} & \dxuse{\dxuse{CLEO.Gamma93by60.pub.RICHICHI.99-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma93by60.pub.RICHICHI.99-pdgref}-cite}%
}
\dxdef{Gamma94-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma94-gn} = \dxuse{Gamma94-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma94} \\
\dxuse{ALEPH.Gamma94.pub.BARATE.98-vu} & \dxuse{\dxuse{ALEPH.Gamma94.pub.BARATE.98-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma94.pub.BARATE.98-pdgref}-cite} \\
\dxuse{CLEO3.Gamma94.pub.ARMS.05-vu} & \dxuse{\dxuse{CLEO3.Gamma94.pub.ARMS.05-pdgref}-exp} & \dxuse{\dxuse{CLEO3.Gamma94.pub.ARMS.05-pdgref}-cite}%
}
\dxdef{Gamma94by69-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma94by69-gn} = \dxuse{Gamma94by69-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma94by69} \\
\dxuse{CLEO.Gamma94by69.pub.RICHICHI.99-vu} & \dxuse{\dxuse{CLEO.Gamma94by69.pub.RICHICHI.99-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma94by69.pub.RICHICHI.99-pdgref}-cite}%
}
\dxdef{Gamma96-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma96-gn} = \dxuse{Gamma96-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma96} \\
\dxuse{BaBar.Gamma96.pub.AUBERT.08-vu} & \dxuse{\dxuse{BaBar.Gamma96.pub.AUBERT.08-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma96.pub.AUBERT.08-pdgref}-cite} \\
\dxuse{Belle.Gamma96.pub.LEE.10-vu} & \dxuse{\dxuse{Belle.Gamma96.pub.LEE.10-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma96.pub.LEE.10-pdgref}-cite}%
}
\dxdef{Gamma102-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma102-gn} = \dxuse{Gamma102-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma102} \\
\dxuse{CLEO.Gamma102.pub.GIBAUT.94B-vu} & \dxuse{\dxuse{CLEO.Gamma102.pub.GIBAUT.94B-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma102.pub.GIBAUT.94B-pdgref}-cite} \\
\dxuse{HRS.Gamma102.pub.BYLSMA.87-vu} & \dxuse{\dxuse{HRS.Gamma102.pub.BYLSMA.87-pdgref}-exp} & \dxuse{\dxuse{HRS.Gamma102.pub.BYLSMA.87-pdgref}-cite} \\
\dxuse{L3.Gamma102.pub.ACHARD.01D-vu} & \dxuse{\dxuse{L3.Gamma102.pub.ACHARD.01D-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma102.pub.ACHARD.01D-pdgref}-cite}%
}
\dxdef{Gamma103-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma103-gn} = \dxuse{Gamma103-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma103} \\
\dxuse{ALEPH.Gamma103.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma103.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma103.pub.SCHAEL.05C-pdgref}-cite} \\
\dxuse{ARGUS.Gamma103.pub.ALBRECHT.88B-vu} & \dxuse{\dxuse{ARGUS.Gamma103.pub.ALBRECHT.88B-pdgref}-exp} & \dxuse{\dxuse{ARGUS.Gamma103.pub.ALBRECHT.88B-pdgref}-cite} \\
\dxuse{CLEO.Gamma103.pub.GIBAUT.94B-vu} & \dxuse{\dxuse{CLEO.Gamma103.pub.GIBAUT.94B-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma103.pub.GIBAUT.94B-pdgref}-cite} \\
\dxuse{DELPHI.Gamma103.pub.ABDALLAH.06A-vu} & \dxuse{\dxuse{DELPHI.Gamma103.pub.ABDALLAH.06A-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma103.pub.ABDALLAH.06A-pdgref}-cite} \\
\dxuse{HRS.Gamma103.pub.BYLSMA.87-vu} & \dxuse{\dxuse{HRS.Gamma103.pub.BYLSMA.87-pdgref}-exp} & \dxuse{\dxuse{HRS.Gamma103.pub.BYLSMA.87-pdgref}-cite} \\
\dxuse{OPAL.Gamma103.pub.ACKERSTAFF.99E-vu} & \dxuse{\dxuse{OPAL.Gamma103.pub.ACKERSTAFF.99E-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma103.pub.ACKERSTAFF.99E-pdgref}-cite}%
}
\dxdef{Gamma104-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma104-gn} = \dxuse{Gamma104-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma104} \\
\dxuse{ALEPH.Gamma104.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma104.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma104.pub.SCHAEL.05C-pdgref}-cite} \\
\dxuse{CLEO.Gamma104.pub.ANASTASSOV.01-vu} & \dxuse{\dxuse{CLEO.Gamma104.pub.ANASTASSOV.01-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma104.pub.ANASTASSOV.01-pdgref}-cite} \\
\dxuse{DELPHI.Gamma104.pub.ABDALLAH.06A-vu} & \dxuse{\dxuse{DELPHI.Gamma104.pub.ABDALLAH.06A-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma104.pub.ABDALLAH.06A-pdgref}-cite} \\
\dxuse{OPAL.Gamma104.pub.ACKERSTAFF.99E-vu} & \dxuse{\dxuse{OPAL.Gamma104.pub.ACKERSTAFF.99E-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma104.pub.ACKERSTAFF.99E-pdgref}-cite}%
}
\dxdef{Gamma106-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma106-gn} = \dxuse{Gamma106-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma106}%
}
\dxdef{Gamma110-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma110-gn} = \dxuse{Gamma110-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma110}%
}
\dxdef{Gamma126-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma126-gn} = \dxuse{Gamma126-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma126} \\
\dxuse{ALEPH.Gamma126.pub.BUSKULIC.97C-vu} & \dxuse{\dxuse{ALEPH.Gamma126.pub.BUSKULIC.97C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma126.pub.BUSKULIC.97C-pdgref}-cite} \\
\dxuse{Belle.Gamma126.pub.INAMI.09-vu} & \dxuse{\dxuse{Belle.Gamma126.pub.INAMI.09-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma126.pub.INAMI.09-pdgref}-cite} \\
\dxuse{CLEO.Gamma126.pub.ARTUSO.92-vu} & \dxuse{\dxuse{CLEO.Gamma126.pub.ARTUSO.92-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma126.pub.ARTUSO.92-pdgref}-cite}%
}
\dxdef{Gamma128-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma128-gn} = \dxuse{Gamma128-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma128} \\
\dxuse{ALEPH.Gamma128.pub.BUSKULIC.97C-vu} & \dxuse{\dxuse{ALEPH.Gamma128.pub.BUSKULIC.97C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma128.pub.BUSKULIC.97C-pdgref}-cite} \\
\dxuse{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E-vu} & \dxuse{\dxuse{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E-pdgref}-cite} \\
\dxuse{Belle.Gamma128.pub.INAMI.09-vu} & \dxuse{\dxuse{Belle.Gamma128.pub.INAMI.09-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma128.pub.INAMI.09-pdgref}-cite} \\
\dxuse{CLEO.Gamma128.pub.BARTELT.96-vu} & \dxuse{\dxuse{CLEO.Gamma128.pub.BARTELT.96-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma128.pub.BARTELT.96-pdgref}-cite}%
}
\dxdef{Gamma130-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma130-gn} = \dxuse{Gamma130-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma130} \\
\dxuse{Belle.Gamma130.pub.INAMI.09-vu} & \dxuse{\dxuse{Belle.Gamma130.pub.INAMI.09-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma130.pub.INAMI.09-pdgref}-cite} \\
\dxuse{CLEO.Gamma130.pub.BISHAI.99-vu} & \dxuse{\dxuse{CLEO.Gamma130.pub.BISHAI.99-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma130.pub.BISHAI.99-pdgref}-cite}%
}
\dxdef{Gamma132-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma132-gn} = \dxuse{Gamma132-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma132} \\
\dxuse{Belle.Gamma132.pub.INAMI.09-vu} & \dxuse{\dxuse{Belle.Gamma132.pub.INAMI.09-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma132.pub.INAMI.09-pdgref}-cite} \\
\dxuse{CLEO.Gamma132.pub.BISHAI.99-vu} & \dxuse{\dxuse{CLEO.Gamma132.pub.BISHAI.99-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma132.pub.BISHAI.99-pdgref}-cite}%
}
\dxdef{Gamma136-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma136-gn} = \dxuse{Gamma136-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma136}%
}
\dxdef{Gamma149-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma149-gn} = \dxuse{Gamma149-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma149}%
}
\dxdef{Gamma150-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma150-gn} = \dxuse{Gamma150-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma150} \\
\dxuse{ALEPH.Gamma150.pub.BUSKULIC.97C-vu} & \dxuse{\dxuse{ALEPH.Gamma150.pub.BUSKULIC.97C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma150.pub.BUSKULIC.97C-pdgref}-cite} \\
\dxuse{CLEO.Gamma150.pub.BARINGER.87-vu} & \dxuse{\dxuse{CLEO.Gamma150.pub.BARINGER.87-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma150.pub.BARINGER.87-pdgref}-cite}%
}
\dxdef{Gamma150by66-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma150by66-gn} = \dxuse{Gamma150by66-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma150by66} \\
\dxuse{ALEPH.Gamma150by66.pub.BUSKULIC.96-vu} & \dxuse{\dxuse{ALEPH.Gamma150by66.pub.BUSKULIC.96-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma150by66.pub.BUSKULIC.96-pdgref}-cite} \\
\dxuse{CLEO.Gamma150by66.pub.BALEST.95C-vu} & \dxuse{\dxuse{CLEO.Gamma150by66.pub.BALEST.95C-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma150by66.pub.BALEST.95C-pdgref}-cite}%
}
\dxdef{Gamma151-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma151-gn} = \dxuse{Gamma151-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma151} \\
\dxuse{CLEO3.Gamma151.pub.ARMS.05-vu} & \dxuse{\dxuse{CLEO3.Gamma151.pub.ARMS.05-pdgref}-exp} & \dxuse{\dxuse{CLEO3.Gamma151.pub.ARMS.05-pdgref}-cite}%
}
\dxdef{Gamma152-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma152-gn} = \dxuse{Gamma152-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma152} \\
\dxuse{ALEPH.Gamma152.pub.BUSKULIC.97C-vu} & \dxuse{\dxuse{ALEPH.Gamma152.pub.BUSKULIC.97C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma152.pub.BUSKULIC.97C-pdgref}-cite}%
}
\dxdef{Gamma152by54-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma152by54-gn} = \dxuse{Gamma152by54-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma152by54}%
}
\dxdef{Gamma152by76-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma152by76-gn} = \dxuse{Gamma152by76-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma152by76} \\
\dxuse{CLEO.Gamma152by76.pub.BORTOLETTO.93-vu} & \dxuse{\dxuse{CLEO.Gamma152by76.pub.BORTOLETTO.93-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma152by76.pub.BORTOLETTO.93-pdgref}-cite}%
}
\dxdef{Gamma167-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma167-gn} = \dxuse{Gamma167-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma167}%
}
\dxdef{Gamma168-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma168-gn} = \dxuse{Gamma168-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma168}%
}
\dxdef{Gamma169-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma169-gn} = \dxuse{Gamma169-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma169}%
}
\dxdef{Gamma800-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma800-gn} = \dxuse{Gamma800-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma800}%
}
\dxdef{Gamma802-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma802-gn} = \dxuse{Gamma802-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma802}%
}
\dxdef{Gamma803-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma803-gn} = \dxuse{Gamma803-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma803}%
}
\dxdef{Gamma804-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma804-gn} = \dxuse{Gamma804-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma804}%
}
\dxdef{Gamma805-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma805-gn} = \dxuse{Gamma805-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma805}%
}
\dxdef{Gamma806-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma806-gn} = \dxuse{Gamma806-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma806}%
}
\dxdef{Gamma810-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma810-gn} = \dxuse{Gamma810-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma810}%
}
\dxdef{Gamma811-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma811-gn} = \dxuse{Gamma811-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma811} \\
\dxuse{BaBar.Gamma811.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma811.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma811.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma812-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma812-gn} = \dxuse{Gamma812-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma812} \\
\dxuse{BaBar.Gamma812.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma812.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma812.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma820-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma820-gn} = \dxuse{Gamma820-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma820}%
}
\dxdef{Gamma821-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma821-gn} = \dxuse{Gamma821-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma821} \\
\dxuse{BaBar.Gamma821.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma821.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma821.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma822-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma822-gn} = \dxuse{Gamma822-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma822} \\
\dxuse{BaBar.Gamma822.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma822.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma822.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma830-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma830-gn} = \dxuse{Gamma830-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma830}%
}
\dxdef{Gamma831-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma831-gn} = \dxuse{Gamma831-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma831} \\
\dxuse{BaBar.Gamma831.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma831.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma831.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma832-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma832-gn} = \dxuse{Gamma832-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma832} \\
\dxuse{BaBar.Gamma832.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma832.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma832.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma833-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma833-gn} = \dxuse{Gamma833-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma833} \\
\dxuse{BaBar.Gamma833.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma833.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma833.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma910-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma910-gn} = \dxuse{Gamma910-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma910} \\
\dxuse{BaBar.Gamma910.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma910.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma910.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma911-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma911-gn} = \dxuse{Gamma911-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma911} \\
\dxuse{BaBar.Gamma911.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma911.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma911.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma920-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma920-gn} = \dxuse{Gamma920-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma920} \\
\dxuse{BaBar.Gamma920.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma920.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma920.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma930-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma930-gn} = \dxuse{Gamma930-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma930} \\
\dxuse{BaBar.Gamma930.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma930.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma930.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma944-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma944-gn} = \dxuse{Gamma944-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma944} \\
\dxuse{BaBar.Gamma944.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma944.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma944.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma945-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma945-gn} = \dxuse{Gamma945-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma945}%
}
\dxdef{GammaAll-qm}{%
\begin{ensuredisplaymath}
\dxuse{GammaAll-gn} = \dxuse{GammaAll-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{GammaAll}%
}
\dxdef{Gamma980-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma980-gn} = \dxuse{Gamma980-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma980} \\
\dxuse{ALEPH.Gamma980.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma980.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma980.pub.SCHAEL.05C-pdgref}-cite}%
}
\dxdef{TauBrVarMeasTable}{%
\dxuse{Gamma1-qm} \\[1.5ex]
\dxuse{Gamma2-qm} \\[1.5ex]
\dxuse{Gamma3-qm} \\[1.5ex]
\dxuse{Gamma3by5-qm} \\[1.5ex]
\dxuse{Gamma5-qm} \\[1.5ex]
\dxuse{Gamma7-qm} \\[1.5ex]
\dxuse{Gamma8-qm} \\[1.5ex]
\dxuse{Gamma8by5-qm} \\[1.5ex]
\dxuse{Gamma9-qm} \\[1.5ex]
\dxuse{Gamma9by5-qm} \\[1.5ex]
\dxuse{Gamma10-qm} \\[1.5ex]
\dxuse{Gamma10by5-qm} \\[1.5ex]
\dxuse{Gamma10by9-qm} \\[1.5ex]
\dxuse{Gamma11-qm} \\[1.5ex]
\dxuse{Gamma12-qm} \\[1.5ex]
\dxuse{Gamma13-qm} \\[1.5ex]
\dxuse{Gamma14-qm} \\[1.5ex]
\dxuse{Gamma16-qm} \\[1.5ex]
\dxuse{Gamma17-qm} \\[1.5ex]
\dxuse{Gamma18-qm} \\[1.5ex]
\dxuse{Gamma19-qm} \\[1.5ex]
\dxuse{Gamma19by13-qm} \\[1.5ex]
\dxuse{Gamma20-qm} \\[1.5ex]
\dxuse{Gamma23-qm} \\[1.5ex]
\dxuse{Gamma24-qm} \\[1.5ex]
\dxuse{Gamma25-qm} \\[1.5ex]
\dxuse{Gamma26-qm} \\[1.5ex]
\dxuse{Gamma26by13-qm} \\[1.5ex]
\dxuse{Gamma27-qm} \\[1.5ex]
\dxuse{Gamma28-qm} \\[1.5ex]
\dxuse{Gamma29-qm} \\[1.5ex]
\dxuse{Gamma30-qm} \\[1.5ex]
\dxuse{Gamma31-qm} \\[1.5ex]
\dxuse{Gamma32-qm} \\[1.5ex]
\dxuse{Gamma33-qm} \\[1.5ex]
\dxuse{Gamma34-qm} \\[1.5ex]
\dxuse{Gamma35-qm} \\[1.5ex]
\dxuse{Gamma37-qm} \\[1.5ex]
\dxuse{Gamma38-qm} \\[1.5ex]
\dxuse{Gamma39-qm} \\[1.5ex]
\dxuse{Gamma40-qm} \\[1.5ex]
\dxuse{Gamma42-qm} \\[1.5ex]
\dxuse{Gamma43-qm} \\[1.5ex]
\dxuse{Gamma44-qm} \\[1.5ex]
\dxuse{Gamma46-qm} \\[1.5ex]
\dxuse{Gamma47-qm} \\[1.5ex]
\dxuse{Gamma48-qm} \\[1.5ex]
\dxuse{Gamma49-qm} \\[1.5ex]
\dxuse{Gamma50-qm} \\[1.5ex]
\dxuse{Gamma51-qm} \\[1.5ex]
\dxuse{Gamma53-qm} \\[1.5ex]
\dxuse{Gamma54-qm} \\[1.5ex]
\dxuse{Gamma55-qm} \\[1.5ex]
\dxuse{Gamma56-qm} \\[1.5ex]
\dxuse{Gamma57-qm} \\[1.5ex]
\dxuse{Gamma57by55-qm} \\[1.5ex]
\dxuse{Gamma58-qm} \\[1.5ex]
\dxuse{Gamma59-qm} \\[1.5ex]
\dxuse{Gamma60-qm} \\[1.5ex]
\dxuse{Gamma62-qm} \\[1.5ex]
\dxuse{Gamma63-qm} \\[1.5ex]
\dxuse{Gamma64-qm} \\[1.5ex]
\dxuse{Gamma65-qm} \\[1.5ex]
\dxuse{Gamma66-qm} \\[1.5ex]
\dxuse{Gamma67-qm} \\[1.5ex]
\dxuse{Gamma68-qm} \\[1.5ex]
\dxuse{Gamma69-qm} \\[1.5ex]
\dxuse{Gamma70-qm} \\[1.5ex]
\dxuse{Gamma74-qm} \\[1.5ex]
\dxuse{Gamma75-qm} \\[1.5ex]
\dxuse{Gamma76-qm} \\[1.5ex]
\dxuse{Gamma76by54-qm} \\[1.5ex]
\dxuse{Gamma77-qm} \\[1.5ex]
\dxuse{Gamma78-qm} \\[1.5ex]
\dxuse{Gamma79-qm} \\[1.5ex]
\dxuse{Gamma80-qm} \\[1.5ex]
\dxuse{Gamma80by60-qm} \\[1.5ex]
\dxuse{Gamma81-qm} \\[1.5ex]
\dxuse{Gamma81by69-qm} \\[1.5ex]
\dxuse{Gamma82-qm} \\[1.5ex]
\dxuse{Gamma83-qm} \\[1.5ex]
\dxuse{Gamma84-qm} \\[1.5ex]
\dxuse{Gamma85-qm} \\[1.5ex]
\dxuse{Gamma85by60-qm} \\[1.5ex]
\dxuse{Gamma87-qm} \\[1.5ex]
\dxuse{Gamma88-qm} \\[1.5ex]
\dxuse{Gamma89-qm} \\[1.5ex]
\dxuse{Gamma92-qm} \\[1.5ex]
\dxuse{Gamma93-qm} \\[1.5ex]
\dxuse{Gamma93by60-qm} \\[1.5ex]
\dxuse{Gamma94-qm} \\[1.5ex]
\dxuse{Gamma94by69-qm} \\[1.5ex]
\dxuse{Gamma96-qm} \\[1.5ex]
\dxuse{Gamma102-qm} \\[1.5ex]
\dxuse{Gamma103-qm} \\[1.5ex]
\dxuse{Gamma104-qm} \\[1.5ex]
\dxuse{Gamma106-qm} \\[1.5ex]
\dxuse{Gamma110-qm} \\[1.5ex]
\dxuse{Gamma126-qm} \\[1.5ex]
\dxuse{Gamma128-qm} \\[1.5ex]
\dxuse{Gamma130-qm} \\[1.5ex]
\dxuse{Gamma132-qm} \\[1.5ex]
\dxuse{Gamma136-qm} \\[1.5ex]
\dxuse{Gamma149-qm} \\[1.5ex]
\dxuse{Gamma150-qm} \\[1.5ex]
\dxuse{Gamma150by66-qm} \\[1.5ex]
\dxuse{Gamma151-qm} \\[1.5ex]
\dxuse{Gamma152-qm} \\[1.5ex]
\dxuse{Gamma152by54-qm} \\[1.5ex]
\dxuse{Gamma152by76-qm} \\[1.5ex]
\dxuse{Gamma167-qm} \\[1.5ex]
\dxuse{Gamma168-qm} \\[1.5ex]
\dxuse{Gamma169-qm} \\[1.5ex]
\dxuse{Gamma800-qm} \\[1.5ex]
\dxuse{Gamma802-qm} \\[1.5ex]
\dxuse{Gamma803-qm} \\[1.5ex]
\dxuse{Gamma804-qm} \\[1.5ex]
\dxuse{Gamma805-qm} \\[1.5ex]
\dxuse{Gamma806-qm} \\[1.5ex]
\dxuse{Gamma810-qm} \\[1.5ex]
\dxuse{Gamma811-qm} \\[1.5ex]
\dxuse{Gamma812-qm} \\[1.5ex]
\dxuse{Gamma820-qm} \\[1.5ex]
\dxuse{Gamma821-qm} \\[1.5ex]
\dxuse{Gamma822-qm} \\[1.5ex]
\dxuse{Gamma830-qm} \\[1.5ex]
\dxuse{Gamma831-qm} \\[1.5ex]
\dxuse{Gamma832-qm} \\[1.5ex]
\dxuse{Gamma833-qm} \\[1.5ex]
\dxuse{Gamma910-qm} \\[1.5ex]
\dxuse{Gamma911-qm} \\[1.5ex]
\dxuse{Gamma920-qm} \\[1.5ex]
\dxuse{Gamma930-qm} \\[1.5ex]
\dxuse{Gamma944-qm} \\[1.5ex]
\dxuse{Gamma945-qm} \\[1.5ex]
\dxuse{GammaAll-qm}%
}
\dxdef{TauBrNuisMeasTable}{%
\dxuse{Gamma980-qm}%
}
\dxdef{BARATE 98-ref}{Barate:1997ma}
\dxdef{BARATE 98-cite}{\cite{Barate:1997ma}}
\dxdef{BARATE 98-exp}{ALEPH}
\dxdef{BARATE 98-type}{pub}
\dxdef{BARATE 98-label}{BARATE 98 (ALEPH)}
\dxdef{BARATE 98-meas}{%
\multicolumn{2}{l}{\dxuse{BARATE 98-label}\,\dxuse{BARATE 98-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma85-gn} = \dxuse{Gamma85-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma85.pub.BARATE.98-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma88-gn} = \dxuse{Gamma88-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma88.pub.BARATE.98-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma93-gn} = \dxuse{Gamma93-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma93.pub.BARATE.98-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma94-gn} = \dxuse{Gamma94-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma94.pub.BARATE.98-vu}%
}
\dxdef{BARATE 98E-ref}{Barate:1997tt}
\dxdef{BARATE 98E-cite}{\cite{Barate:1997tt}}
\dxdef{BARATE 98E-exp}{ALEPH}
\dxdef{BARATE 98E-type}{pub}
\dxdef{BARATE 98E-label}{BARATE 98E (ALEPH)}
\dxdef{BARATE 98E-meas}{%
\multicolumn{2}{l}{\dxuse{BARATE 98E-label}\,\dxuse{BARATE 98E-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma33-gn} = \dxuse{Gamma33-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma33.pub.BARATE.98E-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma37-gn} = \dxuse{Gamma37-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma37.pub.BARATE.98E-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma40-gn} = \dxuse{Gamma40-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma40.pub.BARATE.98E-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma42-gn} = \dxuse{Gamma42-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma42.pub.BARATE.98E-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma47-gn} = \dxuse{Gamma47-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma47.pub.BARATE.98E-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma48-gn} = \dxuse{Gamma48-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma48.pub.BARATE.98E-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma51-gn} = \dxuse{Gamma51-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma51.pub.BARATE.98E-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma53-gn} = \dxuse{Gamma53-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma53.pub.BARATE.98E-vu}%
}
\dxdef{BARATE 99K-ref}{Barate:1999hi}
\dxdef{BARATE 99K-cite}{\cite{Barate:1999hi}}
\dxdef{BARATE 99K-exp}{ALEPH}
\dxdef{BARATE 99K-type}{pub}
\dxdef{BARATE 99K-label}{BARATE 99K (ALEPH)}
\dxdef{BARATE 99K-meas}{%
\multicolumn{2}{l}{\dxuse{BARATE 99K-label}\,\dxuse{BARATE 99K-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma10-gn} = \dxuse{Gamma10-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma10.pub.BARATE.99K-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma16-gn} = \dxuse{Gamma16-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma16.pub.BARATE.99K-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma23-gn} = \dxuse{Gamma23-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma23.pub.BARATE.99K-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma28-gn} = \dxuse{Gamma28-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma28.pub.BARATE.99K-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma35-gn} = \dxuse{Gamma35-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma35.pub.BARATE.99K-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma37-gn} = \dxuse{Gamma37-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma37.pub.BARATE.99K-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma40-gn} = \dxuse{Gamma40-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma40.pub.BARATE.99K-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma42-gn} = \dxuse{Gamma42-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma42.pub.BARATE.99K-vu}%
}
\dxdef{BARATE 99R-ref}{Barate:1999hj}
\dxdef{BARATE 99R-cite}{\cite{Barate:1999hj}}
\dxdef{BARATE 99R-exp}{ALEPH}
\dxdef{BARATE 99R-type}{pub}
\dxdef{BARATE 99R-label}{BARATE 99R (ALEPH)}
\dxdef{BARATE 99R-meas}{%
\multicolumn{2}{l}{\dxuse{BARATE 99R-label}\,\dxuse{BARATE 99R-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma44-gn} = \dxuse{Gamma44-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma44.pub.BARATE.99R-vu}%
}
\dxdef{BUSKULIC 96-ref}{Buskulic:1995ty}
\dxdef{BUSKULIC 96-cite}{\cite{Buskulic:1995ty}}
\dxdef{BUSKULIC 96-exp}{ALEPH}
\dxdef{BUSKULIC 96-type}{pub}
\dxdef{BUSKULIC 96-label}{BUSKULIC 96 (ALEPH)}
\dxdef{BUSKULIC 96-meas}{%
\multicolumn{2}{l}{\dxuse{BUSKULIC 96-label}\,\dxuse{BUSKULIC 96-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma150by66-gn} = \dxuse{Gamma150by66-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma150by66.pub.BUSKULIC.96-vu}%
}
\dxdef{BUSKULIC 97C-ref}{Buskulic:1996qs}
\dxdef{BUSKULIC 97C-cite}{\cite{Buskulic:1996qs}}
\dxdef{BUSKULIC 97C-exp}{ALEPH}
\dxdef{BUSKULIC 97C-type}{pub}
\dxdef{BUSKULIC 97C-label}{BUSKULIC 97C (ALEPH)}
\dxdef{BUSKULIC 97C-meas}{%
\multicolumn{2}{l}{\dxuse{BUSKULIC 97C-label}\,\dxuse{BUSKULIC 97C-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma126-gn} = \dxuse{Gamma126-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma126.pub.BUSKULIC.97C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma128-gn} = \dxuse{Gamma128-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma128.pub.BUSKULIC.97C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma150-gn} = \dxuse{Gamma150-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma150.pub.BUSKULIC.97C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma152-gn} = \dxuse{Gamma152-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma152.pub.BUSKULIC.97C-vu}%
}
\dxdef{SCHAEL 05C-ref}{Schael:2005am}
\dxdef{SCHAEL 05C-cite}{\cite{Schael:2005am}}
\dxdef{SCHAEL 05C-exp}{ALEPH}
\dxdef{SCHAEL 05C-type}{pub}
\dxdef{SCHAEL 05C-label}{SCHAEL 05C (ALEPH)}
\dxdef{SCHAEL 05C-meas}{%
\multicolumn{2}{l}{\dxuse{SCHAEL 05C-label}\,\dxuse{SCHAEL 05C-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma3-gn} = \dxuse{Gamma3-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma3.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma5-gn} = \dxuse{Gamma5-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma5.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma9-gn} = \dxuse{Gamma9-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma9.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma14-gn} = \dxuse{Gamma14-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma14.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma20-gn} = \dxuse{Gamma20-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma20.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma27-gn} = \dxuse{Gamma27-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma27.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma30-gn} = \dxuse{Gamma30-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma30.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma62-gn} = \dxuse{Gamma62-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma62.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma69-gn} = \dxuse{Gamma69-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma69.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma76-gn} = \dxuse{Gamma76-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma76.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma103-gn} = \dxuse{Gamma103-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma103.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma104-gn} = \dxuse{Gamma104-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma104.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma980-gn} = \dxuse{Gamma980-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma980.pub.SCHAEL.05C-vu}%
}
\dxdef{ALBRECHT 88B-ref}{Albrecht:1987zf}
\dxdef{ALBRECHT 88B-cite}{\cite{Albrecht:1987zf}}
\dxdef{ALBRECHT 88B-exp}{ARGUS}
\dxdef{ALBRECHT 88B-type}{pub}
\dxdef{ALBRECHT 88B-label}{ALBRECHT 88B (ARGUS)}
\dxdef{ALBRECHT 88B-meas}{%
\multicolumn{2}{l}{\dxuse{ALBRECHT 88B-label}\,\dxuse{ALBRECHT 88B-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma103-gn} = \dxuse{Gamma103-td}
\end{ensuredisplaymath} & \dxuse{ARGUS.Gamma103.pub.ALBRECHT.88B-vu}%
}
\dxdef{ALBRECHT 92D-ref}{Albrecht:1991rh}
\dxdef{ALBRECHT 92D-cite}{\cite{Albrecht:1991rh}}
\dxdef{ALBRECHT 92D-exp}{ARGUS}
\dxdef{ALBRECHT 92D-type}{pub}
\dxdef{ALBRECHT 92D-label}{ALBRECHT 92D (ARGUS)}
\dxdef{ALBRECHT 92D-meas}{%
\multicolumn{2}{l}{\dxuse{ALBRECHT 92D-label}\,\dxuse{ALBRECHT 92D-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma3by5-gn} = \dxuse{Gamma3by5-td}
\end{ensuredisplaymath} & \dxuse{ARGUS.Gamma3by5.pub.ALBRECHT.92D-vu}%
}
\dxdef{AUBERT 07AP-ref}{Aubert:2007jh}
\dxdef{AUBERT 07AP-cite}{\cite{Aubert:2007jh}}
\dxdef{AUBERT 07AP-exp}{\babar}
\dxdef{AUBERT 07AP-type}{pub}
\dxdef{AUBERT 07AP-label}{AUBERT 07AP (\babar)}
\dxdef{AUBERT 07AP-meas}{%
\multicolumn{2}{l}{\dxuse{AUBERT 07AP-label}\,\dxuse{AUBERT 07AP-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma16-gn} = \dxuse{Gamma16-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma16.pub.AUBERT.07AP-vu}%
}
\dxdef{AUBERT 08-ref}{Aubert:2007mh}
\dxdef{AUBERT 08-cite}{\cite{Aubert:2007mh}}
\dxdef{AUBERT 08-exp}{\babar}
\dxdef{AUBERT 08-type}{pub}
\dxdef{AUBERT 08-label}{AUBERT 08 (\babar)}
\dxdef{AUBERT 08-meas}{%
\multicolumn{2}{l}{\dxuse{AUBERT 08-label}\,\dxuse{AUBERT 08-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma60-gn} = \dxuse{Gamma60-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma60.pub.AUBERT.08-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma85-gn} = \dxuse{Gamma85-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma85.pub.AUBERT.08-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma93-gn} = \dxuse{Gamma93-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma93.pub.AUBERT.08-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma96-gn} = \dxuse{Gamma96-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma96.pub.AUBERT.08-vu}%
}
\dxdef{AUBERT 10F-ref}{Aubert:2009qj}
\dxdef{AUBERT 10F-cite}{\cite{Aubert:2009qj}}
\dxdef{AUBERT 10F-exp}{\babar}
\dxdef{AUBERT 10F-type}{pub}
\dxdef{AUBERT 10F-label}{AUBERT 10F (\babar)}
\dxdef{AUBERT 10F-meas}{%
\multicolumn{2}{l}{\dxuse{AUBERT 10F-label}\,\dxuse{AUBERT 10F-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma3by5-gn} = \dxuse{Gamma3by5-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma3by5.pub.AUBERT.10F-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma9by5-gn} = \dxuse{Gamma9by5-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma9by5.pub.AUBERT.10F-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma10by5-gn} = \dxuse{Gamma10by5-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma10by5.pub.AUBERT.10F-vu}%
}
\dxdef{DEL-AMO-SANCHEZ 11E-ref}{delAmoSanchez:2010pc}
\dxdef{DEL-AMO-SANCHEZ 11E-cite}{\cite{delAmoSanchez:2010pc}}
\dxdef{DEL-AMO-SANCHEZ 11E-exp}{\babar}
\dxdef{DEL-AMO-SANCHEZ 11E-type}{pub}
\dxdef{DEL-AMO-SANCHEZ 11E-label}{DEL-AMO-SANCHEZ 11E (\babar)}
\dxdef{DEL-AMO-SANCHEZ 11E-meas}{%
\multicolumn{2}{l}{\dxuse{DEL-AMO-SANCHEZ 11E-label}\,\dxuse{DEL-AMO-SANCHEZ 11E-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma128-gn} = \dxuse{Gamma128-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E-vu}%
}
\dxdef{LEES 12X-ref}{Lees:2012ks}
\dxdef{LEES 12X-cite}{\cite{Lees:2012ks}}
\dxdef{LEES 12X-exp}{\babar}
\dxdef{LEES 12X-type}{pub}
\dxdef{LEES 12X-label}{LEES 12X (\babar)}
\dxdef{LEES 12X-meas}{%
\multicolumn{2}{l}{\dxuse{LEES 12X-label}\,\dxuse{LEES 12X-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma811-gn} = \dxuse{Gamma811-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma811.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma812-gn} = \dxuse{Gamma812-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma812.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma821-gn} = \dxuse{Gamma821-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma821.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma822-gn} = \dxuse{Gamma822-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma822.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma831-gn} = \dxuse{Gamma831-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma831.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma832-gn} = \dxuse{Gamma832-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma832.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma833-gn} = \dxuse{Gamma833-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma833.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma910-gn} = \dxuse{Gamma910-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma910.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma911-gn} = \dxuse{Gamma911-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma911.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma920-gn} = \dxuse{Gamma920-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma920.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma930-gn} = \dxuse{Gamma930-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma930.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma944-gn} = \dxuse{Gamma944-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma944.pub.LEES.12X-vu}%
}
\dxdef{LEES 12Y-ref}{Lees:2012de}
\dxdef{LEES 12Y-cite}{\cite{Lees:2012de}}
\dxdef{LEES 12Y-exp}{\babar}
\dxdef{LEES 12Y-type}{pub}
\dxdef{LEES 12Y-label}{LEES 12Y (\babar)}
\dxdef{LEES 12Y-meas}{%
\multicolumn{2}{l}{\dxuse{LEES 12Y-label}\,\dxuse{LEES 12Y-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma47-gn} = \dxuse{Gamma47-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma47.pub.LEES.12Y-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma50-gn} = \dxuse{Gamma50-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma50.pub.LEES.12Y-vu}%
}
\dxdef{LEES 18B-ref}{BaBar:2018qry}
\dxdef{LEES 18B-cite}{\cite{BaBar:2018qry}}
\dxdef{LEES 18B-exp}{\babar}
\dxdef{LEES 18B-type}{pub}
\dxdef{LEES 18B-label}{LEES 18B (\babar)}
\dxdef{LEES 18B-meas}{%
\multicolumn{2}{l}{\dxuse{LEES 18B-label}\,\dxuse{LEES 18B-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma37-gn} = \dxuse{Gamma37-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma37.pub.LEES.18B-vu}%
}
\dxdef{FUJIKAWA 08-ref}{Fujikawa:2008ma}
\dxdef{FUJIKAWA 08-cite}{\cite{Fujikawa:2008ma}}
\dxdef{FUJIKAWA 08-exp}{Belle}
\dxdef{FUJIKAWA 08-type}{pub}
\dxdef{FUJIKAWA 08-label}{FUJIKAWA 08 (Belle)}
\dxdef{FUJIKAWA 08-meas}{%
\multicolumn{2}{l}{\dxuse{FUJIKAWA 08-label}\,\dxuse{FUJIKAWA 08-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma13-gn} = \dxuse{Gamma13-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma13.pub.FUJIKAWA.08-vu}%
}
\dxdef{INAMI 09-ref}{Inami:2008ar}
\dxdef{INAMI 09-cite}{\cite{Inami:2008ar}}
\dxdef{INAMI 09-exp}{Belle}
\dxdef{INAMI 09-type}{pub}
\dxdef{INAMI 09-label}{INAMI 09 (Belle)}
\dxdef{INAMI 09-meas}{%
\multicolumn{2}{l}{\dxuse{INAMI 09-label}\,\dxuse{INAMI 09-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma126-gn} = \dxuse{Gamma126-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma126.pub.INAMI.09-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma128-gn} = \dxuse{Gamma128-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma128.pub.INAMI.09-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma130-gn} = \dxuse{Gamma130-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma130.pub.INAMI.09-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma132-gn} = \dxuse{Gamma132-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma132.pub.INAMI.09-vu}%
}
\dxdef{LEE 10-ref}{Lee:2010tc}
\dxdef{LEE 10-cite}{\cite{Lee:2010tc}}
\dxdef{LEE 10-exp}{Belle}
\dxdef{LEE 10-type}{pub}
\dxdef{LEE 10-label}{LEE 10 (Belle)}
\dxdef{LEE 10-meas}{%
\multicolumn{2}{l}{\dxuse{LEE 10-label}\,\dxuse{LEE 10-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma60-gn} = \dxuse{Gamma60-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma60.pub.LEE.10-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma85-gn} = \dxuse{Gamma85-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma85.pub.LEE.10-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma93-gn} = \dxuse{Gamma93-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma93.pub.LEE.10-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma96-gn} = \dxuse{Gamma96-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma96.pub.LEE.10-vu}%
}
\dxdef{RYU 14vpc-ref}{Ryu:2014vpc}
\dxdef{RYU 14vpc-cite}{\cite{Ryu:2014vpc}}
\dxdef{RYU 14vpc-exp}{Belle}
\dxdef{RYU 14vpc-type}{pub}
\dxdef{RYU 14vpc-label}{RYU 14vpc (Belle)}
\dxdef{RYU 14vpc-meas}{%
\multicolumn{2}{l}{\dxuse{RYU 14vpc-label}\,\dxuse{RYU 14vpc-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma35-gn} = \dxuse{Gamma35-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma35.pub.RYU.14vpc-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma37-gn} = \dxuse{Gamma37-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma37.pub.RYU.14vpc-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma40-gn} = \dxuse{Gamma40-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma40.pub.RYU.14vpc-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma42-gn} = \dxuse{Gamma42-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma42.pub.RYU.14vpc-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma47-gn} = \dxuse{Gamma47-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma47.pub.RYU.14vpc-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma50-gn} = \dxuse{Gamma50-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma50.pub.RYU.14vpc-vu}%
}
\dxdef{Belle2 ADACHI 2024-ref}{Belle-II:2024vvr}
\dxdef{Belle2 ADACHI 2024-cite}{\cite{Belle-II:2024vvr}}
\dxdef{Belle2 ADACHI 2024-exp}{Belle\,II}
\dxdef{Belle2 ADACHI 2024-type}{ADACHI}
\dxdef{Belle2 ADACHI 2024-label}{Belle\,II ADACHI 2024}
\dxdef{Belle2 ADACHI 2024-meas}{%
\multicolumn{2}{l}{\dxuse{Belle2 ADACHI 2024-label}\,\dxuse{Belle2 ADACHI 2024-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma3by5-gn} = \dxuse{Gamma3by5-td}
\end{ensuredisplaymath} & \dxuse{Belle2.Gamma3by5.ADACHI.2024-vu}%
}
\dxdef{BEHREND 89B-ref}{Behrend:1989wc}
\dxdef{BEHREND 89B-cite}{\cite{Behrend:1989wc}}
\dxdef{BEHREND 89B-exp}{CELLO}
\dxdef{BEHREND 89B-type}{pub}
\dxdef{BEHREND 89B-label}{BEHREND 89B (CELLO)}
\dxdef{BEHREND 89B-meas}{%
\multicolumn{2}{l}{\dxuse{BEHREND 89B-label}\,\dxuse{BEHREND 89B-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma54-gn} = \dxuse{Gamma54-td}
\end{ensuredisplaymath} & \dxuse{CELLO.Gamma54.pub.BEHREND.89B-vu}%
}
\dxdef{ANASTASSOV 01-ref}{Anastassov:2000xu}
\dxdef{ANASTASSOV 01-cite}{\cite{Anastassov:2000xu}}
\dxdef{ANASTASSOV 01-exp}{CLEO}
\dxdef{ANASTASSOV 01-type}{pub}
\dxdef{ANASTASSOV 01-label}{ANASTASSOV 01 (CLEO)}
\dxdef{ANASTASSOV 01-meas}{%
\multicolumn{2}{l}{\dxuse{ANASTASSOV 01-label}\,\dxuse{ANASTASSOV 01-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma78-gn} = \dxuse{Gamma78-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma78.pub.ANASTASSOV.01-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma104-gn} = \dxuse{Gamma104-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma104.pub.ANASTASSOV.01-vu}%
}
\dxdef{ANASTASSOV 97-ref}{CLEO:1996oro}
\dxdef{ANASTASSOV 97-cite}{\cite{CLEO:1996oro}}
\dxdef{ANASTASSOV 97-exp}{CLEO}
\dxdef{ANASTASSOV 97-type}{pub}
\dxdef{ANASTASSOV 97-label}{ANASTASSOV 97 (CLEO)}
\dxdef{ANASTASSOV 97-meas}{%
\multicolumn{2}{l}{\dxuse{ANASTASSOV 97-label}\,\dxuse{ANASTASSOV 97-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma3by5-gn} = \dxuse{Gamma3by5-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma3by5.pub.ANASTASSOV.97-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma5-gn} = \dxuse{Gamma5-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma5.pub.ANASTASSOV.97-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma8-gn} = \dxuse{Gamma8-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma8.pub.ANASTASSOV.97-vu}%
}
\dxdef{ARTUSO 92-ref}{Artuso:1992qu}
\dxdef{ARTUSO 92-cite}{\cite{Artuso:1992qu}}
\dxdef{ARTUSO 92-exp}{CLEO}
\dxdef{ARTUSO 92-type}{pub}
\dxdef{ARTUSO 92-label}{ARTUSO 92 (CLEO)}
\dxdef{ARTUSO 92-meas}{%
\multicolumn{2}{l}{\dxuse{ARTUSO 92-label}\,\dxuse{ARTUSO 92-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma126-gn} = \dxuse{Gamma126-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma126.pub.ARTUSO.92-vu}%
}
\dxdef{ARTUSO 94-ref}{Artuso:1994ii}
\dxdef{ARTUSO 94-cite}{\cite{Artuso:1994ii}}
\dxdef{ARTUSO 94-exp}{CLEO}
\dxdef{ARTUSO 94-type}{pub}
\dxdef{ARTUSO 94-label}{ARTUSO 94 (CLEO)}
\dxdef{ARTUSO 94-meas}{%
\multicolumn{2}{l}{\dxuse{ARTUSO 94-label}\,\dxuse{ARTUSO 94-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma13-gn} = \dxuse{Gamma13-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma13.pub.ARTUSO.94-vu}%
}
\dxdef{BALEST 95C-ref}{Balest:1995kq}
\dxdef{BALEST 95C-cite}{\cite{Balest:1995kq}}
\dxdef{BALEST 95C-exp}{CLEO}
\dxdef{BALEST 95C-type}{pub}
\dxdef{BALEST 95C-label}{BALEST 95C (CLEO)}
\dxdef{BALEST 95C-meas}{%
\multicolumn{2}{l}{\dxuse{BALEST 95C-label}\,\dxuse{BALEST 95C-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma57-gn} = \dxuse{Gamma57-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma57.pub.BALEST.95C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma66-gn} = \dxuse{Gamma66-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma66.pub.BALEST.95C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma150by66-gn} = \dxuse{Gamma150by66-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma150by66.pub.BALEST.95C-vu}%
}
\dxdef{BARINGER 87-ref}{Baringer:1987tr}
\dxdef{BARINGER 87-cite}{\cite{Baringer:1987tr}}
\dxdef{BARINGER 87-exp}{CLEO}
\dxdef{BARINGER 87-type}{pub}
\dxdef{BARINGER 87-label}{BARINGER 87 (CLEO)}
\dxdef{BARINGER 87-meas}{%
\multicolumn{2}{l}{\dxuse{BARINGER 87-label}\,\dxuse{BARINGER 87-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma150-gn} = \dxuse{Gamma150-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma150.pub.BARINGER.87-vu}%
}
\dxdef{BARTELT 96-ref}{Bartelt:1996iv}
\dxdef{BARTELT 96-cite}{\cite{Bartelt:1996iv}}
\dxdef{BARTELT 96-exp}{CLEO}
\dxdef{BARTELT 96-type}{pub}
\dxdef{BARTELT 96-label}{BARTELT 96 (CLEO)}
\dxdef{BARTELT 96-meas}{%
\multicolumn{2}{l}{\dxuse{BARTELT 96-label}\,\dxuse{BARTELT 96-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma128-gn} = \dxuse{Gamma128-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma128.pub.BARTELT.96-vu}%
}
\dxdef{BATTLE 94-ref}{Battle:1994by}
\dxdef{BATTLE 94-cite}{\cite{Battle:1994by}}
\dxdef{BATTLE 94-exp}{CLEO}
\dxdef{BATTLE 94-type}{pub}
\dxdef{BATTLE 94-label}{BATTLE 94 (CLEO)}
\dxdef{BATTLE 94-meas}{%
\multicolumn{2}{l}{\dxuse{BATTLE 94-label}\,\dxuse{BATTLE 94-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma10-gn} = \dxuse{Gamma10-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma10.pub.BATTLE.94-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma16-gn} = \dxuse{Gamma16-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma16.pub.BATTLE.94-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma23-gn} = \dxuse{Gamma23-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma23.pub.BATTLE.94-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma31-gn} = \dxuse{Gamma31-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma31.pub.BATTLE.94-vu}%
}
\dxdef{BISHAI 99-ref}{Bishai:1998gf}
\dxdef{BISHAI 99-cite}{\cite{Bishai:1998gf}}
\dxdef{BISHAI 99-exp}{CLEO}
\dxdef{BISHAI 99-type}{pub}
\dxdef{BISHAI 99-label}{BISHAI 99 (CLEO)}
\dxdef{BISHAI 99-meas}{%
\multicolumn{2}{l}{\dxuse{BISHAI 99-label}\,\dxuse{BISHAI 99-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma130-gn} = \dxuse{Gamma130-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma130.pub.BISHAI.99-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma132-gn} = \dxuse{Gamma132-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma132.pub.BISHAI.99-vu}%
}
\dxdef{BORTOLETTO 93-ref}{Bortoletto:1993px}
\dxdef{BORTOLETTO 93-cite}{\cite{Bortoletto:1993px}}
\dxdef{BORTOLETTO 93-exp}{CLEO}
\dxdef{BORTOLETTO 93-type}{pub}
\dxdef{BORTOLETTO 93-label}{BORTOLETTO 93 (CLEO)}
\dxdef{BORTOLETTO 93-meas}{%
\multicolumn{2}{l}{\dxuse{BORTOLETTO 93-label}\,\dxuse{BORTOLETTO 93-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma76by54-gn} = \dxuse{Gamma76by54-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma76by54.pub.BORTOLETTO.93-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma152by76-gn} = \dxuse{Gamma152by76-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma152by76.pub.BORTOLETTO.93-vu}%
}
\dxdef{COAN 96-ref}{Coan:1996iu}
\dxdef{COAN 96-cite}{\cite{Coan:1996iu}}
\dxdef{COAN 96-exp}{CLEO}
\dxdef{COAN 96-type}{pub}
\dxdef{COAN 96-label}{COAN 96 (CLEO)}
\dxdef{COAN 96-meas}{%
\multicolumn{2}{l}{\dxuse{COAN 96-label}\,\dxuse{COAN 96-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma34-gn} = \dxuse{Gamma34-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma34.pub.COAN.96-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma37-gn} = \dxuse{Gamma37-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma37.pub.COAN.96-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma39-gn} = \dxuse{Gamma39-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma39.pub.COAN.96-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma42-gn} = \dxuse{Gamma42-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma42.pub.COAN.96-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma47-gn} = \dxuse{Gamma47-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma47.pub.COAN.96-vu}%
}
\dxdef{EDWARDS 00A-ref}{Edwards:1999fj}
\dxdef{EDWARDS 00A-cite}{\cite{Edwards:1999fj}}
\dxdef{EDWARDS 00A-exp}{CLEO}
\dxdef{EDWARDS 00A-type}{pub}
\dxdef{EDWARDS 00A-label}{EDWARDS 00A (CLEO)}
\dxdef{EDWARDS 00A-meas}{%
\multicolumn{2}{l}{\dxuse{EDWARDS 00A-label}\,\dxuse{EDWARDS 00A-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma69-gn} = \dxuse{Gamma69-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma69.pub.EDWARDS.00A-vu}%
}
\dxdef{GIBAUT 94B-ref}{Gibaut:1994ik}
\dxdef{GIBAUT 94B-cite}{\cite{Gibaut:1994ik}}
\dxdef{GIBAUT 94B-exp}{CLEO}
\dxdef{GIBAUT 94B-type}{pub}
\dxdef{GIBAUT 94B-label}{GIBAUT 94B (CLEO)}
\dxdef{GIBAUT 94B-meas}{%
\multicolumn{2}{l}{\dxuse{GIBAUT 94B-label}\,\dxuse{GIBAUT 94B-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma102-gn} = \dxuse{Gamma102-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma102.pub.GIBAUT.94B-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma103-gn} = \dxuse{Gamma103-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma103.pub.GIBAUT.94B-vu}%
}
\dxdef{PROCARIO 93-ref}{Procario:1992hd}
\dxdef{PROCARIO 93-cite}{\cite{Procario:1992hd}}
\dxdef{PROCARIO 93-exp}{CLEO}
\dxdef{PROCARIO 93-type}{pub}
\dxdef{PROCARIO 93-label}{PROCARIO 93 (CLEO)}
\dxdef{PROCARIO 93-meas}{%
\multicolumn{2}{l}{\dxuse{PROCARIO 93-label}\,\dxuse{PROCARIO 93-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma19by13-gn} = \dxuse{Gamma19by13-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma19by13.pub.PROCARIO.93-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma26by13-gn} = \dxuse{Gamma26by13-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma26by13.pub.PROCARIO.93-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma29-gn} = \dxuse{Gamma29-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma29.pub.PROCARIO.93-vu}%
}
\dxdef{RICHICHI 99-ref}{Richichi:1998bc}
\dxdef{RICHICHI 99-cite}{\cite{Richichi:1998bc}}
\dxdef{RICHICHI 99-exp}{CLEO}
\dxdef{RICHICHI 99-type}{pub}
\dxdef{RICHICHI 99-label}{RICHICHI 99 (CLEO)}
\dxdef{RICHICHI 99-meas}{%
\multicolumn{2}{l}{\dxuse{RICHICHI 99-label}\,\dxuse{RICHICHI 99-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma80by60-gn} = \dxuse{Gamma80by60-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma80by60.pub.RICHICHI.99-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma81by69-gn} = \dxuse{Gamma81by69-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma81by69.pub.RICHICHI.99-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma93by60-gn} = \dxuse{Gamma93by60-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma93by60.pub.RICHICHI.99-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma94by69-gn} = \dxuse{Gamma94by69-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma94by69.pub.RICHICHI.99-vu}%
}
\dxdef{ARMS 05-ref}{Arms:2005qg}
\dxdef{ARMS 05-cite}{\cite{Arms:2005qg}}
\dxdef{ARMS 05-exp}{CLEO3}
\dxdef{ARMS 05-type}{pub}
\dxdef{ARMS 05-label}{ARMS 05 (CLEO3)}
\dxdef{ARMS 05-meas}{%
\multicolumn{2}{l}{\dxuse{ARMS 05-label}\,\dxuse{ARMS 05-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma88-gn} = \dxuse{Gamma88-td}
\end{ensuredisplaymath} & \dxuse{CLEO3.Gamma88.pub.ARMS.05-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma94-gn} = \dxuse{Gamma94-td}
\end{ensuredisplaymath} & \dxuse{CLEO3.Gamma94.pub.ARMS.05-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma151-gn} = \dxuse{Gamma151-td}
\end{ensuredisplaymath} & \dxuse{CLEO3.Gamma151.pub.ARMS.05-vu}%
}
\dxdef{BRIERE 03-ref}{Briere:2003fr}
\dxdef{BRIERE 03-cite}{\cite{Briere:2003fr}}
\dxdef{BRIERE 03-exp}{CLEO3}
\dxdef{BRIERE 03-type}{pub}
\dxdef{BRIERE 03-label}{BRIERE 03 (CLEO3)}
\dxdef{BRIERE 03-meas}{%
\multicolumn{2}{l}{\dxuse{BRIERE 03-label}\,\dxuse{BRIERE 03-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma60-gn} = \dxuse{Gamma60-td}
\end{ensuredisplaymath} & \dxuse{CLEO3.Gamma60.pub.BRIERE.03-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma85-gn} = \dxuse{Gamma85-td}
\end{ensuredisplaymath} & \dxuse{CLEO3.Gamma85.pub.BRIERE.03-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma93-gn} = \dxuse{Gamma93-td}
\end{ensuredisplaymath} & \dxuse{CLEO3.Gamma93.pub.BRIERE.03-vu}%
}
\dxdef{ABDALLAH 06A-ref}{Abdallah:2003cw}
\dxdef{ABDALLAH 06A-cite}{\cite{Abdallah:2003cw}}
\dxdef{ABDALLAH 06A-exp}{DELPHI}
\dxdef{ABDALLAH 06A-type}{pub}
\dxdef{ABDALLAH 06A-label}{ABDALLAH 06A (DELPHI)}
\dxdef{ABDALLAH 06A-meas}{%
\multicolumn{2}{l}{\dxuse{ABDALLAH 06A-label}\,\dxuse{ABDALLAH 06A-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma8-gn} = \dxuse{Gamma8-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma8.pub.ABDALLAH.06A-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma13-gn} = \dxuse{Gamma13-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma13.pub.ABDALLAH.06A-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma19-gn} = \dxuse{Gamma19-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma19.pub.ABDALLAH.06A-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma25-gn} = \dxuse{Gamma25-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma25.pub.ABDALLAH.06A-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma57-gn} = \dxuse{Gamma57-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma57.pub.ABDALLAH.06A-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma66-gn} = \dxuse{Gamma66-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma66.pub.ABDALLAH.06A-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma74-gn} = \dxuse{Gamma74-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma74.pub.ABDALLAH.06A-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma103-gn} = \dxuse{Gamma103-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma103.pub.ABDALLAH.06A-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma104-gn} = \dxuse{Gamma104-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma104.pub.ABDALLAH.06A-vu}%
}
\dxdef{ABREU 92N-ref}{Abreu:1992gn}
\dxdef{ABREU 92N-cite}{\cite{Abreu:1992gn}}
\dxdef{ABREU 92N-exp}{DELPHI}
\dxdef{ABREU 92N-type}{pub}
\dxdef{ABREU 92N-label}{ABREU 92N (DELPHI)}
\dxdef{ABREU 92N-meas}{%
\multicolumn{2}{l}{\dxuse{ABREU 92N-label}\,\dxuse{ABREU 92N-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma7-gn} = \dxuse{Gamma7-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma7.pub.ABREU.92N-vu}%
}
\dxdef{ABREU 94K-ref}{Abreu:1994fi}
\dxdef{ABREU 94K-cite}{\cite{Abreu:1994fi}}
\dxdef{ABREU 94K-exp}{DELPHI}
\dxdef{ABREU 94K-type}{pub}
\dxdef{ABREU 94K-label}{ABREU 94K (DELPHI)}
\dxdef{ABREU 94K-meas}{%
\multicolumn{2}{l}{\dxuse{ABREU 94K-label}\,\dxuse{ABREU 94K-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma10-gn} = \dxuse{Gamma10-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma10.pub.ABREU.94K-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma31-gn} = \dxuse{Gamma31-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma31.pub.ABREU.94K-vu}%
}
\dxdef{ABREU 99X-ref}{Abreu:1999rb}
\dxdef{ABREU 99X-cite}{\cite{Abreu:1999rb}}
\dxdef{ABREU 99X-exp}{DELPHI}
\dxdef{ABREU 99X-type}{pub}
\dxdef{ABREU 99X-label}{ABREU 99X (DELPHI)}
\dxdef{ABREU 99X-meas}{%
\multicolumn{2}{l}{\dxuse{ABREU 99X-label}\,\dxuse{ABREU 99X-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma3-gn} = \dxuse{Gamma3-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma3.pub.ABREU.99X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma5-gn} = \dxuse{Gamma5-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma5.pub.ABREU.99X-vu}%
}
\dxdef{BYLSMA 87-ref}{Bylsma:1986zy}
\dxdef{BYLSMA 87-cite}{\cite{Bylsma:1986zy}}
\dxdef{BYLSMA 87-exp}{HRS}
\dxdef{BYLSMA 87-type}{pub}
\dxdef{BYLSMA 87-label}{BYLSMA 87 (HRS)}
\dxdef{BYLSMA 87-meas}{%
\multicolumn{2}{l}{\dxuse{BYLSMA 87-label}\,\dxuse{BYLSMA 87-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma102-gn} = \dxuse{Gamma102-td}
\end{ensuredisplaymath} & \dxuse{HRS.Gamma102.pub.BYLSMA.87-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma103-gn} = \dxuse{Gamma103-td}
\end{ensuredisplaymath} & \dxuse{HRS.Gamma103.pub.BYLSMA.87-vu}%
}
\dxdef{ACCIARRI 01F-ref}{Acciarri:2001sg}
\dxdef{ACCIARRI 01F-cite}{\cite{Acciarri:2001sg}}
\dxdef{ACCIARRI 01F-exp}{L3}
\dxdef{ACCIARRI 01F-type}{pub}
\dxdef{ACCIARRI 01F-label}{ACCIARRI 01F (L3)}
\dxdef{ACCIARRI 01F-meas}{%
\multicolumn{2}{l}{\dxuse{ACCIARRI 01F-label}\,\dxuse{ACCIARRI 01F-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma3-gn} = \dxuse{Gamma3-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma3.pub.ACCIARRI.01F-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma5-gn} = \dxuse{Gamma5-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma5.pub.ACCIARRI.01F-vu}%
}
\dxdef{ACCIARRI 95-ref}{Acciarri:1994vr}
\dxdef{ACCIARRI 95-cite}{\cite{Acciarri:1994vr}}
\dxdef{ACCIARRI 95-exp}{L3}
\dxdef{ACCIARRI 95-type}{pub}
\dxdef{ACCIARRI 95-label}{ACCIARRI 95 (L3)}
\dxdef{ACCIARRI 95-meas}{%
\multicolumn{2}{l}{\dxuse{ACCIARRI 95-label}\,\dxuse{ACCIARRI 95-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma7-gn} = \dxuse{Gamma7-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma7.pub.ACCIARRI.95-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma13-gn} = \dxuse{Gamma13-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma13.pub.ACCIARRI.95-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma19-gn} = \dxuse{Gamma19-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma19.pub.ACCIARRI.95-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma26-gn} = \dxuse{Gamma26-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma26.pub.ACCIARRI.95-vu}%
}
\dxdef{ACCIARRI 95F-ref}{Acciarri:1995kx}
\dxdef{ACCIARRI 95F-cite}{\cite{Acciarri:1995kx}}
\dxdef{ACCIARRI 95F-exp}{L3}
\dxdef{ACCIARRI 95F-type}{pub}
\dxdef{ACCIARRI 95F-label}{ACCIARRI 95F (L3)}
\dxdef{ACCIARRI 95F-meas}{%
\multicolumn{2}{l}{\dxuse{ACCIARRI 95F-label}\,\dxuse{ACCIARRI 95F-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma35-gn} = \dxuse{Gamma35-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma35.pub.ACCIARRI.95F-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma40-gn} = \dxuse{Gamma40-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma40.pub.ACCIARRI.95F-vu}%
}
\dxdef{ACHARD 01D-ref}{Achard:2001pk}
\dxdef{ACHARD 01D-cite}{\cite{Achard:2001pk}}
\dxdef{ACHARD 01D-exp}{L3}
\dxdef{ACHARD 01D-type}{pub}
\dxdef{ACHARD 01D-label}{ACHARD 01D (L3)}
\dxdef{ACHARD 01D-meas}{%
\multicolumn{2}{l}{\dxuse{ACHARD 01D-label}\,\dxuse{ACHARD 01D-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma55-gn} = \dxuse{Gamma55-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma55.pub.ACHARD.01D-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma102-gn} = \dxuse{Gamma102-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma102.pub.ACHARD.01D-vu}%
}
\dxdef{ADEVA 91F-ref}{Adeva:1991qq}
\dxdef{ADEVA 91F-cite}{\cite{Adeva:1991qq}}
\dxdef{ADEVA 91F-exp}{L3}
\dxdef{ADEVA 91F-type}{pub}
\dxdef{ADEVA 91F-label}{ADEVA 91F (L3)}
\dxdef{ADEVA 91F-meas}{%
\multicolumn{2}{l}{\dxuse{ADEVA 91F-label}\,\dxuse{ADEVA 91F-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma54-gn} = \dxuse{Gamma54-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma54.pub.ADEVA.91F-vu}%
}
\dxdef{ABBIENDI 00C-ref}{Abbiendi:1999pm}
\dxdef{ABBIENDI 00C-cite}{\cite{Abbiendi:1999pm}}
\dxdef{ABBIENDI 00C-exp}{OPAL}
\dxdef{ABBIENDI 00C-type}{pub}
\dxdef{ABBIENDI 00C-label}{ABBIENDI 00C (OPAL)}
\dxdef{ABBIENDI 00C-meas}{%
\multicolumn{2}{l}{\dxuse{ABBIENDI 00C-label}\,\dxuse{ABBIENDI 00C-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma35-gn} = \dxuse{Gamma35-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma35.pub.ABBIENDI.00C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma38-gn} = \dxuse{Gamma38-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma38.pub.ABBIENDI.00C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma43-gn} = \dxuse{Gamma43-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma43.pub.ABBIENDI.00C-vu}%
}
\dxdef{ABBIENDI 00D-ref}{Abbiendi:1999cq}
\dxdef{ABBIENDI 00D-cite}{\cite{Abbiendi:1999cq}}
\dxdef{ABBIENDI 00D-exp}{OPAL}
\dxdef{ABBIENDI 00D-type}{pub}
\dxdef{ABBIENDI 00D-label}{ABBIENDI 00D (OPAL)}
\dxdef{ABBIENDI 00D-meas}{%
\multicolumn{2}{l}{\dxuse{ABBIENDI 00D-label}\,\dxuse{ABBIENDI 00D-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma92-gn} = \dxuse{Gamma92-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma92.pub.ABBIENDI.00D-vu}%
}
\dxdef{ABBIENDI 01J-ref}{Abbiendi:2000ee}
\dxdef{ABBIENDI 01J-cite}{\cite{Abbiendi:2000ee}}
\dxdef{ABBIENDI 01J-exp}{OPAL}
\dxdef{ABBIENDI 01J-type}{pub}
\dxdef{ABBIENDI 01J-label}{ABBIENDI 01J (OPAL)}
\dxdef{ABBIENDI 01J-meas}{%
\multicolumn{2}{l}{\dxuse{ABBIENDI 01J-label}\,\dxuse{ABBIENDI 01J-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma10-gn} = \dxuse{Gamma10-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma10.pub.ABBIENDI.01J-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma31-gn} = \dxuse{Gamma31-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma31.pub.ABBIENDI.01J-vu}%
}
\dxdef{ABBIENDI 03-ref}{Abbiendi:2002jw}
\dxdef{ABBIENDI 03-cite}{\cite{Abbiendi:2002jw}}
\dxdef{ABBIENDI 03-exp}{OPAL}
\dxdef{ABBIENDI 03-type}{pub}
\dxdef{ABBIENDI 03-label}{ABBIENDI 03 (OPAL)}
\dxdef{ABBIENDI 03-meas}{%
\multicolumn{2}{l}{\dxuse{ABBIENDI 03-label}\,\dxuse{ABBIENDI 03-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma3-gn} = \dxuse{Gamma3-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma3.pub.ABBIENDI.03-vu}%
}
\dxdef{ABBIENDI 04J-ref}{Abbiendi:2004xa}
\dxdef{ABBIENDI 04J-cite}{\cite{Abbiendi:2004xa}}
\dxdef{ABBIENDI 04J-exp}{OPAL}
\dxdef{ABBIENDI 04J-type}{pub}
\dxdef{ABBIENDI 04J-label}{ABBIENDI 04J (OPAL)}
\dxdef{ABBIENDI 04J-meas}{%
\multicolumn{2}{l}{\dxuse{ABBIENDI 04J-label}\,\dxuse{ABBIENDI 04J-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma16-gn} = \dxuse{Gamma16-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma16.pub.ABBIENDI.04J-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma85-gn} = \dxuse{Gamma85-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma85.pub.ABBIENDI.04J-vu}%
}
\dxdef{ABBIENDI 99H-ref}{Abbiendi:1998cx}
\dxdef{ABBIENDI 99H-cite}{\cite{Abbiendi:1998cx}}
\dxdef{ABBIENDI 99H-exp}{OPAL}
\dxdef{ABBIENDI 99H-type}{pub}
\dxdef{ABBIENDI 99H-label}{ABBIENDI 99H (OPAL)}
\dxdef{ABBIENDI 99H-meas}{%
\multicolumn{2}{l}{\dxuse{ABBIENDI 99H-label}\,\dxuse{ABBIENDI 99H-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma5-gn} = \dxuse{Gamma5-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma5.pub.ABBIENDI.99H-vu}%
}
\dxdef{ACKERSTAFF 98M-ref}{Ackerstaff:1997tx}
\dxdef{ACKERSTAFF 98M-cite}{\cite{Ackerstaff:1997tx}}
\dxdef{ACKERSTAFF 98M-exp}{OPAL}
\dxdef{ACKERSTAFF 98M-type}{pub}
\dxdef{ACKERSTAFF 98M-label}{ACKERSTAFF 98M (OPAL)}
\dxdef{ACKERSTAFF 98M-meas}{%
\multicolumn{2}{l}{\dxuse{ACKERSTAFF 98M-label}\,\dxuse{ACKERSTAFF 98M-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma8-gn} = \dxuse{Gamma8-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma8.pub.ACKERSTAFF.98M-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma13-gn} = \dxuse{Gamma13-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma13.pub.ACKERSTAFF.98M-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma17-gn} = \dxuse{Gamma17-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma17.pub.ACKERSTAFF.98M-vu}%
}
\dxdef{ACKERSTAFF 99E-ref}{Ackerstaff:1998ia}
\dxdef{ACKERSTAFF 99E-cite}{\cite{Ackerstaff:1998ia}}
\dxdef{ACKERSTAFF 99E-exp}{OPAL}
\dxdef{ACKERSTAFF 99E-type}{pub}
\dxdef{ACKERSTAFF 99E-label}{ACKERSTAFF 99E (OPAL)}
\dxdef{ACKERSTAFF 99E-meas}{%
\multicolumn{2}{l}{\dxuse{ACKERSTAFF 99E-label}\,\dxuse{ACKERSTAFF 99E-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma103-gn} = \dxuse{Gamma103-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma103.pub.ACKERSTAFF.99E-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma104-gn} = \dxuse{Gamma104-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma104.pub.ACKERSTAFF.99E-vu}%
}
\dxdef{AKERS 94G-ref}{Akers:1994td}
\dxdef{AKERS 94G-cite}{\cite{Akers:1994td}}
\dxdef{AKERS 94G-exp}{OPAL}
\dxdef{AKERS 94G-type}{pub}
\dxdef{AKERS 94G-label}{AKERS 94G (OPAL)}
\dxdef{AKERS 94G-meas}{%
\multicolumn{2}{l}{\dxuse{AKERS 94G-label}\,\dxuse{AKERS 94G-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma33-gn} = \dxuse{Gamma33-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma33.pub.AKERS.94G-vu}%
}
\dxdef{AKERS 95Y-ref}{Akers:1995ry}
\dxdef{AKERS 95Y-cite}{\cite{Akers:1995ry}}
\dxdef{AKERS 95Y-exp}{OPAL}
\dxdef{AKERS 95Y-type}{pub}
\dxdef{AKERS 95Y-label}{AKERS 95Y (OPAL)}
\dxdef{AKERS 95Y-meas}{%
\multicolumn{2}{l}{\dxuse{AKERS 95Y-label}\,\dxuse{AKERS 95Y-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma55-gn} = \dxuse{Gamma55-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma55.pub.AKERS.95Y-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma57by55-gn} = \dxuse{Gamma57by55-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma57by55.pub.AKERS.95Y-vu}%
}
\dxdef{ALEXANDER 91D-ref}{Alexander:1991am}
\dxdef{ALEXANDER 91D-cite}{\cite{Alexander:1991am}}
\dxdef{ALEXANDER 91D-exp}{OPAL}
\dxdef{ALEXANDER 91D-type}{pub}
\dxdef{ALEXANDER 91D-label}{ALEXANDER 91D (OPAL)}
\dxdef{ALEXANDER 91D-meas}{%
\multicolumn{2}{l}{\dxuse{ALEXANDER 91D-label}\,\dxuse{ALEXANDER 91D-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma7-gn} = \dxuse{Gamma7-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma7.pub.ALEXANDER.91D-vu}%
}
\dxdef{AIHARA 87B-ref}{Aihara:1986mw}
\dxdef{AIHARA 87B-cite}{\cite{Aihara:1986mw}}
\dxdef{AIHARA 87B-exp}{TPC}
\dxdef{AIHARA 87B-type}{pub}
\dxdef{AIHARA 87B-label}{AIHARA 87B (TPC)}
\dxdef{AIHARA 87B-meas}{%
\multicolumn{2}{l}{\dxuse{AIHARA 87B-label}\,\dxuse{AIHARA 87B-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma54-gn} = \dxuse{Gamma54-td}
\end{ensuredisplaymath} & \dxuse{TPC.Gamma54.pub.AIHARA.87B-vu}%
}
\dxdef{BAUER 94-ref}{TPCTwoGamma:1993tpi}
\dxdef{BAUER 94-cite}{\cite{TPCTwoGamma:1993tpi}}
\dxdef{BAUER 94-exp}{TPC}
\dxdef{BAUER 94-type}{pub}
\dxdef{BAUER 94-label}{BAUER 94 (TPC)}
\dxdef{BAUER 94-meas}{%
\multicolumn{2}{l}{\dxuse{BAUER 94-label}\,\dxuse{BAUER 94-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma82-gn} = \dxuse{Gamma82-td}
\end{ensuredisplaymath} & \dxuse{TPC.Gamma82.pub.BAUER.94-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma92-gn} = \dxuse{Gamma92-td}
\end{ensuredisplaymath} & \dxuse{TPC.Gamma92.pub.BAUER.94-vu}%
}
\dxdef{TauBrMeasByRef}{%
\dxuse{BARATE 98-meas} \\[1.5ex]
\dxuse{BARATE 98E-meas} \\[1.5ex]
\dxuse{BARATE 99K-meas} \\[1.5ex]
\dxuse{BARATE 99R-meas} \\[1.5ex]
\dxuse{BUSKULIC 96-meas} \\[1.5ex]
\dxuse{BUSKULIC 97C-meas} \\[1.5ex]
\dxuse{SCHAEL 05C-meas} \\[1.5ex]
\dxuse{ALBRECHT 88B-meas} \\[1.5ex]
\dxuse{ALBRECHT 92D-meas} \\[1.5ex]
\dxuse{AUBERT 07AP-meas} \\[1.5ex]
\dxuse{AUBERT 08-meas} \\[1.5ex]
\dxuse{AUBERT 10F-meas} \\[1.5ex]
\dxuse{DEL-AMO-SANCHEZ 11E-meas} \\[1.5ex]
\dxuse{LEES 12X-meas} \\[1.5ex]
\dxuse{LEES 12Y-meas} \\[1.5ex]
\dxuse{LEES 18B-meas} \\[1.5ex]
\dxuse{FUJIKAWA 08-meas} \\[1.5ex]
\dxuse{INAMI 09-meas} \\[1.5ex]
\dxuse{LEE 10-meas} \\[1.5ex]
\dxuse{RYU 14vpc-meas} \\[1.5ex]
\dxuse{Belle2 ADACHI 2024-meas} \\[1.5ex]
\dxuse{BEHREND 89B-meas} \\[1.5ex]
\dxuse{ANASTASSOV 01-meas} \\[1.5ex]
\dxuse{ANASTASSOV 97-meas} \\[1.5ex]
\dxuse{ARTUSO 92-meas} \\[1.5ex]
\dxuse{ARTUSO 94-meas} \\[1.5ex]
\dxuse{BALEST 95C-meas} \\[1.5ex]
\dxuse{BARINGER 87-meas} \\[1.5ex]
\dxuse{BARTELT 96-meas} \\[1.5ex]
\dxuse{BATTLE 94-meas} \\[1.5ex]
\dxuse{BISHAI 99-meas} \\[1.5ex]
\dxuse{BORTOLETTO 93-meas} \\[1.5ex]
\dxuse{COAN 96-meas} \\[1.5ex]
\dxuse{EDWARDS 00A-meas} \\[1.5ex]
\dxuse{GIBAUT 94B-meas} \\[1.5ex]
\dxuse{PROCARIO 93-meas} \\[1.5ex]
\dxuse{RICHICHI 99-meas} \\[1.5ex]
\dxuse{ARMS 05-meas} \\[1.5ex]
\dxuse{BRIERE 03-meas} \\[1.5ex]
\dxuse{ABDALLAH 06A-meas} \\[1.5ex]
\dxuse{ABREU 92N-meas} \\[1.5ex]
\dxuse{ABREU 94K-meas} \\[1.5ex]
\dxuse{ABREU 99X-meas} \\[1.5ex]
\dxuse{BYLSMA 87-meas} \\[1.5ex]
\dxuse{ACCIARRI 01F-meas} \\[1.5ex]
\dxuse{ACCIARRI 95-meas} \\[1.5ex]
\dxuse{ACCIARRI 95F-meas} \\[1.5ex]
\dxuse{ACHARD 01D-meas} \\[1.5ex]
\dxuse{ADEVA 91F-meas} \\[1.5ex]
\dxuse{ABBIENDI 00C-meas} \\[1.5ex]
\dxuse{ABBIENDI 00D-meas} \\[1.5ex]
\dxuse{ABBIENDI 01J-meas} \\[1.5ex]
\dxuse{ABBIENDI 03-meas} \\[1.5ex]
\dxuse{ABBIENDI 04J-meas} \\[1.5ex]
\dxuse{ABBIENDI 99H-meas} \\[1.5ex]
\dxuse{ACKERSTAFF 98M-meas} \\[1.5ex]
\dxuse{ACKERSTAFF 99E-meas} \\[1.5ex]
\dxuse{AKERS 94G-meas} \\[1.5ex]
\dxuse{AKERS 95Y-meas} \\[1.5ex]
\dxuse{ALEXANDER 91D-meas} \\[1.5ex]
\dxuse{AIHARA 87B-meas} \\[1.5ex]
\dxuse{BAUER 94-meas}%
}
\dxdef{TauBrStrangeVal}{%
\dxQuantLine{Gamma10}{0.6965 \pm 0.0096}{-2} 
\dxQuantLine{Gamma16}{0.4328 \pm 0.0148}{-2} 
\dxQuantLine{Gamma23}{0.0647 \pm 0.0218}{-2} 
\dxQuantLine{Gamma28}{0.0477 \pm 0.0212}{-2} 
\dxQuantLine{Gamma35}{0.8384 \pm 0.0138}{-2} 
\dxQuantLine{Gamma40}{0.3817 \pm 0.0129}{-2} 
\dxQuantLine{Gamma44}{0.0263 \pm 0.0226}{-2} 
\dxQuantLine{Gamma53}{0.0247 \pm 0.0199}{-2} 
\dxQuantLine{Gamma128}{0.0155 \pm 0.0008}{-2} 
\dxQuantLine{Gamma130}{0.0048 \pm 0.0012}{-2} 
\dxQuantLine{Gamma132}{0.0094 \pm 0.0015}{-2} 
\dxQuantLine{Gamma151}{0.0410 \pm 0.0092}{-2} 
\dxQuantLine{Gamma168}{0.0022 \pm 0.0008}{-2} 
\dxQuantLine{Gamma169}{0.0015 \pm 0.0006}{-2} 
\dxQuantLine{Gamma802}{0.2927 \pm 0.0068}{-2} 
\dxQuantLine{Gamma803}{0.0394 \pm 0.0142}{-2} 
\dxQuantLine{Gamma822}{0.0001 \pm 0.0001}{-2} 
\dxQuantLine{Gamma833}{0.0001 \pm 0.0001}{-2}%
}
\dxdef{TauBrStrangeTotVal}{%
\dxQuantLine{Gamma110}{2.9196 \pm 0.0442}{-2}%
}
\dxdef{TauBrUnitarityQuants}{%
\dxConstrQuantValWeight{Gamma3}{0.1737 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma5}{0.1785 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma9}{0.1082 \pm 0.0005}{1.0000} 
\dxConstrQuantValWeight{Gamma10}{0.00697 \pm 0.00010}{1.0000} 
\dxConstrQuantValWeight{Gamma14}{0.2549 \pm 0.0009}{1.0000} 
\dxConstrQuantValWeight{Gamma16}{0.00433 \pm 0.00015}{1.0000} 
\dxConstrQuantValWeight{Gamma20}{0.0926 \pm 0.0010}{1.0000} 
\dxConstrQuantValWeight{Gamma23}{(0.65 \pm 0.22)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma27}{0.0104 \pm 0.0007}{1.0000} 
\dxConstrQuantValWeight{Gamma28}{(0.48 \pm 0.21)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma30}{0.0011 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma35}{0.00838 \pm 0.00014}{1.0000} 
\dxConstrQuantValWeight{Gamma37}{0.001486 \pm 0.000034}{1.0000} 
\dxConstrQuantValWeight{Gamma40}{0.00382 \pm 0.00013}{1.0000} 
\dxConstrQuantValWeight{Gamma42}{0.00150 \pm 0.00007}{1.0000} 
\dxConstrQuantValWeight{Gamma44}{(0.26 \pm 0.23)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma47}{(235 \pm 6)\cdot 10^{-6}}{2.0000} 
\dxConstrQuantValWeight{Gamma48}{0.00108 \pm 0.00024}{1.0000} 
\dxConstrQuantValWeight{Gamma50}{(18.2 \pm 2.1)\cdot 10^{-6}}{2.0000} 
\dxConstrQuantValWeight{Gamma51}{(0.32 \pm 0.12)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma53}{(0.25 \pm 0.20)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma62}{0.0899 \pm 0.0005}{1.0000} 
\dxConstrQuantValWeight{Gamma70}{0.0274 \pm 0.0007}{1.0000} 
\dxConstrQuantValWeight{Gamma77}{0.0010 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma93}{0.001435 \pm 0.000027}{1.0000} 
\dxConstrQuantValWeight{Gamma94}{(61 \pm 18)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma126}{0.00139 \pm 0.00007}{1.0000} 
\dxConstrQuantValWeight{Gamma128}{(155 \pm 8)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma130}{(48 \pm 12)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma132}{(94 \pm 15)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma136}{(220 \pm 13)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma151}{(0.41 \pm 0.09)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma152}{0.0041 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma167}{(44 \pm 16)\cdot 10^{-6}}{0.8300} 
\dxConstrQuantValWeight{Gamma800}{0.0195 \pm 0.0006}{1.0000} 
\dxConstrQuantValWeight{Gamma802}{0.00293 \pm 0.00007}{1.0000} 
\dxConstrQuantValWeight{Gamma803}{(0.39 \pm 0.14)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma805}{(0.40 \pm 0.15)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma811}{(72 \pm 16)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma812}{(14 \pm 27)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma821}{(775 \pm 30)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma822}{(0.6 \pm 1.2)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma831}{(84 \pm 6)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma832}{(38 \pm 9)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma833}{(1.1 \pm 0.6)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma920}{(52 \pm 4)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma945}{(0.19 \pm 0.04)\cdot 10^{-3}}{1.0000}%
}
\dxdef{TauBrUnitarityQuantsPdgPatch}{%
\dxConstrQuantValWeight{Gamma3}{0.1737 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma5}{0.1785 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma9}{0.1082 \pm 0.0005}{1.0000} 
\dxConstrQuantValWeight{Gamma10}{0.00697 \pm 0.00010}{1.0000} 
\dxConstrQuantValWeight{Gamma14}{0.2549 \pm 0.0009}{1.0000} 
\dxConstrQuantValWeight{Gamma16}{0.00433 \pm 0.00015}{1.0000} 
\dxConstrQuantValWeight{Gamma20}{0.0926 \pm 0.0010}{1.0022} 
\dxConstrQuantValWeight{Gamma23}{(0.65 \pm 0.22)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma27}{0.0104 \pm 0.0007}{1.0000} 
\dxConstrQuantValWeight{Gamma28}{(0.48 \pm 0.21)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma30}{0.0011 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma35}{0.00838 \pm 0.00014}{1.0000} 
\dxConstrQuantValWeight{Gamma37}{0.001486 \pm 0.000034}{1.0000} 
\dxConstrQuantValWeight{Gamma40}{0.00382 \pm 0.00013}{1.0000} 
\dxConstrQuantValWeight{Gamma42}{0.00150 \pm 0.00007}{1.0000} 
\dxConstrQuantValWeight{Gamma44}{(0.26 \pm 0.23)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma47}{(235 \pm 6)\cdot 10^{-6}}{2.0000} 
\dxConstrQuantValWeight{Gamma48}{0.00108 \pm 0.00024}{1.0000} 
\dxConstrQuantValWeight{Gamma50}{(18.2 \pm 2.1)\cdot 10^{-6}}{2.0000} 
\dxConstrQuantValWeight{Gamma51}{(0.32 \pm 0.12)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma53}{(0.25 \pm 0.20)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma62}{0.0899 \pm 0.0005}{1.0022} 
\dxConstrQuantValWeight{Gamma70}{0.0274 \pm 0.0007}{1.0000} 
\dxConstrQuantValWeight{Gamma77}{0.0010 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma93}{0.001435 \pm 0.000027}{1.0000} 
\dxConstrQuantValWeight{Gamma94}{(61 \pm 18)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma126}{0.00139 \pm 0.00007}{1.0000} 
\dxConstrQuantValWeight{Gamma128}{(155 \pm 8)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma130}{(48 \pm 12)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma132}{(94 \pm 15)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma136}{(220 \pm 13)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma151}{(0.41 \pm 0.09)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma152}{0.0041 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma167}{(44 \pm 16)\cdot 10^{-6}}{0.8300} 
\dxConstrQuantValWeight{Gamma800}{0.0195 \pm 0.0006}{1.0000} 
\dxConstrQuantValWeight{Gamma802}{0.00293 \pm 0.00007}{1.0000} 
\dxConstrQuantValWeight{Gamma803}{(0.39 \pm 0.14)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma811}{(72 \pm 16)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma812}{(14 \pm 27)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma821}{(775 \pm 30)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma822}{(0.6 \pm 1.2)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma831}{(84 \pm 6)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma832}{(38 \pm 9)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma833}{(1.1 \pm 0.6)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma920}{(52 \pm 4)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma945}{(0.19 \pm 0.04)\cdot 10^{-3}}{1.0000}%
}
\dxdef{TauBrBaseQuants}{%
\dxQuantLine{Gamma3}{17.3657 \pm 0.0355}{-2} 
\dxQuantLine{Gamma5}{17.8468 \pm 0.0368}{-2} 
\dxQuantLine{Gamma9}{10.8151 \pm 0.0512}{-2} 
\dxQuantLine{Gamma10}{0.6965 \pm 0.0096}{-2} 
\dxQuantLine{Gamma14}{25.4931 \pm 0.0893}{-2} 
\dxQuantLine{Gamma16}{0.4328 \pm 0.0148}{-2} 
\dxQuantLine{Gamma20}{9.2590 \pm 0.0964}{-2} 
\dxQuantLine{Gamma23}{0.0647 \pm 0.0218}{-2} 
\dxQuantLine{Gamma27}{1.0435 \pm 0.0707}{-2} 
\dxQuantLine{Gamma28}{0.0477 \pm 0.0212}{-2} 
\dxQuantLine{Gamma30}{0.1121 \pm 0.0391}{-2} 
\dxQuantLine{Gamma35}{0.8384 \pm 0.0138}{-2} 
\dxQuantLine{Gamma37}{0.1486 \pm 0.0034}{-2} 
\dxQuantLine{Gamma40}{0.3817 \pm 0.0129}{-2} 
\dxQuantLine{Gamma42}{0.1500 \pm 0.0070}{-2} 
\dxQuantLine{Gamma44}{0.0263 \pm 0.0226}{-2} 
\dxQuantLine{Gamma47}{0.0235 \pm 0.0006}{-2} 
\dxQuantLine{Gamma48}{0.1080 \pm 0.0242}{-2} 
\dxQuantLine{Gamma50}{0.0018 \pm 0.0002}{-2} 
\dxQuantLine{Gamma51}{0.0325 \pm 0.0119}{-2} 
\dxQuantLine{Gamma53}{0.0247 \pm 0.0199}{-2} 
\dxQuantLine{Gamma62}{8.9860 \pm 0.0513}{-2} 
\dxQuantLine{Gamma70}{2.7405 \pm 0.0710}{-2} 
\dxQuantLine{Gamma77}{0.0980 \pm 0.0357}{-2} 
\dxQuantLine{Gamma93}{0.1435 \pm 0.0027}{-2} 
\dxQuantLine{Gamma94}{0.0061 \pm 0.0018}{-2} 
\dxQuantLine{Gamma126}{0.1389 \pm 0.0072}{-2} 
\dxQuantLine{Gamma128}{0.0155 \pm 0.0008}{-2} 
\dxQuantLine{Gamma130}{0.0048 \pm 0.0012}{-2} 
\dxQuantLine{Gamma132}{0.0094 \pm 0.0015}{-2} 
\dxQuantLine{Gamma136}{0.0220 \pm 0.0013}{-2} 
\dxQuantLine{Gamma151}{0.0410 \pm 0.0092}{-2} 
\dxQuantLine{Gamma152}{0.4085 \pm 0.0419}{-2} 
\dxQuantLine{Gamma167}{0.0044 \pm 0.0016}{-2} 
\dxQuantLine{Gamma800}{1.9494 \pm 0.0645}{-2} 
\dxQuantLine{Gamma802}{0.2927 \pm 0.0068}{-2} 
\dxQuantLine{Gamma803}{0.0394 \pm 0.0142}{-2} 
\dxQuantLine{Gamma811}{0.0072 \pm 0.0016}{-2} 
\dxQuantLine{Gamma812}{0.0014 \pm 0.0027}{-2} 
\dxQuantLine{Gamma821}{0.0775 \pm 0.0030}{-2} 
\dxQuantLine{Gamma822}{0.0001 \pm 0.0001}{-2} 
\dxQuantLine{Gamma831}{0.0084 \pm 0.0006}{-2} 
\dxQuantLine{Gamma832}{0.0038 \pm 0.0009}{-2} 
\dxQuantLine{Gamma833}{0.0001 \pm 0.0001}{-2} 
\dxQuantLine{Gamma920}{0.0052 \pm 0.0004}{-2} 
\dxQuantLine{Gamma945}{0.0194 \pm 0.0038}{-2} 
\dxQuantLine{Gamma980}{0.2171 \pm 0.0792}{-2}%
}
\dxdef{TauBrBaseQuantCorr}{%
 & \(\BR_{3}\) & \(\BR_{5}\) & \(\BR_{9}\) & \(\BR_{10}\) & \(\BR_{14}\) & \(\BR_{16}\) & \(\BR_{20}\) & \(\BR_{23}\) & \(\BR_{27}\) & \(\BR_{28}\) & \(\BR_{30}\) & \(\BR_{35}\) & \(\BR_{37}\) & \(\BR_{40}\) \\
\(\BR_{3}\) &  100 &   39 &    2 &    3 &  -20 &   -1 &  -12 &   -1 &   -7 &   -1 &   -5 &   -3 &   -1 &   -2 \\
\(\BR_{5}\) &   39 &  100 &    0 &    4 &  -20 &   -1 &  -12 &    0 &   -6 &   -1 &   -4 &   -3 &   -1 &   -2 \\
\(\BR_{9}\) &    2 &    0 &  100 &    5 &  -17 &    0 &  -14 &   -2 &  -10 &   -1 &  -11 &   -3 &    1 &   -2 \\
\(\BR_{10}\) &    3 &    4 &    5 &  100 &   -5 &   -2 &   -4 &   -3 &   -1 &   -2 &   -1 &   -1 &    0 &   -1 \\
\(\BR_{14}\) &  -20 &  -20 &  -17 &   -5 &  100 &   -9 &  -46 &   -1 &    0 &    0 &   -9 &   -1 &    0 &   -1 \\
\(\BR_{16}\) &   -1 &   -1 &    0 &   -2 &   -9 &  100 &   -1 &  -14 &    1 &  -13 &    0 &   -1 &    0 &    0 \\
\(\BR_{20}\) &  -12 &  -12 &  -14 &   -4 &  -46 &   -1 &  100 &  -10 &  -39 &   -3 &    7 &   -2 &    0 &   -2 \\
\(\BR_{23}\) &   -1 &    0 &   -2 &   -3 &   -1 &  -14 &  -10 &  100 &    1 &  -23 &   -2 &    0 &   -2 &    0 \\
\(\BR_{27}\) &   -7 &   -6 &  -10 &   -1 &    0 &    1 &  -39 &    1 &  100 &  -11 &  -44 &   -1 &    0 &   -1 \\
\(\BR_{28}\) &   -1 &   -1 &   -1 &   -2 &    0 &  -13 &   -3 &  -23 &  -11 &  100 &    2 &    0 &   -2 &    0 \\
\(\BR_{30}\) &   -5 &   -4 &  -11 &   -1 &   -9 &    0 &    7 &   -2 &  -44 &    2 &  100 &    0 &    0 &    0 \\
\(\BR_{35}\) &   -3 &   -3 &   -3 &   -1 &   -1 &   -1 &   -2 &    0 &   -1 &    0 &    0 &  100 &  -15 &  -13 \\
\(\BR_{37}\) &   -1 &   -1 &    1 &    0 &    0 &    0 &    0 &   -2 &    0 &   -2 &    0 &  -15 &  100 &    2 \\
\(\BR_{40}\) &   -2 &   -2 &   -2 &   -1 &   -1 &    0 &   -2 &    0 &   -1 &    0 &    0 &  -13 &    2 &  100 \\[1.5ex]
 & \(\BR_{3}\) & \(\BR_{5}\) & \(\BR_{9}\) & \(\BR_{10}\) & \(\BR_{14}\) & \(\BR_{16}\) & \(\BR_{20}\) & \(\BR_{23}\) & \(\BR_{27}\) & \(\BR_{28}\) & \(\BR_{30}\) & \(\BR_{35}\) & \(\BR_{37}\) & \(\BR_{40}\) \\
\(\BR_{42}\) &   -1 &   -1 &   -1 &   -1 &    0 &   -3 &    0 &   -5 &    0 &   -5 &    0 &   -1 &  -14 &  -20 \\
\(\BR_{44}\) &   -5 &   -5 &   -5 &   -2 &   -3 &   -1 &   -4 &   -2 &   -1 &   -2 &    0 &   -3 &    0 &   -6 \\
\(\BR_{47}\) &   -1 &   -1 &    2 &    0 &   -1 &    2 &   -1 &   -1 &    0 &   -1 &    0 &   -2 &    3 &   -4 \\
\(\BR_{48}\) &   -5 &   -5 &   -5 &   -2 &   -3 &   -1 &   -5 &   -2 &   -1 &   -2 &    0 &   -5 &    0 &   -4 \\
\(\BR_{50}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &   -1 &    0 &    1 &    5 &   -1 \\
\(\BR_{51}\) &   -2 &   -2 &   -2 &   -1 &   -1 &   -1 &   -2 &   -1 &   -1 &   -1 &    0 &   -2 &    0 &   -2 \\
\(\BR_{53}\) &   -5 &   -5 &   -5 &   -2 &   -3 &   -1 &   -4 &   -2 &   -1 &   -2 &    0 &   -2 &    0 &   -2 \\
\(\BR_{62}\) &   -8 &   -9 &    4 &   -2 &   -6 &    3 &  -12 &   -2 &   -7 &   -1 &   -5 &   -2 &    3 &   -2 \\
\(\BR_{70}\) &   -4 &   -4 &   -5 &    0 &   -9 &    0 &    1 &    1 &   -1 &    1 &    3 &    1 &   -1 &    1 \\
\(\BR_{77}\) &    0 &    0 &   -2 &    0 &   -2 &    0 &    0 &    0 &    2 &    0 &    2 &    0 &    0 &    0 \\
\(\BR_{93}\) &   -2 &   -2 &    2 &   -1 &   -1 &    1 &   -2 &   -1 &   -1 &   -1 &   -1 &   -1 &    1 &    0 \\
\(\BR_{94}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{126}\) &   -1 &   -1 &   -1 &    0 &   -1 &    0 &   -2 &   -1 &    0 &   -1 &   -2 &   -1 &    0 &    0 \\
\(\BR_{128}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &   -1 &    0 &    0 &    1 &    0 \\[1.5ex]
 & \(\BR_{3}\) & \(\BR_{5}\) & \(\BR_{9}\) & \(\BR_{10}\) & \(\BR_{14}\) & \(\BR_{16}\) & \(\BR_{20}\) & \(\BR_{23}\) & \(\BR_{27}\) & \(\BR_{28}\) & \(\BR_{30}\) & \(\BR_{35}\) & \(\BR_{37}\) & \(\BR_{40}\) \\
\(\BR_{130}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{132}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{136}\) &   -1 &   -1 &    1 &    0 &   -1 &    1 &   -1 &    0 &   -1 &    0 &   -1 &    0 &    1 &    0 \\
\(\BR_{151}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{152}\) &   -2 &   -2 &   -5 &   -1 &   -3 &    0 &   -2 &   -1 &    2 &   -1 &    2 &   -1 &    0 &    0 \\
\(\BR_{167}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{800}\) &   -3 &   -3 &   -3 &   -1 &   -4 &    0 &   -1 &    0 &   -1 &    0 &    1 &    0 &    0 &    0 \\
\(\BR_{802}\) &   -2 &   -2 &   -1 &   -1 &   -1 &   -1 &   -3 &   -1 &   -2 &   -1 &   -1 &   -1 &    0 &   -1 \\
\(\BR_{803}\) &    1 &    1 &    0 &   -1 &    1 &   -1 &   -1 &   -1 &    0 &   -1 &   -1 &   -1 &    0 &   -1 \\
\(\BR_{811}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{812}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{821}\) &   -1 &   -1 &    1 &    0 &   -1 &    1 &   -2 &   -1 &   -1 &    0 &   -1 &   -1 &    1 &    0 \\
\(\BR_{822}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{831}\) &   -1 &   -1 &    0 &    0 &   -1 &    1 &   -1 &    0 &    0 &    0 &   -1 &    0 &    1 &    0 \\[1.5ex]
 & \(\BR_{3}\) & \(\BR_{5}\) & \(\BR_{9}\) & \(\BR_{10}\) & \(\BR_{14}\) & \(\BR_{16}\) & \(\BR_{20}\) & \(\BR_{23}\) & \(\BR_{27}\) & \(\BR_{28}\) & \(\BR_{30}\) & \(\BR_{35}\) & \(\BR_{37}\) & \(\BR_{40}\) \\
\(\BR_{832}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{833}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{920}\) &   -1 &   -1 &    1 &    0 &    0 &    1 &   -1 &    0 &    0 &    0 &   -1 &    0 &    1 &    0 \\
\(\BR_{945}\) &   -1 &   -1 &    0 &    0 &   -1 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{980}\) &   -4 &   -4 &   -3 &   -1 &   -2 &   -1 &   -3 &   -1 &   -1 &   -1 &    0 &   -1 &    0 &   -1 \\[1.5ex]

 & \(\BR_{42}\) & \(\BR_{44}\) & \(\BR_{47}\) & \(\BR_{48}\) & \(\BR_{50}\) & \(\BR_{51}\) & \(\BR_{53}\) & \(\BR_{62}\) & \(\BR_{70}\) & \(\BR_{77}\) & \(\BR_{93}\) & \(\BR_{94}\) & \(\BR_{126}\) & \(\BR_{128}\) \\
\(\BR_{3}\) &   -1 &   -5 &   -1 &   -5 &    0 &   -2 &   -5 &   -8 &   -4 &    0 &   -2 &    0 &   -1 &    0 \\
\(\BR_{5}\) &   -1 &   -5 &   -1 &   -5 &    0 &   -2 &   -5 &   -9 &   -4 &    0 &   -2 &    0 &   -1 &    0 \\
\(\BR_{9}\) &   -1 &   -5 &    2 &   -5 &    0 &   -2 &   -5 &    4 &   -5 &   -2 &    2 &    0 &   -1 &    0 \\
\(\BR_{10}\) &   -1 &   -2 &    0 &   -2 &    0 &   -1 &   -2 &   -2 &    0 &    0 &   -1 &    0 &    0 &    0 \\
\(\BR_{14}\) &    0 &   -3 &   -1 &   -3 &    0 &   -1 &   -3 &   -6 &   -9 &   -2 &   -1 &    0 &   -1 &    0 \\
\(\BR_{16}\) &   -3 &   -1 &    2 &   -1 &    0 &   -1 &   -1 &    3 &    0 &    0 &    1 &    0 &    0 &    0 \\
\(\BR_{20}\) &    0 &   -4 &   -1 &   -5 &    0 &   -2 &   -4 &  -12 &    1 &    0 &   -2 &    0 &   -2 &    0 \\
\(\BR_{23}\) &   -5 &   -2 &   -1 &   -2 &   -1 &   -1 &   -2 &   -2 &    1 &    0 &   -1 &    0 &   -1 &   -1 \\
\(\BR_{27}\) &    0 &   -1 &    0 &   -1 &    0 &   -1 &   -1 &   -7 &   -1 &    2 &   -1 &    0 &    0 &    0 \\
\(\BR_{28}\) &   -5 &   -2 &   -1 &   -2 &   -1 &   -1 &   -2 &   -1 &    1 &    0 &   -1 &    0 &   -1 &   -1 \\
\(\BR_{30}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -5 &    3 &    2 &   -1 &    0 &   -2 &    0 \\
\(\BR_{35}\) &   -1 &   -3 &   -2 &   -5 &    1 &   -2 &   -2 &   -2 &    1 &    0 &   -1 &    0 &   -1 &    0 \\
\(\BR_{37}\) &  -14 &    0 &    3 &    0 &    5 &    0 &    0 &    3 &   -1 &    0 &    1 &    0 &    0 &    1 \\
\(\BR_{40}\) &  -20 &   -6 &   -4 &   -4 &   -1 &   -2 &   -2 &   -2 &    1 &    0 &    0 &    0 &    0 &    0 \\[1.5ex]
 & \(\BR_{42}\) & \(\BR_{44}\) & \(\BR_{47}\) & \(\BR_{48}\) & \(\BR_{50}\) & \(\BR_{51}\) & \(\BR_{53}\) & \(\BR_{62}\) & \(\BR_{70}\) & \(\BR_{77}\) & \(\BR_{93}\) & \(\BR_{94}\) & \(\BR_{126}\) & \(\BR_{128}\) \\
\(\BR_{42}\) &  100 &    0 &    1 &   -1 &    6 &   -1 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{44}\) &    0 &  100 &    0 &  -10 &    0 &   -4 &   -4 &   -4 &    2 &    0 &   -1 &    0 &   -1 &    0 \\
\(\BR_{47}\) &    1 &    0 &  100 &   -1 &   -7 &    0 &    0 &    5 &   -1 &    0 &    2 &    0 &    0 &    1 \\
\(\BR_{48}\) &   -1 &  -10 &   -1 &  100 &    0 &   -8 &   -4 &   -4 &    2 &    0 &   -1 &    0 &   -1 &    0 \\
\(\BR_{50}\) &    6 &    0 &   -7 &    0 &  100 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{51}\) &   -1 &   -4 &    0 &   -8 &    0 &  100 &   -2 &   -2 &    1 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{53}\) &    0 &   -4 &    0 &   -4 &    0 &   -2 &  100 &   -4 &    2 &    0 &   -1 &    0 &   -1 &    0 \\
\(\BR_{62}\) &   -1 &   -4 &    5 &   -4 &    0 &   -2 &   -4 &  100 &  -19 &   -1 &   15 &   -1 &    0 &    2 \\
\(\BR_{70}\) &    0 &    2 &   -1 &    2 &    0 &    1 &    2 &  -19 &  100 &   -8 &   -4 &   -1 &    0 &    0 \\
\(\BR_{77}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &   -8 &  100 &    0 &    0 &   -5 &    0 \\
\(\BR_{93}\) &    0 &   -1 &    2 &   -1 &    0 &    0 &   -1 &   15 &   -4 &    0 &  100 &    0 &    0 &    1 \\
\(\BR_{94}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &   -1 &    0 &    0 &  100 &    0 &    0 \\
\(\BR_{126}\) &    0 &   -1 &    0 &   -1 &    0 &    0 &   -1 &    0 &    0 &   -5 &    0 &    0 &  100 &    4 \\
\(\BR_{128}\) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    2 &    0 &    0 &    1 &    0 &    4 &  100 \\[1.5ex]
 & \(\BR_{42}\) & \(\BR_{44}\) & \(\BR_{47}\) & \(\BR_{48}\) & \(\BR_{50}\) & \(\BR_{51}\) & \(\BR_{53}\) & \(\BR_{62}\) & \(\BR_{70}\) & \(\BR_{77}\) & \(\BR_{93}\) & \(\BR_{94}\) & \(\BR_{126}\) & \(\BR_{128}\) \\
\(\BR_{130}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    1 &    1 \\
\(\BR_{132}\) &    0 &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    2 &    1 \\
\(\BR_{136}\) &    0 &   -1 &    1 &   -1 &    0 &    0 &   -1 &    1 &   -1 &    0 &    1 &    0 &    0 &    0 \\
\(\BR_{151}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   12 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{152}\) &    0 &   -1 &    0 &   -1 &    0 &    0 &   -1 &   -2 &  -11 &  -64 &   -1 &    0 &    0 &    0 \\
\(\BR_{167}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    1 &    0 &    0 &    0 \\
\(\BR_{800}\) &    0 &   -1 &    0 &   -1 &    0 &    0 &   -1 &   -9 &  -67 &   -3 &   -2 &    0 &    0 &    0 \\
\(\BR_{802}\) &    0 &   -2 &    0 &   -2 &    0 &   -1 &   -2 &   19 &   -6 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{803}\) &    0 &   -1 &    0 &   -1 &    0 &   -1 &   -1 &   -4 &  -14 &   -1 &   -1 &   -3 &    0 &   -1 \\
\(\BR_{811}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{812}\) &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &   -1 &   -1 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{821}\) &    0 &   -1 &    2 &   -1 &    0 &    0 &   -1 &    3 &   -1 &    0 &    1 &    0 &    0 &    1 \\
\(\BR_{822}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{831}\) &    0 &    0 &    1 &   -1 &    0 &    0 &    0 &    1 &   -1 &    0 &    1 &    0 &    0 &    0 \\[1.5ex]
 & \(\BR_{42}\) & \(\BR_{44}\) & \(\BR_{47}\) & \(\BR_{48}\) & \(\BR_{50}\) & \(\BR_{51}\) & \(\BR_{53}\) & \(\BR_{62}\) & \(\BR_{70}\) & \(\BR_{77}\) & \(\BR_{93}\) & \(\BR_{94}\) & \(\BR_{126}\) & \(\BR_{128}\) \\
\(\BR_{832}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{833}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{920}\) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    1 &    0 &    0 &    1 &    0 &    0 &    0 \\
\(\BR_{945}\) &    0 &   -1 &    0 &   -1 &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{980}\) &    0 &   -3 &    0 &   -3 &    0 &   -1 &   -3 &   -3 &    1 &    0 &   -1 &    0 &   -1 &    0 \\[1.5ex]

 & \(\BR_{130}\) & \(\BR_{132}\) & \(\BR_{136}\) & \(\BR_{151}\) & \(\BR_{152}\) & \(\BR_{167}\) & \(\BR_{800}\) & \(\BR_{802}\) & \(\BR_{803}\) & \(\BR_{811}\) & \(\BR_{812}\) & \(\BR_{821}\) & \(\BR_{822}\) & \(\BR_{831}\) \\
\(\BR_{3}\) &    0 &    0 &   -1 &    0 &   -2 &    0 &   -3 &   -2 &    1 &    0 &    0 &   -1 &    0 &   -1 \\
\(\BR_{5}\) &    0 &    0 &   -1 &    0 &   -2 &    0 &   -3 &   -2 &    1 &    0 &    0 &   -1 &    0 &   -1 \\
\(\BR_{9}\) &    0 &    0 &    1 &    0 &   -5 &    0 &   -3 &   -1 &    0 &    0 &    0 &    1 &    0 &    0 \\
\(\BR_{10}\) &    0 &    0 &    0 &    0 &   -1 &    0 &   -1 &   -1 &   -1 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{14}\) &    0 &    0 &   -1 &    0 &   -3 &    0 &   -4 &   -1 &    1 &    0 &    0 &   -1 &    0 &   -1 \\
\(\BR_{16}\) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &   -1 &   -1 &    0 &    0 &    1 &    0 &    1 \\
\(\BR_{20}\) &    0 &    0 &   -1 &    0 &   -2 &    0 &   -1 &   -3 &   -1 &    0 &    0 &   -2 &    0 &   -1 \\
\(\BR_{23}\) &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &   -1 &   -1 &    0 &    0 &   -1 &    0 &    0 \\
\(\BR_{27}\) &    0 &    0 &   -1 &    0 &    2 &    0 &   -1 &   -2 &    0 &    0 &    0 &   -1 &    0 &    0 \\
\(\BR_{28}\) &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &   -1 &   -1 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{30}\) &    0 &    0 &   -1 &    0 &    2 &    0 &    1 &   -1 &   -1 &    0 &    0 &   -1 &    0 &   -1 \\
\(\BR_{35}\) &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &   -1 &   -1 &    0 &    0 &   -1 &    0 &    0 \\
\(\BR_{37}\) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    1 &    0 &    1 \\
\(\BR_{40}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &   -1 &    0 &    0 &    0 &    0 &    0 \\[1.5ex]
 & \(\BR_{130}\) & \(\BR_{132}\) & \(\BR_{136}\) & \(\BR_{151}\) & \(\BR_{152}\) & \(\BR_{167}\) & \(\BR_{800}\) & \(\BR_{802}\) & \(\BR_{803}\) & \(\BR_{811}\) & \(\BR_{812}\) & \(\BR_{821}\) & \(\BR_{822}\) & \(\BR_{831}\) \\
\(\BR_{42}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{44}\) &    0 &    0 &   -1 &    0 &   -1 &    0 &   -1 &   -2 &   -1 &    0 &    0 &   -1 &    0 &    0 \\
\(\BR_{47}\) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    2 &    0 &    1 \\
\(\BR_{48}\) &    0 &   -1 &   -1 &    0 &   -1 &    0 &   -1 &   -2 &   -1 &    0 &    0 &   -1 &    0 &   -1 \\
\(\BR_{50}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    0 \\
\(\BR_{51}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &   -1 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{53}\) &    0 &    0 &   -1 &    0 &   -1 &    0 &   -1 &   -2 &   -1 &    0 &    0 &   -1 &    0 &    0 \\
\(\BR_{62}\) &    0 &    0 &    1 &    0 &   -2 &   -1 &   -9 &   19 &   -4 &    0 &   -1 &    3 &    0 &    1 \\
\(\BR_{70}\) &    0 &    0 &   -1 &   12 &  -11 &    0 &  -67 &   -6 &  -14 &    0 &   -1 &   -1 &    0 &   -1 \\
\(\BR_{77}\) &   -1 &    0 &    0 &    0 &  -64 &    0 &   -3 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{93}\) &    0 &    0 &    1 &    0 &   -1 &    1 &   -2 &    0 &   -1 &    0 &    0 &    1 &    0 &    1 \\
\(\BR_{94}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -3 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{126}\) &    1 &    2 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{128}\) &    1 &    1 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    1 &    0 &    0 \\[1.5ex]
 & \(\BR_{130}\) & \(\BR_{132}\) & \(\BR_{136}\) & \(\BR_{151}\) & \(\BR_{152}\) & \(\BR_{167}\) & \(\BR_{800}\) & \(\BR_{802}\) & \(\BR_{803}\) & \(\BR_{811}\) & \(\BR_{812}\) & \(\BR_{821}\) & \(\BR_{822}\) & \(\BR_{831}\) \\
\(\BR_{130}\) &  100 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{132}\) &    0 &  100 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &   -2 &    0 &    0 &    0 \\
\(\BR_{136}\) &    0 &    0 &  100 &    0 &    0 &    0 &    0 &   -1 &    0 &   20 &   -8 &   46 &   -1 &   38 \\
\(\BR_{151}\) &    0 &    0 &    0 &  100 &    0 &    0 &  -14 &   -2 &  -58 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{152}\) &    0 &    0 &    0 &    0 &  100 &    0 &   -4 &   -1 &   -1 &    0 &   -1 &    0 &    0 &    0 \\
\(\BR_{167}\) &    0 &    0 &    0 &    0 &    0 &  100 &    0 &    1 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{800}\) &    0 &    0 &    0 &  -14 &   -4 &    0 &  100 &   -2 &   10 &    0 &    0 &   -1 &    0 &    0 \\
\(\BR_{802}\) &    0 &    0 &   -1 &   -2 &   -1 &    1 &   -2 &  100 &   -1 &    0 &    0 &   -1 &    0 &    0 \\
\(\BR_{803}\) &    0 &    0 &    0 &  -58 &   -1 &    0 &   10 &   -1 &  100 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{811}\) &    0 &   -1 &   20 &    0 &    0 &    0 &    0 &    0 &    0 &  100 &  -16 &    7 &    0 &   14 \\
\(\BR_{812}\) &    0 &   -2 &   -8 &    0 &   -1 &    0 &    0 &    0 &    0 &  -16 &  100 &   -4 &    0 &   -4 \\
\(\BR_{821}\) &    0 &    0 &   46 &    0 &    0 &    0 &   -1 &   -1 &    0 &    7 &   -4 &  100 &   -1 &   39 \\
\(\BR_{822}\) &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &  100 &   -1 \\
\(\BR_{831}\) &    0 &    0 &   38 &    0 &    0 &    0 &    0 &    0 &    0 &   14 &   -4 &   39 &   -1 &  100 \\[1.5ex]
 & \(\BR_{130}\) & \(\BR_{132}\) & \(\BR_{136}\) & \(\BR_{151}\) & \(\BR_{152}\) & \(\BR_{167}\) & \(\BR_{800}\) & \(\BR_{802}\) & \(\BR_{803}\) & \(\BR_{811}\) & \(\BR_{812}\) & \(\BR_{821}\) & \(\BR_{822}\) & \(\BR_{831}\) \\
\(\BR_{832}\) &    0 &    0 &    3 &    0 &    0 &    0 &    0 &    0 &    0 &    2 &    0 &    3 &    0 &   -2 \\
\(\BR_{833}\) &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &   -1 \\
\(\BR_{920}\) &    0 &    0 &   20 &    0 &    0 &    0 &    0 &    0 &    0 &    3 &   -2 &   34 &   -1 &   17 \\
\(\BR_{945}\) &    0 &   -1 &   25 &    0 &    0 &    0 &    0 &    0 &    0 &   10 &  -11 &    9 &    0 &   17 \\
\(\BR_{980}\) &    0 &    0 &    0 &    0 &   -1 &    0 &   -1 &   -1 &   -1 &    0 &    0 &   -1 &    0 &    0 \\[1.5ex]

 & \(\BR_{832}\) & \(\BR_{833}\) & \(\BR_{920}\) & \(\BR_{945}\) & \(\BR_{980}\) &  &  &  &  &  &  &  &  &  \\
\(\BR_{3}\) &    0 &    0 &   -1 &   -1 &   -4 &      &      &      &      &      &      &      &      &      \\
\(\BR_{5}\) &    0 &    0 &   -1 &   -1 &   -4 &      &      &      &      &      &      &      &      &      \\
\(\BR_{9}\) &    0 &    0 &    1 &    0 &   -3 &      &      &      &      &      &      &      &      &      \\
\(\BR_{10}\) &    0 &    0 &    0 &    0 &   -1 &      &      &      &      &      &      &      &      &      \\
\(\BR_{14}\) &    0 &    0 &    0 &   -1 &   -2 &      &      &      &      &      &      &      &      &      \\
\(\BR_{16}\) &    0 &    0 &    1 &    0 &   -1 &      &      &      &      &      &      &      &      &      \\
\(\BR_{20}\) &    0 &    0 &   -1 &   -1 &   -3 &      &      &      &      &      &      &      &      &      \\
\(\BR_{23}\) &    0 &    0 &    0 &    0 &   -1 &      &      &      &      &      &      &      &      &      \\
\(\BR_{27}\) &    0 &    0 &    0 &    0 &   -1 &      &      &      &      &      &      &      &      &      \\
\(\BR_{28}\) &    0 &    0 &    0 &    0 &   -1 &      &      &      &      &      &      &      &      &      \\
\(\BR_{30}\) &    0 &    0 &   -1 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{35}\) &    0 &    0 &    0 &    0 &   -1 &      &      &      &      &      &      &      &      &      \\
\(\BR_{37}\) &    0 &    0 &    1 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{40}\) &    0 &    0 &    0 &    0 &   -1 &      &      &      &      &      &      &      &      &      \\[1.5ex]
 & \(\BR_{832}\) & \(\BR_{833}\) & \(\BR_{920}\) & \(\BR_{945}\) & \(\BR_{980}\) &  &  &  &  &  &  &  &  &  \\
\(\BR_{42}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{44}\) &    0 &    0 &    0 &   -1 &   -3 &      &      &      &      &      &      &      &      &      \\
\(\BR_{47}\) &    0 &    0 &    1 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{48}\) &    0 &    0 &    0 &   -1 &   -3 &      &      &      &      &      &      &      &      &      \\
\(\BR_{50}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{51}\) &    0 &    0 &    0 &    0 &   -1 &      &      &      &      &      &      &      &      &      \\
\(\BR_{53}\) &    0 &    0 &    0 &   -1 &   -3 &      &      &      &      &      &      &      &      &      \\
\(\BR_{62}\) &    0 &    0 &    1 &    0 &   -3 &      &      &      &      &      &      &      &      &      \\
\(\BR_{70}\) &    0 &    0 &    0 &    0 &    1 &      &      &      &      &      &      &      &      &      \\
\(\BR_{77}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{93}\) &    0 &    0 &    1 &    0 &   -1 &      &      &      &      &      &      &      &      &      \\
\(\BR_{94}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{126}\) &    0 &    0 &    0 &    0 &   -1 &      &      &      &      &      &      &      &      &      \\
\(\BR_{128}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\[1.5ex]
 & \(\BR_{832}\) & \(\BR_{833}\) & \(\BR_{920}\) & \(\BR_{945}\) & \(\BR_{980}\) &  &  &  &  &  &  &  &  &  \\
\(\BR_{130}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{132}\) &    0 &    0 &    0 &   -1 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{136}\) &    3 &   -1 &   20 &   25 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{151}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{152}\) &    0 &    0 &    0 &    0 &   -1 &      &      &      &      &      &      &      &      &      \\
\(\BR_{167}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{800}\) &    0 &    0 &    0 &    0 &   -1 &      &      &      &      &      &      &      &      &      \\
\(\BR_{802}\) &    0 &    0 &    0 &    0 &   -1 &      &      &      &      &      &      &      &      &      \\
\(\BR_{803}\) &    0 &    0 &    0 &    0 &   -1 &      &      &      &      &      &      &      &      &      \\
\(\BR_{811}\) &    2 &    0 &    3 &   10 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{812}\) &    0 &    0 &   -2 &  -11 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{821}\) &    3 &   -1 &   34 &    9 &   -1 &      &      &      &      &      &      &      &      &      \\
\(\BR_{822}\) &    0 &    0 &   -1 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{831}\) &   -2 &   -1 &   17 &   17 &    0 &      &      &      &      &      &      &      &      &      \\[1.5ex]
 & \(\BR_{832}\) & \(\BR_{833}\) & \(\BR_{920}\) & \(\BR_{945}\) & \(\BR_{980}\) &  &  &  &  &  &  &  &  &  \\
\(\BR_{832}\) &  100 &   -1 &    1 &    2 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{833}\) &   -1 &  100 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{920}\) &    1 &    0 &  100 &    4 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{945}\) &    2 &    0 &    4 &  100 &   -1 &      &      &      &      &      &      &      &      &      \\
\(\BR_{980}\) &    0 &    0 &    0 &   -1 &  100 &      &      &      &      &      &      &      &      &     %
}
\dxConstrDef{Gamma1}{\BR_{1}}{\BR_{3} + \BR_{5} + \BR_{9} + \BR_{10} + \BR_{14} + \BR_{16} \\
  {}& + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35} \\
  {}& + \BR_{40} + \BR_{44} + \BR_{37} + \BR_{42} + \BR_{47} + \BR_{48} \\
  {}& + \BR_{804} + \BR_{50} + \BR_{51} + \BR_{806} + \BR_{126}\cdot{}\BR_{\eta\to\text{neutral}} \\
  {}& + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{132}\cdot{}\BR_{\eta\to\text{neutral}} \\
  {}& + \BR_{800}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{151}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{152}\cdot{}\BR_{\omega\to\pi^0\gamma} \\
  {}& + \BR_{167}\cdot{}\BR_{\phi\to K_S K_L}}
\dxConstrDef{Gamma2}{\BR_{2}}{\BR_{3} + \BR_{5} + \BR_{9} + \BR_{10} + \BR_{14} + \BR_{16} \\
  {}& + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\\
  {}& +\BR_{<\bar{K}^0|K_L>}) + \BR_{40}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{44}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\\
  {}& +\BR_{<\bar{K}^0|K_L>}) + \BR_{37}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{42}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\\
  {}& +\BR_{<\bar{K}^0|K_L>}) + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{48}\cdot{}\BR_{K_S\to\pi^0\pi^0} \\
  {}& + \BR_{804} + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{51}\cdot{}\BR_{K_S\to\pi^0\pi^0} \\
  {}& + \BR_{806} + \BR_{126}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} \\
  {}& + \BR_{132}\cdot{}(\BR_{\eta\to\text{neutral}}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>})) + \BR_{800}\cdot{}\BR_{\omega\to\pi^0\gamma} \\
  {}& + \BR_{151}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{152}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{167}\cdot{}(\BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^0\pi^0})}
\dxConstrDef{Gamma3by5}{\BR_{3 / 5}}{\frac{\BR_{3}}{\BR_{5}}}
\dxConstrDef{Gamma7}{\BR_{7}}{\BR_{35}\cdot{}\BR_{<\bar{K}^0|K_L>} + \BR_{9} + \BR_{804} + \BR_{37}\cdot{}\BR_{<K^0|K_L>} \\
  {}& + \BR_{10}}
\dxConstrDef{Gamma8}{\BR_{8}}{\BR_{9} + \BR_{10}}
\dxConstrDef{Gamma8by5}{\BR_{8 / 5}}{\frac{\BR_{8}}{\BR_{5}}}
\dxConstrDef{Gamma9by5}{\BR_{9 / 5}}{\frac{\BR_{9}}{\BR_{5}}}
\dxConstrDef{Gamma10by5}{\BR_{10 / 5}}{\frac{\BR_{10}}{\BR_{5}}}
\dxConstrDef{Gamma10by9}{\BR_{10 / 9}}{\frac{\BR_{10}}{\BR_{9}}}
\dxConstrDef{Gamma11}{\BR_{11}}{\BR_{14} + \BR_{16} + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} \\
  {}& + \BR_{30} + \BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{126}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} \\
  {}& + \BR_{132}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to\text{neutral}}) + \BR_{151}\cdot{}\BR_{\omega\to\pi^0\gamma} \\
  {}& + \BR_{152}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{800}\cdot{}\BR_{\omega\to\pi^0\gamma}}
\dxConstrDef{Gamma12}{\BR_{12}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{30} + \BR_{23} + \BR_{28} + \BR_{14} \\
  {}& + \BR_{16} + \BR_{20} + \BR_{27} + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}
\dxConstrDef{Gamma13}{\BR_{13}}{\BR_{14} + \BR_{16}}
\dxConstrDef{Gamma17}{\BR_{17}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{30} + \BR_{23} + \BR_{28} + \BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{20} + \BR_{27} + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}
\dxConstrDef{Gamma18}{\BR_{18}}{\BR_{23} + \BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{20} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0})}
\dxConstrDef{Gamma19}{\BR_{19}}{\BR_{23} + \BR_{20}}
\dxConstrDef{Gamma19by13}{\BR_{19 / 13}}{\frac{\BR_{19}}{\BR_{13}}}
\dxConstrDef{Gamma24}{\BR_{24}}{\BR_{27} + \BR_{28} + \BR_{30} + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{128}\cdot{}\BR_{\eta\to3\pi^0} \\
  {}& + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{132}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to3\pi^0})}
\dxConstrDef{Gamma25}{\BR_{25}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{30} + \BR_{28} + \BR_{27} + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} \\
  {}& + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}
\dxConstrDef{Gamma26}{\BR_{26}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{28} + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{27}}
\dxConstrDef{Gamma26by13}{\BR_{26 / 13}}{\frac{\BR_{26}}{\BR_{13}}}
\dxConstrDef{Gamma29}{\BR_{29}}{\BR_{30} + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}
\dxConstrDef{Gamma31}{\BR_{31}}{\BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{23} + \BR_{28} + \BR_{42} + \BR_{16} \\
  {}& + \BR_{37} + \BR_{10} + \BR_{167}\cdot{}(\BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^0\pi^0})}
\dxConstrDef{Gamma32}{\BR_{32}}{\BR_{16} + \BR_{23} + \BR_{28} + \BR_{37} + \BR_{42} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} \\
  {}& + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{167}\cdot{}(\BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^0\pi^0})}
\dxConstrDef{Gamma33}{\BR_{33}}{\BR_{35}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{40}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{42}\cdot{}\BR_{<K^0|K_S>} \\
  {}& + \BR_{47} + \BR_{48} + \BR_{50} + \BR_{51} + \BR_{37}\cdot{}\BR_{<K^0|K_S>} \\
  {}& + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{\eta\to\text{neutral}}) + \BR_{44}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{167}\cdot{}\BR_{\phi\to K_S K_L}}
\dxConstrDef{Gamma34}{\BR_{34}}{\BR_{35} + \BR_{37}}
\dxConstrDef{Gamma38}{\BR_{38}}{\BR_{42} + \BR_{37}}
\dxConstrDef{Gamma39}{\BR_{39}}{\BR_{40} + \BR_{42}}
\dxConstrDef{Gamma43}{\BR_{43}}{\BR_{40} + \BR_{44}}
\dxConstrDef{Gamma46}{\BR_{46}}{\BR_{48} + \BR_{47} + \BR_{804}}
\dxConstrDef{Gamma49}{\BR_{49}}{\BR_{50} + \BR_{51} + \BR_{806}}
\dxConstrDef{Gamma54}{\BR_{54}}{\BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) \\
  {}& + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) \\
  {}& + \BR_{47}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{48}\cdot{}\BR_{K_S\to\pi^+\pi^-} \\
  {}& + \BR_{50}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{51}\cdot{}\BR_{K_S\to\pi^+\pi^-} \\
  {}& + \BR_{53}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{62} + \BR_{70} \\
  {}& + \BR_{77} + \BR_{78} + \BR_{93} + \BR_{94} + \BR_{126}\cdot{}\BR_{\eta\to\text{charged}} \\
  {}& + \BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{130}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_L>}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} \\
  {}& + \BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{\eta\to3\pi^0}) \\
  {}& + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) \\
  {}& + \BR_{167}\cdot{}(\BR_{\phi\to K^+K^-} + \BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{802} + \BR_{803} \\
  {}& + \BR_{800}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-})}
\dxConstrDef{Gamma55}{\BR_{55}}{\BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{78} \\
  {}& + \BR_{77} + \BR_{94} + \BR_{62} + \BR_{70} + \BR_{93} + \BR_{126}\cdot{}\BR_{\eta\to\text{charged}} \\
  {}& + \BR_{802} + \BR_{803} + \BR_{800}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}\\
  {}& +\BR_{\omega\to\pi^+\pi^-}) + \BR_{130}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{168}}
\dxConstrDef{Gamma56}{\BR_{56}}{\BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{62} + \BR_{93} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) \\
  {}& + \BR_{802} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{168}}
\dxConstrDef{Gamma57}{\BR_{57}}{\BR_{62} + \BR_{93} + \BR_{802} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-} \\
  {}& + \BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}
\dxConstrDef{Gamma57by55}{\BR_{57 / 55}}{\frac{\BR_{57}}{\BR_{55}}}
\dxConstrDef{Gamma58}{\BR_{58}}{\BR_{62} + \BR_{93} + \BR_{802} + \BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}
\dxConstrDef{Gamma59}{\BR_{59}}{\BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{62} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-}}
\dxConstrDef{Gamma60}{\BR_{60}}{\BR_{62} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-}}
\dxConstrDef{Gamma63}{\BR_{63}}{\BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) \\
  {}& + \BR_{47}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{70} + \BR_{77} + \BR_{78} + \BR_{94} + \BR_{126}\cdot{}\BR_{\eta\to\text{charged}} \\
  {}& + \BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{130}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{\eta\to\text{neutral}} \\
  {}& + \BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to\text{charged}}) + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}\\
  {}& +\BR_{\omega\to\pi^+\pi^-}) + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}
\dxConstrDef{Gamma64}{\BR_{64}}{\BR_{78} + \BR_{77} + \BR_{94} + \BR_{70} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} \\
  {}& + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} \\
  {}& + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{803}}
\dxConstrDef{Gamma65}{\BR_{65}}{\BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) \\
  {}& + \BR_{70} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} \\
  {}& + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}
\dxConstrDef{Gamma66}{\BR_{66}}{\BR_{70} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} \\
  {}& + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}
\dxConstrDef{Gamma67}{\BR_{67}}{\BR_{70} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{803}}
\dxConstrDef{Gamma68}{\BR_{68}}{\BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{70} + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} \\
  {}& + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma69}{\BR_{69}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{70} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma74}{\BR_{74}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{78} + \BR_{77} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} \\
  {}& + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma75}{\BR_{75}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{47}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{77} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma76}{\BR_{76}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{77} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma76by54}{\BR_{76 / 54}}{\frac{\BR_{76}}{\BR_{54}}}
\dxConstrDef{Gamma78}{\BR_{78}}{\BR_{810} + \BR_{50}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{\eta\to3\pi^0})}
\dxConstrDef{Gamma79}{\BR_{79}}{\BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) \\
  {}& + \BR_{93} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}\\
  {}& +\BR_{\omega\to\pi^+\pi^-}) + \BR_{168} + \BR_{802} + \BR_{803}}
\dxConstrDef{Gamma80}{\BR_{80}}{\BR_{93} + \BR_{802} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-}}
\dxConstrDef{Gamma80by60}{\BR_{80 / 60}}{\frac{\BR_{80}}{\BR_{60}}}
\dxConstrDef{Gamma81}{\BR_{81}}{\BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{94} + \BR_{803} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma81by69}{\BR_{81 / 69}}{\frac{\BR_{81}}{\BR_{69}}}
\dxConstrDef{Gamma82}{\BR_{82}}{\BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{802} \\
  {}& + \BR_{803} + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})}
\dxConstrDef{Gamma83}{\BR_{83}}{\BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{802} + \BR_{803} + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}\\
  {}& +\BR_{\omega\to\pi^+\pi^-})}
\dxConstrDef{Gamma84}{\BR_{84}}{\BR_{802} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})}
\dxConstrDef{Gamma85}{\BR_{85}}{\BR_{802} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-}}
\dxConstrDef{Gamma85by60}{\BR_{85 / 60}}{\frac{\BR_{85}}{\BR_{60}}}
\dxConstrDef{Gamma87}{\BR_{87}}{\BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} \\
  {}& + \BR_{803}}
\dxConstrDef{Gamma88}{\BR_{88}}{\BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{803} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma89}{\BR_{89}}{\BR_{803} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma92}{\BR_{92}}{\BR_{94} + \BR_{93}}
\dxConstrDef{Gamma93by60}{\BR_{93 / 60}}{\frac{\BR_{93}}{\BR_{60}}}
\dxConstrDef{Gamma94by69}{\BR_{94 / 69}}{\frac{\BR_{94}}{\BR_{69}}}
\dxConstrDef{Gamma96}{\BR_{96}}{\BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}
\dxConstrDef{Gamma102}{\BR_{102}}{\BR_{103} + \BR_{104}}
\dxConstrDef{Gamma103}{\BR_{103}}{\BR_{820} + \BR_{822} + \BR_{831}\cdot{}\BR_{\omega\to\pi^+\pi^-}}
\dxConstrDef{Gamma104}{\BR_{104}}{\BR_{830} + \BR_{833}}
\dxConstrDef{Gamma106}{\BR_{106}}{\BR_{30} + \BR_{44}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{47} + \BR_{53}\cdot{}\BR_{<K^0|K_S>} \\
  {}& + \BR_{77} + \BR_{103} + \BR_{126}\cdot{}(\BR_{\eta\to3\pi^0}+\BR_{\eta\to\pi^+\pi^-\pi^0}) + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma110}{\BR_{110}}{\BR_{10} + \BR_{16} + \BR_{23} + \BR_{28} + \BR_{35} + \BR_{40} \\
  {}& + \BR_{128} + \BR_{802} + \BR_{803} + \BR_{151} + \BR_{130} + \BR_{132} \\
  {}& + \BR_{44} + \BR_{53} + \BR_{168} + \BR_{169} + \BR_{822} + \BR_{833}}
\dxConstrDef{Gamma149}{\BR_{149}}{\BR_{152} + \BR_{800} + \BR_{151}}
\dxConstrDef{Gamma150}{\BR_{150}}{\BR_{800} + \BR_{151}}
\dxConstrDef{Gamma150by66}{\BR_{150 / 66}}{\frac{\BR_{150}}{\BR_{66}}}
\dxConstrDef{Gamma152by54}{\BR_{152 / 54}}{\frac{\BR_{152}}{\BR_{54}}}
\dxConstrDef{Gamma152by76}{\BR_{152 / 76}}{\frac{\BR_{152}}{\BR_{76}}}
\dxConstrDef{Gamma168}{\BR_{168}}{\BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}
\dxConstrDef{Gamma169}{\BR_{169}}{\BR_{167}\cdot{}\BR_{\phi\to K_S K_L}}
\dxConstrDef{Gamma804}{\BR_{804}}{\BR_{47} \cdot{} ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))}
\dxConstrDef{Gamma805}{\BR_{805}}{\BR_{980}/(1-\BR_{980})\cdot{}(\BR_{20} + \BR_{62})}
\dxConstrDef{Gamma806}{\BR_{806}}{\BR_{50} \cdot{} ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))}
\dxConstrDef{Gamma810}{\BR_{810}}{\BR_{910} + \BR_{911} + \BR_{811}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{812}}
\dxConstrDef{Gamma820}{\BR_{820}}{\BR_{920} + \BR_{821}}
\dxConstrDef{Gamma830}{\BR_{830}}{\BR_{930} + \BR_{831}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{832}}
\dxConstrDef{Gamma910}{\BR_{910}}{\BR_{136}\cdot{}\BR_{\eta\to3\pi^0}}
\dxConstrDef{Gamma911}{\BR_{911}}{\BR_{945}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma930}{\BR_{930}}{\BR_{136}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma944}{\BR_{944}}{\BR_{136}\cdot{}\BR_{\eta\to\gamma\gamma}}
\dxConstrDef{GammaAll}{\BR_{\text{all}}}{\BR_{3} + \BR_{5} + \BR_{9} + \BR_{10} + \BR_{14} + \BR_{16} \\
  {}& + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35} \\
  {}& + \BR_{37} + \BR_{40} + \BR_{42} + \BR_{47}\cdot{}(1 + ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))) \\
  {}& + \BR_{48} + \BR_{62} + \BR_{70} + \BR_{77} + \BR_{811} + \BR_{812} \\
  {}& + \BR_{93} + \BR_{94} + \BR_{832} + \BR_{833} + \BR_{126} + \BR_{128} \\
  {}& + \BR_{802} + \BR_{803} + \BR_{800} + \BR_{151} + \BR_{130} + \BR_{132} \\
  {}& + \BR_{44} + \BR_{53} + \BR_{50}\cdot{}(1 + ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))) \\
  {}& + \BR_{51} + \BR_{167}\cdot{}(\BR_{\phi\to K^+K^-}+\BR_{\phi\to K_S K_L}) + \BR_{152} + \BR_{920} \\
  {}& + \BR_{821} + \BR_{822} + \BR_{831} + \BR_{136} + \BR_{945} + \BR_{805}}
\dxConstrDef{Unitarity}{1}{\BR_{\text{all}}}
\dxdef{TauBrConstrEqs}{%
\begin{align*}
\dxuse{Gamma1-left} ={}& \dxuse{Gamma1-right}
\end{align*}
\begin{align*}
\dxuse{Gamma2-left} ={}& \dxuse{Gamma2-right}
\end{align*}
\begin{align*}
\dxuse{Gamma3by5-left} ={}& \dxuse{Gamma3by5-right}
\end{align*}
\begin{align*}
\dxuse{Gamma7-left} ={}& \dxuse{Gamma7-right}
\end{align*}
\begin{align*}
\dxuse{Gamma8-left} ={}& \dxuse{Gamma8-right}
\end{align*}
\begin{align*}
\dxuse{Gamma8by5-left} ={}& \dxuse{Gamma8by5-right}
\end{align*}
\begin{align*}
\dxuse{Gamma9by5-left} ={}& \dxuse{Gamma9by5-right}
\end{align*}
\begin{align*}
\dxuse{Gamma10by5-left} ={}& \dxuse{Gamma10by5-right}
\end{align*}
\begin{align*}
\dxuse{Gamma10by9-left} ={}& \dxuse{Gamma10by9-right}
\end{align*}
\begin{align*}
\dxuse{Gamma11-left} ={}& \dxuse{Gamma11-right}
\end{align*}
\begin{align*}
\dxuse{Gamma12-left} ={}& \dxuse{Gamma12-right}
\end{align*}
\begin{align*}
\dxuse{Gamma13-left} ={}& \dxuse{Gamma13-right}
\end{align*}
\begin{align*}
\dxuse{Gamma17-left} ={}& \dxuse{Gamma17-right}
\end{align*}
\begin{align*}
\dxuse{Gamma18-left} ={}& \dxuse{Gamma18-right}
\end{align*}
\begin{align*}
\dxuse{Gamma19-left} ={}& \dxuse{Gamma19-right}
\end{align*}
\begin{align*}
\dxuse{Gamma19by13-left} ={}& \dxuse{Gamma19by13-right}
\end{align*}
\begin{align*}
\dxuse{Gamma24-left} ={}& \dxuse{Gamma24-right}
\end{align*}
\begin{align*}
\dxuse{Gamma25-left} ={}& \dxuse{Gamma25-right}
\end{align*}
\begin{align*}
\dxuse{Gamma26-left} ={}& \dxuse{Gamma26-right}
\end{align*}
\begin{align*}
\dxuse{Gamma26by13-left} ={}& \dxuse{Gamma26by13-right}
\end{align*}
\begin{align*}
\dxuse{Gamma29-left} ={}& \dxuse{Gamma29-right}
\end{align*}
\begin{align*}
\dxuse{Gamma31-left} ={}& \dxuse{Gamma31-right}
\end{align*}
\begin{align*}
\dxuse{Gamma32-left} ={}& \dxuse{Gamma32-right}
\end{align*}
\begin{align*}
\dxuse{Gamma33-left} ={}& \dxuse{Gamma33-right}
\end{align*}
\begin{align*}
\dxuse{Gamma34-left} ={}& \dxuse{Gamma34-right}
\end{align*}
\begin{align*}
\dxuse{Gamma38-left} ={}& \dxuse{Gamma38-right}
\end{align*}
\begin{align*}
\dxuse{Gamma39-left} ={}& \dxuse{Gamma39-right}
\end{align*}
\begin{align*}
\dxuse{Gamma43-left} ={}& \dxuse{Gamma43-right}
\end{align*}
\begin{align*}
\dxuse{Gamma46-left} ={}& \dxuse{Gamma46-right}
\end{align*}
\begin{align*}
\dxuse{Gamma49-left} ={}& \dxuse{Gamma49-right}
\end{align*}
\begin{align*}
\dxuse{Gamma54-left} ={}& \dxuse{Gamma54-right}
\end{align*}
\begin{align*}
\dxuse{Gamma55-left} ={}& \dxuse{Gamma55-right}
\end{align*}
\begin{align*}
\dxuse{Gamma56-left} ={}& \dxuse{Gamma56-right}
\end{align*}
\begin{align*}
\dxuse{Gamma57-left} ={}& \dxuse{Gamma57-right}
\end{align*}
\begin{align*}
\dxuse{Gamma57by55-left} ={}& \dxuse{Gamma57by55-right}
\end{align*}
\begin{align*}
\dxuse{Gamma58-left} ={}& \dxuse{Gamma58-right}
\end{align*}
\begin{align*}
\dxuse{Gamma59-left} ={}& \dxuse{Gamma59-right}
\end{align*}
\begin{align*}
\dxuse{Gamma60-left} ={}& \dxuse{Gamma60-right}
\end{align*}
\begin{align*}
\dxuse{Gamma63-left} ={}& \dxuse{Gamma63-right}
\end{align*}
\begin{align*}
\dxuse{Gamma64-left} ={}& \dxuse{Gamma64-right}
\end{align*}
\begin{align*}
\dxuse{Gamma65-left} ={}& \dxuse{Gamma65-right}
\end{align*}
\begin{align*}
\dxuse{Gamma66-left} ={}& \dxuse{Gamma66-right}
\end{align*}
\begin{align*}
\dxuse{Gamma67-left} ={}& \dxuse{Gamma67-right}
\end{align*}
\begin{align*}
\dxuse{Gamma68-left} ={}& \dxuse{Gamma68-right}
\end{align*}
\begin{align*}
\dxuse{Gamma69-left} ={}& \dxuse{Gamma69-right}
\end{align*}
\begin{align*}
\dxuse{Gamma74-left} ={}& \dxuse{Gamma74-right}
\end{align*}
\begin{align*}
\dxuse{Gamma75-left} ={}& \dxuse{Gamma75-right}
\end{align*}
\begin{align*}
\dxuse{Gamma76-left} ={}& \dxuse{Gamma76-right}
\end{align*}
\begin{align*}
\dxuse{Gamma76by54-left} ={}& \dxuse{Gamma76by54-right}
\end{align*}
\begin{align*}
\dxuse{Gamma78-left} ={}& \dxuse{Gamma78-right}
\end{align*}
\begin{align*}
\dxuse{Gamma79-left} ={}& \dxuse{Gamma79-right}
\end{align*}
\begin{align*}
\dxuse{Gamma80-left} ={}& \dxuse{Gamma80-right}
\end{align*}
\begin{align*}
\dxuse{Gamma80by60-left} ={}& \dxuse{Gamma80by60-right}
\end{align*}
\begin{align*}
\dxuse{Gamma81-left} ={}& \dxuse{Gamma81-right}
\end{align*}
\begin{align*}
\dxuse{Gamma81by69-left} ={}& \dxuse{Gamma81by69-right}
\end{align*}
\begin{align*}
\dxuse{Gamma82-left} ={}& \dxuse{Gamma82-right}
\end{align*}
\begin{align*}
\dxuse{Gamma83-left} ={}& \dxuse{Gamma83-right}
\end{align*}
\begin{align*}
\dxuse{Gamma84-left} ={}& \dxuse{Gamma84-right}
\end{align*}
\begin{align*}
\dxuse{Gamma85-left} ={}& \dxuse{Gamma85-right}
\end{align*}
\begin{align*}
\dxuse{Gamma85by60-left} ={}& \dxuse{Gamma85by60-right}
\end{align*}
\begin{align*}
\dxuse{Gamma87-left} ={}& \dxuse{Gamma87-right}
\end{align*}
\begin{align*}
\dxuse{Gamma88-left} ={}& \dxuse{Gamma88-right}
\end{align*}
\begin{align*}
\dxuse{Gamma89-left} ={}& \dxuse{Gamma89-right}
\end{align*}
\begin{align*}
\dxuse{Gamma92-left} ={}& \dxuse{Gamma92-right}
\end{align*}
\begin{align*}
\dxuse{Gamma93by60-left} ={}& \dxuse{Gamma93by60-right}
\end{align*}
\begin{align*}
\dxuse{Gamma94by69-left} ={}& \dxuse{Gamma94by69-right}
\end{align*}
\begin{align*}
\dxuse{Gamma96-left} ={}& \dxuse{Gamma96-right}
\end{align*}
\begin{align*}
\dxuse{Gamma102-left} ={}& \dxuse{Gamma102-right}
\end{align*}
\begin{align*}
\dxuse{Gamma103-left} ={}& \dxuse{Gamma103-right}
\end{align*}
\begin{align*}
\dxuse{Gamma104-left} ={}& \dxuse{Gamma104-right}
\end{align*}
\begin{align*}
\dxuse{Gamma106-left} ={}& \dxuse{Gamma106-right}
\end{align*}
\begin{align*}
\dxuse{Gamma110-left} ={}& \dxuse{Gamma110-right}
\end{align*}
\begin{align*}
\dxuse{Gamma149-left} ={}& \dxuse{Gamma149-right}
\end{align*}
\begin{align*}
\dxuse{Gamma150-left} ={}& \dxuse{Gamma150-right}
\end{align*}
\begin{align*}
\dxuse{Gamma150by66-left} ={}& \dxuse{Gamma150by66-right}
\end{align*}
\begin{align*}
\dxuse{Gamma152by54-left} ={}& \dxuse{Gamma152by54-right}
\end{align*}
\begin{align*}
\dxuse{Gamma152by76-left} ={}& \dxuse{Gamma152by76-right}
\end{align*}
\begin{align*}
\dxuse{Gamma168-left} ={}& \dxuse{Gamma168-right}
\end{align*}
\begin{align*}
\dxuse{Gamma169-left} ={}& \dxuse{Gamma169-right}
\end{align*}
\begin{align*}
\dxuse{Gamma804-left} ={}& \dxuse{Gamma804-right}
\end{align*}
\begin{align*}
\dxuse{Gamma805-left} ={}& \dxuse{Gamma805-right}
\end{align*}
\begin{align*}
\dxuse{Gamma806-left} ={}& \dxuse{Gamma806-right}
\end{align*}
\begin{align*}
\dxuse{Gamma810-left} ={}& \dxuse{Gamma810-right}
\end{align*}
\begin{align*}
\dxuse{Gamma820-left} ={}& \dxuse{Gamma820-right}
\end{align*}
\begin{align*}
\dxuse{Gamma830-left} ={}& \dxuse{Gamma830-right}
\end{align*}
\begin{align*}
\dxuse{Gamma910-left} ={}& \dxuse{Gamma910-right}
\end{align*}
\begin{align*}
\dxuse{Gamma911-left} ={}& \dxuse{Gamma911-right}
\end{align*}
\begin{align*}
\dxuse{Gamma930-left} ={}& \dxuse{Gamma930-right}
\end{align*}
\begin{align*}
\dxuse{Gamma944-left} ={}& \dxuse{Gamma944-right}
\end{align*}
\begin{align*}
\dxuse{GammaAll-left} ={}& \dxuse{GammaAll-right}
\end{align*}
\begin{align*}
\dxuse{Unitarity-left} ={}& \dxuse{Unitarity-right}
\end{align*}%
}


==> tau/avg-taubr-2023.tex <==
\dxdef{TauBrMeasNum}{171}
\dxdef{TauBrMeasNumAll}{172}
\dxdef{TauBrMeasNumNuisance}{1}
\dxdef{TauBrQuantNum}{137}
\dxdef{TauBrQuantNumAll}{138}
\dxdef{TauBrQuantNumNuisance}{1}
\dxdef{TauBrBaseQuantNum}{47}
\dxdef{TauBrBaseVarNum}{46}
\dxdef{TauBrConstrNum}{91}
\dxdef{TauBrChisq}{138}
\dxdef{TauBrDof}{125}
\dxdef{TauBrChisqProb}{20.2\%}
\dxdef{TauBrChisq_full}{138}
\dxdef{TauBrDof_full}{125}
\dxdef{TauBrChisqProb_full}{20.2\%}
\dxdef{TauBrUnitarityResid}{(0.07 \pm 0.11)\%}
\dxdef{TauBrUnitarityQuantNum}{47}
\dxdef{TauBrPdgQuantNum}{129}
\dxdef{TauBrPdgQuantNumNonRatio}{112}
\dxdef{TauBrPdgQuantNumRatio}{17}
\dxdef{TauBrPdgQuantNumWithMeas}{85}
\dxdef{TauBrPdgQuantNumNonRatioWithMeas}{72}
\dxdef{TauBrPdgQuantNumRatioWithMeas}{13}
\dxdef{TauBrPdgConstrNum}{83}
\dxdef{TauBrNumMeasALEPH}{39}
\dxdef{TauBrNumMeasARGUS}{2}
\dxdef{TauBrNumMeasBaBar}{24}
\dxdef{TauBrNumMeasBelle}{15}
\dxdef{TauBrNumMeasBelle2}{1}
\dxdef{TauBrNumMeasCELLO}{1}
\dxdef{TauBrNumMeasCLEO}{35}
\dxdef{TauBrNumMeasCLEO3}{6}
\dxdef{TauBrNumMeasDELPHI}{14}
\dxdef{TauBrNumMeasHRS}{2}
\dxdef{TauBrNumMeasL3}{11}
\dxdef{TauBrNumMeasOPAL}{19}
\dxdef{TauBrNumMeasTPC}{3}
\dxQuantDef{Gamma1}{\BR_{1}}{\BR(\tau^- \to \text{particle}^- \ge{} 0\, \text{neutrals} \ge{} 0\,  K^0\, \nu_\tau)}{0.8518 \pm 0.0011}{0.8518}{\pm 0.0011}
\dxQuantDef{Gamma2}{\BR_{2}}{\BR(\tau^- \to \text{particle}^- \ge{} 0\, \text{neutrals} \ge{} 0\,  K_L^0\, \nu_\tau)}{0.8452 \pm 0.0010}{0.8452}{\pm 0.0010}
\dxQuantDef{Gamma3}{\BR_{3}}{\BR(\tau^- \to \mu^- \bar{\nu}_\mu \nu_\tau)}{0.17360 \pm 0.00037}{0.17360}{\pm 0.00037}
\dxMeasDef{ALEPH.Gamma3.pub.SCHAEL.05C}{Gamma3}{SCHAEL 05C}{0.17319 \pm 0.00070 \pm 0.00032}{0.17319}{\pm 0.00070}{\pm 0.00032}
\dxMeasDef{DELPHI.Gamma3.pub.ABREU.99X}{Gamma3}{ABREU 99X}{0.17325 \pm 0.00095 \pm 0.00077}{0.17325}{\pm 0.00095}{\pm 0.00077}
\dxMeasDef{L3.Gamma3.pub.ACCIARRI.01F}{Gamma3}{ACCIARRI 01F}{0.17342 \pm 0.00110 \pm 0.00067}{0.17342}{\pm 0.00110}{\pm 0.00067}
\dxMeasDef{OPAL.Gamma3.pub.ABBIENDI.03}{Gamma3}{ABBIENDI 03}{0.17340 \pm 0.00090 \pm 0.00060}{0.17340}{\pm 0.00090}{\pm 0.00060}
\dxQuantDef{Gamma3by5}{\BR_{3 / 5}}{\frac{\BR(\tau^- \to \mu^- \bar{\nu}_\mu \nu_\tau)}{\BR(\tau^- \to e^- \bar{\nu}_e \nu_\tau)}}{0.9730 \pm 0.0022}{0.9730}{\pm 0.0022}
\dxMeasDef{ARGUS.Gamma3by5.pub.ALBRECHT.92D}{Gamma3by5}{ALBRECHT 92D}{0.9970 \pm 0.0350 \pm 0.0400}{0.9970}{\pm 0.0350}{\pm 0.0400}
\dxMeasDef{BaBar.Gamma3by5.pub.AUBERT.10F}{Gamma3by5}{AUBERT 10F}{0.9796 \pm 0.0016 \pm 0.0036}{0.9796}{\pm 0.0016}{\pm 0.0036}
\dxMeasDef{Belle2.Gamma3by5.ADACHI.2024}{Gamma3by5}{Belle2 ADACHI 2024}{0.9675 \pm 0.0007 \pm 0.0036}{0.9675}{\pm 0.0007}{\pm 0.0036}
\dxMeasDef{CLEO.Gamma3by5.pub.ANASTASSOV.97}{Gamma3by5}{ANASTASSOV 97}{0.9777 \pm 0.0063 \pm 0.0087}{0.9777}{\pm 0.0063}{\pm 0.0087}
\dxQuantDef{Gamma5}{\BR_{5}}{\BR(\tau^- \to e^- \bar{\nu}_e \nu_\tau)}{0.1784 \pm 0.0004}{0.1784}{\pm 0.0004}
\dxMeasDef{ALEPH.Gamma5.pub.SCHAEL.05C}{Gamma5}{SCHAEL 05C}{0.1784 \pm 0.0007 \pm 0.0004}{0.1784}{\pm 0.0007}{\pm 0.0004}
\dxMeasDef{CLEO.Gamma5.pub.ANASTASSOV.97}{Gamma5}{ANASTASSOV 97}{0.1776 \pm 0.0006 \pm 0.0017}{0.1776}{\pm 0.0006}{\pm 0.0017}
\dxMeasDef{DELPHI.Gamma5.pub.ABREU.99X}{Gamma5}{ABREU 99X}{0.1788 \pm 0.0011 \pm 0.0011}{0.1788}{\pm 0.0011}{\pm 0.0011}
\dxMeasDef{L3.Gamma5.pub.ACCIARRI.01F}{Gamma5}{ACCIARRI 01F}{0.1781 \pm 0.0010 \pm 0.0008}{0.1781}{\pm 0.0010}{\pm 0.0008}
\dxMeasDef{OPAL.Gamma5.pub.ABBIENDI.99H}{Gamma5}{ABBIENDI 99H}{0.1781 \pm 0.0009 \pm 0.0006}{0.1781}{\pm 0.0009}{\pm 0.0006}
\dxQuantDef{Gamma7}{\BR_{7}}{\BR(\tau^- \to h^- \ge{} 0\,  K_L^0\, \nu_\tau)}{0.1202 \pm 0.0005}{0.1202}{\pm 0.0005}
\dxMeasDef{DELPHI.Gamma7.pub.ABREU.92N}{Gamma7}{ABREU 92N}{0.1240 \pm 0.0070 \pm 0.0070}{0.1240}{\pm 0.0070}{\pm 0.0070}
\dxMeasDef{L3.Gamma7.pub.ACCIARRI.95}{Gamma7}{ACCIARRI 95}{0.1247 \pm 0.0026 \pm 0.0043}{0.1247}{\pm 0.0026}{\pm 0.0043}
\dxMeasDef{OPAL.Gamma7.pub.ALEXANDER.91D}{Gamma7}{ALEXANDER 91D}{0.1210 \pm 0.0070 \pm 0.0050}{0.1210}{\pm 0.0070}{\pm 0.0050}
\dxQuantDef{Gamma8}{\BR_{8}}{\BR(\tau^- \to h^- \nu_\tau)}{0.1150 \pm 0.0005}{0.1150}{\pm 0.0005}
\dxMeasDef{CLEO.Gamma8.pub.ANASTASSOV.97}{Gamma8}{ANASTASSOV 97}{0.1152 \pm 0.0005 \pm 0.0012}{0.1152}{\pm 0.0005}{\pm 0.0012}
\dxMeasDef{DELPHI.Gamma8.pub.ABDALLAH.06A}{Gamma8}{ABDALLAH 06A}{0.1157 \pm 0.0012 \pm 0.0011}{0.1157}{\pm 0.0012}{\pm 0.0011}
\dxMeasDef{OPAL.Gamma8.pub.ACKERSTAFF.98M}{Gamma8}{ACKERSTAFF 98M}{0.1198 \pm 0.0013 \pm 0.0016}{0.1198}{\pm 0.0013}{\pm 0.0016}
\dxQuantDef{Gamma8by5}{\BR_{8 / 5}}{\frac{\BR(\tau^- \to h^- \nu_\tau)}{\BR(\tau^- \to e^- \bar{\nu}_e \nu_\tau)}}{0.6448 \pm 0.0032}{0.6448}{\pm 0.0032}
\dxQuantDef{Gamma9}{\BR_{9}}{\BR(\tau^- \to \pi^- \nu_\tau)}{0.1081 \pm 0.0005}{0.1081}{\pm 0.0005}
\dxMeasDef{ALEPH.Gamma9.pub.SCHAEL.05C}{Gamma9}{SCHAEL 05C}{0.1083 \pm 0.0007 \pm 0.0008}{0.1083}{\pm 0.0007}{\pm 0.0008}
\dxQuantDef{Gamma9by5}{\BR_{9 / 5}}{\frac{\BR(\tau^- \to \pi^- \nu_\tau)}{\BR(\tau^- \to e^- \bar{\nu}_e \nu_\tau)}}{0.6058 \pm 0.0032}{0.6058}{\pm 0.0032}
\dxMeasDef{BaBar.Gamma9by5.pub.AUBERT.10F}{Gamma9by5}{AUBERT 10F}{0.5945 \pm 0.0014 \pm 0.0061}{0.5945}{\pm 0.0014}{\pm 0.0061}
\dxQuantDef{Gamma10}{\BR_{10}}{\BR(\tau^- \to K^- \nu_\tau)}{0.00696 \pm 0.00010}{0.00696}{\pm 0.00010}
\dxMeasDef{ALEPH.Gamma10.pub.BARATE.99K}{Gamma10}{BARATE 99K}{0.00696 \pm 0.00025 \pm 0.00014}{0.00696}{\pm 0.00025}{\pm 0.00014}
\dxMeasDef{CLEO.Gamma10.pub.BATTLE.94}{Gamma10}{BATTLE 94}{0.00660 \pm 0.00070 \pm 0.00090}{0.00660}{\pm 0.00070}{\pm 0.00090}
\dxMeasDef{DELPHI.Gamma10.pub.ABREU.94K}{Gamma10}{ABREU 94K}{0.00850 \pm 0.00180 \pm 0.00000}{0.00850}{\pm 0.00180}{\pm 0.00000}
\dxMeasDef{OPAL.Gamma10.pub.ABBIENDI.01J}{Gamma10}{ABBIENDI 01J}{0.00658 \pm 0.00027 \pm 0.00029}{0.00658}{\pm 0.00027}{\pm 0.00029}
\dxQuantDef{Gamma10by5}{\BR_{10 / 5}}{\frac{\BR(\tau^- \to K^- \nu_\tau)}{\BR(\tau^- \to e^- \bar{\nu}_e \nu_\tau)}}{0.03901 \pm 0.00054}{0.03901}{\pm 0.00054}
\dxMeasDef{BaBar.Gamma10by5.pub.AUBERT.10F}{Gamma10by5}{AUBERT 10F}{0.03882 \pm 0.00032 \pm 0.00057}{0.03882}{\pm 0.00032}{\pm 0.00057}
\dxQuantDef{Gamma10by9}{\BR_{10 / 9}}{\frac{\BR(\tau^- \to K^- \nu_\tau)}{\BR(\tau^- \to \pi^- \nu_\tau)}}{0.0644 \pm 0.0009}{0.0644}{\pm 0.0009}
\dxQuantDef{Gamma11}{\BR_{11}}{\BR(\tau^- \to h^- \ge{} 1\,  \text{neutrals}\, \nu_\tau)}{0.3698 \pm 0.0010}{0.3698}{\pm 0.0010}
\dxQuantDef{Gamma12}{\BR_{12}}{\BR(\tau^- \to h^- \ge{} 1\, \pi^0\, \nu_\tau\;(\text{ex.}K^0))}{0.3648 \pm 0.0010}{0.3648}{\pm 0.0010}
\dxQuantDef{Gamma13}{\BR_{13}}{\BR(\tau^- \to h^- \pi^0 \nu_\tau)}{0.25917 \pm 0.00090}{0.25917}{\pm 0.00090}
\dxMeasDef{Belle.Gamma13.pub.FUJIKAWA.08}{Gamma13}{FUJIKAWA 08}{0.25670 \pm 0.00010 \pm 0.00390}{0.25670}{\pm 0.00010}{\pm 0.00390}
\dxMeasDef{CLEO.Gamma13.pub.ARTUSO.94}{Gamma13}{ARTUSO 94}{0.25870 \pm 0.00120 \pm 0.00420}{0.25870}{\pm 0.00120}{\pm 0.00420}
\dxMeasDef{DELPHI.Gamma13.pub.ABDALLAH.06A}{Gamma13}{ABDALLAH 06A}{0.25740 \pm 0.00201 \pm 0.00138}{0.25740}{\pm 0.00201}{\pm 0.00138}
\dxMeasDef{L3.Gamma13.pub.ACCIARRI.95}{Gamma13}{ACCIARRI 95}{0.25050 \pm 0.00350 \pm 0.00500}{0.25050}{\pm 0.00350}{\pm 0.00500}
\dxMeasDef{OPAL.Gamma13.pub.ACKERSTAFF.98M}{Gamma13}{ACKERSTAFF 98M}{0.25890 \pm 0.00170 \pm 0.00290}{0.25890}{\pm 0.00170}{\pm 0.00290}
\dxQuantDef{Gamma14}{\BR_{14}}{\BR(\tau^- \to \pi^- \pi^0 \nu_\tau)}{0.2548 \pm 0.0009}{0.2548}{\pm 0.0009}
\dxMeasDef{ALEPH.Gamma14.pub.SCHAEL.05C}{Gamma14}{SCHAEL 05C}{0.2547 \pm 0.0010 \pm 0.0008}{0.2547}{\pm 0.0010}{\pm 0.0008}
\dxQuantDef{Gamma16}{\BR_{16}}{\BR(\tau^- \to K^- \pi^0 \nu_\tau)}{0.004321 \pm 0.000148}{0.004321}{\pm 0.000148}
\dxMeasDef{ALEPH.Gamma16.pub.BARATE.99K}{Gamma16}{BARATE 99K}{0.004440 \pm 0.000260 \pm 0.000240}{0.004440}{\pm 0.000260}{\pm 0.000240}
\dxMeasDef{BaBar.Gamma16.pub.AUBERT.07AP}{Gamma16}{AUBERT 07AP}{0.004160 \pm 0.000030 \pm 0.000180}{0.004160}{\pm 0.000030}{\pm 0.000180}
\dxMeasDef{CLEO.Gamma16.pub.BATTLE.94}{Gamma16}{BATTLE 94}{0.005100 \pm 0.001000 \pm 0.000700}{0.005100}{\pm 0.001000}{\pm 0.000700}
\dxMeasDef{OPAL.Gamma16.pub.ABBIENDI.04J}{Gamma16}{ABBIENDI 04J}{0.004710 \pm 0.000590 \pm 0.000230}{0.004710}{\pm 0.000590}{\pm 0.000230}
\dxQuantDef{Gamma17}{\BR_{17}}{\BR(\tau^- \to h^- \ge{} 2\,  \pi^0\, \nu_\tau)}{0.1079 \pm 0.0010}{0.1079}{\pm 0.0010}
\dxMeasDef{OPAL.Gamma17.pub.ACKERSTAFF.98M}{Gamma17}{ACKERSTAFF 98M}{0.0991 \pm 0.0031 \pm 0.0027}{0.0991}{\pm 0.0031}{\pm 0.0027}
\dxQuantDef{Gamma18}{\BR_{18}}{\BR(\tau^- \to h^- 2\pi^0 \nu_\tau)}{0.0946 \pm 0.0010}{0.0946}{\pm 0.0010}
\dxQuantDef{Gamma19}{\BR_{19}}{\BR(\tau^- \to h^- 2\pi^0 \nu_\tau\;(\text{ex.}K^0))}{0.0931 \pm 0.0010}{0.0931}{\pm 0.0010}
\dxMeasDef{DELPHI.Gamma19.pub.ABDALLAH.06A}{Gamma19}{ABDALLAH 06A}{0.0950 \pm 0.0032 \pm 0.0027}{0.0950}{\pm 0.0032}{\pm 0.0027}
\dxMeasDef{L3.Gamma19.pub.ACCIARRI.95}{Gamma19}{ACCIARRI 95}{0.0888 \pm 0.0037 \pm 0.0042}{0.0888}{\pm 0.0037}{\pm 0.0042}
\dxQuantDef{Gamma19by13}{\BR_{19 / 13}}{\frac{\BR(\tau^- \to h^- 2\pi^0 \nu_\tau\;(\text{ex.}K^0))}{\BR(\tau^- \to h^- \pi^0 \nu_\tau)}}{0.359 \pm 0.005}{0.359}{\pm 0.005}
\dxMeasDef{CLEO.Gamma19by13.pub.PROCARIO.93}{Gamma19by13}{PROCARIO 93}{0.342 \pm 0.006 \pm 0.016}{0.342}{\pm 0.006}{\pm 0.016}
\dxQuantDef{Gamma20}{\BR_{20}}{\BR(\tau^- \to \pi^- 2\pi^0 \nu_\tau\;(\text{ex.}K^0))}{0.0925 \pm 0.0010}{0.0925}{\pm 0.0010}
\dxMeasDef{ALEPH.Gamma20.pub.SCHAEL.05C}{Gamma20}{SCHAEL 05C}{0.0924 \pm 0.0009 \pm 0.0009}{0.0924}{\pm 0.0009}{\pm 0.0009}
\dxQuantDef{Gamma23}{\BR_{23}}{\BR(\tau^- \to K^- 2\pi^0 \nu_\tau\;(\text{ex.}K^0))}{0.00063 \pm 0.00022}{0.00063}{\pm 0.00022}
\dxMeasDef{ALEPH.Gamma23.pub.BARATE.99K}{Gamma23}{BARATE 99K}{0.00056 \pm 0.00020 \pm 0.00015}{0.00056}{\pm 0.00020}{\pm 0.00015}
\dxMeasDef{CLEO.Gamma23.pub.BATTLE.94}{Gamma23}{BATTLE 94}{0.00090 \pm 0.00100 \pm 0.00030}{0.00090}{\pm 0.00100}{\pm 0.00030}
\dxQuantDef{Gamma24}{\BR_{24}}{\BR(\tau^- \to h^- \ge{} 3\, \pi^0\, \nu_\tau)}{0.0134 \pm 0.0007}{0.0134}{\pm 0.0007}
\dxQuantDef{Gamma25}{\BR_{25}}{\BR(\tau^- \to h^- \ge{} 3\, \pi^0\, \nu_\tau\;(\text{ex.}K^0))}{0.0125 \pm 0.0007}{0.0125}{\pm 0.0007}
\dxMeasDef{DELPHI.Gamma25.pub.ABDALLAH.06A}{Gamma25}{ABDALLAH 06A}{0.0140 \pm 0.0021 \pm 0.0022}{0.0140}{\pm 0.0021}{\pm 0.0022}
\dxQuantDef{Gamma26}{\BR_{26}}{\BR(\tau^- \to h^- 3\pi^0 \nu_\tau)}{0.0117 \pm 0.0007}{0.0117}{\pm 0.0007}
\dxMeasDef{L3.Gamma26.pub.ACCIARRI.95}{Gamma26}{ACCIARRI 95}{0.0170 \pm 0.0024 \pm 0.0038}{0.0170}{\pm 0.0024}{\pm 0.0038}
\dxQuantDef{Gamma26by13}{\BR_{26 / 13}}{\frac{\BR(\tau^- \to h^- 3\pi^0 \nu_\tau)}{\BR(\tau^- \to h^- \pi^0 \nu_\tau)}}{0.0453 \pm 0.0028}{0.0453}{\pm 0.0028}
\dxMeasDef{CLEO.Gamma26by13.pub.PROCARIO.93}{Gamma26by13}{PROCARIO 93}{0.0440 \pm 0.0030 \pm 0.0050}{0.0440}{\pm 0.0030}{\pm 0.0050}
\dxQuantDef{Gamma27}{\BR_{27}}{\BR(\tau^- \to \pi^- 3\pi^0 \nu_\tau\;(\text{ex.}K^0))}{0.0104 \pm 0.0007}{0.0104}{\pm 0.0007}
\dxMeasDef{ALEPH.Gamma27.pub.SCHAEL.05C}{Gamma27}{SCHAEL 05C}{0.0098 \pm 0.0007 \pm 0.0006}{0.0098}{\pm 0.0007}{\pm 0.0006}
\dxQuantDef{Gamma28}{\BR_{28}}{\BR(\tau^- \to K^- 3\pi^0 \nu_\tau\;(\text{ex.}K^0,\eta))}{(0.46 \pm 0.21)\cdot 10^{-3}}{0.46 \cdot 10^{-3}}{\pm 0.21 \cdot 10^{-3}}
\dxMeasDef{ALEPH.Gamma28.pub.BARATE.99K}{Gamma28}{BARATE 99K}{(0.37 \pm 0.21 \pm 0.11)\cdot 10^{-3}}{0.37 \cdot 10^{-3}}{\pm 0.21 \cdot 10^{-3}}{\pm 0.11 \cdot 10^{-3}}
\dxQuantDef{Gamma29}{\BR_{29}}{\BR(\tau^- \to h^- 4\pi^0 \nu_\tau\;(\text{ex.}K^0))}{0.0016 \pm 0.0004}{0.0016}{\pm 0.0004}
\dxMeasDef{CLEO.Gamma29.pub.PROCARIO.93}{Gamma29}{PROCARIO 93}{0.0016 \pm 0.0005 \pm 0.0005}{0.0016}{\pm 0.0005}{\pm 0.0005}
\dxQuantDef{Gamma30}{\BR_{30}}{\BR(\tau^- \to h^- 4\pi^0 \nu_\tau\;(\text{ex.}K^0,\eta))}{0.00112 \pm 0.00039}{0.00112}{\pm 0.00039}
\dxMeasDef{ALEPH.Gamma30.pub.SCHAEL.05C}{Gamma30}{SCHAEL 05C}{0.00112 \pm 0.00037 \pm 0.00035}{0.00112}{\pm 0.00037}{\pm 0.00035}
\dxQuantDef{Gamma31}{\BR_{31}}{\BR(\tau^- \to K^- \ge{} 0\, \pi^0 \ge{} 0\, K^0 \ge{} 0\, \gamma \nu_\tau)}{0.01548 \pm 0.00029}{0.01548}{\pm 0.00029}
\dxMeasDef{CLEO.Gamma31.pub.BATTLE.94}{Gamma31}{BATTLE 94}{0.01700 \pm 0.00120 \pm 0.00190}{0.01700}{\pm 0.00120}{\pm 0.00190}
\dxMeasDef{DELPHI.Gamma31.pub.ABREU.94K}{Gamma31}{ABREU 94K}{0.01540 \pm 0.00240 \pm 0.00000}{0.01540}{\pm 0.00240}{\pm 0.00000}
\dxMeasDef{OPAL.Gamma31.pub.ABBIENDI.01J}{Gamma31}{ABBIENDI 01J}{0.01528 \pm 0.00039 \pm 0.00040}{0.01528}{\pm 0.00039}{\pm 0.00040}
\dxQuantDef{Gamma32}{\BR_{32}}{\BR(\tau^- \to K^- \ge{} 1\, (\pi^0\,\text{or}\,K^0\,\text{or}\,\gamma) \nu_\tau)}{0.00856 \pm 0.00028}{0.00856}{\pm 0.00028}
\dxQuantDef{Gamma33}{\BR_{33}}{\BR(\tau^- \to K_S^0 (\text{particle}s)^- \nu_\tau)}{0.00937 \pm 0.00029}{0.00937}{\pm 0.00029}
\dxMeasDef{ALEPH.Gamma33.pub.BARATE.98E}{Gamma33}{BARATE 98E}{0.00970 \pm 0.00058 \pm 0.00062}{0.00970}{\pm 0.00058}{\pm 0.00062}
\dxMeasDef{OPAL.Gamma33.pub.AKERS.94G}{Gamma33}{AKERS 94G}{0.00970 \pm 0.00090 \pm 0.00060}{0.00970}{\pm 0.00090}{\pm 0.00060}
\dxQuantDef{Gamma34}{\BR_{34}}{\BR(\tau^- \to h^- \bar{K}^0 \nu_\tau)}{0.00986 \pm 0.00014}{0.00986}{\pm 0.00014}
\dxMeasDef{CLEO.Gamma34.pub.COAN.96}{Gamma34}{COAN 96}{0.00855 \pm 0.00036 \pm 0.00073}{0.00855}{\pm 0.00036}{\pm 0.00073}
\dxQuantDef{Gamma35}{\BR_{35}}{\BR(\tau^- \to \pi^- \bar{K}^0 \nu_\tau)}{0.008375 \pm 0.000139}{0.008375}{\pm 0.000139}
\dxMeasDef{ALEPH.Gamma35.pub.BARATE.99K}{Gamma35}{BARATE 99K}{0.009280 \pm 0.000450 \pm 0.000340}{0.009280}{\pm 0.000450}{\pm 0.000340}
\dxMeasDef{Belle.Gamma35.pub.RYU.14vpc}{Gamma35}{RYU 14vpc}{0.008320 \pm 0.000025 \pm 0.000150}{0.008320}{\pm 0.000025}{\pm 0.000150}
\dxMeasDef{L3.Gamma35.pub.ACCIARRI.95F}{Gamma35}{ACCIARRI 95F}{0.009500 \pm 0.001500 \pm 0.000600}{0.009500}{\pm 0.001500}{\pm 0.000600}
\dxMeasDef{OPAL.Gamma35.pub.ABBIENDI.00C}{Gamma35}{ABBIENDI 00C}{0.009330 \pm 0.000680 \pm 0.000490}{0.009330}{\pm 0.000680}{\pm 0.000490}
\dxQuantDef{Gamma37}{\BR_{37}}{\BR(\tau^- \to K^- K^0 \nu_\tau)}{0.001486 \pm 0.000034}{0.001486}{\pm 0.000034}
\dxMeasDef{ALEPH.Gamma37.pub.BARATE.98E}{Gamma37}{BARATE 98E}{0.001580 \pm 0.000420 \pm 0.000170}{0.001580}{\pm 0.000420}{\pm 0.000170}
\dxMeasDef{ALEPH.Gamma37.pub.BARATE.99K}{Gamma37}{BARATE 99K}{0.001620 \pm 0.000210 \pm 0.000110}{0.001620}{\pm 0.000210}{\pm 0.000110}
\dxMeasDef{BaBar.Gamma37.pub.LEES.18B}{Gamma37}{LEES 18B}{0.001478 \pm 0.000022 \pm 0.000040}{0.001478}{\pm 0.000022}{\pm 0.000040}
\dxMeasDef{Belle.Gamma37.pub.RYU.14vpc}{Gamma37}{RYU 14vpc}{0.001480 \pm 0.000013 \pm 0.000055}{0.001480}{\pm 0.000013}{\pm 0.000055}
\dxMeasDef{CLEO.Gamma37.pub.COAN.96}{Gamma37}{COAN 96}{0.001510 \pm 0.000210 \pm 0.000220}{0.001510}{\pm 0.000210}{\pm 0.000220}
\dxQuantDef{Gamma38}{\BR_{38}}{\BR(\tau^- \to K^- K^0 \ge{} 0\,  \pi^0\, \nu_\tau)}{0.00298 \pm 0.00007}{0.00298}{\pm 0.00007}
\dxMeasDef{OPAL.Gamma38.pub.ABBIENDI.00C}{Gamma38}{ABBIENDI 00C}{0.00330 \pm 0.00055 \pm 0.00039}{0.00330}{\pm 0.00055}{\pm 0.00039}
\dxQuantDef{Gamma39}{\BR_{39}}{\BR(\tau^- \to h^- \bar{K}^0 \pi^0 \nu_\tau)}{0.00531 \pm 0.00013}{0.00531}{\pm 0.00013}
\dxMeasDef{CLEO.Gamma39.pub.COAN.96}{Gamma39}{COAN 96}{0.00562 \pm 0.00050 \pm 0.00048}{0.00562}{\pm 0.00050}{\pm 0.00048}
\dxQuantDef{Gamma40}{\BR_{40}}{\BR(\tau^- \to \pi^- \bar{K}^0 \pi^0 \nu_\tau)}{0.003810 \pm 0.000129}{0.003810}{\pm 0.000129}
\dxMeasDef{ALEPH.Gamma40.pub.BARATE.98E}{Gamma40}{BARATE 98E}{0.002940 \pm 0.000730 \pm 0.000370}{0.002940}{\pm 0.000730}{\pm 0.000370}
\dxMeasDef{ALEPH.Gamma40.pub.BARATE.99K}{Gamma40}{BARATE 99K}{0.003470 \pm 0.000530 \pm 0.000370}{0.003470}{\pm 0.000530}{\pm 0.000370}
\dxMeasDef{Belle.Gamma40.pub.RYU.14vpc}{Gamma40}{RYU 14vpc}{0.003860 \pm 0.000031 \pm 0.000135}{0.003860}{\pm 0.000031}{\pm 0.000135}
\dxMeasDef{L3.Gamma40.pub.ACCIARRI.95F}{Gamma40}{ACCIARRI 95F}{0.004100 \pm 0.001200 \pm 0.000300}{0.004100}{\pm 0.001200}{\pm 0.000300}
\dxQuantDef{Gamma42}{\BR_{42}}{\BR(\tau^- \to K^- K^0 \pi^0 \nu_\tau)}{0.001499 \pm 0.000070}{0.001499}{\pm 0.000070}
\dxMeasDef{ALEPH.Gamma42.pub.BARATE.98E}{Gamma42}{BARATE 98E}{0.001520 \pm 0.000760 \pm 0.000210}{0.001520}{\pm 0.000760}{\pm 0.000210}
\dxMeasDef{ALEPH.Gamma42.pub.BARATE.99K}{Gamma42}{BARATE 99K}{0.001430 \pm 0.000250 \pm 0.000150}{0.001430}{\pm 0.000250}{\pm 0.000150}
\dxMeasDef{Belle.Gamma42.pub.RYU.14vpc}{Gamma42}{RYU 14vpc}{0.001496 \pm 0.000019 \pm 0.000073}{0.001496}{\pm 0.000019}{\pm 0.000073}
\dxMeasDef{CLEO.Gamma42.pub.COAN.96}{Gamma42}{COAN 96}{0.001450 \pm 0.000360 \pm 0.000200}{0.001450}{\pm 0.000360}{\pm 0.000200}
\dxQuantDef{Gamma43}{\BR_{43}}{\BR(\tau^- \to \pi^- \bar{K}^0 \ge{} 1\,  \pi^0\, \nu_\tau)}{0.00404 \pm 0.00026}{0.00404}{\pm 0.00026}
\dxMeasDef{OPAL.Gamma43.pub.ABBIENDI.00C}{Gamma43}{ABBIENDI 00C}{0.00324 \pm 0.00074 \pm 0.00066}{0.00324}{\pm 0.00074}{\pm 0.00066}
\dxQuantDef{Gamma44}{\BR_{44}}{\BR(\tau^- \to \pi^- \bar{K}^0 2\pi^0 \nu_\tau\;(\text{ex.}K^0))}{(0.23 \pm 0.23)\cdot 10^{-3}}{0.23 \cdot 10^{-3}}{\pm 0.23 \cdot 10^{-3}}
\dxMeasDef{ALEPH.Gamma44.pub.BARATE.99R}{Gamma44}{BARATE 99R}{(0.26 \pm 0.24 \pm 0.00)\cdot 10^{-3}}{0.26 \cdot 10^{-3}}{\pm 0.24 \cdot 10^{-3}}{\pm 0.00 \cdot 10^{-3}}
\dxQuantDef{Gamma46}{\BR_{46}}{\BR(\tau^- \to \pi^- K^0 \bar{K}^0 \nu_\tau)}{0.00152 \pm 0.00025}{0.00152}{\pm 0.00025}
\dxQuantDef{Gamma47}{\BR_{47}}{\BR(\tau^- \to \pi^- K_S^0 K_S^0 \nu_\tau)}{(234.8 \pm 6.5)\cdot 10^{-6}}{234.8 \cdot 10^{-6}}{\pm 6.5 \cdot 10^{-6}}
\dxMeasDef{ALEPH.Gamma47.pub.BARATE.98E}{Gamma47}{BARATE 98E}{(260.0 \pm 100.0 \pm 50.0)\cdot 10^{-6}}{260.0 \cdot 10^{-6}}{\pm 100.0 \cdot 10^{-6}}{\pm 50.0 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma47.pub.LEES.12Y}{Gamma47}{LEES 12Y}{(231.0 \pm 4.0 \pm 8.0)\cdot 10^{-6}}{231.0 \cdot 10^{-6}}{\pm 4.0 \cdot 10^{-6}}{\pm 8.0 \cdot 10^{-6}}
\dxMeasDef{Belle.Gamma47.pub.RYU.14vpc}{Gamma47}{RYU 14vpc}{(233.0 \pm 3.3 \pm 9.3)\cdot 10^{-6}}{233.0 \cdot 10^{-6}}{\pm 3.3 \cdot 10^{-6}}{\pm 9.3 \cdot 10^{-6}}
\dxMeasDef{CLEO.Gamma47.pub.COAN.96}{Gamma47}{COAN 96}{(230.0 \pm 50.0 \pm 30.0)\cdot 10^{-6}}{230.0 \cdot 10^{-6}}{\pm 50.0 \cdot 10^{-6}}{\pm 30.0 \cdot 10^{-6}}
\dxQuantDef{Gamma48}{\BR_{48}}{\BR(\tau^- \to \pi^- K_S^0 K_L^0 \nu_\tau)}{0.00105 \pm 0.00025}{0.00105}{\pm 0.00025}
\dxMeasDef{ALEPH.Gamma48.pub.BARATE.98E}{Gamma48}{BARATE 98E}{0.00101 \pm 0.00023 \pm 0.00013}{0.00101}{\pm 0.00023}{\pm 0.00013}
\dxQuantDef{Gamma49}{\BR_{49}}{\BR(\tau^- \to \pi^- \pi^0 K^0 \bar{K}^0 \nu_\tau)}{(0.35 \pm 0.12)\cdot 10^{-3}}{0.35 \cdot 10^{-3}}{\pm 0.12 \cdot 10^{-3}}
\dxQuantDef{Gamma50}{\BR_{50}}{\BR(\tau^- \to \pi^- K_S^0 K_S^0 \pi^0 \nu_\tau)}{(18.2 \pm 2.1)\cdot 10^{-6}}{18.2 \cdot 10^{-6}}{\pm 2.1 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma50.pub.LEES.12Y}{Gamma50}{LEES 12Y}{(16.0 \pm 2.0 \pm 2.2)\cdot 10^{-6}}{16.0 \cdot 10^{-6}}{\pm 2.0 \cdot 10^{-6}}{\pm 2.2 \cdot 10^{-6}}
\dxMeasDef{Belle.Gamma50.pub.RYU.14vpc}{Gamma50}{RYU 14vpc}{(20.0 \pm 2.2 \pm 2.0)\cdot 10^{-6}}{20.0 \cdot 10^{-6}}{\pm 2.2 \cdot 10^{-6}}{\pm 2.0 \cdot 10^{-6}}
\dxQuantDef{Gamma51}{\BR_{51}}{\BR(\tau^- \to \pi^- K_S^0 K_L^0 \pi^0 \nu_\tau)}{(0.32 \pm 0.12)\cdot 10^{-3}}{0.32 \cdot 10^{-3}}{\pm 0.12 \cdot 10^{-3}}
\dxMeasDef{ALEPH.Gamma51.pub.BARATE.98E}{Gamma51}{BARATE 98E}{(0.31 \pm 0.11 \pm 0.05)\cdot 10^{-3}}{0.31 \cdot 10^{-3}}{\pm 0.11 \cdot 10^{-3}}{\pm 0.05 \cdot 10^{-3}}
\dxQuantDef{Gamma53}{\BR_{53}}{\BR(\tau^- \to \bar{K}^0 h^- h^- h^+ \nu_\tau)}{(0.22 \pm 0.20)\cdot 10^{-3}}{0.22 \cdot 10^{-3}}{\pm 0.20 \cdot 10^{-3}}
\dxMeasDef{ALEPH.Gamma53.pub.BARATE.98E}{Gamma53}{BARATE 98E}{(0.23 \pm 0.19 \pm 0.07)\cdot 10^{-3}}{0.23 \cdot 10^{-3}}{\pm 0.19 \cdot 10^{-3}}{\pm 0.07 \cdot 10^{-3}}
\dxQuantDef{Gamma54}{\BR_{54}}{\BR(\tau^- \to h^- h^- h^+ \ge{} 0\, \text{neutrals} \ge{} 0\,  K_L^0\, \nu_\tau)}{0.1519 \pm 0.0006}{0.1519}{\pm 0.0006}
\dxMeasDef{CELLO.Gamma54.pub.BEHREND.89B}{Gamma54}{BEHREND 89B}{0.1500 \pm 0.0040 \pm 0.0030}{0.1500}{\pm 0.0040}{\pm 0.0030}
\dxMeasDef{L3.Gamma54.pub.ADEVA.91F}{Gamma54}{ADEVA 91F}{0.1440 \pm 0.0060 \pm 0.0030}{0.1440}{\pm 0.0060}{\pm 0.0030}
\dxMeasDef{TPC.Gamma54.pub.AIHARA.87B}{Gamma54}{AIHARA 87B}{0.1510 \pm 0.0080 \pm 0.0060}{0.1510}{\pm 0.0080}{\pm 0.0060}
\dxQuantDef{Gamma55}{\BR_{55}}{\BR(\tau^- \to h^- h^- h^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau\;(\text{ex.}K^0))}{0.1454 \pm 0.0006}{0.1454}{\pm 0.0006}
\dxMeasDef{L3.Gamma55.pub.ACHARD.01D}{Gamma55}{ACHARD 01D}{0.1456 \pm 0.0010 \pm 0.0008}{0.1456}{\pm 0.0010}{\pm 0.0008}
\dxMeasDef{OPAL.Gamma55.pub.AKERS.95Y}{Gamma55}{AKERS 95Y}{0.1496 \pm 0.0009 \pm 0.0022}{0.1496}{\pm 0.0009}{\pm 0.0022}
\dxQuantDef{Gamma56}{\BR_{56}}{\BR(\tau^- \to h^- h^- h^+ \nu_\tau)}{0.0979 \pm 0.0005}{0.0979}{\pm 0.0005}
\dxQuantDef{Gamma57}{\BR_{57}}{\BR(\tau^- \to h^- h^- h^+ \nu_\tau\;(\text{ex.}K^0))}{0.0945 \pm 0.0005}{0.0945}{\pm 0.0005}
\dxMeasDef{CLEO.Gamma57.pub.BALEST.95C}{Gamma57}{BALEST 95C}{0.0951 \pm 0.0007 \pm 0.0020}{0.0951}{\pm 0.0007}{\pm 0.0020}
\dxMeasDef{DELPHI.Gamma57.pub.ABDALLAH.06A}{Gamma57}{ABDALLAH 06A}{0.0932 \pm 0.0009 \pm 0.0008}{0.0932}{\pm 0.0009}{\pm 0.0008}
\dxQuantDef{Gamma57by55}{\BR_{57 / 55}}{\frac{\BR(\tau^- \to h^- h^- h^+ \nu_\tau\;(\text{ex.}K^0))}{\BR(\tau^- \to h^- h^- h^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau\;(\text{ex.}K^0))}}{0.6496 \pm 0.0031}{0.6496}{\pm 0.0031}
\dxMeasDef{OPAL.Gamma57by55.pub.AKERS.95Y}{Gamma57by55}{AKERS 95Y}{0.6600 \pm 0.0040 \pm 0.0140}{0.6600}{\pm 0.0040}{\pm 0.0140}
\dxQuantDef{Gamma58}{\BR_{58}}{\BR(\tau^- \to h^- h^- h^+ \nu_\tau\;(\text{ex.}K^0,\omega))}{0.0942 \pm 0.0005}{0.0942}{\pm 0.0005}
\dxQuantDef{Gamma59}{\BR_{59}}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \nu_\tau)}{0.0930 \pm 0.0005}{0.0930}{\pm 0.0005}
\dxQuantDef{Gamma60}{\BR_{60}}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0))}{0.09010 \pm 0.00052}{0.09010}{\pm 0.00052}
\dxMeasDef{BaBar.Gamma60.pub.AUBERT.08}{Gamma60}{AUBERT 08}{0.08830 \pm 0.00010 \pm 0.00130}{0.08830}{\pm 0.00010}{\pm 0.00130}
\dxMeasDef{Belle.Gamma60.pub.LEE.10}{Gamma60}{LEE 10}{0.08420 \pm 0.00000 {}^{+0.00260}_{-0.00250}}{0.08420}{\pm 0.00000}{{}^{+0.00260}_{-0.00250}}
\dxMeasDef{CLEO3.Gamma60.pub.BRIERE.03}{Gamma60}{BRIERE 03}{0.09130 \pm 0.00050 \pm 0.00460}{0.09130}{\pm 0.00050}{\pm 0.00460}
\dxQuantDef{Gamma62}{\BR_{62}}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0,\omega))}{0.0898 \pm 0.0005}{0.0898}{\pm 0.0005}
\dxMeasDef{ALEPH.Gamma62.pub.SCHAEL.05C}{Gamma62}{SCHAEL 05C}{0.0904 \pm 0.0006 \pm 0.0008}{0.0904}{\pm 0.0006}{\pm 0.0008}
\dxQuantDef{Gamma63}{\BR_{63}}{\BR(\tau^- \to h^- h^- h^+ \ge{} 1\,  \text{neutrals}\, \nu_\tau)}{0.0529 \pm 0.0005}{0.0529}{\pm 0.0005}
\dxQuantDef{Gamma64}{\BR_{64}}{\BR(\tau^- \to h^- h^- h^+ \ge{} 1\,  \pi^0\, \nu_\tau\;(\text{ex.}K^0))}{0.0509 \pm 0.0005}{0.0509}{\pm 0.0005}
\dxQuantDef{Gamma65}{\BR_{65}}{\BR(\tau^- \to h^- h^- h^+ \pi^0 \nu_\tau)}{0.0476 \pm 0.0005}{0.0476}{\pm 0.0005}
\dxQuantDef{Gamma66}{\BR_{66}}{\BR(\tau^- \to h^- h^- h^+ \pi^0 \nu_\tau\;(\text{ex.}K^0))}{0.0457 \pm 0.0005}{0.0457}{\pm 0.0005}
\dxMeasDef{CLEO.Gamma66.pub.BALEST.95C}{Gamma66}{BALEST 95C}{0.0423 \pm 0.0006 \pm 0.0022}{0.0423}{\pm 0.0006}{\pm 0.0022}
\dxMeasDef{DELPHI.Gamma66.pub.ABDALLAH.06A}{Gamma66}{ABDALLAH 06A}{0.0454 \pm 0.0011 \pm 0.0010}{0.0454}{\pm 0.0011}{\pm 0.0010}
\dxQuantDef{Gamma67}{\BR_{67}}{\BR(\tau^- \to h^- h^- h^+ \pi^0 \nu_\tau\;(\text{ex.}K^0,\omega))}{0.0279 \pm 0.0007}{0.0279}{\pm 0.0007}
\dxQuantDef{Gamma68}{\BR_{68}}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \pi^0 \nu_\tau)}{0.0462 \pm 0.0005}{0.0462}{\pm 0.0005}
\dxQuantDef{Gamma69}{\BR_{69}}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \pi^0 \nu_\tau\;(\text{ex.}K^0))}{0.0449 \pm 0.0005}{0.0449}{\pm 0.0005}
\dxMeasDef{ALEPH.Gamma69.pub.SCHAEL.05C}{Gamma69}{SCHAEL 05C}{0.0460 \pm 0.0006 \pm 0.0006}{0.0460}{\pm 0.0006}{\pm 0.0006}
\dxMeasDef{CLEO.Gamma69.pub.EDWARDS.00A}{Gamma69}{EDWARDS 00A}{0.0419 \pm 0.0010 \pm 0.0021}{0.0419}{\pm 0.0010}{\pm 0.0021}
\dxQuantDef{Gamma70}{\BR_{70}}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \pi^0 \nu_\tau\;(\text{ex.}K^0,\omega))}{0.0274 \pm 0.0007}{0.0274}{\pm 0.0007}
\dxQuantDef{Gamma74}{\BR_{74}}{\BR(\tau^- \to h^- h^- h^+ \ge{} 2\, \pi^0\, \nu_\tau\;(\text{ex.}K^0))}{0.00515 \pm 0.00031}{0.00515}{\pm 0.00031}
\dxMeasDef{DELPHI.Gamma74.pub.ABDALLAH.06A}{Gamma74}{ABDALLAH 06A}{0.00561 \pm 0.00068 \pm 0.00095}{0.00561}{\pm 0.00068}{\pm 0.00095}
\dxQuantDef{Gamma75}{\BR_{75}}{\BR(\tau^- \to h^- h^- h^+ 2\pi^0 \nu_\tau)}{0.00504 \pm 0.00031}{0.00504}{\pm 0.00031}
\dxQuantDef{Gamma76}{\BR_{76}}{\BR(\tau^- \to h^- h^- h^+ 2\pi^0 \nu_\tau\;(\text{ex.}K^0))}{0.00494 \pm 0.00031}{0.00494}{\pm 0.00031}
\dxMeasDef{ALEPH.Gamma76.pub.SCHAEL.05C}{Gamma76}{SCHAEL 05C}{0.00435 \pm 0.00030 \pm 0.00035}{0.00435}{\pm 0.00030}{\pm 0.00035}
\dxQuantDef{Gamma76by54}{\BR_{76 / 54}}{\frac{\BR(\tau^- \to h^- h^- h^+ 2\pi^0 \nu_\tau\;(\text{ex.}K^0))}{\BR(\tau^- \to h^- h^- h^+ \ge{} 0\, \text{neutrals} \ge{} 0\,  K_L^0\, \nu_\tau)}}{0.0325 \pm 0.0020}{0.0325}{\pm 0.0020}
\dxMeasDef{CLEO.Gamma76by54.pub.BORTOLETTO.93}{Gamma76by54}{BORTOLETTO 93}{0.0340 \pm 0.0020 \pm 0.0030}{0.0340}{\pm 0.0020}{\pm 0.0030}
\dxQuantDef{Gamma77}{\BR_{77}}{\BR(\tau^- \to h^- h^- h^+ 2\pi^0 \nu_\tau\;(\text{ex.}K^0,\omega,\eta))}{0.0010 \pm 0.0004}{0.0010}{\pm 0.0004}
\dxQuantDef{Gamma78}{\BR_{78}}{\BR(\tau^- \to h^- h^- h^+ 3\pi^0 \nu_\tau)}{(212 \pm 30)\cdot 10^{-6}}{212 \cdot 10^{-6}}{\pm 30 \cdot 10^{-6}}
\dxMeasDef{CLEO.Gamma78.pub.ANASTASSOV.01}{Gamma78}{ANASTASSOV 01}{(220 \pm 30 \pm 40)\cdot 10^{-6}}{220 \cdot 10^{-6}}{\pm 30 \cdot 10^{-6}}{\pm 40 \cdot 10^{-6}}
\dxQuantDef{Gamma79}{\BR_{79}}{\BR(\tau^- \to K^- h^- h^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau)}{0.00628 \pm 0.00014}{0.00628}{\pm 0.00014}
\dxQuantDef{Gamma80}{\BR_{80}}{\BR(\tau^- \to K^- \pi^- h^+ \nu_\tau\;(\text{ex.}K^0))}{0.00436 \pm 0.00007}{0.00436}{\pm 0.00007}
\dxQuantDef{Gamma80by60}{\BR_{80 / 60}}{\frac{\BR(\tau^- \to K^- \pi^- h^+ \nu_\tau\;(\text{ex.}K^0))}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0))}}{0.0484 \pm 0.0008}{0.0484}{\pm 0.0008}
\dxMeasDef{CLEO.Gamma80by60.pub.RICHICHI.99}{Gamma80by60}{RICHICHI 99}{0.0544 \pm 0.0021 \pm 0.0053}{0.0544}{\pm 0.0021}{\pm 0.0053}
\dxQuantDef{Gamma81}{\BR_{81}}{\BR(\tau^- \to K^- \pi^- h^+ \pi^0 \nu_\tau\;(\text{ex.}K^0))}{(0.85 \pm 0.12)\cdot 10^{-3}}{0.85 \cdot 10^{-3}}{\pm 0.12 \cdot 10^{-3}}
\dxQuantDef{Gamma81by69}{\BR_{81 / 69}}{\frac{\BR(\tau^- \to K^- \pi^- h^+ \pi^0 \nu_\tau\;(\text{ex.}K^0))}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \pi^0 \nu_\tau\;(\text{ex.}K^0))}}{0.0189 \pm 0.0026}{0.0189}{\pm 0.0026}
\dxMeasDef{CLEO.Gamma81by69.pub.RICHICHI.99}{Gamma81by69}{RICHICHI 99}{0.0261 \pm 0.0045 \pm 0.0042}{0.0261}{\pm 0.0045}{\pm 0.0042}
\dxQuantDef{Gamma82}{\BR_{82}}{\BR(\tau^- \to K^- \pi^- \pi^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau)}{0.00476 \pm 0.00014}{0.00476}{\pm 0.00014}
\dxMeasDef{TPC.Gamma82.pub.BAUER.94}{Gamma82}{BAUER 94}{0.00580 {}^{+0.00150}_{-0.00130} \pm 0.00120}{0.00580}{{}^{+0.00150}_{-0.00130}}{\pm 0.00120}
\dxQuantDef{Gamma83}{\BR_{83}}{\BR(\tau^- \to K^- \pi^- \pi^+ \ge{} 0\,  \pi^0\, \nu_\tau\;(\text{ex.}K^0))}{0.00372 \pm 0.00013}{0.00372}{\pm 0.00013}
\dxQuantDef{Gamma84}{\BR_{84}}{\BR(\tau^- \to K^- \pi^- \pi^+ \nu_\tau)}{0.00344 \pm 0.00007}{0.00344}{\pm 0.00007}
\dxQuantDef{Gamma85}{\BR_{85}}{\BR(\tau^- \to K^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0))}{0.002930 \pm 0.000068}{0.002930}{\pm 0.000068}
\dxMeasDef{ALEPH.Gamma85.pub.BARATE.98}{Gamma85}{BARATE 98}{0.002140 \pm 0.000370 \pm 0.000290}{0.002140}{\pm 0.000370}{\pm 0.000290}
\dxMeasDef{BaBar.Gamma85.pub.AUBERT.08}{Gamma85}{AUBERT 08}{0.002730 \pm 0.000020 \pm 0.000090}{0.002730}{\pm 0.000020}{\pm 0.000090}
\dxMeasDef{Belle.Gamma85.pub.LEE.10}{Gamma85}{LEE 10}{0.003300 \pm 0.000010 {}^{+0.000160}_{-0.000170}}{0.003300}{\pm 0.000010}{{}^{+0.000160}_{-0.000170}}
\dxMeasDef{CLEO3.Gamma85.pub.BRIERE.03}{Gamma85}{BRIERE 03}{0.003840 \pm 0.000140 \pm 0.000380}{0.003840}{\pm 0.000140}{\pm 0.000380}
\dxMeasDef{OPAL.Gamma85.pub.ABBIENDI.04J}{Gamma85}{ABBIENDI 04J}{0.004150 \pm 0.000530 \pm 0.000400}{0.004150}{\pm 0.000530}{\pm 0.000400}
\dxQuantDef{Gamma85by60}{\BR_{85 / 60}}{\frac{\BR(\tau^- \to K^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0))}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0))}}{0.0325 \pm 0.0007}{0.0325}{\pm 0.0007}
\dxQuantDef{Gamma87}{\BR_{87}}{\BR(\tau^- \to K^- \pi^- \pi^+ \pi^0 \nu_\tau)}{0.00131 \pm 0.00012}{0.00131}{\pm 0.00012}
\dxQuantDef{Gamma88}{\BR_{88}}{\BR(\tau^- \to K^- \pi^- \pi^+ \pi^0 \nu_\tau\;(\text{ex.}K^0))}{(0.79 \pm 0.12)\cdot 10^{-3}}{0.79 \cdot 10^{-3}}{\pm 0.12 \cdot 10^{-3}}
\dxMeasDef{ALEPH.Gamma88.pub.BARATE.98}{Gamma88}{BARATE 98}{(0.61 \pm 0.39 \pm 0.18)\cdot 10^{-3}}{0.61 \cdot 10^{-3}}{\pm 0.39 \cdot 10^{-3}}{\pm 0.18 \cdot 10^{-3}}
\dxMeasDef{CLEO3.Gamma88.pub.ARMS.05}{Gamma88}{ARMS 05}{(0.74 \pm 0.08 \pm 0.11)\cdot 10^{-3}}{0.74 \cdot 10^{-3}}{\pm 0.08 \cdot 10^{-3}}{\pm 0.11 \cdot 10^{-3}}
\dxQuantDef{Gamma89}{\BR_{89}}{\BR(\tau^- \to K^- \pi^- \pi^+ \pi^0 \nu_\tau\;(\text{ex.}K^0,\eta))}{(0.75 \pm 0.12)\cdot 10^{-3}}{0.75 \cdot 10^{-3}}{\pm 0.12 \cdot 10^{-3}}
\dxQuantDef{Gamma92}{\BR_{92}}{\BR(\tau^- \to \pi^- K^- K^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau)}{0.001495 \pm 0.000033}{0.001495}{\pm 0.000033}
\dxMeasDef{OPAL.Gamma92.pub.ABBIENDI.00D}{Gamma92}{ABBIENDI 00D}{0.001590 \pm 0.000530 \pm 0.000200}{0.001590}{\pm 0.000530}{\pm 0.000200}
\dxMeasDef{TPC.Gamma92.pub.BAUER.94}{Gamma92}{BAUER 94}{0.001500 {}^{+0.000900}_{-0.000700} \pm 0.000300}{0.001500}{{}^{+0.000900}_{-0.000700}}{\pm 0.000300}
\dxQuantDef{Gamma93}{\BR_{93}}{\BR(\tau^- \to \pi^- K^- K^+ \nu_\tau)}{0.001434 \pm 0.000027}{0.001434}{\pm 0.000027}
\dxMeasDef{ALEPH.Gamma93.pub.BARATE.98}{Gamma93}{BARATE 98}{0.001630 \pm 0.000210 \pm 0.000170}{0.001630}{\pm 0.000210}{\pm 0.000170}
\dxMeasDef{BaBar.Gamma93.pub.AUBERT.08}{Gamma93}{AUBERT 08}{0.001346 \pm 0.000010 \pm 0.000036}{0.001346}{\pm 0.000010}{\pm 0.000036}
\dxMeasDef{Belle.Gamma93.pub.LEE.10}{Gamma93}{LEE 10}{0.001550 \pm 0.000010 {}^{+0.000060}_{-0.000050}}{0.001550}{\pm 0.000010}{{}^{+0.000060}_{-0.000050}}
\dxMeasDef{CLEO3.Gamma93.pub.BRIERE.03}{Gamma93}{BRIERE 03}{0.001550 \pm 0.000060 \pm 0.000090}{0.001550}{\pm 0.000060}{\pm 0.000090}
\dxQuantDef{Gamma93by60}{\BR_{93 / 60}}{\frac{\BR(\tau^- \to \pi^- K^- K^+ \nu_\tau)}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0))}}{0.01592 \pm 0.00030}{0.01592}{\pm 0.00030}
\dxMeasDef{CLEO.Gamma93by60.pub.RICHICHI.99}{Gamma93by60}{RICHICHI 99}{0.01600 \pm 0.00150 \pm 0.00300}{0.01600}{\pm 0.00150}{\pm 0.00300}
\dxQuantDef{Gamma94}{\BR_{94}}{\BR(\tau^- \to \pi^- K^- K^+ \pi^0 \nu_\tau)}{(61 \pm 18)\cdot 10^{-6}}{61 \cdot 10^{-6}}{\pm 18 \cdot 10^{-6}}
\dxMeasDef{ALEPH.Gamma94.pub.BARATE.98}{Gamma94}{BARATE 98}{(750 \pm 290 \pm 150)\cdot 10^{-6}}{750 \cdot 10^{-6}}{\pm 290 \cdot 10^{-6}}{\pm 150 \cdot 10^{-6}}
\dxMeasDef{CLEO3.Gamma94.pub.ARMS.05}{Gamma94}{ARMS 05}{(55 \pm 14 \pm 12)\cdot 10^{-6}}{55 \cdot 10^{-6}}{\pm 14 \cdot 10^{-6}}{\pm 12 \cdot 10^{-6}}
\dxQuantDef{Gamma94by69}{\BR_{94 / 69}}{\frac{\BR(\tau^- \to \pi^- K^- K^+ \pi^0 \nu_\tau)}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \pi^0 \nu_\tau\;(\text{ex.}K^0))}}{0.0014 \pm 0.0004}{0.0014}{\pm 0.0004}
\dxMeasDef{CLEO.Gamma94by69.pub.RICHICHI.99}{Gamma94by69}{RICHICHI 99}{0.0079 \pm 0.0044 \pm 0.0016}{0.0079}{\pm 0.0044}{\pm 0.0016}
\dxQuantDef{Gamma96}{\BR_{96}}{\BR(\tau^- \to K^- K^- K^+ \nu_\tau)}{(21.7 \pm 8.0)\cdot 10^{-6}}{21.7 \cdot 10^{-6}}{\pm 8.0 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma96.pub.AUBERT.08}{Gamma96}{AUBERT 08}{(15.8 \pm 1.3 \pm 1.2)\cdot 10^{-6}}{15.8 \cdot 10^{-6}}{\pm 1.3 \cdot 10^{-6}}{\pm 1.2 \cdot 10^{-6}}
\dxMeasDef{Belle.Gamma96.pub.LEE.10}{Gamma96}{LEE 10}{(32.9 \pm 1.7 {}^{+1.9}_{-2.0})\cdot 10^{-6}}{32.9 \cdot 10^{-6}}{\pm 1.7 \cdot 10^{-6}}{{}^{+1.9}_{-2.0} \cdot 10^{-6}}
\dxQuantDef{Gamma102}{\BR_{102}}{\BR(\tau^- \to 3h^- 2h^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau\;(\text{ex.}K^0))}{0.00099 \pm 0.00004}{0.00099}{\pm 0.00004}
\dxMeasDef{CLEO.Gamma102.pub.GIBAUT.94B}{Gamma102}{GIBAUT 94B}{0.00097 \pm 0.00005 \pm 0.00011}{0.00097}{\pm 0.00005}{\pm 0.00011}
\dxMeasDef{HRS.Gamma102.pub.BYLSMA.87}{Gamma102}{BYLSMA 87}{0.00102 \pm 0.00029 \pm 0.00000}{0.00102}{\pm 0.00029}{\pm 0.00000}
\dxMeasDef{L3.Gamma102.pub.ACHARD.01D}{Gamma102}{ACHARD 01D}{0.00170 \pm 0.00022 \pm 0.00026}{0.00170}{\pm 0.00022}{\pm 0.00026}
\dxQuantDef{Gamma103}{\BR_{103}}{\BR(\tau^- \to 3h^- 2h^+ \nu_\tau\;(\text{ex.}K^0))}{(828 \pm 31)\cdot 10^{-6}}{828 \cdot 10^{-6}}{\pm 31 \cdot 10^{-6}}
\dxMeasDef{ALEPH.Gamma103.pub.SCHAEL.05C}{Gamma103}{SCHAEL 05C}{(720 \pm 90 \pm 120)\cdot 10^{-6}}{720 \cdot 10^{-6}}{\pm 90 \cdot 10^{-6}}{\pm 120 \cdot 10^{-6}}
\dxMeasDef{ARGUS.Gamma103.pub.ALBRECHT.88B}{Gamma103}{ALBRECHT 88B}{(640 \pm 230 \pm 100)\cdot 10^{-6}}{640 \cdot 10^{-6}}{\pm 230 \cdot 10^{-6}}{\pm 100 \cdot 10^{-6}}
\dxMeasDef{CLEO.Gamma103.pub.GIBAUT.94B}{Gamma103}{GIBAUT 94B}{(770 \pm 50 \pm 90)\cdot 10^{-6}}{770 \cdot 10^{-6}}{\pm 50 \cdot 10^{-6}}{\pm 90 \cdot 10^{-6}}
\dxMeasDef{DELPHI.Gamma103.pub.ABDALLAH.06A}{Gamma103}{ABDALLAH 06A}{(970 \pm 150 \pm 50)\cdot 10^{-6}}{970 \cdot 10^{-6}}{\pm 150 \cdot 10^{-6}}{\pm 50 \cdot 10^{-6}}
\dxMeasDef{HRS.Gamma103.pub.BYLSMA.87}{Gamma103}{BYLSMA 87}{(510 \pm 200 \pm 0)\cdot 10^{-6}}{510 \cdot 10^{-6}}{\pm 200 \cdot 10^{-6}}{\pm 0 \cdot 10^{-6}}
\dxMeasDef{OPAL.Gamma103.pub.ACKERSTAFF.99E}{Gamma103}{ACKERSTAFF 99E}{(910 \pm 140 \pm 60)\cdot 10^{-6}}{910 \cdot 10^{-6}}{\pm 140 \cdot 10^{-6}}{\pm 60 \cdot 10^{-6}}
\dxQuantDef{Gamma104}{\BR_{104}}{\BR(\tau^- \to 3h^- 2h^+ \pi^0 \nu_\tau\;(\text{ex.}K^0))}{(165 \pm 11)\cdot 10^{-6}}{165 \cdot 10^{-6}}{\pm 11 \cdot 10^{-6}}
\dxMeasDef{ALEPH.Gamma104.pub.SCHAEL.05C}{Gamma104}{SCHAEL 05C}{(210 \pm 70 \pm 90)\cdot 10^{-6}}{210 \cdot 10^{-6}}{\pm 70 \cdot 10^{-6}}{\pm 90 \cdot 10^{-6}}
\dxMeasDef{CLEO.Gamma104.pub.ANASTASSOV.01}{Gamma104}{ANASTASSOV 01}{(170 \pm 20 \pm 20)\cdot 10^{-6}}{170 \cdot 10^{-6}}{\pm 20 \cdot 10^{-6}}{\pm 20 \cdot 10^{-6}}
\dxMeasDef{DELPHI.Gamma104.pub.ABDALLAH.06A}{Gamma104}{ABDALLAH 06A}{(160 \pm 120 \pm 60)\cdot 10^{-6}}{160 \cdot 10^{-6}}{\pm 120 \cdot 10^{-6}}{\pm 60 \cdot 10^{-6}}
\dxMeasDef{OPAL.Gamma104.pub.ACKERSTAFF.99E}{Gamma104}{ACKERSTAFF 99E}{(270 \pm 180 \pm 90)\cdot 10^{-6}}{270 \cdot 10^{-6}}{\pm 180 \cdot 10^{-6}}{\pm 90 \cdot 10^{-6}}
\dxQuantDef{Gamma106}{\BR_{106}}{\BR(\tau^- \to (5\pi)^- \nu_\tau)}{0.0078 \pm 0.0005}{0.0078}{\pm 0.0005}
\dxQuantDef{Gamma110}{\BR_{110}}{\BR(\tau^- \to X_s^- \nu_\tau)}{0.0291 \pm 0.0005}{0.0291}{\pm 0.0005}
\dxQuantDef{Gamma126}{\BR_{126}}{\BR(\tau^- \to \pi^- \pi^0 \eta \nu_\tau)}{0.001386 \pm 0.000072}{0.001386}{\pm 0.000072}
\dxMeasDef{ALEPH.Gamma126.pub.BUSKULIC.97C}{Gamma126}{BUSKULIC 97C}{0.001800 \pm 0.000400 \pm 0.000200}{0.001800}{\pm 0.000400}{\pm 0.000200}
\dxMeasDef{Belle.Gamma126.pub.INAMI.09}{Gamma126}{INAMI 09}{0.001350 \pm 0.000030 \pm 0.000070}{0.001350}{\pm 0.000030}{\pm 0.000070}
\dxMeasDef{CLEO.Gamma126.pub.ARTUSO.92}{Gamma126}{ARTUSO 92}{0.001700 \pm 0.000200 \pm 0.000200}{0.001700}{\pm 0.000200}{\pm 0.000200}
\dxQuantDef{Gamma128}{\BR_{128}}{\BR(\tau^- \to K^- \eta \nu_\tau)}{(155 \pm 8)\cdot 10^{-6}}{155 \cdot 10^{-6}}{\pm 8 \cdot 10^{-6}}
\dxMeasDef{ALEPH.Gamma128.pub.BUSKULIC.97C}{Gamma128}{BUSKULIC 97C}{(290 {}^{+130}_{-120} \pm 70)\cdot 10^{-6}}{290 \cdot 10^{-6}}{{}^{+130}_{-120} \cdot 10^{-6}}{\pm 70 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E}{Gamma128}{DEL-AMO-SANCHEZ 11E}{(142 \pm 11 \pm 7)\cdot 10^{-6}}{142 \cdot 10^{-6}}{\pm 11 \cdot 10^{-6}}{\pm 7 \cdot 10^{-6}}
\dxMeasDef{Belle.Gamma128.pub.INAMI.09}{Gamma128}{INAMI 09}{(158 \pm 5 \pm 9)\cdot 10^{-6}}{158 \cdot 10^{-6}}{\pm 5 \cdot 10^{-6}}{\pm 9 \cdot 10^{-6}}
\dxMeasDef{CLEO.Gamma128.pub.BARTELT.96}{Gamma128}{BARTELT 96}{(260 \pm 50 \pm 50)\cdot 10^{-6}}{260 \cdot 10^{-6}}{\pm 50 \cdot 10^{-6}}{\pm 50 \cdot 10^{-6}}
\dxQuantDef{Gamma130}{\BR_{130}}{\BR(\tau^- \to K^- \pi^0 \eta \nu_\tau)}{(48 \pm 12)\cdot 10^{-6}}{48 \cdot 10^{-6}}{\pm 12 \cdot 10^{-6}}
\dxMeasDef{Belle.Gamma130.pub.INAMI.09}{Gamma130}{INAMI 09}{(46 \pm 11 \pm 4)\cdot 10^{-6}}{46 \cdot 10^{-6}}{\pm 11 \cdot 10^{-6}}{\pm 4 \cdot 10^{-6}}
\dxMeasDef{CLEO.Gamma130.pub.BISHAI.99}{Gamma130}{BISHAI 99}{(177 \pm 56 \pm 71)\cdot 10^{-6}}{177 \cdot 10^{-6}}{\pm 56 \cdot 10^{-6}}{\pm 71 \cdot 10^{-6}}
\dxQuantDef{Gamma132}{\BR_{132}}{\BR(\tau^- \to \pi^- \bar{K}^0 \eta \nu_\tau)}{(94 \pm 15)\cdot 10^{-6}}{94 \cdot 10^{-6}}{\pm 15 \cdot 10^{-6}}
\dxMeasDef{Belle.Gamma132.pub.INAMI.09}{Gamma132}{INAMI 09}{(88 \pm 14 \pm 6)\cdot 10^{-6}}{88 \cdot 10^{-6}}{\pm 14 \cdot 10^{-6}}{\pm 6 \cdot 10^{-6}}
\dxMeasDef{CLEO.Gamma132.pub.BISHAI.99}{Gamma132}{BISHAI 99}{(220 \pm 70 \pm 22)\cdot 10^{-6}}{220 \cdot 10^{-6}}{\pm 70 \cdot 10^{-6}}{\pm 22 \cdot 10^{-6}}
\dxQuantDef{Gamma136}{\BR_{136}}{\BR(\tau^- \to \pi^- \pi^+ \pi^- \eta \nu_\tau\;(\text{ex.}K^0))}{(220 \pm 13)\cdot 10^{-6}}{220 \cdot 10^{-6}}{\pm 13 \cdot 10^{-6}}
\dxQuantDef{Gamma149}{\BR_{149}}{\BR(\tau^- \to h^- \omega \ge{} 0\,  \text{neutrals}\, \nu_\tau)}{0.0240 \pm 0.0008}{0.0240}{\pm 0.0008}
\dxQuantDef{Gamma150}{\BR_{150}}{\BR(\tau^- \to h^- \omega \nu_\tau)}{0.0199 \pm 0.0006}{0.0199}{\pm 0.0006}
\dxMeasDef{ALEPH.Gamma150.pub.BUSKULIC.97C}{Gamma150}{BUSKULIC 97C}{0.0191 \pm 0.0007 \pm 0.0006}{0.0191}{\pm 0.0007}{\pm 0.0006}
\dxMeasDef{CLEO.Gamma150.pub.BARINGER.87}{Gamma150}{BARINGER 87}{0.0160 \pm 0.0027 \pm 0.0041}{0.0160}{\pm 0.0027}{\pm 0.0041}
\dxQuantDef{Gamma150by66}{\BR_{150 / 66}}{\frac{\BR(\tau^- \to h^- \omega \nu_\tau)}{\BR(\tau^- \to h^- h^- h^+ \pi^0 \nu_\tau\;(\text{ex.}K^0))}}{0.435 \pm 0.014}{0.435}{\pm 0.014}
\dxMeasDef{ALEPH.Gamma150by66.pub.BUSKULIC.96}{Gamma150by66}{BUSKULIC 96}{0.431 \pm 0.033 \pm 0.000}{0.431}{\pm 0.033}{\pm 0.000}
\dxMeasDef{CLEO.Gamma150by66.pub.BALEST.95C}{Gamma150by66}{BALEST 95C}{0.464 \pm 0.016 \pm 0.017}{0.464}{\pm 0.016}{\pm 0.017}
\dxQuantDef{Gamma151}{\BR_{151}}{\BR(\tau^- \to K^- \omega \nu_\tau)}{(0.41 \pm 0.09)\cdot 10^{-3}}{0.41 \cdot 10^{-3}}{\pm 0.09 \cdot 10^{-3}}
\dxMeasDef{CLEO3.Gamma151.pub.ARMS.05}{Gamma151}{ARMS 05}{(0.41 \pm 0.06 \pm 0.07)\cdot 10^{-3}}{0.41 \cdot 10^{-3}}{\pm 0.06 \cdot 10^{-3}}{\pm 0.07 \cdot 10^{-3}}
\dxQuantDef{Gamma152}{\BR_{152}}{\BR(\tau^- \to h^- \pi^0 \omega \nu_\tau)}{0.0041 \pm 0.0004}{0.0041}{\pm 0.0004}
\dxMeasDef{ALEPH.Gamma152.pub.BUSKULIC.97C}{Gamma152}{BUSKULIC 97C}{0.0043 \pm 0.0006 \pm 0.0005}{0.0043}{\pm 0.0006}{\pm 0.0005}
\dxQuantDef{Gamma152by54}{\BR_{152 / 54}}{\frac{\BR(\tau^- \to h^- \omega \pi^0 \nu_\tau)}{\BR(\tau^- \to h^- h^- h^+ \ge{} 0\, \text{neutrals} \ge{} 0\,  K_L^0\, \nu_\tau)}}{0.0268 \pm 0.0028}{0.0268}{\pm 0.0028}
\dxQuantDef{Gamma152by76}{\BR_{152 / 76}}{\frac{\BR(\tau^- \to h^- \omega \pi^0 \nu_\tau)}{\BR(\tau^- \to h^- h^- h^+ 2\pi^0 \nu_\tau\;(\text{ex.}K^0))}}{0.82 \pm 0.08}{0.82}{\pm 0.08}
\dxMeasDef{CLEO.Gamma152by76.pub.BORTOLETTO.93}{Gamma152by76}{BORTOLETTO 93}{0.81 \pm 0.06 \pm 0.06}{0.81}{\pm 0.06}{\pm 0.06}
\dxQuantDef{Gamma167}{\BR_{167}}{\BR(\tau^- \to K^- \phi \nu_\tau)}{(44 \pm 16)\cdot 10^{-6}}{44 \cdot 10^{-6}}{\pm 16 \cdot 10^{-6}}
\dxQuantDef{Gamma168}{\BR_{168}}{\BR(\tau^- \to K^- \phi(K^+ K^-) \nu_\tau)}{(22 \pm 8)\cdot 10^{-6}}{22 \cdot 10^{-6}}{\pm 8 \cdot 10^{-6}}
\dxQuantDef{Gamma169}{\BR_{169}}{\BR(\tau^- \to K^- \phi(K_S^0 K_L^0) \nu_\tau)}{(15 \pm 6)\cdot 10^{-6}}{15 \cdot 10^{-6}}{\pm 6 \cdot 10^{-6}}
\dxQuantDef{Gamma800}{\BR_{800}}{\BR(\tau^- \to \pi^- \omega \nu_\tau)}{0.0195 \pm 0.0006}{0.0195}{\pm 0.0006}
\dxQuantDef{Gamma802}{\BR_{802}}{\BR(\tau^- \to K^- \pi^- \pi^+ \nu_\tau\;(\text{ex.}K^0,\omega))}{0.00292 \pm 0.00007}{0.00292}{\pm 0.00007}
\dxQuantDef{Gamma803}{\BR_{803}}{\BR(\tau^- \to K^- \pi^- \pi^+ \pi^0 \nu_\tau\;(\text{ex.}K^0,\omega,\eta))}{(0.39 \pm 0.14)\cdot 10^{-3}}{0.39 \cdot 10^{-3}}{\pm 0.14 \cdot 10^{-3}}
\dxQuantDef{Gamma804}{\BR_{804}}{\BR(\tau^- \to \pi^- K_L^0 K_L^0 \nu_\tau)}{(235 \pm 6)\cdot 10^{-6}}{235 \cdot 10^{-6}}{\pm 6 \cdot 10^{-6}}
\dxQuantDef{Gamma805}{\BR_{805}}{\BR(\tau^- \to a_1^-(\pi^- \gamma) \nu_\tau)}{(0.38 \pm 0.15)\cdot 10^{-3}}{0.38 \cdot 10^{-3}}{\pm 0.15 \cdot 10^{-3}}
\dxQuantDef{Gamma806}{\BR_{806}}{\BR(\tau^- \to \pi^- K_L^0 K_L^0 \pi^0 \nu_\tau)}{(18.2 \pm 2.1)\cdot 10^{-6}}{18.2 \cdot 10^{-6}}{\pm 2.1 \cdot 10^{-6}}
\dxQuantDef{Gamma810}{\BR_{810}}{\BR(\tau^- \to 2\pi^- \pi^+ 3\pi^0 \nu_\tau\;(\text{ex.}K^0))}{(194 \pm 30)\cdot 10^{-6}}{194 \cdot 10^{-6}}{\pm 30 \cdot 10^{-6}}
\dxQuantDef{Gamma811}{\BR_{811}}{\BR(\tau^- \to \pi^- 2\pi^0 \omega \nu_\tau)}{(72 \pm 16)\cdot 10^{-6}}{72 \cdot 10^{-6}}{\pm 16 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma811.pub.LEES.12X}{Gamma811}{LEES 12X}{(73 \pm 12 \pm 12)\cdot 10^{-6}}{73 \cdot 10^{-6}}{\pm 12 \cdot 10^{-6}}{\pm 12 \cdot 10^{-6}}
\dxQuantDef{Gamma812}{\BR_{812}}{\BR(\tau^- \to 2\pi^- \pi^+ 3\pi^0 \nu_\tau\;(\text{ex.}K^0,\eta,\omega,f_1))}{(14 \pm 27)\cdot 10^{-6}}{14 \cdot 10^{-6}}{\pm 27 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma812.pub.LEES.12X}{Gamma812}{LEES 12X}{(10 \pm 8 \pm 30)\cdot 10^{-6}}{10 \cdot 10^{-6}}{\pm 8 \cdot 10^{-6}}{\pm 30 \cdot 10^{-6}}
\dxQuantDef{Gamma820}{\BR_{820}}{\BR(\tau^- \to 3\pi^- 2\pi^+ \nu_\tau\;(\text{ex.}K^0,\omega))}{(826 \pm 31)\cdot 10^{-6}}{826 \cdot 10^{-6}}{\pm 31 \cdot 10^{-6}}
\dxQuantDef{Gamma821}{\BR_{821}}{\BR(\tau^- \to 3\pi^- 2\pi^+ \nu_\tau\;(\text{ex.}K^0,\omega,f_1))}{(774 \pm 30)\cdot 10^{-6}}{774 \cdot 10^{-6}}{\pm 30 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma821.pub.LEES.12X}{Gamma821}{LEES 12X}{(768 \pm 4 \pm 40)\cdot 10^{-6}}{768 \cdot 10^{-6}}{\pm 4 \cdot 10^{-6}}{\pm 40 \cdot 10^{-6}}
\dxQuantDef{Gamma822}{\BR_{822}}{\BR(\tau^- \to K^- 2\pi^- 2\pi^+ \nu_\tau\;(\text{ex.}K^0))}{(0.6 \pm 1.2)\cdot 10^{-6}}{0.6 \cdot 10^{-6}}{\pm 1.2 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma822.pub.LEES.12X}{Gamma822}{LEES 12X}{(0.6 \pm 0.5 \pm 1.1)\cdot 10^{-6}}{0.6 \cdot 10^{-6}}{\pm 0.5 \cdot 10^{-6}}{\pm 1.1 \cdot 10^{-6}}
\dxQuantDef{Gamma830}{\BR_{830}}{\BR(\tau^- \to 3\pi^- 2\pi^+ \pi^0 \nu_\tau\;(\text{ex.}K^0))}{(163 \pm 11)\cdot 10^{-6}}{163 \cdot 10^{-6}}{\pm 11 \cdot 10^{-6}}
\dxQuantDef{Gamma831}{\BR_{831}}{\BR(\tau^- \to 2\pi^- \pi^+ \omega \nu_\tau\;(\text{ex.}K^0))}{(84 \pm 6)\cdot 10^{-6}}{84 \cdot 10^{-6}}{\pm 6 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma831.pub.LEES.12X}{Gamma831}{LEES 12X}{(84 \pm 4 \pm 6)\cdot 10^{-6}}{84 \cdot 10^{-6}}{\pm 4 \cdot 10^{-6}}{\pm 6 \cdot 10^{-6}}
\dxQuantDef{Gamma832}{\BR_{832}}{\BR(\tau^- \to 3\pi^- 2\pi^+ \pi^0 \nu_\tau\;(\text{ex.}K^0,\eta,\omega,f_1))}{(37.7 \pm 8.7)\cdot 10^{-6}}{37.7 \cdot 10^{-6}}{\pm 8.7 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma832.pub.LEES.12X}{Gamma832}{LEES 12X}{(36.0 \pm 3.0 \pm 9.0)\cdot 10^{-6}}{36.0 \cdot 10^{-6}}{\pm 3.0 \cdot 10^{-6}}{\pm 9.0 \cdot 10^{-6}}
\dxQuantDef{Gamma833}{\BR_{833}}{\BR(\tau^- \to K^- 2\pi^- 2\pi^+ \pi^0 \nu_\tau\;(\text{ex.}K^0))}{(1.1 \pm 0.6)\cdot 10^{-6}}{1.1 \cdot 10^{-6}}{\pm 0.6 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma833.pub.LEES.12X}{Gamma833}{LEES 12X}{(1.1 \pm 0.4 \pm 0.4)\cdot 10^{-6}}{1.1 \cdot 10^{-6}}{\pm 0.4 \cdot 10^{-6}}{\pm 0.4 \cdot 10^{-6}}
\dxQuantDef{Gamma910}{\BR_{910}}{\BR(\tau^- \to 2\pi^- \pi^+ \eta(3\pi^0) \nu_\tau\;(\text{ex.}K^0))}{(72 \pm 4)\cdot 10^{-6}}{72 \cdot 10^{-6}}{\pm 4 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma910.pub.LEES.12X}{Gamma910}{LEES 12X}{(83 \pm 9 \pm 8)\cdot 10^{-6}}{83 \cdot 10^{-6}}{\pm 9 \cdot 10^{-6}}{\pm 8 \cdot 10^{-6}}
\dxQuantDef{Gamma911}{\BR_{911}}{\BR(\tau^- \to \pi^- 2\pi^0 \eta(\pi^+ \pi^- \pi^0) \nu_\tau\;(\text{ex.}K^0))}{(45 \pm 9)\cdot 10^{-6}}{45 \cdot 10^{-6}}{\pm 9 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma911.pub.LEES.12X}{Gamma911}{LEES 12X}{(46 \pm 8 \pm 5)\cdot 10^{-6}}{46 \cdot 10^{-6}}{\pm 8 \cdot 10^{-6}}{\pm 5 \cdot 10^{-6}}
\dxQuantDef{Gamma920}{\BR_{920}}{\BR(\tau^- \to \pi^- f_1(2\pi^- 2\pi^+) \nu_\tau)}{(52.4 \pm 4.4)\cdot 10^{-6}}{52.4 \cdot 10^{-6}}{\pm 4.4 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma920.pub.LEES.12X}{Gamma920}{LEES 12X}{(52.0 \pm 3.1 \pm 3.7)\cdot 10^{-6}}{52.0 \cdot 10^{-6}}{\pm 3.1 \cdot 10^{-6}}{\pm 3.7 \cdot 10^{-6}}
\dxQuantDef{Gamma930}{\BR_{930}}{\BR(\tau^- \to 2\pi^- \pi^+ \eta(\pi^+ \pi^- \pi^0) \nu_\tau\;(\text{ex.}K^0))}{(50.7 \pm 3.0)\cdot 10^{-6}}{50.7 \cdot 10^{-6}}{\pm 3.0 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma930.pub.LEES.12X}{Gamma930}{LEES 12X}{(53.9 \pm 2.7 \pm 4.1)\cdot 10^{-6}}{53.9 \cdot 10^{-6}}{\pm 2.7 \cdot 10^{-6}}{\pm 4.1 \cdot 10^{-6}}
\dxQuantDef{Gamma944}{\BR_{944}}{\BR(\tau^- \to 2\pi^- \pi^+ \eta(\gamma \gamma) \nu_\tau\;(\text{ex.}K^0))}{(86.6 \pm 5.1)\cdot 10^{-6}}{86.6 \cdot 10^{-6}}{\pm 5.1 \cdot 10^{-6}}
\dxMeasDef{BaBar.Gamma944.pub.LEES.12X}{Gamma944}{LEES 12X}{(82.6 \pm 3.5 \pm 5.1)\cdot 10^{-6}}{82.6 \cdot 10^{-6}}{\pm 3.5 \cdot 10^{-6}}{\pm 5.1 \cdot 10^{-6}}
\dxQuantDef{Gamma945}{\BR_{945}}{\BR(\tau^- \to \pi^- 2\pi^0 \eta \nu_\tau\;(\text{ex.}K^0))}{(0.19 \pm 0.04)\cdot 10^{-3}}{0.19 \cdot 10^{-3}}{\pm 0.04 \cdot 10^{-3}}
\dxQuantDef{GammaUnitResid}{\BR_{\text{ur}}}{\BR(\tau^- \text{unitarity residual})}{0.0007 \pm 0.0011}{0.0007}{\pm 0.0011}
\dxQuantDef{GammaAll}{\BR_{\text{all}}}{\BR(\tau^- \to \text{all modes})}{0.9993 \pm 0.0011}{0.9993}{\pm 0.0011}
\dxQuantDef{Gamma980}{\BR_{980}}{\BR(a_1^- \to \pi^- \gamma)}{0.0021 \pm 0.0008}{0.0021}{\pm 0.0008}
\dxMeasDef{ALEPH.Gamma980.pub.SCHAEL.05C}{Gamma980}{SCHAEL 05C}{0.0021 \pm 0.0008 \pm 0.0000}{0.0021}{\pm 0.0008}{\pm 0.0000}
\dxdef{Gamma1-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma1-gn} = \dxuse{Gamma1-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma1}%
}
\dxdef{Gamma2-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma2-gn} = \dxuse{Gamma2-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma2}%
}
\dxdef{Gamma3-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma3-gn} = \dxuse{Gamma3-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma3} \\
\dxuse{ALEPH.Gamma3.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma3.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma3.pub.SCHAEL.05C-pdgref}-cite} \\
\dxuse{DELPHI.Gamma3.pub.ABREU.99X-vu} & \dxuse{\dxuse{DELPHI.Gamma3.pub.ABREU.99X-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma3.pub.ABREU.99X-pdgref}-cite} \\
\dxuse{L3.Gamma3.pub.ACCIARRI.01F-vu} & \dxuse{\dxuse{L3.Gamma3.pub.ACCIARRI.01F-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma3.pub.ACCIARRI.01F-pdgref}-cite} \\
\dxuse{OPAL.Gamma3.pub.ABBIENDI.03-vu} & \dxuse{\dxuse{OPAL.Gamma3.pub.ABBIENDI.03-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma3.pub.ABBIENDI.03-pdgref}-cite}%
}
\dxdef{Gamma3by5-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma3by5-gn} = \dxuse{Gamma3by5-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma3by5} \\
\dxuse{ARGUS.Gamma3by5.pub.ALBRECHT.92D-vu} & \dxuse{\dxuse{ARGUS.Gamma3by5.pub.ALBRECHT.92D-pdgref}-exp} & \dxuse{\dxuse{ARGUS.Gamma3by5.pub.ALBRECHT.92D-pdgref}-cite} \\
\dxuse{BaBar.Gamma3by5.pub.AUBERT.10F-vu} & \dxuse{\dxuse{BaBar.Gamma3by5.pub.AUBERT.10F-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma3by5.pub.AUBERT.10F-pdgref}-cite} \\
\dxuse{Belle2.Gamma3by5.ADACHI.2024-vu} & \dxuse{\dxuse{Belle2.Gamma3by5.ADACHI.2024-pdgref}-exp} & \dxuse{\dxuse{Belle2.Gamma3by5.ADACHI.2024-pdgref}-cite} \\
\dxuse{CLEO.Gamma3by5.pub.ANASTASSOV.97-vu} & \dxuse{\dxuse{CLEO.Gamma3by5.pub.ANASTASSOV.97-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma3by5.pub.ANASTASSOV.97-pdgref}-cite}%
}
\dxdef{Gamma5-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma5-gn} = \dxuse{Gamma5-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma5} \\
\dxuse{ALEPH.Gamma5.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma5.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma5.pub.SCHAEL.05C-pdgref}-cite} \\
\dxuse{CLEO.Gamma5.pub.ANASTASSOV.97-vu} & \dxuse{\dxuse{CLEO.Gamma5.pub.ANASTASSOV.97-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma5.pub.ANASTASSOV.97-pdgref}-cite} \\
\dxuse{DELPHI.Gamma5.pub.ABREU.99X-vu} & \dxuse{\dxuse{DELPHI.Gamma5.pub.ABREU.99X-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma5.pub.ABREU.99X-pdgref}-cite} \\
\dxuse{L3.Gamma5.pub.ACCIARRI.01F-vu} & \dxuse{\dxuse{L3.Gamma5.pub.ACCIARRI.01F-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma5.pub.ACCIARRI.01F-pdgref}-cite} \\
\dxuse{OPAL.Gamma5.pub.ABBIENDI.99H-vu} & \dxuse{\dxuse{OPAL.Gamma5.pub.ABBIENDI.99H-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma5.pub.ABBIENDI.99H-pdgref}-cite}%
}
\dxdef{Gamma7-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma7-gn} = \dxuse{Gamma7-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma7} \\
\dxuse{DELPHI.Gamma7.pub.ABREU.92N-vu} & \dxuse{\dxuse{DELPHI.Gamma7.pub.ABREU.92N-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma7.pub.ABREU.92N-pdgref}-cite} \\
\dxuse{L3.Gamma7.pub.ACCIARRI.95-vu} & \dxuse{\dxuse{L3.Gamma7.pub.ACCIARRI.95-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma7.pub.ACCIARRI.95-pdgref}-cite} \\
\dxuse{OPAL.Gamma7.pub.ALEXANDER.91D-vu} & \dxuse{\dxuse{OPAL.Gamma7.pub.ALEXANDER.91D-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma7.pub.ALEXANDER.91D-pdgref}-cite}%
}
\dxdef{Gamma8-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma8-gn} = \dxuse{Gamma8-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma8} \\
\dxuse{CLEO.Gamma8.pub.ANASTASSOV.97-vu} & \dxuse{\dxuse{CLEO.Gamma8.pub.ANASTASSOV.97-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma8.pub.ANASTASSOV.97-pdgref}-cite} \\
\dxuse{DELPHI.Gamma8.pub.ABDALLAH.06A-vu} & \dxuse{\dxuse{DELPHI.Gamma8.pub.ABDALLAH.06A-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma8.pub.ABDALLAH.06A-pdgref}-cite} \\
\dxuse{OPAL.Gamma8.pub.ACKERSTAFF.98M-vu} & \dxuse{\dxuse{OPAL.Gamma8.pub.ACKERSTAFF.98M-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma8.pub.ACKERSTAFF.98M-pdgref}-cite}%
}
\dxdef{Gamma8by5-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma8by5-gn} = \dxuse{Gamma8by5-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma8by5}%
}
\dxdef{Gamma9-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma9-gn} = \dxuse{Gamma9-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma9} \\
\dxuse{ALEPH.Gamma9.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma9.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma9.pub.SCHAEL.05C-pdgref}-cite}%
}
\dxdef{Gamma9by5-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma9by5-gn} = \dxuse{Gamma9by5-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma9by5} \\
\dxuse{BaBar.Gamma9by5.pub.AUBERT.10F-vu} & \dxuse{\dxuse{BaBar.Gamma9by5.pub.AUBERT.10F-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma9by5.pub.AUBERT.10F-pdgref}-cite}%
}
\dxdef{Gamma10-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma10-gn} = \dxuse{Gamma10-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma10} \\
\dxuse{ALEPH.Gamma10.pub.BARATE.99K-vu} & \dxuse{\dxuse{ALEPH.Gamma10.pub.BARATE.99K-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma10.pub.BARATE.99K-pdgref}-cite} \\
\dxuse{CLEO.Gamma10.pub.BATTLE.94-vu} & \dxuse{\dxuse{CLEO.Gamma10.pub.BATTLE.94-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma10.pub.BATTLE.94-pdgref}-cite} \\
\dxuse{DELPHI.Gamma10.pub.ABREU.94K-vu} & \dxuse{\dxuse{DELPHI.Gamma10.pub.ABREU.94K-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma10.pub.ABREU.94K-pdgref}-cite} \\
\dxuse{OPAL.Gamma10.pub.ABBIENDI.01J-vu} & \dxuse{\dxuse{OPAL.Gamma10.pub.ABBIENDI.01J-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma10.pub.ABBIENDI.01J-pdgref}-cite}%
}
\dxdef{Gamma10by5-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma10by5-gn} = \dxuse{Gamma10by5-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma10by5} \\
\dxuse{BaBar.Gamma10by5.pub.AUBERT.10F-vu} & \dxuse{\dxuse{BaBar.Gamma10by5.pub.AUBERT.10F-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma10by5.pub.AUBERT.10F-pdgref}-cite}%
}
\dxdef{Gamma10by9-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma10by9-gn} = \dxuse{Gamma10by9-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma10by9}%
}
\dxdef{Gamma11-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma11-gn} = \dxuse{Gamma11-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma11}%
}
\dxdef{Gamma12-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma12-gn} = \dxuse{Gamma12-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma12}%
}
\dxdef{Gamma13-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma13-gn} = \dxuse{Gamma13-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma13} \\
\dxuse{Belle.Gamma13.pub.FUJIKAWA.08-vu} & \dxuse{\dxuse{Belle.Gamma13.pub.FUJIKAWA.08-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma13.pub.FUJIKAWA.08-pdgref}-cite} \\
\dxuse{CLEO.Gamma13.pub.ARTUSO.94-vu} & \dxuse{\dxuse{CLEO.Gamma13.pub.ARTUSO.94-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma13.pub.ARTUSO.94-pdgref}-cite} \\
\dxuse{DELPHI.Gamma13.pub.ABDALLAH.06A-vu} & \dxuse{\dxuse{DELPHI.Gamma13.pub.ABDALLAH.06A-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma13.pub.ABDALLAH.06A-pdgref}-cite} \\
\dxuse{L3.Gamma13.pub.ACCIARRI.95-vu} & \dxuse{\dxuse{L3.Gamma13.pub.ACCIARRI.95-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma13.pub.ACCIARRI.95-pdgref}-cite} \\
\dxuse{OPAL.Gamma13.pub.ACKERSTAFF.98M-vu} & \dxuse{\dxuse{OPAL.Gamma13.pub.ACKERSTAFF.98M-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma13.pub.ACKERSTAFF.98M-pdgref}-cite}%
}
\dxdef{Gamma14-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma14-gn} = \dxuse{Gamma14-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma14} \\
\dxuse{ALEPH.Gamma14.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma14.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma14.pub.SCHAEL.05C-pdgref}-cite}%
}
\dxdef{Gamma16-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma16-gn} = \dxuse{Gamma16-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma16} \\
\dxuse{ALEPH.Gamma16.pub.BARATE.99K-vu} & \dxuse{\dxuse{ALEPH.Gamma16.pub.BARATE.99K-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma16.pub.BARATE.99K-pdgref}-cite} \\
\dxuse{BaBar.Gamma16.pub.AUBERT.07AP-vu} & \dxuse{\dxuse{BaBar.Gamma16.pub.AUBERT.07AP-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma16.pub.AUBERT.07AP-pdgref}-cite} \\
\dxuse{CLEO.Gamma16.pub.BATTLE.94-vu} & \dxuse{\dxuse{CLEO.Gamma16.pub.BATTLE.94-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma16.pub.BATTLE.94-pdgref}-cite} \\
\dxuse{OPAL.Gamma16.pub.ABBIENDI.04J-vu} & \dxuse{\dxuse{OPAL.Gamma16.pub.ABBIENDI.04J-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma16.pub.ABBIENDI.04J-pdgref}-cite}%
}
\dxdef{Gamma17-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma17-gn} = \dxuse{Gamma17-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma17} \\
\dxuse{OPAL.Gamma17.pub.ACKERSTAFF.98M-vu} & \dxuse{\dxuse{OPAL.Gamma17.pub.ACKERSTAFF.98M-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma17.pub.ACKERSTAFF.98M-pdgref}-cite}%
}
\dxdef{Gamma18-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma18-gn} = \dxuse{Gamma18-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma18}%
}
\dxdef{Gamma19-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma19-gn} = \dxuse{Gamma19-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma19} \\
\dxuse{DELPHI.Gamma19.pub.ABDALLAH.06A-vu} & \dxuse{\dxuse{DELPHI.Gamma19.pub.ABDALLAH.06A-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma19.pub.ABDALLAH.06A-pdgref}-cite} \\
\dxuse{L3.Gamma19.pub.ACCIARRI.95-vu} & \dxuse{\dxuse{L3.Gamma19.pub.ACCIARRI.95-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma19.pub.ACCIARRI.95-pdgref}-cite}%
}
\dxdef{Gamma19by13-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma19by13-gn} = \dxuse{Gamma19by13-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma19by13} \\
\dxuse{CLEO.Gamma19by13.pub.PROCARIO.93-vu} & \dxuse{\dxuse{CLEO.Gamma19by13.pub.PROCARIO.93-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma19by13.pub.PROCARIO.93-pdgref}-cite}%
}
\dxdef{Gamma20-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma20-gn} = \dxuse{Gamma20-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma20} \\
\dxuse{ALEPH.Gamma20.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma20.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma20.pub.SCHAEL.05C-pdgref}-cite}%
}
\dxdef{Gamma23-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma23-gn} = \dxuse{Gamma23-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma23} \\
\dxuse{ALEPH.Gamma23.pub.BARATE.99K-vu} & \dxuse{\dxuse{ALEPH.Gamma23.pub.BARATE.99K-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma23.pub.BARATE.99K-pdgref}-cite} \\
\dxuse{CLEO.Gamma23.pub.BATTLE.94-vu} & \dxuse{\dxuse{CLEO.Gamma23.pub.BATTLE.94-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma23.pub.BATTLE.94-pdgref}-cite}%
}
\dxdef{Gamma24-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma24-gn} = \dxuse{Gamma24-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma24}%
}
\dxdef{Gamma25-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma25-gn} = \dxuse{Gamma25-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma25} \\
\dxuse{DELPHI.Gamma25.pub.ABDALLAH.06A-vu} & \dxuse{\dxuse{DELPHI.Gamma25.pub.ABDALLAH.06A-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma25.pub.ABDALLAH.06A-pdgref}-cite}%
}
\dxdef{Gamma26-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma26-gn} = \dxuse{Gamma26-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma26} \\
\dxuse{L3.Gamma26.pub.ACCIARRI.95-vu} & \dxuse{\dxuse{L3.Gamma26.pub.ACCIARRI.95-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma26.pub.ACCIARRI.95-pdgref}-cite}%
}
\dxdef{Gamma26by13-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma26by13-gn} = \dxuse{Gamma26by13-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma26by13} \\
\dxuse{CLEO.Gamma26by13.pub.PROCARIO.93-vu} & \dxuse{\dxuse{CLEO.Gamma26by13.pub.PROCARIO.93-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma26by13.pub.PROCARIO.93-pdgref}-cite}%
}
\dxdef{Gamma27-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma27-gn} = \dxuse{Gamma27-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma27} \\
\dxuse{ALEPH.Gamma27.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma27.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma27.pub.SCHAEL.05C-pdgref}-cite}%
}
\dxdef{Gamma28-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma28-gn} = \dxuse{Gamma28-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma28} \\
\dxuse{ALEPH.Gamma28.pub.BARATE.99K-vu} & \dxuse{\dxuse{ALEPH.Gamma28.pub.BARATE.99K-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma28.pub.BARATE.99K-pdgref}-cite}%
}
\dxdef{Gamma29-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma29-gn} = \dxuse{Gamma29-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma29} \\
\dxuse{CLEO.Gamma29.pub.PROCARIO.93-vu} & \dxuse{\dxuse{CLEO.Gamma29.pub.PROCARIO.93-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma29.pub.PROCARIO.93-pdgref}-cite}%
}
\dxdef{Gamma30-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma30-gn} = \dxuse{Gamma30-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma30} \\
\dxuse{ALEPH.Gamma30.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma30.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma30.pub.SCHAEL.05C-pdgref}-cite}%
}
\dxdef{Gamma31-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma31-gn} = \dxuse{Gamma31-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma31} \\
\dxuse{CLEO.Gamma31.pub.BATTLE.94-vu} & \dxuse{\dxuse{CLEO.Gamma31.pub.BATTLE.94-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma31.pub.BATTLE.94-pdgref}-cite} \\
\dxuse{DELPHI.Gamma31.pub.ABREU.94K-vu} & \dxuse{\dxuse{DELPHI.Gamma31.pub.ABREU.94K-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma31.pub.ABREU.94K-pdgref}-cite} \\
\dxuse{OPAL.Gamma31.pub.ABBIENDI.01J-vu} & \dxuse{\dxuse{OPAL.Gamma31.pub.ABBIENDI.01J-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma31.pub.ABBIENDI.01J-pdgref}-cite}%
}
\dxdef{Gamma32-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma32-gn} = \dxuse{Gamma32-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma32}%
}
\dxdef{Gamma33-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma33-gn} = \dxuse{Gamma33-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma33} \\
\dxuse{ALEPH.Gamma33.pub.BARATE.98E-vu} & \dxuse{\dxuse{ALEPH.Gamma33.pub.BARATE.98E-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma33.pub.BARATE.98E-pdgref}-cite} \\
\dxuse{OPAL.Gamma33.pub.AKERS.94G-vu} & \dxuse{\dxuse{OPAL.Gamma33.pub.AKERS.94G-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma33.pub.AKERS.94G-pdgref}-cite}%
}
\dxdef{Gamma34-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma34-gn} = \dxuse{Gamma34-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma34} \\
\dxuse{CLEO.Gamma34.pub.COAN.96-vu} & \dxuse{\dxuse{CLEO.Gamma34.pub.COAN.96-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma34.pub.COAN.96-pdgref}-cite}%
}
\dxdef{Gamma35-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma35-gn} = \dxuse{Gamma35-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma35} \\
\dxuse{ALEPH.Gamma35.pub.BARATE.99K-vu} & \dxuse{\dxuse{ALEPH.Gamma35.pub.BARATE.99K-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma35.pub.BARATE.99K-pdgref}-cite} \\
\dxuse{Belle.Gamma35.pub.RYU.14vpc-vu} & \dxuse{\dxuse{Belle.Gamma35.pub.RYU.14vpc-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma35.pub.RYU.14vpc-pdgref}-cite} \\
\dxuse{L3.Gamma35.pub.ACCIARRI.95F-vu} & \dxuse{\dxuse{L3.Gamma35.pub.ACCIARRI.95F-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma35.pub.ACCIARRI.95F-pdgref}-cite} \\
\dxuse{OPAL.Gamma35.pub.ABBIENDI.00C-vu} & \dxuse{\dxuse{OPAL.Gamma35.pub.ABBIENDI.00C-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma35.pub.ABBIENDI.00C-pdgref}-cite}%
}
\dxdef{Gamma37-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma37-gn} = \dxuse{Gamma37-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma37} \\
\dxuse{ALEPH.Gamma37.pub.BARATE.98E-vu} & \dxuse{\dxuse{ALEPH.Gamma37.pub.BARATE.98E-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma37.pub.BARATE.98E-pdgref}-cite} \\
\dxuse{ALEPH.Gamma37.pub.BARATE.99K-vu} & \dxuse{\dxuse{ALEPH.Gamma37.pub.BARATE.99K-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma37.pub.BARATE.99K-pdgref}-cite} \\
\dxuse{BaBar.Gamma37.pub.LEES.18B-vu} & \dxuse{\dxuse{BaBar.Gamma37.pub.LEES.18B-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma37.pub.LEES.18B-pdgref}-cite} \\
\dxuse{Belle.Gamma37.pub.RYU.14vpc-vu} & \dxuse{\dxuse{Belle.Gamma37.pub.RYU.14vpc-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma37.pub.RYU.14vpc-pdgref}-cite} \\
\dxuse{CLEO.Gamma37.pub.COAN.96-vu} & \dxuse{\dxuse{CLEO.Gamma37.pub.COAN.96-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma37.pub.COAN.96-pdgref}-cite}%
}
\dxdef{Gamma38-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma38-gn} = \dxuse{Gamma38-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma38} \\
\dxuse{OPAL.Gamma38.pub.ABBIENDI.00C-vu} & \dxuse{\dxuse{OPAL.Gamma38.pub.ABBIENDI.00C-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma38.pub.ABBIENDI.00C-pdgref}-cite}%
}
\dxdef{Gamma39-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma39-gn} = \dxuse{Gamma39-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma39} \\
\dxuse{CLEO.Gamma39.pub.COAN.96-vu} & \dxuse{\dxuse{CLEO.Gamma39.pub.COAN.96-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma39.pub.COAN.96-pdgref}-cite}%
}
\dxdef{Gamma40-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma40-gn} = \dxuse{Gamma40-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma40} \\
\dxuse{ALEPH.Gamma40.pub.BARATE.98E-vu} & \dxuse{\dxuse{ALEPH.Gamma40.pub.BARATE.98E-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma40.pub.BARATE.98E-pdgref}-cite} \\
\dxuse{ALEPH.Gamma40.pub.BARATE.99K-vu} & \dxuse{\dxuse{ALEPH.Gamma40.pub.BARATE.99K-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma40.pub.BARATE.99K-pdgref}-cite} \\
\dxuse{Belle.Gamma40.pub.RYU.14vpc-vu} & \dxuse{\dxuse{Belle.Gamma40.pub.RYU.14vpc-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma40.pub.RYU.14vpc-pdgref}-cite} \\
\dxuse{L3.Gamma40.pub.ACCIARRI.95F-vu} & \dxuse{\dxuse{L3.Gamma40.pub.ACCIARRI.95F-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma40.pub.ACCIARRI.95F-pdgref}-cite}%
}
\dxdef{Gamma42-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma42-gn} = \dxuse{Gamma42-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma42} \\
\dxuse{ALEPH.Gamma42.pub.BARATE.98E-vu} & \dxuse{\dxuse{ALEPH.Gamma42.pub.BARATE.98E-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma42.pub.BARATE.98E-pdgref}-cite} \\
\dxuse{ALEPH.Gamma42.pub.BARATE.99K-vu} & \dxuse{\dxuse{ALEPH.Gamma42.pub.BARATE.99K-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma42.pub.BARATE.99K-pdgref}-cite} \\
\dxuse{Belle.Gamma42.pub.RYU.14vpc-vu} & \dxuse{\dxuse{Belle.Gamma42.pub.RYU.14vpc-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma42.pub.RYU.14vpc-pdgref}-cite} \\
\dxuse{CLEO.Gamma42.pub.COAN.96-vu} & \dxuse{\dxuse{CLEO.Gamma42.pub.COAN.96-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma42.pub.COAN.96-pdgref}-cite}%
}
\dxdef{Gamma43-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma43-gn} = \dxuse{Gamma43-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma43} \\
\dxuse{OPAL.Gamma43.pub.ABBIENDI.00C-vu} & \dxuse{\dxuse{OPAL.Gamma43.pub.ABBIENDI.00C-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma43.pub.ABBIENDI.00C-pdgref}-cite}%
}
\dxdef{Gamma44-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma44-gn} = \dxuse{Gamma44-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma44} \\
\dxuse{ALEPH.Gamma44.pub.BARATE.99R-vu} & \dxuse{\dxuse{ALEPH.Gamma44.pub.BARATE.99R-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma44.pub.BARATE.99R-pdgref}-cite}%
}
\dxdef{Gamma46-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma46-gn} = \dxuse{Gamma46-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma46}%
}
\dxdef{Gamma47-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma47-gn} = \dxuse{Gamma47-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma47} \\
\dxuse{ALEPH.Gamma47.pub.BARATE.98E-vu} & \dxuse{\dxuse{ALEPH.Gamma47.pub.BARATE.98E-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma47.pub.BARATE.98E-pdgref}-cite} \\
\dxuse{BaBar.Gamma47.pub.LEES.12Y-vu} & \dxuse{\dxuse{BaBar.Gamma47.pub.LEES.12Y-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma47.pub.LEES.12Y-pdgref}-cite} \\
\dxuse{Belle.Gamma47.pub.RYU.14vpc-vu} & \dxuse{\dxuse{Belle.Gamma47.pub.RYU.14vpc-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma47.pub.RYU.14vpc-pdgref}-cite} \\
\dxuse{CLEO.Gamma47.pub.COAN.96-vu} & \dxuse{\dxuse{CLEO.Gamma47.pub.COAN.96-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma47.pub.COAN.96-pdgref}-cite}%
}
\dxdef{Gamma48-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma48-gn} = \dxuse{Gamma48-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma48} \\
\dxuse{ALEPH.Gamma48.pub.BARATE.98E-vu} & \dxuse{\dxuse{ALEPH.Gamma48.pub.BARATE.98E-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma48.pub.BARATE.98E-pdgref}-cite}%
}
\dxdef{Gamma49-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma49-gn} = \dxuse{Gamma49-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma49}%
}
\dxdef{Gamma50-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma50-gn} = \dxuse{Gamma50-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma50} \\
\dxuse{BaBar.Gamma50.pub.LEES.12Y-vu} & \dxuse{\dxuse{BaBar.Gamma50.pub.LEES.12Y-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma50.pub.LEES.12Y-pdgref}-cite} \\
\dxuse{Belle.Gamma50.pub.RYU.14vpc-vu} & \dxuse{\dxuse{Belle.Gamma50.pub.RYU.14vpc-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma50.pub.RYU.14vpc-pdgref}-cite}%
}
\dxdef{Gamma51-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma51-gn} = \dxuse{Gamma51-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma51} \\
\dxuse{ALEPH.Gamma51.pub.BARATE.98E-vu} & \dxuse{\dxuse{ALEPH.Gamma51.pub.BARATE.98E-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma51.pub.BARATE.98E-pdgref}-cite}%
}
\dxdef{Gamma53-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma53-gn} = \dxuse{Gamma53-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma53} \\
\dxuse{ALEPH.Gamma53.pub.BARATE.98E-vu} & \dxuse{\dxuse{ALEPH.Gamma53.pub.BARATE.98E-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma53.pub.BARATE.98E-pdgref}-cite}%
}
\dxdef{Gamma54-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma54-gn} = \dxuse{Gamma54-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma54} \\
\dxuse{CELLO.Gamma54.pub.BEHREND.89B-vu} & \dxuse{\dxuse{CELLO.Gamma54.pub.BEHREND.89B-pdgref}-exp} & \dxuse{\dxuse{CELLO.Gamma54.pub.BEHREND.89B-pdgref}-cite} \\
\dxuse{L3.Gamma54.pub.ADEVA.91F-vu} & \dxuse{\dxuse{L3.Gamma54.pub.ADEVA.91F-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma54.pub.ADEVA.91F-pdgref}-cite} \\
\dxuse{TPC.Gamma54.pub.AIHARA.87B-vu} & \dxuse{\dxuse{TPC.Gamma54.pub.AIHARA.87B-pdgref}-exp} & \dxuse{\dxuse{TPC.Gamma54.pub.AIHARA.87B-pdgref}-cite}%
}
\dxdef{Gamma55-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma55-gn} = \dxuse{Gamma55-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma55} \\
\dxuse{L3.Gamma55.pub.ACHARD.01D-vu} & \dxuse{\dxuse{L3.Gamma55.pub.ACHARD.01D-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma55.pub.ACHARD.01D-pdgref}-cite} \\
\dxuse{OPAL.Gamma55.pub.AKERS.95Y-vu} & \dxuse{\dxuse{OPAL.Gamma55.pub.AKERS.95Y-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma55.pub.AKERS.95Y-pdgref}-cite}%
}
\dxdef{Gamma56-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma56-gn} = \dxuse{Gamma56-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma56}%
}
\dxdef{Gamma57-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma57-gn} = \dxuse{Gamma57-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma57} \\
\dxuse{CLEO.Gamma57.pub.BALEST.95C-vu} & \dxuse{\dxuse{CLEO.Gamma57.pub.BALEST.95C-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma57.pub.BALEST.95C-pdgref}-cite} \\
\dxuse{DELPHI.Gamma57.pub.ABDALLAH.06A-vu} & \dxuse{\dxuse{DELPHI.Gamma57.pub.ABDALLAH.06A-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma57.pub.ABDALLAH.06A-pdgref}-cite}%
}
\dxdef{Gamma57by55-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma57by55-gn} = \dxuse{Gamma57by55-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma57by55} \\
\dxuse{OPAL.Gamma57by55.pub.AKERS.95Y-vu} & \dxuse{\dxuse{OPAL.Gamma57by55.pub.AKERS.95Y-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma57by55.pub.AKERS.95Y-pdgref}-cite}%
}
\dxdef{Gamma58-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma58-gn} = \dxuse{Gamma58-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma58}%
}
\dxdef{Gamma59-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma59-gn} = \dxuse{Gamma59-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma59}%
}
\dxdef{Gamma60-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma60-gn} = \dxuse{Gamma60-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma60} \\
\dxuse{BaBar.Gamma60.pub.AUBERT.08-vu} & \dxuse{\dxuse{BaBar.Gamma60.pub.AUBERT.08-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma60.pub.AUBERT.08-pdgref}-cite} \\
\dxuse{Belle.Gamma60.pub.LEE.10-vu} & \dxuse{\dxuse{Belle.Gamma60.pub.LEE.10-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma60.pub.LEE.10-pdgref}-cite} \\
\dxuse{CLEO3.Gamma60.pub.BRIERE.03-vu} & \dxuse{\dxuse{CLEO3.Gamma60.pub.BRIERE.03-pdgref}-exp} & \dxuse{\dxuse{CLEO3.Gamma60.pub.BRIERE.03-pdgref}-cite}%
}
\dxdef{Gamma62-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma62-gn} = \dxuse{Gamma62-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma62} \\
\dxuse{ALEPH.Gamma62.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma62.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma62.pub.SCHAEL.05C-pdgref}-cite}%
}
\dxdef{Gamma63-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma63-gn} = \dxuse{Gamma63-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma63}%
}
\dxdef{Gamma64-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma64-gn} = \dxuse{Gamma64-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma64}%
}
\dxdef{Gamma65-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma65-gn} = \dxuse{Gamma65-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma65}%
}
\dxdef{Gamma66-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma66-gn} = \dxuse{Gamma66-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma66} \\
\dxuse{CLEO.Gamma66.pub.BALEST.95C-vu} & \dxuse{\dxuse{CLEO.Gamma66.pub.BALEST.95C-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma66.pub.BALEST.95C-pdgref}-cite} \\
\dxuse{DELPHI.Gamma66.pub.ABDALLAH.06A-vu} & \dxuse{\dxuse{DELPHI.Gamma66.pub.ABDALLAH.06A-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma66.pub.ABDALLAH.06A-pdgref}-cite}%
}
\dxdef{Gamma67-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma67-gn} = \dxuse{Gamma67-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma67}%
}
\dxdef{Gamma68-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma68-gn} = \dxuse{Gamma68-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma68}%
}
\dxdef{Gamma69-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma69-gn} = \dxuse{Gamma69-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma69} \\
\dxuse{ALEPH.Gamma69.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma69.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma69.pub.SCHAEL.05C-pdgref}-cite} \\
\dxuse{CLEO.Gamma69.pub.EDWARDS.00A-vu} & \dxuse{\dxuse{CLEO.Gamma69.pub.EDWARDS.00A-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma69.pub.EDWARDS.00A-pdgref}-cite}%
}
\dxdef{Gamma70-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma70-gn} = \dxuse{Gamma70-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma70}%
}
\dxdef{Gamma74-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma74-gn} = \dxuse{Gamma74-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma74} \\
\dxuse{DELPHI.Gamma74.pub.ABDALLAH.06A-vu} & \dxuse{\dxuse{DELPHI.Gamma74.pub.ABDALLAH.06A-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma74.pub.ABDALLAH.06A-pdgref}-cite}%
}
\dxdef{Gamma75-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma75-gn} = \dxuse{Gamma75-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma75}%
}
\dxdef{Gamma76-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma76-gn} = \dxuse{Gamma76-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma76} \\
\dxuse{ALEPH.Gamma76.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma76.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma76.pub.SCHAEL.05C-pdgref}-cite}%
}
\dxdef{Gamma76by54-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma76by54-gn} = \dxuse{Gamma76by54-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma76by54} \\
\dxuse{CLEO.Gamma76by54.pub.BORTOLETTO.93-vu} & \dxuse{\dxuse{CLEO.Gamma76by54.pub.BORTOLETTO.93-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma76by54.pub.BORTOLETTO.93-pdgref}-cite}%
}
\dxdef{Gamma77-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma77-gn} = \dxuse{Gamma77-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma77}%
}
\dxdef{Gamma78-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma78-gn} = \dxuse{Gamma78-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma78} \\
\dxuse{CLEO.Gamma78.pub.ANASTASSOV.01-vu} & \dxuse{\dxuse{CLEO.Gamma78.pub.ANASTASSOV.01-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma78.pub.ANASTASSOV.01-pdgref}-cite}%
}
\dxdef{Gamma79-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma79-gn} = \dxuse{Gamma79-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma79}%
}
\dxdef{Gamma80-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma80-gn} = \dxuse{Gamma80-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma80}%
}
\dxdef{Gamma80by60-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma80by60-gn} = \dxuse{Gamma80by60-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma80by60} \\
\dxuse{CLEO.Gamma80by60.pub.RICHICHI.99-vu} & \dxuse{\dxuse{CLEO.Gamma80by60.pub.RICHICHI.99-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma80by60.pub.RICHICHI.99-pdgref}-cite}%
}
\dxdef{Gamma81-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma81-gn} = \dxuse{Gamma81-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma81}%
}
\dxdef{Gamma81by69-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma81by69-gn} = \dxuse{Gamma81by69-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma81by69} \\
\dxuse{CLEO.Gamma81by69.pub.RICHICHI.99-vu} & \dxuse{\dxuse{CLEO.Gamma81by69.pub.RICHICHI.99-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma81by69.pub.RICHICHI.99-pdgref}-cite}%
}
\dxdef{Gamma82-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma82-gn} = \dxuse{Gamma82-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma82} \\
\dxuse{TPC.Gamma82.pub.BAUER.94-vu} & \dxuse{\dxuse{TPC.Gamma82.pub.BAUER.94-pdgref}-exp} & \dxuse{\dxuse{TPC.Gamma82.pub.BAUER.94-pdgref}-cite}%
}
\dxdef{Gamma83-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma83-gn} = \dxuse{Gamma83-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma83}%
}
\dxdef{Gamma84-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma84-gn} = \dxuse{Gamma84-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma84}%
}
\dxdef{Gamma85-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma85-gn} = \dxuse{Gamma85-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma85} \\
\dxuse{ALEPH.Gamma85.pub.BARATE.98-vu} & \dxuse{\dxuse{ALEPH.Gamma85.pub.BARATE.98-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma85.pub.BARATE.98-pdgref}-cite} \\
\dxuse{BaBar.Gamma85.pub.AUBERT.08-vu} & \dxuse{\dxuse{BaBar.Gamma85.pub.AUBERT.08-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma85.pub.AUBERT.08-pdgref}-cite} \\
\dxuse{Belle.Gamma85.pub.LEE.10-vu} & \dxuse{\dxuse{Belle.Gamma85.pub.LEE.10-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma85.pub.LEE.10-pdgref}-cite} \\
\dxuse{CLEO3.Gamma85.pub.BRIERE.03-vu} & \dxuse{\dxuse{CLEO3.Gamma85.pub.BRIERE.03-pdgref}-exp} & \dxuse{\dxuse{CLEO3.Gamma85.pub.BRIERE.03-pdgref}-cite} \\
\dxuse{OPAL.Gamma85.pub.ABBIENDI.04J-vu} & \dxuse{\dxuse{OPAL.Gamma85.pub.ABBIENDI.04J-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma85.pub.ABBIENDI.04J-pdgref}-cite}%
}
\dxdef{Gamma85by60-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma85by60-gn} = \dxuse{Gamma85by60-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma85by60}%
}
\dxdef{Gamma87-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma87-gn} = \dxuse{Gamma87-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma87}%
}
\dxdef{Gamma88-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma88-gn} = \dxuse{Gamma88-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma88} \\
\dxuse{ALEPH.Gamma88.pub.BARATE.98-vu} & \dxuse{\dxuse{ALEPH.Gamma88.pub.BARATE.98-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma88.pub.BARATE.98-pdgref}-cite} \\
\dxuse{CLEO3.Gamma88.pub.ARMS.05-vu} & \dxuse{\dxuse{CLEO3.Gamma88.pub.ARMS.05-pdgref}-exp} & \dxuse{\dxuse{CLEO3.Gamma88.pub.ARMS.05-pdgref}-cite}%
}
\dxdef{Gamma89-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma89-gn} = \dxuse{Gamma89-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma89}%
}
\dxdef{Gamma92-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma92-gn} = \dxuse{Gamma92-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma92} \\
\dxuse{OPAL.Gamma92.pub.ABBIENDI.00D-vu} & \dxuse{\dxuse{OPAL.Gamma92.pub.ABBIENDI.00D-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma92.pub.ABBIENDI.00D-pdgref}-cite} \\
\dxuse{TPC.Gamma92.pub.BAUER.94-vu} & \dxuse{\dxuse{TPC.Gamma92.pub.BAUER.94-pdgref}-exp} & \dxuse{\dxuse{TPC.Gamma92.pub.BAUER.94-pdgref}-cite}%
}
\dxdef{Gamma93-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma93-gn} = \dxuse{Gamma93-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma93} \\
\dxuse{ALEPH.Gamma93.pub.BARATE.98-vu} & \dxuse{\dxuse{ALEPH.Gamma93.pub.BARATE.98-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma93.pub.BARATE.98-pdgref}-cite} \\
\dxuse{BaBar.Gamma93.pub.AUBERT.08-vu} & \dxuse{\dxuse{BaBar.Gamma93.pub.AUBERT.08-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma93.pub.AUBERT.08-pdgref}-cite} \\
\dxuse{Belle.Gamma93.pub.LEE.10-vu} & \dxuse{\dxuse{Belle.Gamma93.pub.LEE.10-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma93.pub.LEE.10-pdgref}-cite} \\
\dxuse{CLEO3.Gamma93.pub.BRIERE.03-vu} & \dxuse{\dxuse{CLEO3.Gamma93.pub.BRIERE.03-pdgref}-exp} & \dxuse{\dxuse{CLEO3.Gamma93.pub.BRIERE.03-pdgref}-cite}%
}
\dxdef{Gamma93by60-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma93by60-gn} = \dxuse{Gamma93by60-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma93by60} \\
\dxuse{CLEO.Gamma93by60.pub.RICHICHI.99-vu} & \dxuse{\dxuse{CLEO.Gamma93by60.pub.RICHICHI.99-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma93by60.pub.RICHICHI.99-pdgref}-cite}%
}
\dxdef{Gamma94-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma94-gn} = \dxuse{Gamma94-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma94} \\
\dxuse{ALEPH.Gamma94.pub.BARATE.98-vu} & \dxuse{\dxuse{ALEPH.Gamma94.pub.BARATE.98-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma94.pub.BARATE.98-pdgref}-cite} \\
\dxuse{CLEO3.Gamma94.pub.ARMS.05-vu} & \dxuse{\dxuse{CLEO3.Gamma94.pub.ARMS.05-pdgref}-exp} & \dxuse{\dxuse{CLEO3.Gamma94.pub.ARMS.05-pdgref}-cite}%
}
\dxdef{Gamma94by69-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma94by69-gn} = \dxuse{Gamma94by69-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma94by69} \\
\dxuse{CLEO.Gamma94by69.pub.RICHICHI.99-vu} & \dxuse{\dxuse{CLEO.Gamma94by69.pub.RICHICHI.99-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma94by69.pub.RICHICHI.99-pdgref}-cite}%
}
\dxdef{Gamma96-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma96-gn} = \dxuse{Gamma96-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma96} \\
\dxuse{BaBar.Gamma96.pub.AUBERT.08-vu} & \dxuse{\dxuse{BaBar.Gamma96.pub.AUBERT.08-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma96.pub.AUBERT.08-pdgref}-cite} \\
\dxuse{Belle.Gamma96.pub.LEE.10-vu} & \dxuse{\dxuse{Belle.Gamma96.pub.LEE.10-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma96.pub.LEE.10-pdgref}-cite}%
}
\dxdef{Gamma102-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma102-gn} = \dxuse{Gamma102-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma102} \\
\dxuse{CLEO.Gamma102.pub.GIBAUT.94B-vu} & \dxuse{\dxuse{CLEO.Gamma102.pub.GIBAUT.94B-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma102.pub.GIBAUT.94B-pdgref}-cite} \\
\dxuse{HRS.Gamma102.pub.BYLSMA.87-vu} & \dxuse{\dxuse{HRS.Gamma102.pub.BYLSMA.87-pdgref}-exp} & \dxuse{\dxuse{HRS.Gamma102.pub.BYLSMA.87-pdgref}-cite} \\
\dxuse{L3.Gamma102.pub.ACHARD.01D-vu} & \dxuse{\dxuse{L3.Gamma102.pub.ACHARD.01D-pdgref}-exp} & \dxuse{\dxuse{L3.Gamma102.pub.ACHARD.01D-pdgref}-cite}%
}
\dxdef{Gamma103-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma103-gn} = \dxuse{Gamma103-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma103} \\
\dxuse{ALEPH.Gamma103.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma103.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma103.pub.SCHAEL.05C-pdgref}-cite} \\
\dxuse{ARGUS.Gamma103.pub.ALBRECHT.88B-vu} & \dxuse{\dxuse{ARGUS.Gamma103.pub.ALBRECHT.88B-pdgref}-exp} & \dxuse{\dxuse{ARGUS.Gamma103.pub.ALBRECHT.88B-pdgref}-cite} \\
\dxuse{CLEO.Gamma103.pub.GIBAUT.94B-vu} & \dxuse{\dxuse{CLEO.Gamma103.pub.GIBAUT.94B-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma103.pub.GIBAUT.94B-pdgref}-cite} \\
\dxuse{DELPHI.Gamma103.pub.ABDALLAH.06A-vu} & \dxuse{\dxuse{DELPHI.Gamma103.pub.ABDALLAH.06A-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma103.pub.ABDALLAH.06A-pdgref}-cite} \\
\dxuse{HRS.Gamma103.pub.BYLSMA.87-vu} & \dxuse{\dxuse{HRS.Gamma103.pub.BYLSMA.87-pdgref}-exp} & \dxuse{\dxuse{HRS.Gamma103.pub.BYLSMA.87-pdgref}-cite} \\
\dxuse{OPAL.Gamma103.pub.ACKERSTAFF.99E-vu} & \dxuse{\dxuse{OPAL.Gamma103.pub.ACKERSTAFF.99E-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma103.pub.ACKERSTAFF.99E-pdgref}-cite}%
}
\dxdef{Gamma104-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma104-gn} = \dxuse{Gamma104-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma104} \\
\dxuse{ALEPH.Gamma104.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma104.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma104.pub.SCHAEL.05C-pdgref}-cite} \\
\dxuse{CLEO.Gamma104.pub.ANASTASSOV.01-vu} & \dxuse{\dxuse{CLEO.Gamma104.pub.ANASTASSOV.01-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma104.pub.ANASTASSOV.01-pdgref}-cite} \\
\dxuse{DELPHI.Gamma104.pub.ABDALLAH.06A-vu} & \dxuse{\dxuse{DELPHI.Gamma104.pub.ABDALLAH.06A-pdgref}-exp} & \dxuse{\dxuse{DELPHI.Gamma104.pub.ABDALLAH.06A-pdgref}-cite} \\
\dxuse{OPAL.Gamma104.pub.ACKERSTAFF.99E-vu} & \dxuse{\dxuse{OPAL.Gamma104.pub.ACKERSTAFF.99E-pdgref}-exp} & \dxuse{\dxuse{OPAL.Gamma104.pub.ACKERSTAFF.99E-pdgref}-cite}%
}
\dxdef{Gamma106-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma106-gn} = \dxuse{Gamma106-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma106}%
}
\dxdef{Gamma110-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma110-gn} = \dxuse{Gamma110-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma110}%
}
\dxdef{Gamma126-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma126-gn} = \dxuse{Gamma126-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma126} \\
\dxuse{ALEPH.Gamma126.pub.BUSKULIC.97C-vu} & \dxuse{\dxuse{ALEPH.Gamma126.pub.BUSKULIC.97C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma126.pub.BUSKULIC.97C-pdgref}-cite} \\
\dxuse{Belle.Gamma126.pub.INAMI.09-vu} & \dxuse{\dxuse{Belle.Gamma126.pub.INAMI.09-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma126.pub.INAMI.09-pdgref}-cite} \\
\dxuse{CLEO.Gamma126.pub.ARTUSO.92-vu} & \dxuse{\dxuse{CLEO.Gamma126.pub.ARTUSO.92-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma126.pub.ARTUSO.92-pdgref}-cite}%
}
\dxdef{Gamma128-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma128-gn} = \dxuse{Gamma128-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma128} \\
\dxuse{ALEPH.Gamma128.pub.BUSKULIC.97C-vu} & \dxuse{\dxuse{ALEPH.Gamma128.pub.BUSKULIC.97C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma128.pub.BUSKULIC.97C-pdgref}-cite} \\
\dxuse{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E-vu} & \dxuse{\dxuse{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E-pdgref}-cite} \\
\dxuse{Belle.Gamma128.pub.INAMI.09-vu} & \dxuse{\dxuse{Belle.Gamma128.pub.INAMI.09-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma128.pub.INAMI.09-pdgref}-cite} \\
\dxuse{CLEO.Gamma128.pub.BARTELT.96-vu} & \dxuse{\dxuse{CLEO.Gamma128.pub.BARTELT.96-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma128.pub.BARTELT.96-pdgref}-cite}%
}
\dxdef{Gamma130-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma130-gn} = \dxuse{Gamma130-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma130} \\
\dxuse{Belle.Gamma130.pub.INAMI.09-vu} & \dxuse{\dxuse{Belle.Gamma130.pub.INAMI.09-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma130.pub.INAMI.09-pdgref}-cite} \\
\dxuse{CLEO.Gamma130.pub.BISHAI.99-vu} & \dxuse{\dxuse{CLEO.Gamma130.pub.BISHAI.99-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma130.pub.BISHAI.99-pdgref}-cite}%
}
\dxdef{Gamma132-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma132-gn} = \dxuse{Gamma132-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma132} \\
\dxuse{Belle.Gamma132.pub.INAMI.09-vu} & \dxuse{\dxuse{Belle.Gamma132.pub.INAMI.09-pdgref}-exp} & \dxuse{\dxuse{Belle.Gamma132.pub.INAMI.09-pdgref}-cite} \\
\dxuse{CLEO.Gamma132.pub.BISHAI.99-vu} & \dxuse{\dxuse{CLEO.Gamma132.pub.BISHAI.99-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma132.pub.BISHAI.99-pdgref}-cite}%
}
\dxdef{Gamma136-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma136-gn} = \dxuse{Gamma136-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma136}%
}
\dxdef{Gamma149-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma149-gn} = \dxuse{Gamma149-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma149}%
}
\dxdef{Gamma150-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma150-gn} = \dxuse{Gamma150-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma150} \\
\dxuse{ALEPH.Gamma150.pub.BUSKULIC.97C-vu} & \dxuse{\dxuse{ALEPH.Gamma150.pub.BUSKULIC.97C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma150.pub.BUSKULIC.97C-pdgref}-cite} \\
\dxuse{CLEO.Gamma150.pub.BARINGER.87-vu} & \dxuse{\dxuse{CLEO.Gamma150.pub.BARINGER.87-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma150.pub.BARINGER.87-pdgref}-cite}%
}
\dxdef{Gamma150by66-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma150by66-gn} = \dxuse{Gamma150by66-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma150by66} \\
\dxuse{ALEPH.Gamma150by66.pub.BUSKULIC.96-vu} & \dxuse{\dxuse{ALEPH.Gamma150by66.pub.BUSKULIC.96-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma150by66.pub.BUSKULIC.96-pdgref}-cite} \\
\dxuse{CLEO.Gamma150by66.pub.BALEST.95C-vu} & \dxuse{\dxuse{CLEO.Gamma150by66.pub.BALEST.95C-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma150by66.pub.BALEST.95C-pdgref}-cite}%
}
\dxdef{Gamma151-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma151-gn} = \dxuse{Gamma151-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma151} \\
\dxuse{CLEO3.Gamma151.pub.ARMS.05-vu} & \dxuse{\dxuse{CLEO3.Gamma151.pub.ARMS.05-pdgref}-exp} & \dxuse{\dxuse{CLEO3.Gamma151.pub.ARMS.05-pdgref}-cite}%
}
\dxdef{Gamma152-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma152-gn} = \dxuse{Gamma152-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma152} \\
\dxuse{ALEPH.Gamma152.pub.BUSKULIC.97C-vu} & \dxuse{\dxuse{ALEPH.Gamma152.pub.BUSKULIC.97C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma152.pub.BUSKULIC.97C-pdgref}-cite}%
}
\dxdef{Gamma152by54-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma152by54-gn} = \dxuse{Gamma152by54-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma152by54}%
}
\dxdef{Gamma152by76-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma152by76-gn} = \dxuse{Gamma152by76-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma152by76} \\
\dxuse{CLEO.Gamma152by76.pub.BORTOLETTO.93-vu} & \dxuse{\dxuse{CLEO.Gamma152by76.pub.BORTOLETTO.93-pdgref}-exp} & \dxuse{\dxuse{CLEO.Gamma152by76.pub.BORTOLETTO.93-pdgref}-cite}%
}
\dxdef{Gamma167-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma167-gn} = \dxuse{Gamma167-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma167}%
}
\dxdef{Gamma168-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma168-gn} = \dxuse{Gamma168-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma168}%
}
\dxdef{Gamma169-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma169-gn} = \dxuse{Gamma169-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma169}%
}
\dxdef{Gamma800-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma800-gn} = \dxuse{Gamma800-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma800}%
}
\dxdef{Gamma802-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma802-gn} = \dxuse{Gamma802-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma802}%
}
\dxdef{Gamma803-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma803-gn} = \dxuse{Gamma803-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma803}%
}
\dxdef{Gamma804-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma804-gn} = \dxuse{Gamma804-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma804}%
}
\dxdef{Gamma805-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma805-gn} = \dxuse{Gamma805-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma805}%
}
\dxdef{Gamma806-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma806-gn} = \dxuse{Gamma806-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma806}%
}
\dxdef{Gamma810-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma810-gn} = \dxuse{Gamma810-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma810}%
}
\dxdef{Gamma811-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma811-gn} = \dxuse{Gamma811-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma811} \\
\dxuse{BaBar.Gamma811.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma811.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma811.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma812-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma812-gn} = \dxuse{Gamma812-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma812} \\
\dxuse{BaBar.Gamma812.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma812.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma812.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma820-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma820-gn} = \dxuse{Gamma820-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma820}%
}
\dxdef{Gamma821-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma821-gn} = \dxuse{Gamma821-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma821} \\
\dxuse{BaBar.Gamma821.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma821.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma821.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma822-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma822-gn} = \dxuse{Gamma822-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma822} \\
\dxuse{BaBar.Gamma822.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma822.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma822.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma830-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma830-gn} = \dxuse{Gamma830-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma830}%
}
\dxdef{Gamma831-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma831-gn} = \dxuse{Gamma831-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma831} \\
\dxuse{BaBar.Gamma831.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma831.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma831.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma832-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma832-gn} = \dxuse{Gamma832-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma832} \\
\dxuse{BaBar.Gamma832.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma832.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma832.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma833-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma833-gn} = \dxuse{Gamma833-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma833} \\
\dxuse{BaBar.Gamma833.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma833.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma833.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma910-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma910-gn} = \dxuse{Gamma910-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma910} \\
\dxuse{BaBar.Gamma910.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma910.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma910.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma911-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma911-gn} = \dxuse{Gamma911-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma911} \\
\dxuse{BaBar.Gamma911.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma911.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma911.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma920-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma920-gn} = \dxuse{Gamma920-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma920} \\
\dxuse{BaBar.Gamma920.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma920.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma920.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma930-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma930-gn} = \dxuse{Gamma930-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma930} \\
\dxuse{BaBar.Gamma930.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma930.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma930.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma944-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma944-gn} = \dxuse{Gamma944-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma944} \\
\dxuse{BaBar.Gamma944.pub.LEES.12X-vu} & \dxuse{\dxuse{BaBar.Gamma944.pub.LEES.12X-pdgref}-exp} & \dxuse{\dxuse{BaBar.Gamma944.pub.LEES.12X-pdgref}-cite}%
}
\dxdef{Gamma945-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma945-gn} = \dxuse{Gamma945-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma945}%
}
\dxdef{GammaUnitResid-qm}{%
\begin{ensuredisplaymath}
\dxuse{GammaUnitResid-gn} = \dxuse{GammaUnitResid-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{GammaUnitResid}%
}
\dxdef{GammaAll-qm}{%
\begin{ensuredisplaymath}
\dxuse{GammaAll-gn} = \dxuse{GammaAll-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{GammaAll}%
}
\dxdef{Gamma980-qm}{%
\begin{ensuredisplaymath}
\dxuse{Gamma980-gn} = \dxuse{Gamma980-td}
\end{ensuredisplaymath} & & \\
\dxQuantMeasLine{Gamma980} \\
\dxuse{ALEPH.Gamma980.pub.SCHAEL.05C-vu} & \dxuse{\dxuse{ALEPH.Gamma980.pub.SCHAEL.05C-pdgref}-exp} & \dxuse{\dxuse{ALEPH.Gamma980.pub.SCHAEL.05C-pdgref}-cite}%
}
\dxdef{TauBrVarMeasTable}{%
\dxuse{Gamma1-qm} \\[1.5ex]
\dxuse{Gamma2-qm} \\[1.5ex]
\dxuse{Gamma3-qm} \\[1.5ex]
\dxuse{Gamma3by5-qm} \\[1.5ex]
\dxuse{Gamma5-qm} \\[1.5ex]
\dxuse{Gamma7-qm} \\[1.5ex]
\dxuse{Gamma8-qm} \\[1.5ex]
\dxuse{Gamma8by5-qm} \\[1.5ex]
\dxuse{Gamma9-qm} \\[1.5ex]
\dxuse{Gamma9by5-qm} \\[1.5ex]
\dxuse{Gamma10-qm} \\[1.5ex]
\dxuse{Gamma10by5-qm} \\[1.5ex]
\dxuse{Gamma10by9-qm} \\[1.5ex]
\dxuse{Gamma11-qm} \\[1.5ex]
\dxuse{Gamma12-qm} \\[1.5ex]
\dxuse{Gamma13-qm} \\[1.5ex]
\dxuse{Gamma14-qm} \\[1.5ex]
\dxuse{Gamma16-qm} \\[1.5ex]
\dxuse{Gamma17-qm} \\[1.5ex]
\dxuse{Gamma18-qm} \\[1.5ex]
\dxuse{Gamma19-qm} \\[1.5ex]
\dxuse{Gamma19by13-qm} \\[1.5ex]
\dxuse{Gamma20-qm} \\[1.5ex]
\dxuse{Gamma23-qm} \\[1.5ex]
\dxuse{Gamma24-qm} \\[1.5ex]
\dxuse{Gamma25-qm} \\[1.5ex]
\dxuse{Gamma26-qm} \\[1.5ex]
\dxuse{Gamma26by13-qm} \\[1.5ex]
\dxuse{Gamma27-qm} \\[1.5ex]
\dxuse{Gamma28-qm} \\[1.5ex]
\dxuse{Gamma29-qm} \\[1.5ex]
\dxuse{Gamma30-qm} \\[1.5ex]
\dxuse{Gamma31-qm} \\[1.5ex]
\dxuse{Gamma32-qm} \\[1.5ex]
\dxuse{Gamma33-qm} \\[1.5ex]
\dxuse{Gamma34-qm} \\[1.5ex]
\dxuse{Gamma35-qm} \\[1.5ex]
\dxuse{Gamma37-qm} \\[1.5ex]
\dxuse{Gamma38-qm} \\[1.5ex]
\dxuse{Gamma39-qm} \\[1.5ex]
\dxuse{Gamma40-qm} \\[1.5ex]
\dxuse{Gamma42-qm} \\[1.5ex]
\dxuse{Gamma43-qm} \\[1.5ex]
\dxuse{Gamma44-qm} \\[1.5ex]
\dxuse{Gamma46-qm} \\[1.5ex]
\dxuse{Gamma47-qm} \\[1.5ex]
\dxuse{Gamma48-qm} \\[1.5ex]
\dxuse{Gamma49-qm} \\[1.5ex]
\dxuse{Gamma50-qm} \\[1.5ex]
\dxuse{Gamma51-qm} \\[1.5ex]
\dxuse{Gamma53-qm} \\[1.5ex]
\dxuse{Gamma54-qm} \\[1.5ex]
\dxuse{Gamma55-qm} \\[1.5ex]
\dxuse{Gamma56-qm} \\[1.5ex]
\dxuse{Gamma57-qm} \\[1.5ex]
\dxuse{Gamma57by55-qm} \\[1.5ex]
\dxuse{Gamma58-qm} \\[1.5ex]
\dxuse{Gamma59-qm} \\[1.5ex]
\dxuse{Gamma60-qm} \\[1.5ex]
\dxuse{Gamma62-qm} \\[1.5ex]
\dxuse{Gamma63-qm} \\[1.5ex]
\dxuse{Gamma64-qm} \\[1.5ex]
\dxuse{Gamma65-qm} \\[1.5ex]
\dxuse{Gamma66-qm} \\[1.5ex]
\dxuse{Gamma67-qm} \\[1.5ex]
\dxuse{Gamma68-qm} \\[1.5ex]
\dxuse{Gamma69-qm} \\[1.5ex]
\dxuse{Gamma70-qm} \\[1.5ex]
\dxuse{Gamma74-qm} \\[1.5ex]
\dxuse{Gamma75-qm} \\[1.5ex]
\dxuse{Gamma76-qm} \\[1.5ex]
\dxuse{Gamma76by54-qm} \\[1.5ex]
\dxuse{Gamma77-qm} \\[1.5ex]
\dxuse{Gamma78-qm} \\[1.5ex]
\dxuse{Gamma79-qm} \\[1.5ex]
\dxuse{Gamma80-qm} \\[1.5ex]
\dxuse{Gamma80by60-qm} \\[1.5ex]
\dxuse{Gamma81-qm} \\[1.5ex]
\dxuse{Gamma81by69-qm} \\[1.5ex]
\dxuse{Gamma82-qm} \\[1.5ex]
\dxuse{Gamma83-qm} \\[1.5ex]
\dxuse{Gamma84-qm} \\[1.5ex]
\dxuse{Gamma85-qm} \\[1.5ex]
\dxuse{Gamma85by60-qm} \\[1.5ex]
\dxuse{Gamma87-qm} \\[1.5ex]
\dxuse{Gamma88-qm} \\[1.5ex]
\dxuse{Gamma89-qm} \\[1.5ex]
\dxuse{Gamma92-qm} \\[1.5ex]
\dxuse{Gamma93-qm} \\[1.5ex]
\dxuse{Gamma93by60-qm} \\[1.5ex]
\dxuse{Gamma94-qm} \\[1.5ex]
\dxuse{Gamma94by69-qm} \\[1.5ex]
\dxuse{Gamma96-qm} \\[1.5ex]
\dxuse{Gamma102-qm} \\[1.5ex]
\dxuse{Gamma103-qm} \\[1.5ex]
\dxuse{Gamma104-qm} \\[1.5ex]
\dxuse{Gamma106-qm} \\[1.5ex]
\dxuse{Gamma110-qm} \\[1.5ex]
\dxuse{Gamma126-qm} \\[1.5ex]
\dxuse{Gamma128-qm} \\[1.5ex]
\dxuse{Gamma130-qm} \\[1.5ex]
\dxuse{Gamma132-qm} \\[1.5ex]
\dxuse{Gamma136-qm} \\[1.5ex]
\dxuse{Gamma149-qm} \\[1.5ex]
\dxuse{Gamma150-qm} \\[1.5ex]
\dxuse{Gamma150by66-qm} \\[1.5ex]
\dxuse{Gamma151-qm} \\[1.5ex]
\dxuse{Gamma152-qm} \\[1.5ex]
\dxuse{Gamma152by54-qm} \\[1.5ex]
\dxuse{Gamma152by76-qm} \\[1.5ex]
\dxuse{Gamma167-qm} \\[1.5ex]
\dxuse{Gamma168-qm} \\[1.5ex]
\dxuse{Gamma169-qm} \\[1.5ex]
\dxuse{Gamma800-qm} \\[1.5ex]
\dxuse{Gamma802-qm} \\[1.5ex]
\dxuse{Gamma803-qm} \\[1.5ex]
\dxuse{Gamma804-qm} \\[1.5ex]
\dxuse{Gamma805-qm} \\[1.5ex]
\dxuse{Gamma806-qm} \\[1.5ex]
\dxuse{Gamma810-qm} \\[1.5ex]
\dxuse{Gamma811-qm} \\[1.5ex]
\dxuse{Gamma812-qm} \\[1.5ex]
\dxuse{Gamma820-qm} \\[1.5ex]
\dxuse{Gamma821-qm} \\[1.5ex]
\dxuse{Gamma822-qm} \\[1.5ex]
\dxuse{Gamma830-qm} \\[1.5ex]
\dxuse{Gamma831-qm} \\[1.5ex]
\dxuse{Gamma832-qm} \\[1.5ex]
\dxuse{Gamma833-qm} \\[1.5ex]
\dxuse{Gamma910-qm} \\[1.5ex]
\dxuse{Gamma911-qm} \\[1.5ex]
\dxuse{Gamma920-qm} \\[1.5ex]
\dxuse{Gamma930-qm} \\[1.5ex]
\dxuse{Gamma944-qm} \\[1.5ex]
\dxuse{Gamma945-qm} \\[1.5ex]
\dxuse{GammaUnitResid-qm} \\[1.5ex]
\dxuse{GammaAll-qm}%
}
\dxdef{TauBrNuisMeasTable}{%
\dxuse{Gamma980-qm}%
}
\dxdef{BARATE 98-ref}{Barate:1997ma}
\dxdef{BARATE 98-cite}{\cite{Barate:1997ma}}
\dxdef{BARATE 98-exp}{ALEPH}
\dxdef{BARATE 98-type}{pub}
\dxdef{BARATE 98-label}{BARATE 98 (ALEPH)}
\dxdef{BARATE 98-meas}{%
\multicolumn{2}{l}{\dxuse{BARATE 98-label}\,\dxuse{BARATE 98-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma85-gn} = \dxuse{Gamma85-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma85.pub.BARATE.98-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma88-gn} = \dxuse{Gamma88-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma88.pub.BARATE.98-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma93-gn} = \dxuse{Gamma93-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma93.pub.BARATE.98-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma94-gn} = \dxuse{Gamma94-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma94.pub.BARATE.98-vu}%
}
\dxdef{BARATE 98E-ref}{Barate:1997tt}
\dxdef{BARATE 98E-cite}{\cite{Barate:1997tt}}
\dxdef{BARATE 98E-exp}{ALEPH}
\dxdef{BARATE 98E-type}{pub}
\dxdef{BARATE 98E-label}{BARATE 98E (ALEPH)}
\dxdef{BARATE 98E-meas}{%
\multicolumn{2}{l}{\dxuse{BARATE 98E-label}\,\dxuse{BARATE 98E-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma33-gn} = \dxuse{Gamma33-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma33.pub.BARATE.98E-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma37-gn} = \dxuse{Gamma37-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma37.pub.BARATE.98E-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma40-gn} = \dxuse{Gamma40-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma40.pub.BARATE.98E-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma42-gn} = \dxuse{Gamma42-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma42.pub.BARATE.98E-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma47-gn} = \dxuse{Gamma47-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma47.pub.BARATE.98E-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma48-gn} = \dxuse{Gamma48-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma48.pub.BARATE.98E-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma51-gn} = \dxuse{Gamma51-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma51.pub.BARATE.98E-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma53-gn} = \dxuse{Gamma53-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma53.pub.BARATE.98E-vu}%
}
\dxdef{BARATE 99K-ref}{Barate:1999hi}
\dxdef{BARATE 99K-cite}{\cite{Barate:1999hi}}
\dxdef{BARATE 99K-exp}{ALEPH}
\dxdef{BARATE 99K-type}{pub}
\dxdef{BARATE 99K-label}{BARATE 99K (ALEPH)}
\dxdef{BARATE 99K-meas}{%
\multicolumn{2}{l}{\dxuse{BARATE 99K-label}\,\dxuse{BARATE 99K-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma10-gn} = \dxuse{Gamma10-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma10.pub.BARATE.99K-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma16-gn} = \dxuse{Gamma16-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma16.pub.BARATE.99K-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma23-gn} = \dxuse{Gamma23-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma23.pub.BARATE.99K-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma28-gn} = \dxuse{Gamma28-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma28.pub.BARATE.99K-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma35-gn} = \dxuse{Gamma35-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma35.pub.BARATE.99K-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma37-gn} = \dxuse{Gamma37-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma37.pub.BARATE.99K-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma40-gn} = \dxuse{Gamma40-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma40.pub.BARATE.99K-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma42-gn} = \dxuse{Gamma42-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma42.pub.BARATE.99K-vu}%
}
\dxdef{BARATE 99R-ref}{Barate:1999hj}
\dxdef{BARATE 99R-cite}{\cite{Barate:1999hj}}
\dxdef{BARATE 99R-exp}{ALEPH}
\dxdef{BARATE 99R-type}{pub}
\dxdef{BARATE 99R-label}{BARATE 99R (ALEPH)}
\dxdef{BARATE 99R-meas}{%
\multicolumn{2}{l}{\dxuse{BARATE 99R-label}\,\dxuse{BARATE 99R-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma44-gn} = \dxuse{Gamma44-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma44.pub.BARATE.99R-vu}%
}
\dxdef{BUSKULIC 96-ref}{Buskulic:1995ty}
\dxdef{BUSKULIC 96-cite}{\cite{Buskulic:1995ty}}
\dxdef{BUSKULIC 96-exp}{ALEPH}
\dxdef{BUSKULIC 96-type}{pub}
\dxdef{BUSKULIC 96-label}{BUSKULIC 96 (ALEPH)}
\dxdef{BUSKULIC 96-meas}{%
\multicolumn{2}{l}{\dxuse{BUSKULIC 96-label}\,\dxuse{BUSKULIC 96-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma150by66-gn} = \dxuse{Gamma150by66-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma150by66.pub.BUSKULIC.96-vu}%
}
\dxdef{BUSKULIC 97C-ref}{Buskulic:1996qs}
\dxdef{BUSKULIC 97C-cite}{\cite{Buskulic:1996qs}}
\dxdef{BUSKULIC 97C-exp}{ALEPH}
\dxdef{BUSKULIC 97C-type}{pub}
\dxdef{BUSKULIC 97C-label}{BUSKULIC 97C (ALEPH)}
\dxdef{BUSKULIC 97C-meas}{%
\multicolumn{2}{l}{\dxuse{BUSKULIC 97C-label}\,\dxuse{BUSKULIC 97C-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma126-gn} = \dxuse{Gamma126-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma126.pub.BUSKULIC.97C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma128-gn} = \dxuse{Gamma128-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma128.pub.BUSKULIC.97C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma150-gn} = \dxuse{Gamma150-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma150.pub.BUSKULIC.97C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma152-gn} = \dxuse{Gamma152-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma152.pub.BUSKULIC.97C-vu}%
}
\dxdef{SCHAEL 05C-ref}{Schael:2005am}
\dxdef{SCHAEL 05C-cite}{\cite{Schael:2005am}}
\dxdef{SCHAEL 05C-exp}{ALEPH}
\dxdef{SCHAEL 05C-type}{pub}
\dxdef{SCHAEL 05C-label}{SCHAEL 05C (ALEPH)}
\dxdef{SCHAEL 05C-meas}{%
\multicolumn{2}{l}{\dxuse{SCHAEL 05C-label}\,\dxuse{SCHAEL 05C-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma3-gn} = \dxuse{Gamma3-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma3.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma5-gn} = \dxuse{Gamma5-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma5.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma9-gn} = \dxuse{Gamma9-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma9.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma14-gn} = \dxuse{Gamma14-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma14.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma20-gn} = \dxuse{Gamma20-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma20.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma27-gn} = \dxuse{Gamma27-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma27.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma30-gn} = \dxuse{Gamma30-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma30.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma62-gn} = \dxuse{Gamma62-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma62.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma69-gn} = \dxuse{Gamma69-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma69.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma76-gn} = \dxuse{Gamma76-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma76.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma103-gn} = \dxuse{Gamma103-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma103.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma104-gn} = \dxuse{Gamma104-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma104.pub.SCHAEL.05C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma980-gn} = \dxuse{Gamma980-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.Gamma980.pub.SCHAEL.05C-vu}%
}
\dxdef{ALBRECHT 88B-ref}{Albrecht:1987zf}
\dxdef{ALBRECHT 88B-cite}{\cite{Albrecht:1987zf}}
\dxdef{ALBRECHT 88B-exp}{ARGUS}
\dxdef{ALBRECHT 88B-type}{pub}
\dxdef{ALBRECHT 88B-label}{ALBRECHT 88B (ARGUS)}
\dxdef{ALBRECHT 88B-meas}{%
\multicolumn{2}{l}{\dxuse{ALBRECHT 88B-label}\,\dxuse{ALBRECHT 88B-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma103-gn} = \dxuse{Gamma103-td}
\end{ensuredisplaymath} & \dxuse{ARGUS.Gamma103.pub.ALBRECHT.88B-vu}%
}
\dxdef{ALBRECHT 92D-ref}{Albrecht:1991rh}
\dxdef{ALBRECHT 92D-cite}{\cite{Albrecht:1991rh}}
\dxdef{ALBRECHT 92D-exp}{ARGUS}
\dxdef{ALBRECHT 92D-type}{pub}
\dxdef{ALBRECHT 92D-label}{ALBRECHT 92D (ARGUS)}
\dxdef{ALBRECHT 92D-meas}{%
\multicolumn{2}{l}{\dxuse{ALBRECHT 92D-label}\,\dxuse{ALBRECHT 92D-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma3by5-gn} = \dxuse{Gamma3by5-td}
\end{ensuredisplaymath} & \dxuse{ARGUS.Gamma3by5.pub.ALBRECHT.92D-vu}%
}
\dxdef{AUBERT 07AP-ref}{Aubert:2007jh}
\dxdef{AUBERT 07AP-cite}{\cite{Aubert:2007jh}}
\dxdef{AUBERT 07AP-exp}{\babar}
\dxdef{AUBERT 07AP-type}{pub}
\dxdef{AUBERT 07AP-label}{AUBERT 07AP (\babar)}
\dxdef{AUBERT 07AP-meas}{%
\multicolumn{2}{l}{\dxuse{AUBERT 07AP-label}\,\dxuse{AUBERT 07AP-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma16-gn} = \dxuse{Gamma16-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma16.pub.AUBERT.07AP-vu}%
}
\dxdef{AUBERT 08-ref}{Aubert:2007mh}
\dxdef{AUBERT 08-cite}{\cite{Aubert:2007mh}}
\dxdef{AUBERT 08-exp}{\babar}
\dxdef{AUBERT 08-type}{pub}
\dxdef{AUBERT 08-label}{AUBERT 08 (\babar)}
\dxdef{AUBERT 08-meas}{%
\multicolumn{2}{l}{\dxuse{AUBERT 08-label}\,\dxuse{AUBERT 08-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma60-gn} = \dxuse{Gamma60-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma60.pub.AUBERT.08-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma85-gn} = \dxuse{Gamma85-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma85.pub.AUBERT.08-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma93-gn} = \dxuse{Gamma93-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma93.pub.AUBERT.08-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma96-gn} = \dxuse{Gamma96-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma96.pub.AUBERT.08-vu}%
}
\dxdef{AUBERT 10F-ref}{Aubert:2009qj}
\dxdef{AUBERT 10F-cite}{\cite{Aubert:2009qj}}
\dxdef{AUBERT 10F-exp}{\babar}
\dxdef{AUBERT 10F-type}{pub}
\dxdef{AUBERT 10F-label}{AUBERT 10F (\babar)}
\dxdef{AUBERT 10F-meas}{%
\multicolumn{2}{l}{\dxuse{AUBERT 10F-label}\,\dxuse{AUBERT 10F-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma3by5-gn} = \dxuse{Gamma3by5-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma3by5.pub.AUBERT.10F-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma9by5-gn} = \dxuse{Gamma9by5-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma9by5.pub.AUBERT.10F-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma10by5-gn} = \dxuse{Gamma10by5-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma10by5.pub.AUBERT.10F-vu}%
}
\dxdef{DEL-AMO-SANCHEZ 11E-ref}{delAmoSanchez:2010pc}
\dxdef{DEL-AMO-SANCHEZ 11E-cite}{\cite{delAmoSanchez:2010pc}}
\dxdef{DEL-AMO-SANCHEZ 11E-exp}{\babar}
\dxdef{DEL-AMO-SANCHEZ 11E-type}{pub}
\dxdef{DEL-AMO-SANCHEZ 11E-label}{DEL-AMO-SANCHEZ 11E (\babar)}
\dxdef{DEL-AMO-SANCHEZ 11E-meas}{%
\multicolumn{2}{l}{\dxuse{DEL-AMO-SANCHEZ 11E-label}\,\dxuse{DEL-AMO-SANCHEZ 11E-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma128-gn} = \dxuse{Gamma128-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E-vu}%
}
\dxdef{LEES 12X-ref}{Lees:2012ks}
\dxdef{LEES 12X-cite}{\cite{Lees:2012ks}}
\dxdef{LEES 12X-exp}{\babar}
\dxdef{LEES 12X-type}{pub}
\dxdef{LEES 12X-label}{LEES 12X (\babar)}
\dxdef{LEES 12X-meas}{%
\multicolumn{2}{l}{\dxuse{LEES 12X-label}\,\dxuse{LEES 12X-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma811-gn} = \dxuse{Gamma811-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma811.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma812-gn} = \dxuse{Gamma812-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma812.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma821-gn} = \dxuse{Gamma821-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma821.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma822-gn} = \dxuse{Gamma822-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma822.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma831-gn} = \dxuse{Gamma831-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma831.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma832-gn} = \dxuse{Gamma832-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma832.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma833-gn} = \dxuse{Gamma833-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma833.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma910-gn} = \dxuse{Gamma910-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma910.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma911-gn} = \dxuse{Gamma911-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma911.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma920-gn} = \dxuse{Gamma920-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma920.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma930-gn} = \dxuse{Gamma930-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma930.pub.LEES.12X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma944-gn} = \dxuse{Gamma944-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma944.pub.LEES.12X-vu}%
}
\dxdef{LEES 12Y-ref}{Lees:2012de}
\dxdef{LEES 12Y-cite}{\cite{Lees:2012de}}
\dxdef{LEES 12Y-exp}{\babar}
\dxdef{LEES 12Y-type}{pub}
\dxdef{LEES 12Y-label}{LEES 12Y (\babar)}
\dxdef{LEES 12Y-meas}{%
\multicolumn{2}{l}{\dxuse{LEES 12Y-label}\,\dxuse{LEES 12Y-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma47-gn} = \dxuse{Gamma47-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma47.pub.LEES.12Y-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma50-gn} = \dxuse{Gamma50-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma50.pub.LEES.12Y-vu}%
}
\dxdef{LEES 18B-ref}{BaBar:2018qry}
\dxdef{LEES 18B-cite}{\cite{BaBar:2018qry}}
\dxdef{LEES 18B-exp}{\babar}
\dxdef{LEES 18B-type}{pub}
\dxdef{LEES 18B-label}{LEES 18B (\babar)}
\dxdef{LEES 18B-meas}{%
\multicolumn{2}{l}{\dxuse{LEES 18B-label}\,\dxuse{LEES 18B-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma37-gn} = \dxuse{Gamma37-td}
\end{ensuredisplaymath} & \dxuse{BaBar.Gamma37.pub.LEES.18B-vu}%
}
\dxdef{FUJIKAWA 08-ref}{Fujikawa:2008ma}
\dxdef{FUJIKAWA 08-cite}{\cite{Fujikawa:2008ma}}
\dxdef{FUJIKAWA 08-exp}{Belle}
\dxdef{FUJIKAWA 08-type}{pub}
\dxdef{FUJIKAWA 08-label}{FUJIKAWA 08 (Belle)}
\dxdef{FUJIKAWA 08-meas}{%
\multicolumn{2}{l}{\dxuse{FUJIKAWA 08-label}\,\dxuse{FUJIKAWA 08-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma13-gn} = \dxuse{Gamma13-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma13.pub.FUJIKAWA.08-vu}%
}
\dxdef{INAMI 09-ref}{Inami:2008ar}
\dxdef{INAMI 09-cite}{\cite{Inami:2008ar}}
\dxdef{INAMI 09-exp}{Belle}
\dxdef{INAMI 09-type}{pub}
\dxdef{INAMI 09-label}{INAMI 09 (Belle)}
\dxdef{INAMI 09-meas}{%
\multicolumn{2}{l}{\dxuse{INAMI 09-label}\,\dxuse{INAMI 09-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma126-gn} = \dxuse{Gamma126-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma126.pub.INAMI.09-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma128-gn} = \dxuse{Gamma128-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma128.pub.INAMI.09-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma130-gn} = \dxuse{Gamma130-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma130.pub.INAMI.09-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma132-gn} = \dxuse{Gamma132-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma132.pub.INAMI.09-vu}%
}
\dxdef{LEE 10-ref}{Lee:2010tc}
\dxdef{LEE 10-cite}{\cite{Lee:2010tc}}
\dxdef{LEE 10-exp}{Belle}
\dxdef{LEE 10-type}{pub}
\dxdef{LEE 10-label}{LEE 10 (Belle)}
\dxdef{LEE 10-meas}{%
\multicolumn{2}{l}{\dxuse{LEE 10-label}\,\dxuse{LEE 10-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma60-gn} = \dxuse{Gamma60-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma60.pub.LEE.10-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma85-gn} = \dxuse{Gamma85-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma85.pub.LEE.10-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma93-gn} = \dxuse{Gamma93-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma93.pub.LEE.10-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma96-gn} = \dxuse{Gamma96-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma96.pub.LEE.10-vu}%
}
\dxdef{RYU 14vpc-ref}{Ryu:2014vpc}
\dxdef{RYU 14vpc-cite}{\cite{Ryu:2014vpc}}
\dxdef{RYU 14vpc-exp}{Belle}
\dxdef{RYU 14vpc-type}{pub}
\dxdef{RYU 14vpc-label}{RYU 14vpc (Belle)}
\dxdef{RYU 14vpc-meas}{%
\multicolumn{2}{l}{\dxuse{RYU 14vpc-label}\,\dxuse{RYU 14vpc-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma35-gn} = \dxuse{Gamma35-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma35.pub.RYU.14vpc-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma37-gn} = \dxuse{Gamma37-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma37.pub.RYU.14vpc-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma40-gn} = \dxuse{Gamma40-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma40.pub.RYU.14vpc-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma42-gn} = \dxuse{Gamma42-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma42.pub.RYU.14vpc-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma47-gn} = \dxuse{Gamma47-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma47.pub.RYU.14vpc-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma50-gn} = \dxuse{Gamma50-td}
\end{ensuredisplaymath} & \dxuse{Belle.Gamma50.pub.RYU.14vpc-vu}%
}
\dxdef{Belle2 ADACHI 2024-ref}{Belle-II:2024vvr}
\dxdef{Belle2 ADACHI 2024-cite}{\cite{Belle-II:2024vvr}}
\dxdef{Belle2 ADACHI 2024-exp}{Belle\,II}
\dxdef{Belle2 ADACHI 2024-type}{ADACHI}
\dxdef{Belle2 ADACHI 2024-label}{Belle\,II ADACHI 2024}
\dxdef{Belle2 ADACHI 2024-meas}{%
\multicolumn{2}{l}{\dxuse{Belle2 ADACHI 2024-label}\,\dxuse{Belle2 ADACHI 2024-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma3by5-gn} = \dxuse{Gamma3by5-td}
\end{ensuredisplaymath} & \dxuse{Belle2.Gamma3by5.ADACHI.2024-vu}%
}
\dxdef{BEHREND 89B-ref}{Behrend:1989wc}
\dxdef{BEHREND 89B-cite}{\cite{Behrend:1989wc}}
\dxdef{BEHREND 89B-exp}{CELLO}
\dxdef{BEHREND 89B-type}{pub}
\dxdef{BEHREND 89B-label}{BEHREND 89B (CELLO)}
\dxdef{BEHREND 89B-meas}{%
\multicolumn{2}{l}{\dxuse{BEHREND 89B-label}\,\dxuse{BEHREND 89B-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma54-gn} = \dxuse{Gamma54-td}
\end{ensuredisplaymath} & \dxuse{CELLO.Gamma54.pub.BEHREND.89B-vu}%
}
\dxdef{ANASTASSOV 01-ref}{Anastassov:2000xu}
\dxdef{ANASTASSOV 01-cite}{\cite{Anastassov:2000xu}}
\dxdef{ANASTASSOV 01-exp}{CLEO}
\dxdef{ANASTASSOV 01-type}{pub}
\dxdef{ANASTASSOV 01-label}{ANASTASSOV 01 (CLEO)}
\dxdef{ANASTASSOV 01-meas}{%
\multicolumn{2}{l}{\dxuse{ANASTASSOV 01-label}\,\dxuse{ANASTASSOV 01-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma78-gn} = \dxuse{Gamma78-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma78.pub.ANASTASSOV.01-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma104-gn} = \dxuse{Gamma104-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma104.pub.ANASTASSOV.01-vu}%
}
\dxdef{ANASTASSOV 97-ref}{CLEO:1996oro}
\dxdef{ANASTASSOV 97-cite}{\cite{CLEO:1996oro}}
\dxdef{ANASTASSOV 97-exp}{CLEO}
\dxdef{ANASTASSOV 97-type}{pub}
\dxdef{ANASTASSOV 97-label}{ANASTASSOV 97 (CLEO)}
\dxdef{ANASTASSOV 97-meas}{%
\multicolumn{2}{l}{\dxuse{ANASTASSOV 97-label}\,\dxuse{ANASTASSOV 97-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma3by5-gn} = \dxuse{Gamma3by5-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma3by5.pub.ANASTASSOV.97-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma5-gn} = \dxuse{Gamma5-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma5.pub.ANASTASSOV.97-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma8-gn} = \dxuse{Gamma8-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma8.pub.ANASTASSOV.97-vu}%
}
\dxdef{ARTUSO 92-ref}{Artuso:1992qu}
\dxdef{ARTUSO 92-cite}{\cite{Artuso:1992qu}}
\dxdef{ARTUSO 92-exp}{CLEO}
\dxdef{ARTUSO 92-type}{pub}
\dxdef{ARTUSO 92-label}{ARTUSO 92 (CLEO)}
\dxdef{ARTUSO 92-meas}{%
\multicolumn{2}{l}{\dxuse{ARTUSO 92-label}\,\dxuse{ARTUSO 92-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma126-gn} = \dxuse{Gamma126-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma126.pub.ARTUSO.92-vu}%
}
\dxdef{ARTUSO 94-ref}{Artuso:1994ii}
\dxdef{ARTUSO 94-cite}{\cite{Artuso:1994ii}}
\dxdef{ARTUSO 94-exp}{CLEO}
\dxdef{ARTUSO 94-type}{pub}
\dxdef{ARTUSO 94-label}{ARTUSO 94 (CLEO)}
\dxdef{ARTUSO 94-meas}{%
\multicolumn{2}{l}{\dxuse{ARTUSO 94-label}\,\dxuse{ARTUSO 94-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma13-gn} = \dxuse{Gamma13-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma13.pub.ARTUSO.94-vu}%
}
\dxdef{BALEST 95C-ref}{Balest:1995kq}
\dxdef{BALEST 95C-cite}{\cite{Balest:1995kq}}
\dxdef{BALEST 95C-exp}{CLEO}
\dxdef{BALEST 95C-type}{pub}
\dxdef{BALEST 95C-label}{BALEST 95C (CLEO)}
\dxdef{BALEST 95C-meas}{%
\multicolumn{2}{l}{\dxuse{BALEST 95C-label}\,\dxuse{BALEST 95C-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma57-gn} = \dxuse{Gamma57-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma57.pub.BALEST.95C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma66-gn} = \dxuse{Gamma66-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma66.pub.BALEST.95C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma150by66-gn} = \dxuse{Gamma150by66-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma150by66.pub.BALEST.95C-vu}%
}
\dxdef{BARINGER 87-ref}{Baringer:1987tr}
\dxdef{BARINGER 87-cite}{\cite{Baringer:1987tr}}
\dxdef{BARINGER 87-exp}{CLEO}
\dxdef{BARINGER 87-type}{pub}
\dxdef{BARINGER 87-label}{BARINGER 87 (CLEO)}
\dxdef{BARINGER 87-meas}{%
\multicolumn{2}{l}{\dxuse{BARINGER 87-label}\,\dxuse{BARINGER 87-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma150-gn} = \dxuse{Gamma150-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma150.pub.BARINGER.87-vu}%
}
\dxdef{BARTELT 96-ref}{Bartelt:1996iv}
\dxdef{BARTELT 96-cite}{\cite{Bartelt:1996iv}}
\dxdef{BARTELT 96-exp}{CLEO}
\dxdef{BARTELT 96-type}{pub}
\dxdef{BARTELT 96-label}{BARTELT 96 (CLEO)}
\dxdef{BARTELT 96-meas}{%
\multicolumn{2}{l}{\dxuse{BARTELT 96-label}\,\dxuse{BARTELT 96-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma128-gn} = \dxuse{Gamma128-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma128.pub.BARTELT.96-vu}%
}
\dxdef{BATTLE 94-ref}{Battle:1994by}
\dxdef{BATTLE 94-cite}{\cite{Battle:1994by}}
\dxdef{BATTLE 94-exp}{CLEO}
\dxdef{BATTLE 94-type}{pub}
\dxdef{BATTLE 94-label}{BATTLE 94 (CLEO)}
\dxdef{BATTLE 94-meas}{%
\multicolumn{2}{l}{\dxuse{BATTLE 94-label}\,\dxuse{BATTLE 94-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma10-gn} = \dxuse{Gamma10-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma10.pub.BATTLE.94-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma16-gn} = \dxuse{Gamma16-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma16.pub.BATTLE.94-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma23-gn} = \dxuse{Gamma23-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma23.pub.BATTLE.94-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma31-gn} = \dxuse{Gamma31-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma31.pub.BATTLE.94-vu}%
}
\dxdef{BISHAI 99-ref}{Bishai:1998gf}
\dxdef{BISHAI 99-cite}{\cite{Bishai:1998gf}}
\dxdef{BISHAI 99-exp}{CLEO}
\dxdef{BISHAI 99-type}{pub}
\dxdef{BISHAI 99-label}{BISHAI 99 (CLEO)}
\dxdef{BISHAI 99-meas}{%
\multicolumn{2}{l}{\dxuse{BISHAI 99-label}\,\dxuse{BISHAI 99-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma130-gn} = \dxuse{Gamma130-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma130.pub.BISHAI.99-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma132-gn} = \dxuse{Gamma132-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma132.pub.BISHAI.99-vu}%
}
\dxdef{BORTOLETTO 93-ref}{Bortoletto:1993px}
\dxdef{BORTOLETTO 93-cite}{\cite{Bortoletto:1993px}}
\dxdef{BORTOLETTO 93-exp}{CLEO}
\dxdef{BORTOLETTO 93-type}{pub}
\dxdef{BORTOLETTO 93-label}{BORTOLETTO 93 (CLEO)}
\dxdef{BORTOLETTO 93-meas}{%
\multicolumn{2}{l}{\dxuse{BORTOLETTO 93-label}\,\dxuse{BORTOLETTO 93-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma76by54-gn} = \dxuse{Gamma76by54-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma76by54.pub.BORTOLETTO.93-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma152by76-gn} = \dxuse{Gamma152by76-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma152by76.pub.BORTOLETTO.93-vu}%
}
\dxdef{COAN 96-ref}{Coan:1996iu}
\dxdef{COAN 96-cite}{\cite{Coan:1996iu}}
\dxdef{COAN 96-exp}{CLEO}
\dxdef{COAN 96-type}{pub}
\dxdef{COAN 96-label}{COAN 96 (CLEO)}
\dxdef{COAN 96-meas}{%
\multicolumn{2}{l}{\dxuse{COAN 96-label}\,\dxuse{COAN 96-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma34-gn} = \dxuse{Gamma34-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma34.pub.COAN.96-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma37-gn} = \dxuse{Gamma37-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma37.pub.COAN.96-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma39-gn} = \dxuse{Gamma39-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma39.pub.COAN.96-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma42-gn} = \dxuse{Gamma42-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma42.pub.COAN.96-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma47-gn} = \dxuse{Gamma47-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma47.pub.COAN.96-vu}%
}
\dxdef{EDWARDS 00A-ref}{Edwards:1999fj}
\dxdef{EDWARDS 00A-cite}{\cite{Edwards:1999fj}}
\dxdef{EDWARDS 00A-exp}{CLEO}
\dxdef{EDWARDS 00A-type}{pub}
\dxdef{EDWARDS 00A-label}{EDWARDS 00A (CLEO)}
\dxdef{EDWARDS 00A-meas}{%
\multicolumn{2}{l}{\dxuse{EDWARDS 00A-label}\,\dxuse{EDWARDS 00A-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma69-gn} = \dxuse{Gamma69-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma69.pub.EDWARDS.00A-vu}%
}
\dxdef{GIBAUT 94B-ref}{Gibaut:1994ik}
\dxdef{GIBAUT 94B-cite}{\cite{Gibaut:1994ik}}
\dxdef{GIBAUT 94B-exp}{CLEO}
\dxdef{GIBAUT 94B-type}{pub}
\dxdef{GIBAUT 94B-label}{GIBAUT 94B (CLEO)}
\dxdef{GIBAUT 94B-meas}{%
\multicolumn{2}{l}{\dxuse{GIBAUT 94B-label}\,\dxuse{GIBAUT 94B-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma102-gn} = \dxuse{Gamma102-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma102.pub.GIBAUT.94B-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma103-gn} = \dxuse{Gamma103-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma103.pub.GIBAUT.94B-vu}%
}
\dxdef{PROCARIO 93-ref}{Procario:1992hd}
\dxdef{PROCARIO 93-cite}{\cite{Procario:1992hd}}
\dxdef{PROCARIO 93-exp}{CLEO}
\dxdef{PROCARIO 93-type}{pub}
\dxdef{PROCARIO 93-label}{PROCARIO 93 (CLEO)}
\dxdef{PROCARIO 93-meas}{%
\multicolumn{2}{l}{\dxuse{PROCARIO 93-label}\,\dxuse{PROCARIO 93-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma19by13-gn} = \dxuse{Gamma19by13-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma19by13.pub.PROCARIO.93-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma26by13-gn} = \dxuse{Gamma26by13-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma26by13.pub.PROCARIO.93-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma29-gn} = \dxuse{Gamma29-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma29.pub.PROCARIO.93-vu}%
}
\dxdef{RICHICHI 99-ref}{Richichi:1998bc}
\dxdef{RICHICHI 99-cite}{\cite{Richichi:1998bc}}
\dxdef{RICHICHI 99-exp}{CLEO}
\dxdef{RICHICHI 99-type}{pub}
\dxdef{RICHICHI 99-label}{RICHICHI 99 (CLEO)}
\dxdef{RICHICHI 99-meas}{%
\multicolumn{2}{l}{\dxuse{RICHICHI 99-label}\,\dxuse{RICHICHI 99-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma80by60-gn} = \dxuse{Gamma80by60-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma80by60.pub.RICHICHI.99-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma81by69-gn} = \dxuse{Gamma81by69-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma81by69.pub.RICHICHI.99-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma93by60-gn} = \dxuse{Gamma93by60-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma93by60.pub.RICHICHI.99-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma94by69-gn} = \dxuse{Gamma94by69-td}
\end{ensuredisplaymath} & \dxuse{CLEO.Gamma94by69.pub.RICHICHI.99-vu}%
}
\dxdef{ARMS 05-ref}{Arms:2005qg}
\dxdef{ARMS 05-cite}{\cite{Arms:2005qg}}
\dxdef{ARMS 05-exp}{CLEO3}
\dxdef{ARMS 05-type}{pub}
\dxdef{ARMS 05-label}{ARMS 05 (CLEO3)}
\dxdef{ARMS 05-meas}{%
\multicolumn{2}{l}{\dxuse{ARMS 05-label}\,\dxuse{ARMS 05-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma88-gn} = \dxuse{Gamma88-td}
\end{ensuredisplaymath} & \dxuse{CLEO3.Gamma88.pub.ARMS.05-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma94-gn} = \dxuse{Gamma94-td}
\end{ensuredisplaymath} & \dxuse{CLEO3.Gamma94.pub.ARMS.05-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma151-gn} = \dxuse{Gamma151-td}
\end{ensuredisplaymath} & \dxuse{CLEO3.Gamma151.pub.ARMS.05-vu}%
}
\dxdef{BRIERE 03-ref}{Briere:2003fr}
\dxdef{BRIERE 03-cite}{\cite{Briere:2003fr}}
\dxdef{BRIERE 03-exp}{CLEO3}
\dxdef{BRIERE 03-type}{pub}
\dxdef{BRIERE 03-label}{BRIERE 03 (CLEO3)}
\dxdef{BRIERE 03-meas}{%
\multicolumn{2}{l}{\dxuse{BRIERE 03-label}\,\dxuse{BRIERE 03-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma60-gn} = \dxuse{Gamma60-td}
\end{ensuredisplaymath} & \dxuse{CLEO3.Gamma60.pub.BRIERE.03-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma85-gn} = \dxuse{Gamma85-td}
\end{ensuredisplaymath} & \dxuse{CLEO3.Gamma85.pub.BRIERE.03-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma93-gn} = \dxuse{Gamma93-td}
\end{ensuredisplaymath} & \dxuse{CLEO3.Gamma93.pub.BRIERE.03-vu}%
}
\dxdef{ABDALLAH 06A-ref}{Abdallah:2003cw}
\dxdef{ABDALLAH 06A-cite}{\cite{Abdallah:2003cw}}
\dxdef{ABDALLAH 06A-exp}{DELPHI}
\dxdef{ABDALLAH 06A-type}{pub}
\dxdef{ABDALLAH 06A-label}{ABDALLAH 06A (DELPHI)}
\dxdef{ABDALLAH 06A-meas}{%
\multicolumn{2}{l}{\dxuse{ABDALLAH 06A-label}\,\dxuse{ABDALLAH 06A-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma8-gn} = \dxuse{Gamma8-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma8.pub.ABDALLAH.06A-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma13-gn} = \dxuse{Gamma13-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma13.pub.ABDALLAH.06A-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma19-gn} = \dxuse{Gamma19-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma19.pub.ABDALLAH.06A-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma25-gn} = \dxuse{Gamma25-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma25.pub.ABDALLAH.06A-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma57-gn} = \dxuse{Gamma57-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma57.pub.ABDALLAH.06A-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma66-gn} = \dxuse{Gamma66-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma66.pub.ABDALLAH.06A-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma74-gn} = \dxuse{Gamma74-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma74.pub.ABDALLAH.06A-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma103-gn} = \dxuse{Gamma103-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma103.pub.ABDALLAH.06A-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma104-gn} = \dxuse{Gamma104-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma104.pub.ABDALLAH.06A-vu}%
}
\dxdef{ABREU 92N-ref}{Abreu:1992gn}
\dxdef{ABREU 92N-cite}{\cite{Abreu:1992gn}}
\dxdef{ABREU 92N-exp}{DELPHI}
\dxdef{ABREU 92N-type}{pub}
\dxdef{ABREU 92N-label}{ABREU 92N (DELPHI)}
\dxdef{ABREU 92N-meas}{%
\multicolumn{2}{l}{\dxuse{ABREU 92N-label}\,\dxuse{ABREU 92N-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma7-gn} = \dxuse{Gamma7-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma7.pub.ABREU.92N-vu}%
}
\dxdef{ABREU 94K-ref}{Abreu:1994fi}
\dxdef{ABREU 94K-cite}{\cite{Abreu:1994fi}}
\dxdef{ABREU 94K-exp}{DELPHI}
\dxdef{ABREU 94K-type}{pub}
\dxdef{ABREU 94K-label}{ABREU 94K (DELPHI)}
\dxdef{ABREU 94K-meas}{%
\multicolumn{2}{l}{\dxuse{ABREU 94K-label}\,\dxuse{ABREU 94K-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma10-gn} = \dxuse{Gamma10-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma10.pub.ABREU.94K-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma31-gn} = \dxuse{Gamma31-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma31.pub.ABREU.94K-vu}%
}
\dxdef{ABREU 99X-ref}{Abreu:1999rb}
\dxdef{ABREU 99X-cite}{\cite{Abreu:1999rb}}
\dxdef{ABREU 99X-exp}{DELPHI}
\dxdef{ABREU 99X-type}{pub}
\dxdef{ABREU 99X-label}{ABREU 99X (DELPHI)}
\dxdef{ABREU 99X-meas}{%
\multicolumn{2}{l}{\dxuse{ABREU 99X-label}\,\dxuse{ABREU 99X-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma3-gn} = \dxuse{Gamma3-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma3.pub.ABREU.99X-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma5-gn} = \dxuse{Gamma5-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.Gamma5.pub.ABREU.99X-vu}%
}
\dxdef{BYLSMA 87-ref}{Bylsma:1986zy}
\dxdef{BYLSMA 87-cite}{\cite{Bylsma:1986zy}}
\dxdef{BYLSMA 87-exp}{HRS}
\dxdef{BYLSMA 87-type}{pub}
\dxdef{BYLSMA 87-label}{BYLSMA 87 (HRS)}
\dxdef{BYLSMA 87-meas}{%
\multicolumn{2}{l}{\dxuse{BYLSMA 87-label}\,\dxuse{BYLSMA 87-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma102-gn} = \dxuse{Gamma102-td}
\end{ensuredisplaymath} & \dxuse{HRS.Gamma102.pub.BYLSMA.87-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma103-gn} = \dxuse{Gamma103-td}
\end{ensuredisplaymath} & \dxuse{HRS.Gamma103.pub.BYLSMA.87-vu}%
}
\dxdef{ACCIARRI 01F-ref}{Acciarri:2001sg}
\dxdef{ACCIARRI 01F-cite}{\cite{Acciarri:2001sg}}
\dxdef{ACCIARRI 01F-exp}{L3}
\dxdef{ACCIARRI 01F-type}{pub}
\dxdef{ACCIARRI 01F-label}{ACCIARRI 01F (L3)}
\dxdef{ACCIARRI 01F-meas}{%
\multicolumn{2}{l}{\dxuse{ACCIARRI 01F-label}\,\dxuse{ACCIARRI 01F-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma3-gn} = \dxuse{Gamma3-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma3.pub.ACCIARRI.01F-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma5-gn} = \dxuse{Gamma5-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma5.pub.ACCIARRI.01F-vu}%
}
\dxdef{ACCIARRI 95-ref}{Acciarri:1994vr}
\dxdef{ACCIARRI 95-cite}{\cite{Acciarri:1994vr}}
\dxdef{ACCIARRI 95-exp}{L3}
\dxdef{ACCIARRI 95-type}{pub}
\dxdef{ACCIARRI 95-label}{ACCIARRI 95 (L3)}
\dxdef{ACCIARRI 95-meas}{%
\multicolumn{2}{l}{\dxuse{ACCIARRI 95-label}\,\dxuse{ACCIARRI 95-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma7-gn} = \dxuse{Gamma7-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma7.pub.ACCIARRI.95-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma13-gn} = \dxuse{Gamma13-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma13.pub.ACCIARRI.95-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma19-gn} = \dxuse{Gamma19-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma19.pub.ACCIARRI.95-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma26-gn} = \dxuse{Gamma26-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma26.pub.ACCIARRI.95-vu}%
}
\dxdef{ACCIARRI 95F-ref}{Acciarri:1995kx}
\dxdef{ACCIARRI 95F-cite}{\cite{Acciarri:1995kx}}
\dxdef{ACCIARRI 95F-exp}{L3}
\dxdef{ACCIARRI 95F-type}{pub}
\dxdef{ACCIARRI 95F-label}{ACCIARRI 95F (L3)}
\dxdef{ACCIARRI 95F-meas}{%
\multicolumn{2}{l}{\dxuse{ACCIARRI 95F-label}\,\dxuse{ACCIARRI 95F-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma35-gn} = \dxuse{Gamma35-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma35.pub.ACCIARRI.95F-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma40-gn} = \dxuse{Gamma40-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma40.pub.ACCIARRI.95F-vu}%
}
\dxdef{ACHARD 01D-ref}{Achard:2001pk}
\dxdef{ACHARD 01D-cite}{\cite{Achard:2001pk}}
\dxdef{ACHARD 01D-exp}{L3}
\dxdef{ACHARD 01D-type}{pub}
\dxdef{ACHARD 01D-label}{ACHARD 01D (L3)}
\dxdef{ACHARD 01D-meas}{%
\multicolumn{2}{l}{\dxuse{ACHARD 01D-label}\,\dxuse{ACHARD 01D-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma55-gn} = \dxuse{Gamma55-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma55.pub.ACHARD.01D-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma102-gn} = \dxuse{Gamma102-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma102.pub.ACHARD.01D-vu}%
}
\dxdef{ADEVA 91F-ref}{Adeva:1991qq}
\dxdef{ADEVA 91F-cite}{\cite{Adeva:1991qq}}
\dxdef{ADEVA 91F-exp}{L3}
\dxdef{ADEVA 91F-type}{pub}
\dxdef{ADEVA 91F-label}{ADEVA 91F (L3)}
\dxdef{ADEVA 91F-meas}{%
\multicolumn{2}{l}{\dxuse{ADEVA 91F-label}\,\dxuse{ADEVA 91F-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma54-gn} = \dxuse{Gamma54-td}
\end{ensuredisplaymath} & \dxuse{L3.Gamma54.pub.ADEVA.91F-vu}%
}
\dxdef{ABBIENDI 00C-ref}{Abbiendi:1999pm}
\dxdef{ABBIENDI 00C-cite}{\cite{Abbiendi:1999pm}}
\dxdef{ABBIENDI 00C-exp}{OPAL}
\dxdef{ABBIENDI 00C-type}{pub}
\dxdef{ABBIENDI 00C-label}{ABBIENDI 00C (OPAL)}
\dxdef{ABBIENDI 00C-meas}{%
\multicolumn{2}{l}{\dxuse{ABBIENDI 00C-label}\,\dxuse{ABBIENDI 00C-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma35-gn} = \dxuse{Gamma35-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma35.pub.ABBIENDI.00C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma38-gn} = \dxuse{Gamma38-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma38.pub.ABBIENDI.00C-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma43-gn} = \dxuse{Gamma43-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma43.pub.ABBIENDI.00C-vu}%
}
\dxdef{ABBIENDI 00D-ref}{Abbiendi:1999cq}
\dxdef{ABBIENDI 00D-cite}{\cite{Abbiendi:1999cq}}
\dxdef{ABBIENDI 00D-exp}{OPAL}
\dxdef{ABBIENDI 00D-type}{pub}
\dxdef{ABBIENDI 00D-label}{ABBIENDI 00D (OPAL)}
\dxdef{ABBIENDI 00D-meas}{%
\multicolumn{2}{l}{\dxuse{ABBIENDI 00D-label}\,\dxuse{ABBIENDI 00D-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma92-gn} = \dxuse{Gamma92-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma92.pub.ABBIENDI.00D-vu}%
}
\dxdef{ABBIENDI 01J-ref}{Abbiendi:2000ee}
\dxdef{ABBIENDI 01J-cite}{\cite{Abbiendi:2000ee}}
\dxdef{ABBIENDI 01J-exp}{OPAL}
\dxdef{ABBIENDI 01J-type}{pub}
\dxdef{ABBIENDI 01J-label}{ABBIENDI 01J (OPAL)}
\dxdef{ABBIENDI 01J-meas}{%
\multicolumn{2}{l}{\dxuse{ABBIENDI 01J-label}\,\dxuse{ABBIENDI 01J-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma10-gn} = \dxuse{Gamma10-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma10.pub.ABBIENDI.01J-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma31-gn} = \dxuse{Gamma31-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma31.pub.ABBIENDI.01J-vu}%
}
\dxdef{ABBIENDI 03-ref}{Abbiendi:2002jw}
\dxdef{ABBIENDI 03-cite}{\cite{Abbiendi:2002jw}}
\dxdef{ABBIENDI 03-exp}{OPAL}
\dxdef{ABBIENDI 03-type}{pub}
\dxdef{ABBIENDI 03-label}{ABBIENDI 03 (OPAL)}
\dxdef{ABBIENDI 03-meas}{%
\multicolumn{2}{l}{\dxuse{ABBIENDI 03-label}\,\dxuse{ABBIENDI 03-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma3-gn} = \dxuse{Gamma3-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma3.pub.ABBIENDI.03-vu}%
}
\dxdef{ABBIENDI 04J-ref}{Abbiendi:2004xa}
\dxdef{ABBIENDI 04J-cite}{\cite{Abbiendi:2004xa}}
\dxdef{ABBIENDI 04J-exp}{OPAL}
\dxdef{ABBIENDI 04J-type}{pub}
\dxdef{ABBIENDI 04J-label}{ABBIENDI 04J (OPAL)}
\dxdef{ABBIENDI 04J-meas}{%
\multicolumn{2}{l}{\dxuse{ABBIENDI 04J-label}\,\dxuse{ABBIENDI 04J-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma16-gn} = \dxuse{Gamma16-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma16.pub.ABBIENDI.04J-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma85-gn} = \dxuse{Gamma85-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma85.pub.ABBIENDI.04J-vu}%
}
\dxdef{ABBIENDI 99H-ref}{Abbiendi:1998cx}
\dxdef{ABBIENDI 99H-cite}{\cite{Abbiendi:1998cx}}
\dxdef{ABBIENDI 99H-exp}{OPAL}
\dxdef{ABBIENDI 99H-type}{pub}
\dxdef{ABBIENDI 99H-label}{ABBIENDI 99H (OPAL)}
\dxdef{ABBIENDI 99H-meas}{%
\multicolumn{2}{l}{\dxuse{ABBIENDI 99H-label}\,\dxuse{ABBIENDI 99H-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma5-gn} = \dxuse{Gamma5-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma5.pub.ABBIENDI.99H-vu}%
}
\dxdef{ACKERSTAFF 98M-ref}{Ackerstaff:1997tx}
\dxdef{ACKERSTAFF 98M-cite}{\cite{Ackerstaff:1997tx}}
\dxdef{ACKERSTAFF 98M-exp}{OPAL}
\dxdef{ACKERSTAFF 98M-type}{pub}
\dxdef{ACKERSTAFF 98M-label}{ACKERSTAFF 98M (OPAL)}
\dxdef{ACKERSTAFF 98M-meas}{%
\multicolumn{2}{l}{\dxuse{ACKERSTAFF 98M-label}\,\dxuse{ACKERSTAFF 98M-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma8-gn} = \dxuse{Gamma8-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma8.pub.ACKERSTAFF.98M-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma13-gn} = \dxuse{Gamma13-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma13.pub.ACKERSTAFF.98M-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma17-gn} = \dxuse{Gamma17-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma17.pub.ACKERSTAFF.98M-vu}%
}
\dxdef{ACKERSTAFF 99E-ref}{Ackerstaff:1998ia}
\dxdef{ACKERSTAFF 99E-cite}{\cite{Ackerstaff:1998ia}}
\dxdef{ACKERSTAFF 99E-exp}{OPAL}
\dxdef{ACKERSTAFF 99E-type}{pub}
\dxdef{ACKERSTAFF 99E-label}{ACKERSTAFF 99E (OPAL)}
\dxdef{ACKERSTAFF 99E-meas}{%
\multicolumn{2}{l}{\dxuse{ACKERSTAFF 99E-label}\,\dxuse{ACKERSTAFF 99E-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma103-gn} = \dxuse{Gamma103-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma103.pub.ACKERSTAFF.99E-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma104-gn} = \dxuse{Gamma104-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma104.pub.ACKERSTAFF.99E-vu}%
}
\dxdef{AKERS 94G-ref}{Akers:1994td}
\dxdef{AKERS 94G-cite}{\cite{Akers:1994td}}
\dxdef{AKERS 94G-exp}{OPAL}
\dxdef{AKERS 94G-type}{pub}
\dxdef{AKERS 94G-label}{AKERS 94G (OPAL)}
\dxdef{AKERS 94G-meas}{%
\multicolumn{2}{l}{\dxuse{AKERS 94G-label}\,\dxuse{AKERS 94G-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma33-gn} = \dxuse{Gamma33-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma33.pub.AKERS.94G-vu}%
}
\dxdef{AKERS 95Y-ref}{Akers:1995ry}
\dxdef{AKERS 95Y-cite}{\cite{Akers:1995ry}}
\dxdef{AKERS 95Y-exp}{OPAL}
\dxdef{AKERS 95Y-type}{pub}
\dxdef{AKERS 95Y-label}{AKERS 95Y (OPAL)}
\dxdef{AKERS 95Y-meas}{%
\multicolumn{2}{l}{\dxuse{AKERS 95Y-label}\,\dxuse{AKERS 95Y-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma55-gn} = \dxuse{Gamma55-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma55.pub.AKERS.95Y-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma57by55-gn} = \dxuse{Gamma57by55-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma57by55.pub.AKERS.95Y-vu}%
}
\dxdef{ALEXANDER 91D-ref}{Alexander:1991am}
\dxdef{ALEXANDER 91D-cite}{\cite{Alexander:1991am}}
\dxdef{ALEXANDER 91D-exp}{OPAL}
\dxdef{ALEXANDER 91D-type}{pub}
\dxdef{ALEXANDER 91D-label}{ALEXANDER 91D (OPAL)}
\dxdef{ALEXANDER 91D-meas}{%
\multicolumn{2}{l}{\dxuse{ALEXANDER 91D-label}\,\dxuse{ALEXANDER 91D-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma7-gn} = \dxuse{Gamma7-td}
\end{ensuredisplaymath} & \dxuse{OPAL.Gamma7.pub.ALEXANDER.91D-vu}%
}
\dxdef{AIHARA 87B-ref}{Aihara:1986mw}
\dxdef{AIHARA 87B-cite}{\cite{Aihara:1986mw}}
\dxdef{AIHARA 87B-exp}{TPC}
\dxdef{AIHARA 87B-type}{pub}
\dxdef{AIHARA 87B-label}{AIHARA 87B (TPC)}
\dxdef{AIHARA 87B-meas}{%
\multicolumn{2}{l}{\dxuse{AIHARA 87B-label}\,\dxuse{AIHARA 87B-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma54-gn} = \dxuse{Gamma54-td}
\end{ensuredisplaymath} & \dxuse{TPC.Gamma54.pub.AIHARA.87B-vu}%
}
\dxdef{BAUER 94-ref}{TPCTwoGamma:1993tpi}
\dxdef{BAUER 94-cite}{\cite{TPCTwoGamma:1993tpi}}
\dxdef{BAUER 94-exp}{TPC}
\dxdef{BAUER 94-type}{pub}
\dxdef{BAUER 94-label}{BAUER 94 (TPC)}
\dxdef{BAUER 94-meas}{%
\multicolumn{2}{l}{\dxuse{BAUER 94-label}\,\dxuse{BAUER 94-cite}} \\
\begin{ensuredisplaymath}
\dxuse{Gamma82-gn} = \dxuse{Gamma82-td}
\end{ensuredisplaymath} & \dxuse{TPC.Gamma82.pub.BAUER.94-vu}
\\
\begin{ensuredisplaymath}
\dxuse{Gamma92-gn} = \dxuse{Gamma92-td}
\end{ensuredisplaymath} & \dxuse{TPC.Gamma92.pub.BAUER.94-vu}%
}
\dxdef{TauBrMeasByRef}{%
\dxuse{BARATE 98-meas} \\[1.5ex]
\dxuse{BARATE 98E-meas} \\[1.5ex]
\dxuse{BARATE 99K-meas} \\[1.5ex]
\dxuse{BARATE 99R-meas} \\[1.5ex]
\dxuse{BUSKULIC 96-meas} \\[1.5ex]
\dxuse{BUSKULIC 97C-meas} \\[1.5ex]
\dxuse{SCHAEL 05C-meas} \\[1.5ex]
\dxuse{ALBRECHT 88B-meas} \\[1.5ex]
\dxuse{ALBRECHT 92D-meas} \\[1.5ex]
\dxuse{AUBERT 07AP-meas} \\[1.5ex]
\dxuse{AUBERT 08-meas} \\[1.5ex]
\dxuse{AUBERT 10F-meas} \\[1.5ex]
\dxuse{DEL-AMO-SANCHEZ 11E-meas} \\[1.5ex]
\dxuse{LEES 12X-meas} \\[1.5ex]
\dxuse{LEES 12Y-meas} \\[1.5ex]
\dxuse{LEES 18B-meas} \\[1.5ex]
\dxuse{FUJIKAWA 08-meas} \\[1.5ex]
\dxuse{INAMI 09-meas} \\[1.5ex]
\dxuse{LEE 10-meas} \\[1.5ex]
\dxuse{RYU 14vpc-meas} \\[1.5ex]
\dxuse{Belle2 ADACHI 2024-meas} \\[1.5ex]
\dxuse{BEHREND 89B-meas} \\[1.5ex]
\dxuse{ANASTASSOV 01-meas} \\[1.5ex]
\dxuse{ANASTASSOV 97-meas} \\[1.5ex]
\dxuse{ARTUSO 92-meas} \\[1.5ex]
\dxuse{ARTUSO 94-meas} \\[1.5ex]
\dxuse{BALEST 95C-meas} \\[1.5ex]
\dxuse{BARINGER 87-meas} \\[1.5ex]
\dxuse{BARTELT 96-meas} \\[1.5ex]
\dxuse{BATTLE 94-meas} \\[1.5ex]
\dxuse{BISHAI 99-meas} \\[1.5ex]
\dxuse{BORTOLETTO 93-meas} \\[1.5ex]
\dxuse{COAN 96-meas} \\[1.5ex]
\dxuse{EDWARDS 00A-meas} \\[1.5ex]
\dxuse{GIBAUT 94B-meas} \\[1.5ex]
\dxuse{PROCARIO 93-meas} \\[1.5ex]
\dxuse{RICHICHI 99-meas} \\[1.5ex]
\dxuse{ARMS 05-meas} \\[1.5ex]
\dxuse{BRIERE 03-meas} \\[1.5ex]
\dxuse{ABDALLAH 06A-meas} \\[1.5ex]
\dxuse{ABREU 92N-meas} \\[1.5ex]
\dxuse{ABREU 94K-meas} \\[1.5ex]
\dxuse{ABREU 99X-meas} \\[1.5ex]
\dxuse{BYLSMA 87-meas} \\[1.5ex]
\dxuse{ACCIARRI 01F-meas} \\[1.5ex]
\dxuse{ACCIARRI 95-meas} \\[1.5ex]
\dxuse{ACCIARRI 95F-meas} \\[1.5ex]
\dxuse{ACHARD 01D-meas} \\[1.5ex]
\dxuse{ADEVA 91F-meas} \\[1.5ex]
\dxuse{ABBIENDI 00C-meas} \\[1.5ex]
\dxuse{ABBIENDI 00D-meas} \\[1.5ex]
\dxuse{ABBIENDI 01J-meas} \\[1.5ex]
\dxuse{ABBIENDI 03-meas} \\[1.5ex]
\dxuse{ABBIENDI 04J-meas} \\[1.5ex]
\dxuse{ABBIENDI 99H-meas} \\[1.5ex]
\dxuse{ACKERSTAFF 98M-meas} \\[1.5ex]
\dxuse{ACKERSTAFF 99E-meas} \\[1.5ex]
\dxuse{AKERS 94G-meas} \\[1.5ex]
\dxuse{AKERS 95Y-meas} \\[1.5ex]
\dxuse{ALEXANDER 91D-meas} \\[1.5ex]
\dxuse{AIHARA 87B-meas} \\[1.5ex]
\dxuse{BAUER 94-meas}%
}
\dxdef{TauBrStrangeVal}{%
\dxQuantLine{Gamma10}{0.6959 \pm 0.0096}{-2} 
\dxQuantLine{Gamma16}{0.4321 \pm 0.0148}{-2} 
\dxQuantLine{Gamma23}{0.0634 \pm 0.0219}{-2} 
\dxQuantLine{Gamma28}{0.0465 \pm 0.0213}{-2} 
\dxQuantLine{Gamma35}{0.8375 \pm 0.0139}{-2} 
\dxQuantLine{Gamma40}{0.3810 \pm 0.0129}{-2} 
\dxQuantLine{Gamma44}{0.0234 \pm 0.0231}{-2} 
\dxQuantLine{Gamma53}{0.0222 \pm 0.0202}{-2} 
\dxQuantLine{Gamma128}{0.0155 \pm 0.0008}{-2} 
\dxQuantLine{Gamma130}{0.0048 \pm 0.0012}{-2} 
\dxQuantLine{Gamma132}{0.0094 \pm 0.0015}{-2} 
\dxQuantLine{Gamma151}{0.0410 \pm 0.0092}{-2} 
\dxQuantLine{Gamma168}{0.0022 \pm 0.0008}{-2} 
\dxQuantLine{Gamma169}{0.0015 \pm 0.0006}{-2} 
\dxQuantLine{Gamma802}{0.2924 \pm 0.0068}{-2} 
\dxQuantLine{Gamma803}{0.0388 \pm 0.0142}{-2} 
\dxQuantLine{Gamma822}{0.0001 \pm 0.0001}{-2} 
\dxQuantLine{Gamma833}{0.0001 \pm 0.0001}{-2}%
}
\dxdef{TauBrStrangeTotVal}{%
\dxQuantLine{Gamma110}{2.9078 \pm 0.0478}{-2}%
}
\dxdef{TauBrUnitarityQuants}{%
\dxConstrQuantValWeight{Gamma3}{0.1736 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma5}{0.1784 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma9}{0.1081 \pm 0.0005}{1.0000} 
\dxConstrQuantValWeight{Gamma10}{0.00696 \pm 0.00010}{1.0000} 
\dxConstrQuantValWeight{Gamma14}{0.2548 \pm 0.0009}{1.0000} 
\dxConstrQuantValWeight{Gamma16}{0.00432 \pm 0.00015}{1.0000} 
\dxConstrQuantValWeight{Gamma20}{0.0925 \pm 0.0010}{1.0000} 
\dxConstrQuantValWeight{Gamma23}{(0.63 \pm 0.22)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma27}{0.0104 \pm 0.0007}{1.0000} 
\dxConstrQuantValWeight{Gamma28}{(0.46 \pm 0.21)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma30}{0.0011 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma35}{0.00838 \pm 0.00014}{1.0000} 
\dxConstrQuantValWeight{Gamma37}{0.001486 \pm 0.000034}{1.0000} 
\dxConstrQuantValWeight{Gamma40}{0.00381 \pm 0.00013}{1.0000} 
\dxConstrQuantValWeight{Gamma42}{0.00150 \pm 0.00007}{1.0000} 
\dxConstrQuantValWeight{Gamma44}{(0.23 \pm 0.23)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma47}{(235 \pm 6)\cdot 10^{-6}}{2.0000} 
\dxConstrQuantValWeight{Gamma48}{0.00105 \pm 0.00025}{1.0000} 
\dxConstrQuantValWeight{Gamma50}{(18.2 \pm 2.1)\cdot 10^{-6}}{2.0000} 
\dxConstrQuantValWeight{Gamma51}{(0.32 \pm 0.12)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma53}{(0.22 \pm 0.20)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma62}{0.0898 \pm 0.0005}{1.0000} 
\dxConstrQuantValWeight{Gamma70}{0.0274 \pm 0.0007}{1.0000} 
\dxConstrQuantValWeight{Gamma77}{0.0010 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma93}{0.001434 \pm 0.000027}{1.0000} 
\dxConstrQuantValWeight{Gamma94}{(61 \pm 18)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma126}{0.00139 \pm 0.00007}{1.0000} 
\dxConstrQuantValWeight{Gamma128}{(155 \pm 8)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma130}{(48 \pm 12)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma132}{(94 \pm 15)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma136}{(220 \pm 13)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma151}{(0.41 \pm 0.09)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma152}{0.0041 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma167}{(44 \pm 16)\cdot 10^{-6}}{0.8300} 
\dxConstrQuantValWeight{Gamma800}{0.0195 \pm 0.0006}{1.0000} 
\dxConstrQuantValWeight{Gamma802}{0.00292 \pm 0.00007}{1.0000} 
\dxConstrQuantValWeight{Gamma803}{(0.39 \pm 0.14)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma805}{(0.38 \pm 0.15)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma811}{(72 \pm 16)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma812}{(14 \pm 27)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma821}{(774 \pm 30)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma822}{(0.6 \pm 1.2)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma831}{(84 \pm 6)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma832}{(38 \pm 9)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma833}{(1.1 \pm 0.6)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma920}{(52 \pm 4)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma945}{(0.19 \pm 0.04)\cdot 10^{-3}}{1.0000}%
}
\dxdef{TauBrUnitarityQuantsPdgPatch}{%
\dxConstrQuantValWeight{Gamma3}{0.1736 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma5}{0.1784 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma9}{0.1081 \pm 0.0005}{1.0000} 
\dxConstrQuantValWeight{Gamma10}{0.00696 \pm 0.00010}{1.0000} 
\dxConstrQuantValWeight{Gamma14}{0.2548 \pm 0.0009}{1.0000} 
\dxConstrQuantValWeight{Gamma16}{0.00432 \pm 0.00015}{1.0000} 
\dxConstrQuantValWeight{Gamma20}{0.0925 \pm 0.0010}{1.0021} 
\dxConstrQuantValWeight{Gamma23}{(0.63 \pm 0.22)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma27}{0.0104 \pm 0.0007}{1.0000} 
\dxConstrQuantValWeight{Gamma28}{(0.46 \pm 0.21)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma30}{0.0011 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma35}{0.00838 \pm 0.00014}{1.0000} 
\dxConstrQuantValWeight{Gamma37}{0.001486 \pm 0.000034}{1.0000} 
\dxConstrQuantValWeight{Gamma40}{0.00381 \pm 0.00013}{1.0000} 
\dxConstrQuantValWeight{Gamma42}{0.00150 \pm 0.00007}{1.0000} 
\dxConstrQuantValWeight{Gamma44}{(0.23 \pm 0.23)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma47}{(235 \pm 6)\cdot 10^{-6}}{2.0000} 
\dxConstrQuantValWeight{Gamma48}{0.00105 \pm 0.00025}{1.0000} 
\dxConstrQuantValWeight{Gamma50}{(18.2 \pm 2.1)\cdot 10^{-6}}{2.0000} 
\dxConstrQuantValWeight{Gamma51}{(0.32 \pm 0.12)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma53}{(0.22 \pm 0.20)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma62}{0.0898 \pm 0.0005}{1.0021} 
\dxConstrQuantValWeight{Gamma70}{0.0274 \pm 0.0007}{1.0000} 
\dxConstrQuantValWeight{Gamma77}{0.0010 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma93}{0.001434 \pm 0.000027}{1.0000} 
\dxConstrQuantValWeight{Gamma94}{(61 \pm 18)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma126}{0.00139 \pm 0.00007}{1.0000} 
\dxConstrQuantValWeight{Gamma128}{(155 \pm 8)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma130}{(48 \pm 12)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma132}{(94 \pm 15)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma136}{(220 \pm 13)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma151}{(0.41 \pm 0.09)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma152}{0.0041 \pm 0.0004}{1.0000} 
\dxConstrQuantValWeight{Gamma167}{(44 \pm 16)\cdot 10^{-6}}{0.8300} 
\dxConstrQuantValWeight{Gamma800}{0.0195 \pm 0.0006}{1.0000} 
\dxConstrQuantValWeight{Gamma802}{0.00292 \pm 0.00007}{1.0000} 
\dxConstrQuantValWeight{Gamma803}{(0.39 \pm 0.14)\cdot 10^{-3}}{1.0000} 
\dxConstrQuantValWeight{Gamma811}{(72 \pm 16)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma812}{(14 \pm 27)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma821}{(774 \pm 30)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma822}{(0.6 \pm 1.2)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma831}{(84 \pm 6)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma832}{(38 \pm 9)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma833}{(1.1 \pm 0.6)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma920}{(52 \pm 4)\cdot 10^{-6}}{1.0000} 
\dxConstrQuantValWeight{Gamma945}{(0.19 \pm 0.04)\cdot 10^{-3}}{1.0000}%
}
\dxdef{TauBrBaseQuants}{%
\dxQuantLine{Gamma3}{17.3596 \pm 0.0368}{-2} 
\dxQuantLine{Gamma5}{17.8405 \pm 0.0381}{-2} 
\dxQuantLine{Gamma9}{10.8071 \pm 0.0527}{-2} 
\dxQuantLine{Gamma10}{0.6959 \pm 0.0096}{-2} 
\dxQuantLine{Gamma14}{25.4849 \pm 0.0902}{-2} 
\dxQuantLine{Gamma16}{0.4321 \pm 0.0148}{-2} 
\dxQuantLine{Gamma20}{9.2451 \pm 0.0988}{-2} 
\dxQuantLine{Gamma23}{0.0634 \pm 0.0219}{-2} 
\dxQuantLine{Gamma27}{1.0408 \pm 0.0708}{-2} 
\dxQuantLine{Gamma28}{0.0465 \pm 0.0213}{-2} 
\dxQuantLine{Gamma30}{0.1121 \pm 0.0391}{-2} 
\dxQuantLine{Gamma35}{0.8375 \pm 0.0139}{-2} 
\dxQuantLine{Gamma37}{0.1486 \pm 0.0034}{-2} 
\dxQuantLine{Gamma40}{0.3810 \pm 0.0129}{-2} 
\dxQuantLine{Gamma42}{0.1499 \pm 0.0070}{-2} 
\dxQuantLine{Gamma44}{0.0234 \pm 0.0231}{-2} 
\dxQuantLine{Gamma47}{0.0235 \pm 0.0006}{-2} 
\dxQuantLine{Gamma48}{0.1048 \pm 0.0247}{-2} 
\dxQuantLine{Gamma50}{0.0018 \pm 0.0002}{-2} 
\dxQuantLine{Gamma51}{0.0318 \pm 0.0119}{-2} 
\dxQuantLine{Gamma53}{0.0222 \pm 0.0202}{-2} 
\dxQuantLine{Gamma62}{8.9799 \pm 0.0521}{-2} 
\dxQuantLine{Gamma70}{2.7447 \pm 0.0714}{-2} 
\dxQuantLine{Gamma77}{0.0982 \pm 0.0356}{-2} 
\dxQuantLine{Gamma93}{0.1434 \pm 0.0027}{-2} 
\dxQuantLine{Gamma94}{0.0061 \pm 0.0018}{-2} 
\dxQuantLine{Gamma126}{0.1386 \pm 0.0072}{-2} 
\dxQuantLine{Gamma128}{0.0155 \pm 0.0008}{-2} 
\dxQuantLine{Gamma130}{0.0048 \pm 0.0012}{-2} 
\dxQuantLine{Gamma132}{0.0094 \pm 0.0015}{-2} 
\dxQuantLine{Gamma136}{0.0220 \pm 0.0013}{-2} 
\dxQuantLine{Gamma151}{0.0410 \pm 0.0092}{-2} 
\dxQuantLine{Gamma152}{0.4070 \pm 0.0419}{-2} 
\dxQuantLine{Gamma167}{0.0044 \pm 0.0016}{-2} 
\dxQuantLine{Gamma800}{1.9474 \pm 0.0646}{-2} 
\dxQuantLine{Gamma802}{0.2924 \pm 0.0068}{-2} 
\dxQuantLine{Gamma803}{0.0388 \pm 0.0142}{-2} 
\dxQuantLine{Gamma811}{0.0072 \pm 0.0016}{-2} 
\dxQuantLine{Gamma812}{0.0014 \pm 0.0027}{-2} 
\dxQuantLine{Gamma821}{0.0774 \pm 0.0030}{-2} 
\dxQuantLine{Gamma822}{0.0001 \pm 0.0001}{-2} 
\dxQuantLine{Gamma831}{0.0084 \pm 0.0006}{-2} 
\dxQuantLine{Gamma832}{0.0038 \pm 0.0009}{-2} 
\dxQuantLine{Gamma833}{0.0001 \pm 0.0001}{-2} 
\dxQuantLine{Gamma920}{0.0052 \pm 0.0004}{-2} 
\dxQuantLine{Gamma945}{0.0194 \pm 0.0038}{-2} 
\dxQuantLine{Gamma980}{0.2100 \pm 0.0800}{-2}%
}
\dxdef{TauBrBaseQuantCorr}{%
 & \(\BR_{3}\) & \(\BR_{5}\) & \(\BR_{9}\) & \(\BR_{10}\) & \(\BR_{14}\) & \(\BR_{16}\) & \(\BR_{20}\) & \(\BR_{23}\) & \(\BR_{27}\) & \(\BR_{28}\) & \(\BR_{30}\) & \(\BR_{35}\) & \(\BR_{37}\) & \(\BR_{40}\) \\
\(\BR_{3}\) &  100 &   43 &    8 &    6 &  -15 &    1 &   -5 &    2 &   -5 &    2 &   -4 &    0 &    0 &    0 \\
\(\BR_{5}\) &   43 &  100 &    6 &    7 &  -16 &    1 &   -6 &    2 &   -4 &    2 &   -4 &    0 &   -1 &    0 \\
\(\BR_{9}\) &    8 &    6 &  100 &    7 &  -13 &    2 &   -8 &    0 &   -8 &    1 &  -10 &    0 &    1 &    0 \\
\(\BR_{10}\) &    6 &    7 &    7 &  100 &   -3 &   -1 &   -1 &   -2 &   -1 &   -1 &   -1 &    0 &    0 &    0 \\
\(\BR_{14}\) &  -15 &  -16 &  -13 &   -3 &  100 &   -8 &  -41 &    0 &    1 &    1 &   -8 &    0 &    0 &    0 \\
\(\BR_{16}\) &    1 &    1 &    2 &   -1 &   -8 &  100 &    1 &  -13 &    1 &  -13 &    0 &    0 &    0 &    1 \\
\(\BR_{20}\) &   -5 &   -6 &   -8 &   -1 &  -41 &    1 &  100 &   -7 &  -36 &   -1 &    6 &    0 &    0 &    0 \\
\(\BR_{23}\) &    2 &    2 &    0 &   -2 &    0 &  -13 &   -7 &  100 &    1 &  -22 &   -2 &    0 &   -2 &    1 \\
\(\BR_{27}\) &   -5 &   -4 &   -8 &   -1 &    1 &    1 &  -36 &    1 &  100 &  -10 &  -44 &    0 &    0 &   -1 \\
\(\BR_{28}\) &    2 &    2 &    1 &   -1 &    1 &  -13 &   -1 &  -22 &  -10 &  100 &    2 &    0 &   -2 &    1 \\
\(\BR_{30}\) &   -4 &   -4 &  -10 &   -1 &   -8 &    0 &    6 &   -2 &  -44 &    2 &  100 &    0 &    0 &    0 \\
\(\BR_{35}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  100 &  -15 &  -12 \\
\(\BR_{37}\) &    0 &   -1 &    1 &    0 &    0 &    0 &    0 &   -2 &    0 &   -2 &    0 &  -15 &  100 &    2 \\
\(\BR_{40}\) &    0 &    0 &    0 &    0 &    0 &    1 &    0 &    1 &   -1 &    1 &    0 &  -12 &    2 &  100 \\[1.5ex]
 & \(\BR_{3}\) & \(\BR_{5}\) & \(\BR_{9}\) & \(\BR_{10}\) & \(\BR_{14}\) & \(\BR_{16}\) & \(\BR_{20}\) & \(\BR_{23}\) & \(\BR_{27}\) & \(\BR_{28}\) & \(\BR_{30}\) & \(\BR_{35}\) & \(\BR_{37}\) & \(\BR_{40}\) \\
\(\BR_{42}\) &    0 &    0 &    0 &    0 &    0 &   -3 &    1 &   -5 &    0 &   -5 &    0 &   -1 &  -14 &  -20 \\
\(\BR_{44}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &   -4 \\
\(\BR_{47}\) &    0 &   -1 &    2 &    0 &    0 &    2 &    0 &    0 &    0 &    0 &    0 &   -1 &    3 &   -4 \\
\(\BR_{48}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -3 &    0 &   -2 \\
\(\BR_{50}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    1 &    5 &    0 \\
\(\BR_{51}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &   -1 \\
\(\BR_{53}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{62}\) &   -3 &   -4 &    8 &    0 &   -3 &    4 &   -7 &    0 &   -6 &    0 &   -5 &   -1 &    3 &    0 \\
\(\BR_{70}\) &   -6 &   -6 &   -7 &   -1 &  -10 &    0 &   -1 &    0 &   -1 &    0 &    3 &    0 &   -1 &    0 \\
\(\BR_{77}\) &   -1 &    0 &   -3 &    0 &   -2 &    0 &    0 &    0 &    2 &    0 &    2 &    0 &    0 &    0 \\
\(\BR_{93}\) &    0 &   -1 &    3 &    0 &   -1 &    2 &   -1 &    0 &   -1 &    0 &   -1 &    0 &    2 &    0 \\
\(\BR_{94}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{126}\) &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    0 &   -2 &    0 &    0 &    0 \\
\(\BR_{128}\) &    0 &    0 &    1 &    0 &    0 &    1 &    0 &   -1 &    0 &   -1 &    0 &    0 &    1 &    0 \\[1.5ex]
 & \(\BR_{3}\) & \(\BR_{5}\) & \(\BR_{9}\) & \(\BR_{10}\) & \(\BR_{14}\) & \(\BR_{16}\) & \(\BR_{20}\) & \(\BR_{23}\) & \(\BR_{27}\) & \(\BR_{28}\) & \(\BR_{30}\) & \(\BR_{35}\) & \(\BR_{37}\) & \(\BR_{40}\) \\
\(\BR_{130}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{132}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{136}\) &    0 &    0 &    1 &    0 &    0 &    1 &    0 &    0 &    0 &    0 &   -1 &    0 &    1 &    0 \\
\(\BR_{151}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{152}\) &   -1 &   -1 &   -3 &    0 &   -2 &    0 &   -1 &    0 &    2 &    0 &    2 &    0 &    0 &    0 \\
\(\BR_{167}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{800}\) &   -2 &   -2 &   -2 &    0 &   -3 &    0 &    0 &    0 &    0 &    0 &    1 &    0 &    0 &    0 \\
\(\BR_{802}\) &    1 &    1 &    1 &    0 &    0 &    0 &   -2 &    0 &   -1 &    0 &   -1 &    0 &    0 &    0 \\
\(\BR_{803}\) &    2 &    2 &    1 &    0 &    2 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    0 \\
\(\BR_{811}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{812}\) &    1 &    1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{821}\) &    0 &    0 &    2 &    0 &    0 &    1 &   -1 &    0 &   -1 &    0 &   -1 &    0 &    1 &    0 \\
\(\BR_{822}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{831}\) &    0 &    0 &    1 &    0 &    0 &    1 &    0 &    0 &    0 &    0 &   -1 &    0 &    1 &    0 \\[1.5ex]
 & \(\BR_{3}\) & \(\BR_{5}\) & \(\BR_{9}\) & \(\BR_{10}\) & \(\BR_{14}\) & \(\BR_{16}\) & \(\BR_{20}\) & \(\BR_{23}\) & \(\BR_{27}\) & \(\BR_{28}\) & \(\BR_{30}\) & \(\BR_{35}\) & \(\BR_{37}\) & \(\BR_{40}\) \\
\(\BR_{832}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{833}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{920}\) &    0 &    0 &    1 &    0 &    0 &    1 &    0 &    0 &    0 &    0 &   -1 &    0 &    1 &    0 \\
\(\BR_{945}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{980}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\[1.5ex]

 & \(\BR_{42}\) & \(\BR_{44}\) & \(\BR_{47}\) & \(\BR_{48}\) & \(\BR_{50}\) & \(\BR_{51}\) & \(\BR_{53}\) & \(\BR_{62}\) & \(\BR_{70}\) & \(\BR_{77}\) & \(\BR_{93}\) & \(\BR_{94}\) & \(\BR_{126}\) & \(\BR_{128}\) \\
\(\BR_{3}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -3 &   -6 &   -1 &    0 &    0 &    0 &    0 \\
\(\BR_{5}\) &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &   -4 &   -6 &    0 &   -1 &    0 &    0 &    0 \\
\(\BR_{9}\) &    0 &    0 &    2 &    0 &    0 &    0 &    0 &    8 &   -7 &   -3 &    3 &    0 &    0 &    1 \\
\(\BR_{10}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{14}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -3 &  -10 &   -2 &   -1 &    0 &    0 &    0 \\
\(\BR_{16}\) &   -3 &    0 &    2 &    0 &    0 &    0 &    0 &    4 &    0 &    0 &    2 &    0 &    0 &    1 \\
\(\BR_{20}\) &    1 &    0 &    0 &    0 &    0 &    0 &    0 &   -7 &   -1 &    0 &   -1 &    0 &   -1 &    0 \\
\(\BR_{23}\) &   -5 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 \\
\(\BR_{27}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -6 &   -1 &    2 &   -1 &    0 &    0 &    0 \\
\(\BR_{28}\) &   -5 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 \\
\(\BR_{30}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -5 &    3 &    2 &   -1 &    0 &   -2 &    0 \\
\(\BR_{35}\) &   -1 &   -1 &   -1 &   -3 &    1 &   -1 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{37}\) &  -14 &    0 &    3 &    0 &    5 &    0 &    0 &    3 &   -1 &    0 &    2 &    0 &    0 &    1 \\
\(\BR_{40}\) &  -20 &   -4 &   -4 &   -2 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\[1.5ex]
 & \(\BR_{42}\) & \(\BR_{44}\) & \(\BR_{47}\) & \(\BR_{48}\) & \(\BR_{50}\) & \(\BR_{51}\) & \(\BR_{53}\) & \(\BR_{62}\) & \(\BR_{70}\) & \(\BR_{77}\) & \(\BR_{93}\) & \(\BR_{94}\) & \(\BR_{126}\) & \(\BR_{128}\) \\
\(\BR_{42}\) &  100 &    0 &    1 &   -1 &    6 &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{44}\) &    0 &  100 &    0 &   -6 &    0 &   -3 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{47}\) &    1 &    0 &  100 &    0 &   -7 &    0 &    0 &    5 &   -1 &    0 &    2 &    0 &    0 &    1 \\
\(\BR_{48}\) &   -1 &   -6 &    0 &  100 &    0 &   -6 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{50}\) &    6 &    0 &   -7 &    0 &  100 &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{51}\) &    0 &   -3 &    0 &   -6 &    0 &  100 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{53}\) &    0 &    0 &    0 &    0 &    0 &    0 &  100 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{62}\) &   -1 &    0 &    5 &    0 &    1 &    0 &    0 &  100 &  -20 &   -1 &   16 &    0 &    1 &    2 \\
\(\BR_{70}\) &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &  -20 &  100 &   -7 &   -4 &   -1 &    0 &    0 \\
\(\BR_{77}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &   -7 &  100 &    0 &    0 &   -5 &    0 \\
\(\BR_{93}\) &    0 &    0 &    2 &    0 &    0 &    0 &    0 &   16 &   -4 &    0 &  100 &    0 &    0 &    1 \\
\(\BR_{94}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &  100 &    0 &    0 \\
\(\BR_{126}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    1 &    0 &   -5 &    0 &    0 &  100 &    4 \\
\(\BR_{128}\) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    2 &    0 &    0 &    1 &    0 &    4 &  100 \\[1.5ex]
 & \(\BR_{42}\) & \(\BR_{44}\) & \(\BR_{47}\) & \(\BR_{48}\) & \(\BR_{50}\) & \(\BR_{51}\) & \(\BR_{53}\) & \(\BR_{62}\) & \(\BR_{70}\) & \(\BR_{77}\) & \(\BR_{93}\) & \(\BR_{94}\) & \(\BR_{126}\) & \(\BR_{128}\) \\
\(\BR_{130}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    1 &    1 \\
\(\BR_{132}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    2 &    1 \\
\(\BR_{136}\) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    2 &   -1 &    0 &    1 &    0 &    0 &    0 \\
\(\BR_{151}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   12 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{152}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &  -11 &  -64 &    0 &    0 &    0 &    0 \\
\(\BR_{167}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    1 &    0 &    0 &    0 \\
\(\BR_{800}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -8 &  -67 &   -3 &   -1 &    0 &    0 &    0 \\
\(\BR_{802}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   20 &   -7 &    0 &    1 &    0 &    0 &    0 \\
\(\BR_{803}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -3 &  -14 &   -1 &   -1 &   -3 &    0 &   -1 \\
\(\BR_{811}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{812}\) &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &   -1 &   -1 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{821}\) &    0 &    0 &    2 &    0 &    0 &    0 &    0 &    3 &   -1 &    0 &    1 &    0 &    0 &    1 \\
\(\BR_{822}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{831}\) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    1 &   -1 &    0 &    1 &    0 &    0 &    0 \\[1.5ex]
 & \(\BR_{42}\) & \(\BR_{44}\) & \(\BR_{47}\) & \(\BR_{48}\) & \(\BR_{50}\) & \(\BR_{51}\) & \(\BR_{53}\) & \(\BR_{62}\) & \(\BR_{70}\) & \(\BR_{77}\) & \(\BR_{93}\) & \(\BR_{94}\) & \(\BR_{126}\) & \(\BR_{128}\) \\
\(\BR_{832}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{833}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{920}\) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    1 &   -1 &    0 &    1 &    0 &    0 &    0 \\
\(\BR_{945}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{980}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\[1.5ex]

 & \(\BR_{130}\) & \(\BR_{132}\) & \(\BR_{136}\) & \(\BR_{151}\) & \(\BR_{152}\) & \(\BR_{167}\) & \(\BR_{800}\) & \(\BR_{802}\) & \(\BR_{803}\) & \(\BR_{811}\) & \(\BR_{812}\) & \(\BR_{821}\) & \(\BR_{822}\) & \(\BR_{831}\) \\
\(\BR_{3}\) &    0 &    0 &    0 &    0 &   -1 &    0 &   -2 &    1 &    2 &    0 &    1 &    0 &    0 &    0 \\
\(\BR_{5}\) &    0 &    0 &    0 &    0 &   -1 &    0 &   -2 &    1 &    2 &    0 &    1 &    0 &    0 &    0 \\
\(\BR_{9}\) &    0 &    0 &    1 &    0 &   -3 &    0 &   -2 &    1 &    1 &    0 &    0 &    2 &    0 &    1 \\
\(\BR_{10}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{14}\) &    0 &    0 &    0 &    0 &   -2 &    0 &   -3 &    0 &    2 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{16}\) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    1 &    0 &    1 \\
\(\BR_{20}\) &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &   -2 &    0 &    0 &    0 &   -1 &    0 &    0 \\
\(\BR_{23}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{27}\) &    0 &    0 &    0 &    0 &    2 &    0 &    0 &   -1 &    0 &    0 &    0 &   -1 &    0 &    0 \\
\(\BR_{28}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{30}\) &    0 &    0 &   -1 &    0 &    2 &    0 &    1 &   -1 &   -1 &    0 &    0 &   -1 &    0 &   -1 \\
\(\BR_{35}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{37}\) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    1 &    0 &    1 \\
\(\BR_{40}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\[1.5ex]
 & \(\BR_{130}\) & \(\BR_{132}\) & \(\BR_{136}\) & \(\BR_{151}\) & \(\BR_{152}\) & \(\BR_{167}\) & \(\BR_{800}\) & \(\BR_{802}\) & \(\BR_{803}\) & \(\BR_{811}\) & \(\BR_{812}\) & \(\BR_{821}\) & \(\BR_{822}\) & \(\BR_{831}\) \\
\(\BR_{42}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{44}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{47}\) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    2 &    0 &    1 \\
\(\BR_{48}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{50}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    0 \\
\(\BR_{51}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{53}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{62}\) &    0 &    0 &    2 &    0 &   -1 &   -1 &   -8 &   20 &   -3 &    0 &   -1 &    3 &    0 &    1 \\
\(\BR_{70}\) &    0 &    0 &   -1 &   12 &  -11 &    0 &  -67 &   -7 &  -14 &   -1 &   -1 &   -1 &    0 &   -1 \\
\(\BR_{77}\) &   -1 &    0 &    0 &    0 &  -64 &    0 &   -3 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{93}\) &    0 &    0 &    1 &    0 &    0 &    1 &   -1 &    1 &   -1 &    0 &    0 &    1 &    0 &    1 \\
\(\BR_{94}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -3 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{126}\) &    1 &    2 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{128}\) &    1 &    1 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    1 &    0 &    0 \\[1.5ex]
 & \(\BR_{130}\) & \(\BR_{132}\) & \(\BR_{136}\) & \(\BR_{151}\) & \(\BR_{152}\) & \(\BR_{167}\) & \(\BR_{800}\) & \(\BR_{802}\) & \(\BR_{803}\) & \(\BR_{811}\) & \(\BR_{812}\) & \(\BR_{821}\) & \(\BR_{822}\) & \(\BR_{831}\) \\
\(\BR_{130}\) &  100 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{132}\) &    0 &  100 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &   -2 &    0 &    0 &    0 \\
\(\BR_{136}\) &    0 &    0 &  100 &    0 &    0 &    0 &    0 &    0 &    0 &   20 &   -8 &   46 &   -1 &   39 \\
\(\BR_{151}\) &    0 &    0 &    0 &  100 &    0 &    0 &  -14 &   -2 &  -58 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{152}\) &    0 &    0 &    0 &    0 &  100 &    0 &   -3 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{167}\) &    0 &    0 &    0 &    0 &    0 &  100 &    0 &    1 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{800}\) &    0 &    0 &    0 &  -14 &   -3 &    0 &  100 &   -2 &   10 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{802}\) &    0 &    0 &    0 &   -2 &    0 &    1 &   -2 &  100 &    0 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{803}\) &    0 &    0 &    0 &  -58 &   -1 &    0 &   10 &    0 &  100 &    0 &    0 &    0 &    0 &    0 \\
\(\BR_{811}\) &    0 &   -1 &   20 &    0 &    0 &    0 &    0 &    0 &    0 &  100 &  -16 &    8 &    0 &   14 \\
\(\BR_{812}\) &    0 &   -2 &   -8 &    0 &    0 &    0 &    0 &    0 &    0 &  -16 &  100 &   -4 &    0 &   -4 \\
\(\BR_{821}\) &    0 &    0 &   46 &    0 &    0 &    0 &    0 &    0 &    0 &    8 &   -4 &  100 &   -1 &   39 \\
\(\BR_{822}\) &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &  100 &   -1 \\
\(\BR_{831}\) &    0 &    0 &   39 &    0 &    0 &    0 &    0 &    0 &    0 &   14 &   -4 &   39 &   -1 &  100 \\[1.5ex]
 & \(\BR_{130}\) & \(\BR_{132}\) & \(\BR_{136}\) & \(\BR_{151}\) & \(\BR_{152}\) & \(\BR_{167}\) & \(\BR_{800}\) & \(\BR_{802}\) & \(\BR_{803}\) & \(\BR_{811}\) & \(\BR_{812}\) & \(\BR_{821}\) & \(\BR_{822}\) & \(\BR_{831}\) \\
\(\BR_{832}\) &    0 &    0 &    3 &    0 &    0 &    0 &    0 &    0 &    0 &    2 &    0 &    3 &    0 &   -2 \\
\(\BR_{833}\) &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &   -1 \\
\(\BR_{920}\) &    0 &    0 &   20 &    0 &    0 &    0 &    0 &    0 &    0 &    3 &   -2 &   34 &   -1 &   17 \\
\(\BR_{945}\) &    0 &   -1 &   25 &    0 &    0 &    0 &    0 &    0 &    0 &   10 &  -11 &   10 &    0 &   17 \\
\(\BR_{980}\) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\[1.5ex]

 & \(\BR_{832}\) & \(\BR_{833}\) & \(\BR_{920}\) & \(\BR_{945}\) & \(\BR_{980}\) &  &  &  &  &  &  &  &  &  \\
\(\BR_{3}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{5}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{9}\) &    0 &    0 &    1 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{10}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{14}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{16}\) &    0 &    0 &    1 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{20}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{23}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{27}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{28}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{30}\) &    0 &    0 &   -1 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{35}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{37}\) &    0 &    0 &    1 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{40}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\[1.5ex]
 & \(\BR_{832}\) & \(\BR_{833}\) & \(\BR_{920}\) & \(\BR_{945}\) & \(\BR_{980}\) &  &  &  &  &  &  &  &  &  \\
\(\BR_{42}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{44}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{47}\) &    0 &    0 &    1 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{48}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{50}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{51}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{53}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{62}\) &    0 &    0 &    1 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{70}\) &    0 &    0 &   -1 &   -1 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{77}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{93}\) &    0 &    0 &    1 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{94}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{126}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{128}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\[1.5ex]
 & \(\BR_{832}\) & \(\BR_{833}\) & \(\BR_{920}\) & \(\BR_{945}\) & \(\BR_{980}\) &  &  &  &  &  &  &  &  &  \\
\(\BR_{130}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{132}\) &    0 &    0 &    0 &   -1 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{136}\) &    3 &   -1 &   20 &   25 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{151}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{152}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{167}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{800}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{802}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{803}\) &    0 &    0 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{811}\) &    2 &    0 &    3 &   10 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{812}\) &    0 &    0 &   -2 &  -11 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{821}\) &    3 &   -1 &   34 &   10 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{822}\) &    0 &    0 &   -1 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{831}\) &   -2 &   -1 &   17 &   17 &    0 &      &      &      &      &      &      &      &      &      \\[1.5ex]
 & \(\BR_{832}\) & \(\BR_{833}\) & \(\BR_{920}\) & \(\BR_{945}\) & \(\BR_{980}\) &  &  &  &  &  &  &  &  &  \\
\(\BR_{832}\) &  100 &   -1 &    1 &    2 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{833}\) &   -1 &  100 &    0 &    0 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{920}\) &    1 &    0 &  100 &    4 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{945}\) &    2 &    0 &    4 &  100 &    0 &      &      &      &      &      &      &      &      &      \\
\(\BR_{980}\) &    0 &    0 &    0 &    0 &  100 &      &      &      &      &      &      &      &      &     %
}
\dxConstrDef{Gamma1}{\BR_{1}}{\BR_{3} + \BR_{5} + \BR_{9} + \BR_{10} + \BR_{14} + \BR_{16} \\
  {}& + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35} \\
  {}& + \BR_{40} + \BR_{44} + \BR_{37} + \BR_{42} + \BR_{47} + \BR_{48} \\
  {}& + \BR_{804} + \BR_{50} + \BR_{51} + \BR_{806} + \BR_{126}\cdot{}\BR_{\eta\to\text{neutral}} \\
  {}& + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{132}\cdot{}\BR_{\eta\to\text{neutral}} \\
  {}& + \BR_{800}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{151}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{152}\cdot{}\BR_{\omega\to\pi^0\gamma} \\
  {}& + \BR_{167}\cdot{}\BR_{\phi\to K_S K_L}}
\dxConstrDef{Gamma2}{\BR_{2}}{\BR_{3} + \BR_{5} + \BR_{9} + \BR_{10} + \BR_{14} + \BR_{16} \\
  {}& + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\\
  {}& +\BR_{<\bar{K}^0|K_L>}) + \BR_{40}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{44}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\\
  {}& +\BR_{<\bar{K}^0|K_L>}) + \BR_{37}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{42}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\\
  {}& +\BR_{<\bar{K}^0|K_L>}) + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{48}\cdot{}\BR_{K_S\to\pi^0\pi^0} \\
  {}& + \BR_{804} + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{51}\cdot{}\BR_{K_S\to\pi^0\pi^0} \\
  {}& + \BR_{806} + \BR_{126}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} \\
  {}& + \BR_{132}\cdot{}(\BR_{\eta\to\text{neutral}}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>})) + \BR_{800}\cdot{}\BR_{\omega\to\pi^0\gamma} \\
  {}& + \BR_{151}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{152}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{167}\cdot{}(\BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^0\pi^0})}
\dxConstrDef{Gamma3by5}{\BR_{3 / 5}}{\frac{\BR_{3}}{\BR_{5}}}
\dxConstrDef{Gamma7}{\BR_{7}}{\BR_{35}\cdot{}\BR_{<\bar{K}^0|K_L>} + \BR_{9} + \BR_{804} + \BR_{37}\cdot{}\BR_{<K^0|K_L>} \\
  {}& + \BR_{10}}
\dxConstrDef{Gamma8}{\BR_{8}}{\BR_{9} + \BR_{10}}
\dxConstrDef{Gamma8by5}{\BR_{8 / 5}}{\frac{\BR_{8}}{\BR_{5}}}
\dxConstrDef{Gamma9by5}{\BR_{9 / 5}}{\frac{\BR_{9}}{\BR_{5}}}
\dxConstrDef{Gamma10by5}{\BR_{10 / 5}}{\frac{\BR_{10}}{\BR_{5}}}
\dxConstrDef{Gamma10by9}{\BR_{10 / 9}}{\frac{\BR_{10}}{\BR_{9}}}
\dxConstrDef{Gamma11}{\BR_{11}}{\BR_{14} + \BR_{16} + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} \\
  {}& + \BR_{30} + \BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{126}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} \\
  {}& + \BR_{132}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to\text{neutral}}) + \BR_{151}\cdot{}\BR_{\omega\to\pi^0\gamma} \\
  {}& + \BR_{152}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{800}\cdot{}\BR_{\omega\to\pi^0\gamma}}
\dxConstrDef{Gamma12}{\BR_{12}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{30} + \BR_{23} + \BR_{28} + \BR_{14} \\
  {}& + \BR_{16} + \BR_{20} + \BR_{27} + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}
\dxConstrDef{Gamma13}{\BR_{13}}{\BR_{14} + \BR_{16}}
\dxConstrDef{Gamma17}{\BR_{17}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{30} + \BR_{23} + \BR_{28} + \BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{20} + \BR_{27} + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}
\dxConstrDef{Gamma18}{\BR_{18}}{\BR_{23} + \BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{20} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0})}
\dxConstrDef{Gamma19}{\BR_{19}}{\BR_{23} + \BR_{20}}
\dxConstrDef{Gamma19by13}{\BR_{19 / 13}}{\frac{\BR_{19}}{\BR_{13}}}
\dxConstrDef{Gamma24}{\BR_{24}}{\BR_{27} + \BR_{28} + \BR_{30} + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{128}\cdot{}\BR_{\eta\to3\pi^0} \\
  {}& + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{132}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to3\pi^0})}
\dxConstrDef{Gamma25}{\BR_{25}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{30} + \BR_{28} + \BR_{27} + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} \\
  {}& + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}
\dxConstrDef{Gamma26}{\BR_{26}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{28} + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{27}}
\dxConstrDef{Gamma26by13}{\BR_{26 / 13}}{\frac{\BR_{26}}{\BR_{13}}}
\dxConstrDef{Gamma29}{\BR_{29}}{\BR_{30} + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}
\dxConstrDef{Gamma31}{\BR_{31}}{\BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{23} + \BR_{28} + \BR_{42} + \BR_{16} \\
  {}& + \BR_{37} + \BR_{10} + \BR_{167}\cdot{}(\BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^0\pi^0})}
\dxConstrDef{Gamma32}{\BR_{32}}{\BR_{16} + \BR_{23} + \BR_{28} + \BR_{37} + \BR_{42} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} \\
  {}& + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{167}\cdot{}(\BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^0\pi^0})}
\dxConstrDef{Gamma33}{\BR_{33}}{\BR_{35}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{40}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{42}\cdot{}\BR_{<K^0|K_S>} \\
  {}& + \BR_{47} + \BR_{48} + \BR_{50} + \BR_{51} + \BR_{37}\cdot{}\BR_{<K^0|K_S>} \\
  {}& + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{\eta\to\text{neutral}}) + \BR_{44}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{167}\cdot{}\BR_{\phi\to K_S K_L}}
\dxConstrDef{Gamma34}{\BR_{34}}{\BR_{35} + \BR_{37}}
\dxConstrDef{Gamma38}{\BR_{38}}{\BR_{42} + \BR_{37}}
\dxConstrDef{Gamma39}{\BR_{39}}{\BR_{40} + \BR_{42}}
\dxConstrDef{Gamma43}{\BR_{43}}{\BR_{40} + \BR_{44}}
\dxConstrDef{Gamma46}{\BR_{46}}{\BR_{48} + \BR_{47} + \BR_{804}}
\dxConstrDef{Gamma49}{\BR_{49}}{\BR_{50} + \BR_{51} + \BR_{806}}
\dxConstrDef{Gamma54}{\BR_{54}}{\BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) \\
  {}& + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) \\
  {}& + \BR_{47}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{48}\cdot{}\BR_{K_S\to\pi^+\pi^-} \\
  {}& + \BR_{50}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{51}\cdot{}\BR_{K_S\to\pi^+\pi^-} \\
  {}& + \BR_{53}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{62} + \BR_{70} \\
  {}& + \BR_{77} + \BR_{78} + \BR_{93} + \BR_{94} + \BR_{126}\cdot{}\BR_{\eta\to\text{charged}} \\
  {}& + \BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{130}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_L>}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} \\
  {}& + \BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{\eta\to3\pi^0}) \\
  {}& + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) \\
  {}& + \BR_{167}\cdot{}(\BR_{\phi\to K^+K^-} + \BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{802} + \BR_{803} \\
  {}& + \BR_{800}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-})}
\dxConstrDef{Gamma55}{\BR_{55}}{\BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{78} \\
  {}& + \BR_{77} + \BR_{94} + \BR_{62} + \BR_{70} + \BR_{93} + \BR_{126}\cdot{}\BR_{\eta\to\text{charged}} \\
  {}& + \BR_{802} + \BR_{803} + \BR_{800}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}\\
  {}& +\BR_{\omega\to\pi^+\pi^-}) + \BR_{130}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{168}}
\dxConstrDef{Gamma56}{\BR_{56}}{\BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{62} + \BR_{93} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) \\
  {}& + \BR_{802} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{168}}
\dxConstrDef{Gamma57}{\BR_{57}}{\BR_{62} + \BR_{93} + \BR_{802} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-} \\
  {}& + \BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}
\dxConstrDef{Gamma57by55}{\BR_{57 / 55}}{\frac{\BR_{57}}{\BR_{55}}}
\dxConstrDef{Gamma58}{\BR_{58}}{\BR_{62} + \BR_{93} + \BR_{802} + \BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}
\dxConstrDef{Gamma59}{\BR_{59}}{\BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{62} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-}}
\dxConstrDef{Gamma60}{\BR_{60}}{\BR_{62} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-}}
\dxConstrDef{Gamma63}{\BR_{63}}{\BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) \\
  {}& + \BR_{47}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{70} + \BR_{77} + \BR_{78} + \BR_{94} + \BR_{126}\cdot{}\BR_{\eta\to\text{charged}} \\
  {}& + \BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{130}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{\eta\to\text{neutral}} \\
  {}& + \BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to\text{charged}}) + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}\\
  {}& +\BR_{\omega\to\pi^+\pi^-}) + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}
\dxConstrDef{Gamma64}{\BR_{64}}{\BR_{78} + \BR_{77} + \BR_{94} + \BR_{70} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} \\
  {}& + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} \\
  {}& + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{803}}
\dxConstrDef{Gamma65}{\BR_{65}}{\BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) \\
  {}& + \BR_{70} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} \\
  {}& + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}
\dxConstrDef{Gamma66}{\BR_{66}}{\BR_{70} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} \\
  {}& + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}
\dxConstrDef{Gamma67}{\BR_{67}}{\BR_{70} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{803}}
\dxConstrDef{Gamma68}{\BR_{68}}{\BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{70} + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} \\
  {}& + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma69}{\BR_{69}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{70} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma74}{\BR_{74}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{78} + \BR_{77} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} \\
  {}& + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma75}{\BR_{75}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{47}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) \\
  {}& + \BR_{77} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma76}{\BR_{76}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{77} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma76by54}{\BR_{76 / 54}}{\frac{\BR_{76}}{\BR_{54}}}
\dxConstrDef{Gamma78}{\BR_{78}}{\BR_{810} + \BR_{50}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{\eta\to3\pi^0})}
\dxConstrDef{Gamma79}{\BR_{79}}{\BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) \\
  {}& + \BR_{93} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}\\
  {}& +\BR_{\omega\to\pi^+\pi^-}) + \BR_{168} + \BR_{802} + \BR_{803}}
\dxConstrDef{Gamma80}{\BR_{80}}{\BR_{93} + \BR_{802} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-}}
\dxConstrDef{Gamma80by60}{\BR_{80 / 60}}{\frac{\BR_{80}}{\BR_{60}}}
\dxConstrDef{Gamma81}{\BR_{81}}{\BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{94} + \BR_{803} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma81by69}{\BR_{81 / 69}}{\frac{\BR_{81}}{\BR_{69}}}
\dxConstrDef{Gamma82}{\BR_{82}}{\BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{802} \\
  {}& + \BR_{803} + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})}
\dxConstrDef{Gamma83}{\BR_{83}}{\BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{802} + \BR_{803} + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}\\
  {}& +\BR_{\omega\to\pi^+\pi^-})}
\dxConstrDef{Gamma84}{\BR_{84}}{\BR_{802} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})}
\dxConstrDef{Gamma85}{\BR_{85}}{\BR_{802} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-}}
\dxConstrDef{Gamma85by60}{\BR_{85 / 60}}{\frac{\BR_{85}}{\BR_{60}}}
\dxConstrDef{Gamma87}{\BR_{87}}{\BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} \\
  {}& + \BR_{803}}
\dxConstrDef{Gamma88}{\BR_{88}}{\BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{803} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma89}{\BR_{89}}{\BR_{803} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma92}{\BR_{92}}{\BR_{94} + \BR_{93}}
\dxConstrDef{Gamma93by60}{\BR_{93 / 60}}{\frac{\BR_{93}}{\BR_{60}}}
\dxConstrDef{Gamma94by69}{\BR_{94 / 69}}{\frac{\BR_{94}}{\BR_{69}}}
\dxConstrDef{Gamma96}{\BR_{96}}{\BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}
\dxConstrDef{Gamma102}{\BR_{102}}{\BR_{103} + \BR_{104}}
\dxConstrDef{Gamma103}{\BR_{103}}{\BR_{820} + \BR_{822} + \BR_{831}\cdot{}\BR_{\omega\to\pi^+\pi^-}}
\dxConstrDef{Gamma104}{\BR_{104}}{\BR_{830} + \BR_{833}}
\dxConstrDef{Gamma106}{\BR_{106}}{\BR_{30} + \BR_{44}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{47} + \BR_{53}\cdot{}\BR_{<K^0|K_S>} \\
  {}& + \BR_{77} + \BR_{103} + \BR_{126}\cdot{}(\BR_{\eta\to3\pi^0}+\BR_{\eta\to\pi^+\pi^-\pi^0}) + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma110}{\BR_{110}}{\BR_{10} + \BR_{16} + \BR_{23} + \BR_{28} + \BR_{35} + \BR_{40} \\
  {}& + \BR_{128} + \BR_{802} + \BR_{803} + \BR_{151} + \BR_{130} + \BR_{132} \\
  {}& + \BR_{44} + \BR_{53} + \BR_{168} + \BR_{169} + \BR_{822} + \BR_{833}}
\dxConstrDef{Gamma149}{\BR_{149}}{\BR_{152} + \BR_{800} + \BR_{151}}
\dxConstrDef{Gamma150}{\BR_{150}}{\BR_{800} + \BR_{151}}
\dxConstrDef{Gamma150by66}{\BR_{150 / 66}}{\frac{\BR_{150}}{\BR_{66}}}
\dxConstrDef{Gamma152by54}{\BR_{152 / 54}}{\frac{\BR_{152}}{\BR_{54}}}
\dxConstrDef{Gamma152by76}{\BR_{152 / 76}}{\frac{\BR_{152}}{\BR_{76}}}
\dxConstrDef{Gamma168}{\BR_{168}}{\BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}
\dxConstrDef{Gamma169}{\BR_{169}}{\BR_{167}\cdot{}\BR_{\phi\to K_S K_L}}
\dxConstrDef{Gamma804}{\BR_{804}}{\BR_{47} \cdot{} ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))}
\dxConstrDef{Gamma805}{\BR_{805}}{\BR_{980}/(1-\BR_{980})\cdot{}(\BR_{20} + \BR_{62})}
\dxConstrDef{Gamma806}{\BR_{806}}{\BR_{50} \cdot{} ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))}
\dxConstrDef{Gamma810}{\BR_{810}}{\BR_{910} + \BR_{911} + \BR_{811}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{812}}
\dxConstrDef{Gamma820}{\BR_{820}}{\BR_{920} + \BR_{821}}
\dxConstrDef{Gamma830}{\BR_{830}}{\BR_{930} + \BR_{831}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{832}}
\dxConstrDef{Gamma910}{\BR_{910}}{\BR_{136}\cdot{}\BR_{\eta\to3\pi^0}}
\dxConstrDef{Gamma911}{\BR_{911}}{\BR_{945}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma930}{\BR_{930}}{\BR_{136}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}
\dxConstrDef{Gamma944}{\BR_{944}}{\BR_{136}\cdot{}\BR_{\eta\to\gamma\gamma}}
\dxConstrDef{GammaUnitResid}{\BR_{\text{ur}}}{1 - \BR_{\text{all}}}
\dxConstrDef{GammaAll}{\BR_{\text{all}}}{\BR_{3} + \BR_{5} + \BR_{9} + \BR_{10} + \BR_{14} + \BR_{16} \\
  {}& + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35} \\
  {}& + \BR_{37} + \BR_{40} + \BR_{42} + \BR_{47}\cdot{}(1 + ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))) \\
  {}& + \BR_{48} + \BR_{62} + \BR_{70} + \BR_{77} + \BR_{811} + \BR_{812} \\
  {}& + \BR_{93} + \BR_{94} + \BR_{832} + \BR_{833} + \BR_{126} + \BR_{128} \\
  {}& + \BR_{802} + \BR_{803} + \BR_{800} + \BR_{151} + \BR_{130} + \BR_{132} \\
  {}& + \BR_{44} + \BR_{53} + \BR_{50}\cdot{}(1 + ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))) \\
  {}& + \BR_{51} + \BR_{167}\cdot{}(\BR_{\phi\to K^+K^-}+\BR_{\phi\to K_S K_L}) + \BR_{152} + \BR_{920} \\
  {}& + \BR_{821} + \BR_{822} + \BR_{831} + \BR_{136} + \BR_{945} + \BR_{805}}
\dxdef{TauBrConstrEqs}{%
\begin{align*}
\dxuse{Gamma1-left} ={}& \dxuse{Gamma1-right}
\end{align*}
\begin{align*}
\dxuse{Gamma2-left} ={}& \dxuse{Gamma2-right}
\end{align*}
\begin{align*}
\dxuse{Gamma3by5-left} ={}& \dxuse{Gamma3by5-right}
\end{align*}
\begin{align*}
\dxuse{Gamma7-left} ={}& \dxuse{Gamma7-right}
\end{align*}
\begin{align*}
\dxuse{Gamma8-left} ={}& \dxuse{Gamma8-right}
\end{align*}
\begin{align*}
\dxuse{Gamma8by5-left} ={}& \dxuse{Gamma8by5-right}
\end{align*}
\begin{align*}
\dxuse{Gamma9by5-left} ={}& \dxuse{Gamma9by5-right}
\end{align*}
\begin{align*}
\dxuse{Gamma10by5-left} ={}& \dxuse{Gamma10by5-right}
\end{align*}
\begin{align*}
\dxuse{Gamma10by9-left} ={}& \dxuse{Gamma10by9-right}
\end{align*}
\begin{align*}
\dxuse{Gamma11-left} ={}& \dxuse{Gamma11-right}
\end{align*}
\begin{align*}
\dxuse{Gamma12-left} ={}& \dxuse{Gamma12-right}
\end{align*}
\begin{align*}
\dxuse{Gamma13-left} ={}& \dxuse{Gamma13-right}
\end{align*}
\begin{align*}
\dxuse{Gamma17-left} ={}& \dxuse{Gamma17-right}
\end{align*}
\begin{align*}
\dxuse{Gamma18-left} ={}& \dxuse{Gamma18-right}
\end{align*}
\begin{align*}
\dxuse{Gamma19-left} ={}& \dxuse{Gamma19-right}
\end{align*}
\begin{align*}
\dxuse{Gamma19by13-left} ={}& \dxuse{Gamma19by13-right}
\end{align*}
\begin{align*}
\dxuse{Gamma24-left} ={}& \dxuse{Gamma24-right}
\end{align*}
\begin{align*}
\dxuse{Gamma25-left} ={}& \dxuse{Gamma25-right}
\end{align*}
\begin{align*}
\dxuse{Gamma26-left} ={}& \dxuse{Gamma26-right}
\end{align*}
\begin{align*}
\dxuse{Gamma26by13-left} ={}& \dxuse{Gamma26by13-right}
\end{align*}
\begin{align*}
\dxuse{Gamma29-left} ={}& \dxuse{Gamma29-right}
\end{align*}
\begin{align*}
\dxuse{Gamma31-left} ={}& \dxuse{Gamma31-right}
\end{align*}
\begin{align*}
\dxuse{Gamma32-left} ={}& \dxuse{Gamma32-right}
\end{align*}
\begin{align*}
\dxuse{Gamma33-left} ={}& \dxuse{Gamma33-right}
\end{align*}
\begin{align*}
\dxuse{Gamma34-left} ={}& \dxuse{Gamma34-right}
\end{align*}
\begin{align*}
\dxuse{Gamma38-left} ={}& \dxuse{Gamma38-right}
\end{align*}
\begin{align*}
\dxuse{Gamma39-left} ={}& \dxuse{Gamma39-right}
\end{align*}
\begin{align*}
\dxuse{Gamma43-left} ={}& \dxuse{Gamma43-right}
\end{align*}
\begin{align*}
\dxuse{Gamma46-left} ={}& \dxuse{Gamma46-right}
\end{align*}
\begin{align*}
\dxuse{Gamma49-left} ={}& \dxuse{Gamma49-right}
\end{align*}
\begin{align*}
\dxuse{Gamma54-left} ={}& \dxuse{Gamma54-right}
\end{align*}
\begin{align*}
\dxuse{Gamma55-left} ={}& \dxuse{Gamma55-right}
\end{align*}
\begin{align*}
\dxuse{Gamma56-left} ={}& \dxuse{Gamma56-right}
\end{align*}
\begin{align*}
\dxuse{Gamma57-left} ={}& \dxuse{Gamma57-right}
\end{align*}
\begin{align*}
\dxuse{Gamma57by55-left} ={}& \dxuse{Gamma57by55-right}
\end{align*}
\begin{align*}
\dxuse{Gamma58-left} ={}& \dxuse{Gamma58-right}
\end{align*}
\begin{align*}
\dxuse{Gamma59-left} ={}& \dxuse{Gamma59-right}
\end{align*}
\begin{align*}
\dxuse{Gamma60-left} ={}& \dxuse{Gamma60-right}
\end{align*}
\begin{align*}
\dxuse{Gamma63-left} ={}& \dxuse{Gamma63-right}
\end{align*}
\begin{align*}
\dxuse{Gamma64-left} ={}& \dxuse{Gamma64-right}
\end{align*}
\begin{align*}
\dxuse{Gamma65-left} ={}& \dxuse{Gamma65-right}
\end{align*}
\begin{align*}
\dxuse{Gamma66-left} ={}& \dxuse{Gamma66-right}
\end{align*}
\begin{align*}
\dxuse{Gamma67-left} ={}& \dxuse{Gamma67-right}
\end{align*}
\begin{align*}
\dxuse{Gamma68-left} ={}& \dxuse{Gamma68-right}
\end{align*}
\begin{align*}
\dxuse{Gamma69-left} ={}& \dxuse{Gamma69-right}
\end{align*}
\begin{align*}
\dxuse{Gamma74-left} ={}& \dxuse{Gamma74-right}
\end{align*}
\begin{align*}
\dxuse{Gamma75-left} ={}& \dxuse{Gamma75-right}
\end{align*}
\begin{align*}
\dxuse{Gamma76-left} ={}& \dxuse{Gamma76-right}
\end{align*}
\begin{align*}
\dxuse{Gamma76by54-left} ={}& \dxuse{Gamma76by54-right}
\end{align*}
\begin{align*}
\dxuse{Gamma78-left} ={}& \dxuse{Gamma78-right}
\end{align*}
\begin{align*}
\dxuse{Gamma79-left} ={}& \dxuse{Gamma79-right}
\end{align*}
\begin{align*}
\dxuse{Gamma80-left} ={}& \dxuse{Gamma80-right}
\end{align*}
\begin{align*}
\dxuse{Gamma80by60-left} ={}& \dxuse{Gamma80by60-right}
\end{align*}
\begin{align*}
\dxuse{Gamma81-left} ={}& \dxuse{Gamma81-right}
\end{align*}
\begin{align*}
\dxuse{Gamma81by69-left} ={}& \dxuse{Gamma81by69-right}
\end{align*}
\begin{align*}
\dxuse{Gamma82-left} ={}& \dxuse{Gamma82-right}
\end{align*}
\begin{align*}
\dxuse{Gamma83-left} ={}& \dxuse{Gamma83-right}
\end{align*}
\begin{align*}
\dxuse{Gamma84-left} ={}& \dxuse{Gamma84-right}
\end{align*}
\begin{align*}
\dxuse{Gamma85-left} ={}& \dxuse{Gamma85-right}
\end{align*}
\begin{align*}
\dxuse{Gamma85by60-left} ={}& \dxuse{Gamma85by60-right}
\end{align*}
\begin{align*}
\dxuse{Gamma87-left} ={}& \dxuse{Gamma87-right}
\end{align*}
\begin{align*}
\dxuse{Gamma88-left} ={}& \dxuse{Gamma88-right}
\end{align*}
\begin{align*}
\dxuse{Gamma89-left} ={}& \dxuse{Gamma89-right}
\end{align*}
\begin{align*}
\dxuse{Gamma92-left} ={}& \dxuse{Gamma92-right}
\end{align*}
\begin{align*}
\dxuse{Gamma93by60-left} ={}& \dxuse{Gamma93by60-right}
\end{align*}
\begin{align*}
\dxuse{Gamma94by69-left} ={}& \dxuse{Gamma94by69-right}
\end{align*}
\begin{align*}
\dxuse{Gamma96-left} ={}& \dxuse{Gamma96-right}
\end{align*}
\begin{align*}
\dxuse{Gamma102-left} ={}& \dxuse{Gamma102-right}
\end{align*}
\begin{align*}
\dxuse{Gamma103-left} ={}& \dxuse{Gamma103-right}
\end{align*}
\begin{align*}
\dxuse{Gamma104-left} ={}& \dxuse{Gamma104-right}
\end{align*}
\begin{align*}
\dxuse{Gamma106-left} ={}& \dxuse{Gamma106-right}
\end{align*}
\begin{align*}
\dxuse{Gamma110-left} ={}& \dxuse{Gamma110-right}
\end{align*}
\begin{align*}
\dxuse{Gamma149-left} ={}& \dxuse{Gamma149-right}
\end{align*}
\begin{align*}
\dxuse{Gamma150-left} ={}& \dxuse{Gamma150-right}
\end{align*}
\begin{align*}
\dxuse{Gamma150by66-left} ={}& \dxuse{Gamma150by66-right}
\end{align*}
\begin{align*}
\dxuse{Gamma152by54-left} ={}& \dxuse{Gamma152by54-right}
\end{align*}
\begin{align*}
\dxuse{Gamma152by76-left} ={}& \dxuse{Gamma152by76-right}
\end{align*}
\begin{align*}
\dxuse{Gamma168-left} ={}& \dxuse{Gamma168-right}
\end{align*}
\begin{align*}
\dxuse{Gamma169-left} ={}& \dxuse{Gamma169-right}
\end{align*}
\begin{align*}
\dxuse{Gamma804-left} ={}& \dxuse{Gamma804-right}
\end{align*}
\begin{align*}
\dxuse{Gamma805-left} ={}& \dxuse{Gamma805-right}
\end{align*}
\begin{align*}
\dxuse{Gamma806-left} ={}& \dxuse{Gamma806-right}
\end{align*}
\begin{align*}
\dxuse{Gamma810-left} ={}& \dxuse{Gamma810-right}
\end{align*}
\begin{align*}
\dxuse{Gamma820-left} ={}& \dxuse{Gamma820-right}
\end{align*}
\begin{align*}
\dxuse{Gamma830-left} ={}& \dxuse{Gamma830-right}
\end{align*}
\begin{align*}
\dxuse{Gamma910-left} ={}& \dxuse{Gamma910-right}
\end{align*}
\begin{align*}
\dxuse{Gamma911-left} ={}& \dxuse{Gamma911-right}
\end{align*}
\begin{align*}
\dxuse{Gamma930-left} ={}& \dxuse{Gamma930-right}
\end{align*}
\begin{align*}
\dxuse{Gamma944-left} ={}& \dxuse{Gamma944-right}
\end{align*}
\begin{align*}
\dxuse{GammaUnitResid-left} ={}& \dxuse{GammaUnitResid-right}
\end{align*}
\begin{align*}
\dxuse{GammaAll-left} ={}& \dxuse{GammaAll-right}
\end{align*}%
}


==> tau/avg-taulife-2023.tex <==
\dxdef{TauLifeMeasNum}{6}
\dxdef{TauLifeMeasNumAll}{6}
\dxdef{TauLifeMeasNumNuisance}{0}
\dxdef{TauLifeQuantNum}{1}
\dxdef{TauLifeQuantNumAll}{1}
\dxdef{TauLifeQuantNumNuisance}{0}
\dxdef{TauLifeBaseQuantNum}{1}
\dxdef{TauLifeBaseVarNum}{1}
\dxdef{TauLifeConstrNum}{0}
\dxdef{TauLifeChisq}{1.87}
\dxdef{TauLifeDof}{5}
\dxdef{TauLifeChisqProb}{87\%}
\dxdef{TauLifeChisq_full}{1.87}
\dxdef{TauLifeDof_full}{5}
\dxdef{TauLifeChisqProb_full}{87\%}
\dxdef{TauLifeNumMeasALEPH}{1}
\dxdef{TauLifeNumMeasBelle}{1}
\dxdef{TauLifeNumMeasCLEO}{1}
\dxdef{TauLifeNumMeasDELPHI}{1}
\dxdef{TauLifeNumMeasL3}{1}
\dxdef{TauLifeNumMeasOPAL}{1}
\dxQuantDef{tau_life}{tau_life}{\tau lifetime [fs]}{290.29 \pm 0.53}{290.29}{\pm 0.53}
\dxMeasDef{ALEPH.tau_life.pub.BARATE.1997R}{tau_life}{BARATE 1997R}{290.10 \pm 1.50 \pm 1.10}{290.10}{\pm 1.50}{\pm 1.10}
\dxMeasDef{Belle.tau_life.pub.BELOUS.2014}{tau_life}{BELOUS 2014}{290.17 \pm 0.53 \pm 0.33}{290.17}{\pm 0.53}{\pm 0.33}
\dxMeasDef{CLEO.tau_life.pub.BALEST.1996}{tau_life}{BALEST 1996}{289.00 \pm 2.80 \pm 4.00}{289.00}{\pm 2.80}{\pm 4.00}
\dxMeasDef{DELPHI.tau_life.pub.ABDALLAH.2004T}{tau_life}{ABDALLAH 2004T}{290.90 \pm 1.40 \pm 1.00}{290.90}{\pm 1.40}{\pm 1.00}
\dxMeasDef{L3.tau_life.pub.ACCIARRI.2000B}{tau_life}{ACCIARRI 2000B}{293.20 \pm 2.00 \pm 1.50}{293.20}{\pm 2.00}{\pm 1.50}
\dxMeasDef{OPAL.tau_life.pub.ALEXANDER.1996E}{tau_life}{ALEXANDER 1996E}{289.20 \pm 1.70 \pm 1.20}{289.20}{\pm 1.70}{\pm 1.20}
\dxdef{tau_life-qm}{%
\dxuse{ALEPH.tau_life.pub.BARATE.1997R-vu} & \dxuse{\dxuse{ALEPH.tau_life.pub.BARATE.1997R-pdgref}-exp} & \dxuse{\dxuse{ALEPH.tau_life.pub.BARATE.1997R-pdgref}-cite} \\
\dxuse{Belle.tau_life.pub.BELOUS.2014-vu} & \dxuse{\dxuse{Belle.tau_life.pub.BELOUS.2014-pdgref}-exp} & \dxuse{\dxuse{Belle.tau_life.pub.BELOUS.2014-pdgref}-cite} \\
\dxuse{CLEO.tau_life.pub.BALEST.1996-vu} & \dxuse{\dxuse{CLEO.tau_life.pub.BALEST.1996-pdgref}-exp} & \dxuse{\dxuse{CLEO.tau_life.pub.BALEST.1996-pdgref}-cite} \\
\dxuse{DELPHI.tau_life.pub.ABDALLAH.2004T-vu} & \dxuse{\dxuse{DELPHI.tau_life.pub.ABDALLAH.2004T-pdgref}-exp} & \dxuse{\dxuse{DELPHI.tau_life.pub.ABDALLAH.2004T-pdgref}-cite} \\
\dxuse{L3.tau_life.pub.ACCIARRI.2000B-vu} & \dxuse{\dxuse{L3.tau_life.pub.ACCIARRI.2000B-pdgref}-exp} & \dxuse{\dxuse{L3.tau_life.pub.ACCIARRI.2000B-pdgref}-cite} \\
\dxuse{OPAL.tau_life.pub.ALEXANDER.1996E-vu} & \dxuse{\dxuse{OPAL.tau_life.pub.ALEXANDER.1996E-pdgref}-exp} & \dxuse{\dxuse{OPAL.tau_life.pub.ALEXANDER.1996E-pdgref}-cite}%
}
\dxdef{TauLifeQuantMeasTable}{%
\dxuse{tau_life-qm}%
}
\dxdef{BARATE 1997R-ref}{ALEPH:1997roz}
\dxdef{BARATE 1997R-cite}{\cite{ALEPH:1997roz}}
\dxdef{BARATE 1997R-exp}{ALEPH}
\dxdef{BARATE 1997R-type}{pub}
\dxdef{BARATE 1997R-label}{BARATE 1997R (ALEPH)}
\dxdef{BARATE 1997R-meas}{%
\multicolumn{2}{l}{\dxuse{BARATE 1997R-label}\,\dxuse{BARATE 1997R-cite}} \\
\begin{ensuredisplaymath}
\dxuse{tau_life-gn} = \dxuse{tau_life-td}
\end{ensuredisplaymath} & \dxuse{ALEPH.tau_life.pub.BARATE.1997R-vu}%
}
\dxdef{BELOUS 2014-ref}{Belle:2013teo}
\dxdef{BELOUS 2014-cite}{\cite{Belle:2013teo}}
\dxdef{BELOUS 2014-exp}{Belle}
\dxdef{BELOUS 2014-type}{pub}
\dxdef{BELOUS 2014-label}{BELOUS 2014 (Belle)}
\dxdef{BELOUS 2014-meas}{%
\multicolumn{2}{l}{\dxuse{BELOUS 2014-label}\,\dxuse{BELOUS 2014-cite}} \\
\begin{ensuredisplaymath}
\dxuse{tau_life-gn} = \dxuse{tau_life-td}
\end{ensuredisplaymath} & \dxuse{Belle.tau_life.pub.BELOUS.2014-vu}%
}
\dxdef{BALEST 1996-ref}{CLEO:1996hqs}
\dxdef{BALEST 1996-cite}{\cite{CLEO:1996hqs}}
\dxdef{BALEST 1996-exp}{CLEO}
\dxdef{BALEST 1996-type}{pub}
\dxdef{BALEST 1996-label}{BALEST 1996 (CLEO)}
\dxdef{BALEST 1996-meas}{%
\multicolumn{2}{l}{\dxuse{BALEST 1996-label}\,\dxuse{BALEST 1996-cite}} \\
\begin{ensuredisplaymath}
\dxuse{tau_life-gn} = \dxuse{tau_life-td}
\end{ensuredisplaymath} & \dxuse{CLEO.tau_life.pub.BALEST.1996-vu}%
}
\dxdef{ABDALLAH 2004T-ref}{DELPHI:2003zcz}
\dxdef{ABDALLAH 2004T-cite}{\cite{DELPHI:2003zcz}}
\dxdef{ABDALLAH 2004T-exp}{DELPHI}
\dxdef{ABDALLAH 2004T-type}{pub}
\dxdef{ABDALLAH 2004T-label}{ABDALLAH 2004T (DELPHI)}
\dxdef{ABDALLAH 2004T-meas}{%
\multicolumn{2}{l}{\dxuse{ABDALLAH 2004T-label}\,\dxuse{ABDALLAH 2004T-cite}} \\
\begin{ensuredisplaymath}
\dxuse{tau_life-gn} = \dxuse{tau_life-td}
\end{ensuredisplaymath} & \dxuse{DELPHI.tau_life.pub.ABDALLAH.2004T-vu}%
}
\dxdef{ACCIARRI 2000B-ref}{L3:2000dya}
\dxdef{ACCIARRI 2000B-cite}{\cite{L3:2000dya}}
\dxdef{ACCIARRI 2000B-exp}{L3}
\dxdef{ACCIARRI 2000B-type}{pub}
\dxdef{ACCIARRI 2000B-label}{ACCIARRI 2000B (L3)}
\dxdef{ACCIARRI 2000B-meas}{%
\multicolumn{2}{l}{\dxuse{ACCIARRI 2000B-label}\,\dxuse{ACCIARRI 2000B-cite}} \\
\begin{ensuredisplaymath}
\dxuse{tau_life-gn} = \dxuse{tau_life-td}
\end{ensuredisplaymath} & \dxuse{L3.tau_life.pub.ACCIARRI.2000B-vu}%
}
\dxdef{ALEXANDER 1996E-ref}{OPAL:1996dap}
\dxdef{ALEXANDER 1996E-cite}{\cite{OPAL:1996dap}}
\dxdef{ALEXANDER 1996E-exp}{OPAL}
\dxdef{ALEXANDER 1996E-type}{pub}
\dxdef{ALEXANDER 1996E-label}{ALEXANDER 1996E (OPAL)}
\dxdef{ALEXANDER 1996E-meas}{%
\multicolumn{2}{l}{\dxuse{ALEXANDER 1996E-label}\,\dxuse{ALEXANDER 1996E-cite}} \\
\begin{ensuredisplaymath}
\dxuse{tau_life-gn} = \dxuse{tau_life-td}
\end{ensuredisplaymath} & \dxuse{OPAL.tau_life.pub.ALEXANDER.1996E-vu}%
}
\dxdef{TauLifeMeasByRef}{%
\dxuse{BARATE 1997R-meas} \\[1.5ex]
\dxuse{BELOUS 2014-meas} \\[1.5ex]
\dxuse{BALEST 1996-meas} \\[1.5ex]
\dxuse{ABDALLAH 2004T-meas} \\[1.5ex]
\dxuse{ACCIARRI 2000B-meas} \\[1.5ex]
\dxuse{ALEXANDER 1996E-meas}%
}


==> tau/avg-taumass-2023.tex <==
\dxdef{TauMassMeasNum}{10}
\dxdef{TauMassMeasNumAll}{10}
\dxdef{TauMassMeasNumNuisance}{0}
\dxdef{TauMassQuantNum}{1}
\dxdef{TauMassQuantNumAll}{1}
\dxdef{TauMassQuantNumNuisance}{0}
\dxdef{TauMassBaseQuantNum}{1}
\dxdef{TauMassBaseVarNum}{1}
\dxdef{TauMassConstrNum}{0}
\dxdef{TauMassChisq}{8.2}
\dxdef{TauMassDof}{9}
\dxdef{TauMassChisqProb}{51\%}
\dxdef{TauMassChisq_full}{8.2}
\dxdef{TauMassDof_full}{9}
\dxdef{TauMassChisqProb_full}{51\%}
\dxdef{TauMassNumMeasARGUS}{1}
\dxdef{TauMassNumMeasBABAR}{1}
\dxdef{TauMassNumMeasBELLE}{1}
\dxdef{TauMassNumMeasBelle2}{1}
\dxdef{TauMassNumMeasBES}{1}
\dxdef{TauMassNumMeasBES3}{1}
\dxdef{TauMassNumMeasCLEO}{1}
\dxdef{TauMassNumMeasDELCO}{1}
\dxdef{TauMassNumMeasKEDR}{1}
\dxdef{TauMassNumMeasOPAL}{1}
\dxQuantDef{tau_mass}{tau_mass}{\tau mass [MeV]}{1776.94 \pm 0.09}{1776.94}{\pm 0.09}
\dxMeasDef{ARGUS.tau_mass.pub.ALBRECHT.1992M}{tau_mass}{ALBRECHT 1992M}{1776.30 \pm 2.40 \pm 1.40}{1776.30}{\pm 2.40}{\pm 1.40}
\dxMeasDef{BABAR.tau_mass.pub.AUBERT.2009AK}{tau_mass}{AUBERT 2009AK}{1776.68 \pm 0.12 \pm 0.41}{1776.68}{\pm 0.12}{\pm 0.41}
\dxMeasDef{BELLE.tau_mass.pub.BELOUS.2007}{tau_mass}{BELOUS 2007}{1776.61 \pm 0.13 \pm 0.35}{1776.61}{\pm 0.13}{\pm 0.35}
\dxMeasDef{Belle2.tau_mass.pub.ADACHI.2023C}{tau_mass}{ADACHI 2023C}{1777.09 \pm 0.08 \pm 0.11}{1777.09}{\pm 0.08}{\pm 0.11}
\dxMeasDef{BES.tau_mass.pub.BAI.1996}{tau_mass}{BAI 1996}{1776.96 {}^{+0.18}_{-0.21} {}^{+0.25}_{-0.17}}{1776.96}{{}^{+0.18}_{-0.21}}{{}^{+0.25}_{-0.17}}
\dxMeasDef{BES3.tau_mass.pub.ABLIKIM.2014D}{tau_mass}{ABLIKIM 2014D}{1776.91 \pm 0.12 {}^{+0.10}_{-0.13}}{1776.91}{\pm 0.12}{{}^{+0.10}_{-0.13}}
\dxMeasDef{CLEO.tau_mass.pub.ANASTASSOV.1997}{tau_mass}{ANASTASSOV 1997}{1778.20 \pm 0.80 \pm 1.20}{1778.20}{\pm 0.80}{\pm 1.20}
\dxMeasDef{DELCO.tau_mass.pub.BACINO.1978B}{tau_mass}{BACINO 1978B}{1783.00 {}^{+3.00}_{-4.00} \pm 0.00}{1783.00}{{}^{+3.00}_{-4.00}}{\pm 0.00}
\dxMeasDef{KEDR.tau_mass.pub.ANASHIN.2023A}{tau_mass}{ANASHIN 2023A}{1776.69 {}^{+0.17}_{-0.19} \pm 0.15}{1776.69}{{}^{+0.17}_{-0.19}}{\pm 0.15}
\dxMeasDef{OPAL.tau_mass.pub.ABBIENDI.2000A}{tau_mass}{ABBIENDI 2000A}{1775.10 \pm 1.60 \pm 1.00}{1775.10}{\pm 1.60}{\pm 1.00}
\dxdef{tau_mass-qm}{%
\dxuse{ARGUS.tau_mass.pub.ALBRECHT.1992M-vu} & \dxuse{\dxuse{ARGUS.tau_mass.pub.ALBRECHT.1992M-pdgref}-exp} & \dxuse{\dxuse{ARGUS.tau_mass.pub.ALBRECHT.1992M-pdgref}-cite} \\
\dxuse{BABAR.tau_mass.pub.AUBERT.2009AK-vu} & \dxuse{\dxuse{BABAR.tau_mass.pub.AUBERT.2009AK-pdgref}-exp} & \dxuse{\dxuse{BABAR.tau_mass.pub.AUBERT.2009AK-pdgref}-cite} \\
\dxuse{BELLE.tau_mass.pub.BELOUS.2007-vu} & \dxuse{\dxuse{BELLE.tau_mass.pub.BELOUS.2007-pdgref}-exp} & \dxuse{\dxuse{BELLE.tau_mass.pub.BELOUS.2007-pdgref}-cite} \\
\dxuse{Belle2.tau_mass.pub.ADACHI.2023C-vu} & \dxuse{\dxuse{Belle2.tau_mass.pub.ADACHI.2023C-pdgref}-exp} & \dxuse{\dxuse{Belle2.tau_mass.pub.ADACHI.2023C-pdgref}-cite} \\
\dxuse{BES.tau_mass.pub.BAI.1996-vu} & \dxuse{\dxuse{BES.tau_mass.pub.BAI.1996-pdgref}-exp} & \dxuse{\dxuse{BES.tau_mass.pub.BAI.1996-pdgref}-cite} \\
\dxuse{BES3.tau_mass.pub.ABLIKIM.2014D-vu} & \dxuse{\dxuse{BES3.tau_mass.pub.ABLIKIM.2014D-pdgref}-exp} & \dxuse{\dxuse{BES3.tau_mass.pub.ABLIKIM.2014D-pdgref}-cite} \\
\dxuse{CLEO.tau_mass.pub.ANASTASSOV.1997-vu} & \dxuse{\dxuse{CLEO.tau_mass.pub.ANASTASSOV.1997-pdgref}-exp} & \dxuse{\dxuse{CLEO.tau_mass.pub.ANASTASSOV.1997-pdgref}-cite} \\
\dxuse{DELCO.tau_mass.pub.BACINO.1978B-vu} & \dxuse{\dxuse{DELCO.tau_mass.pub.BACINO.1978B-pdgref}-exp} & \dxuse{\dxuse{DELCO.tau_mass.pub.BACINO.1978B-pdgref}-cite} \\
\dxuse{KEDR.tau_mass.pub.ANASHIN.2023A-vu} & \dxuse{\dxuse{KEDR.tau_mass.pub.ANASHIN.2023A-pdgref}-exp} & \dxuse{\dxuse{KEDR.tau_mass.pub.ANASHIN.2023A-pdgref}-cite} \\
\dxuse{OPAL.tau_mass.pub.ABBIENDI.2000A-vu} & \dxuse{\dxuse{OPAL.tau_mass.pub.ABBIENDI.2000A-pdgref}-exp} & \dxuse{\dxuse{OPAL.tau_mass.pub.ABBIENDI.2000A-pdgref}-cite}%
}
\dxdef{TauMassQuantMeasTable}{%
\dxuse{tau_mass-qm}%
}
\dxdef{ALBRECHT 1992M-ref}{ARGUS:1992chv}
\dxdef{ALBRECHT 1992M-cite}{\cite{ARGUS:1992chv}}
\dxdef{ALBRECHT 1992M-exp}{ARGUS}
\dxdef{ALBRECHT 1992M-type}{pub}
\dxdef{ALBRECHT 1992M-label}{ALBRECHT 1992M (ARGUS)}
\dxdef{ALBRECHT 1992M-meas}{%
\multicolumn{2}{l}{\dxuse{ALBRECHT 1992M-label}\,\dxuse{ALBRECHT 1992M-cite}} \\
\begin{ensuredisplaymath}
\dxuse{tau_mass-gn} = \dxuse{tau_mass-td}
\end{ensuredisplaymath} & \dxuse{ARGUS.tau_mass.pub.ALBRECHT.1992M-vu}%
}
\dxdef{AUBERT 2009AK-ref}{BaBar:2009qmj}
\dxdef{AUBERT 2009AK-cite}{\cite{BaBar:2009qmj}}
\dxdef{AUBERT 2009AK-exp}{BABAR}
\dxdef{AUBERT 2009AK-type}{pub}
\dxdef{AUBERT 2009AK-label}{AUBERT 2009AK (BABAR)}
\dxdef{AUBERT 2009AK-meas}{%
\multicolumn{2}{l}{\dxuse{AUBERT 2009AK-label}\,\dxuse{AUBERT 2009AK-cite}} \\
\begin{ensuredisplaymath}
\dxuse{tau_mass-gn} = \dxuse{tau_mass-td}
\end{ensuredisplaymath} & \dxuse{BABAR.tau_mass.pub.AUBERT.2009AK-vu}%
}
\dxdef{BELOUS 2007-ref}{Belle:2006qqw}
\dxdef{BELOUS 2007-cite}{\cite{Belle:2006qqw}}
\dxdef{BELOUS 2007-exp}{Belle}
\dxdef{BELOUS 2007-type}{pub}
\dxdef{BELOUS 2007-label}{BELOUS 2007 (Belle)}
\dxdef{BELOUS 2007-meas}{%
\multicolumn{2}{l}{\dxuse{BELOUS 2007-label}\,\dxuse{BELOUS 2007-cite}} \\
\begin{ensuredisplaymath}
\dxuse{tau_mass-gn} = \dxuse{tau_mass-td}
\end{ensuredisplaymath} & \dxuse{BELLE.tau_mass.pub.BELOUS.2007-vu}%
}
\dxdef{ADACHI 2023C-ref}{Belle-II:2023izd}
\dxdef{ADACHI 2023C-cite}{\cite{Belle-II:2023izd}}
\dxdef{ADACHI 2023C-exp}{Belle\,II}
\dxdef{ADACHI 2023C-type}{pub}
\dxdef{ADACHI 2023C-label}{ADACHI 2023C (Belle\,II)}
\dxdef{ADACHI 2023C-meas}{%
\multicolumn{2}{l}{\dxuse{ADACHI 2023C-label}\,\dxuse{ADACHI 2023C-cite}} \\
\begin{ensuredisplaymath}
\dxuse{tau_mass-gn} = \dxuse{tau_mass-td}
\end{ensuredisplaymath} & \dxuse{Belle2.tau_mass.pub.ADACHI.2023C-vu}%
}
\dxdef{BAI 1996-ref}{BES:1995jmv}
\dxdef{BAI 1996-cite}{\cite{BES:1995jmv}}
\dxdef{BAI 1996-exp}{BES}
\dxdef{BAI 1996-type}{pub}
\dxdef{BAI 1996-label}{BAI 1996 (BES)}
\dxdef{BAI 1996-meas}{%
\multicolumn{2}{l}{\dxuse{BAI 1996-label}\,\dxuse{BAI 1996-cite}} \\
\begin{ensuredisplaymath}
\dxuse{tau_mass-gn} = \dxuse{tau_mass-td}
\end{ensuredisplaymath} & \dxuse{BES.tau_mass.pub.BAI.1996-vu}%
}
\dxdef{ABLIKIM 2014D-ref}{BESIII:2014srs}
\dxdef{ABLIKIM 2014D-cite}{\cite{BESIII:2014srs}}
\dxdef{ABLIKIM 2014D-exp}{BES3}
\dxdef{ABLIKIM 2014D-type}{pub}
\dxdef{ABLIKIM 2014D-label}{ABLIKIM 2014D (BES3)}
\dxdef{ABLIKIM 2014D-meas}{%
\multicolumn{2}{l}{\dxuse{ABLIKIM 2014D-label}\,\dxuse{ABLIKIM 2014D-cite}} \\
\begin{ensuredisplaymath}
\dxuse{tau_mass-gn} = \dxuse{tau_mass-td}
\end{ensuredisplaymath} & \dxuse{BES3.tau_mass.pub.ABLIKIM.2014D-vu}%
}
\dxdef{ANASTASSOV 1997-ref}{CLEO:1996oro}
\dxdef{ANASTASSOV 1997-cite}{\cite{CLEO:1996oro}}
\dxdef{ANASTASSOV 1997-exp}{CLEO}
\dxdef{ANASTASSOV 1997-type}{pub}
\dxdef{ANASTASSOV 1997-label}{ANASTASSOV 1997 (CLEO)}
\dxdef{ANASTASSOV 1997-meas}{%
\multicolumn{2}{l}{\dxuse{ANASTASSOV 1997-label}\,\dxuse{ANASTASSOV 1997-cite}} \\
\begin{ensuredisplaymath}
\dxuse{tau_mass-gn} = \dxuse{tau_mass-td}
\end{ensuredisplaymath} & \dxuse{CLEO.tau_mass.pub.ANASTASSOV.1997-vu}%
}
\dxdef{BACINO 1978B-ref}{Bacino:1978gb}
\dxdef{BACINO 1978B-cite}{\cite{Bacino:1978gb}}
\dxdef{BACINO 1978B-exp}{DELCO}
\dxdef{BACINO 1978B-type}{pub}
\dxdef{BACINO 1978B-label}{BACINO 1978B (DELCO)}
\dxdef{BACINO 1978B-meas}{%
\multicolumn{2}{l}{\dxuse{BACINO 1978B-label}\,\dxuse{BACINO 1978B-cite}} \\
\begin{ensuredisplaymath}
\dxuse{tau_mass-gn} = \dxuse{tau_mass-td}
\end{ensuredisplaymath} & \dxuse{DELCO.tau_mass.pub.BACINO.1978B-vu}%
}
\dxdef{ANASHIN 2023A-ref}{Anashin:2023sch}
\dxdef{ANASHIN 2023A-cite}{\cite{Anashin:2023sch}}
\dxdef{ANASHIN 2023A-exp}{KEDR}
\dxdef{ANASHIN 2023A-type}{pub}
\dxdef{ANASHIN 2023A-label}{ANASHIN 2023A (KEDR)}
\dxdef{ANASHIN 2023A-meas}{%
\multicolumn{2}{l}{\dxuse{ANASHIN 2023A-label}\,\dxuse{ANASHIN 2023A-cite}} \\
\begin{ensuredisplaymath}
\dxuse{tau_mass-gn} = \dxuse{tau_mass-td}
\end{ensuredisplaymath} & \dxuse{KEDR.tau_mass.pub.ANASHIN.2023A-vu}%
}
\dxdef{ABBIENDI 2000A-ref}{OPAL:2000svx}
\dxdef{ABBIENDI 2000A-cite}{\cite{OPAL:2000svx}}
\dxdef{ABBIENDI 2000A-exp}{OPAL}
\dxdef{ABBIENDI 2000A-type}{pub}
\dxdef{ABBIENDI 2000A-label}{ABBIENDI 2000A (OPAL)}
\dxdef{ABBIENDI 2000A-meas}{%
\multicolumn{2}{l}{\dxuse{ABBIENDI 2000A-label}\,\dxuse{ABBIENDI 2000A-cite}} \\
\begin{ensuredisplaymath}
\dxuse{tau_mass-gn} = \dxuse{tau_mass-td}
\end{ensuredisplaymath} & \dxuse{OPAL.tau_mass.pub.ABBIENDI.2000A-vu}%
}
\dxdef{TauMassMeasByRef}{%
\dxuse{ALBRECHT 1992M-meas} \\[1.5ex]
\dxuse{AUBERT 2009AK-meas} \\[1.5ex]
\dxuse{BELOUS 2007-meas} \\[1.5ex]
\dxuse{ADACHI 2023C-meas} \\[1.5ex]
\dxuse{BAI 1996-meas} \\[1.5ex]
\dxuse{ABLIKIM 2014D-meas} \\[1.5ex]
\dxuse{ANASTASSOV 1997-meas} \\[1.5ex]
\dxuse{BACINO 1978B-meas} \\[1.5ex]
\dxuse{ANASHIN 2023A-meas} \\[1.5ex]
\dxuse{ABBIENDI 2000A-meas}%
}


==> tau/tau-defs.tex <==
\newcommand{\hflavtau}{HFLAV-Tau\xspace}
\newcommand{\BRF}[2]{#2}
\newcommand{\BRtau}[1]{\ensuremath{\tau^- \to #1}\xspace}
\newcommand{\inlineFrac}[1]{{\renewcommand{\frac}[2]{##1/##2}#1}}
\newcommand{\inlineFracParen}[1]{{\renewcommand{\frac}[2]{(##1)/(##2)}#1}}

%
%
%
%

%
%
%
\newcommand{\lepth}{\mathcal{L}}
\newcommand{\leptl}{\ell}

%
\newcommand{\radRatio}{R}
%
\newcommand{\radDelta}{\delta}

%
\newcommand{\Rhad}{\ensuremath{R_{\text{had}}}\xspace}
\newcommand{\BRhad}{\ensuremath{\BR_{\text{had}}}\xspace}
\newcommand{\Gammahad}{\ensuremath{\Gamma_{\text{had}}}\xspace}
%
\newcommand{\Rstrange}{\ensuremath{R_{us}}\xspace}
\newcommand{\BRstrange}{\ensuremath{\BR_{us}}\xspace}
\newcommand{\Gammastrange}{\ensuremath{\Gamma_{us}}\xspace}
\newcommand{\Rnonstrange}{\ensuremath{R_{ud}}\xspace}
\newcommand{\BRnonstrange}{\ensuremath{\BR_{ud}}\xspace}
\newcommand{\Gammanonstrange}{\ensuremath{\Gamma_{ud}}\xspace}
\newcommand{\deltaRtauSUtb}{\ensuremath{\delta R_{\tau\text{-}SU(3)\text{-break}}}\xspace}
\newcommand{\tauknu}{\ensuremath{\tau^{-} \to K^{-} \nut}\xspace}
\newcommand{\taupinu}{\ensuremath{\tau^{-} \to \pi^{-} \nut}\xspace}
\newcommand{\BFtautoknu}{\ensuremath{\BR(\tauknu)}\xspace}
\newcommand{\BFtautopinu}{\ensuremath{\BR(\taupinu)}\xspace}
\newcommand{\VusUni}{\ensuremath{\Vus_{\text{uni}}}\xspace}
\newcommand{\VusTauIncl}{\ensuremath{\Vus_{\tau s}}\xspace}
\dxdef{VusTauIncl-OPE-1}{\ensuremath{\Vus_{\tau\text{-OPE-1}}}}
\dxdef{VusTauIncl-OPE-2}{\ensuremath{\Vus_{\tau\text{-OPE-2}}}}
\dxdef{VusTauIncl-latt-disp}{\ensuremath{\Vus_{\tau\text{-latt-disp}}}}
\dxdef{VusTauIncl-latt-incl}{\ensuremath{\Vus_{\tau\text{-latt-incl}}}}
\dxdef{VusTauInclbyVud-OPE-1}{\ensuremath{\Vus/\Vud_{\tau\text{-OPE-1}}}}
\dxdef{VusTauInclbyVud-OPE-2}{\ensuremath{\Vus/\Vud_{\tau\text{-OPE-2}}}}
\dxdef{VusTauInclbyVud-latt-disp}{\ensuremath{\Vus/\Vud_{\tau\text{-latt-disp}}}}
\dxdef{VusTauInclbyVud-latt-incl}{\ensuremath{\Vus/\Vud_{\tau\text{-latt-incl}}}}
\newcommand{\VusTauKpi}{\ensuremath{\Vus_{\tau K/\pi}}\xspace}
\newcommand{\VusTauKnu}{\ensuremath{\Vus_{\tau K}}\xspace}
\newcommand{\VusTauKPinu}{\ensuremath{\Vus_{\tau K\pi}}\xspace}
%
\newcommand{\dRradTauhHmu}{\ensuremath{\radDelta_{\tau/h}}\xspace}
\newcommand{\dRradTaupiPimu}{\ensuremath{\radDelta_{\tau/\pi}}\xspace}
\newcommand{\dRradTaukKmu}{\ensuremath{\radDelta_{\tau/K}}\xspace}
\newcommand{\RradKmuPimu}{\ensuremath{\radRatio_{K/\pi}}\xspace}
%
\providecommand{\slashLikeH}{%
  \raisebox{.9ex}{%
    \scalebox{.7}{%
      \rotatebox[origin=c]{18}{$-$}%
    }%
  }%
}
\providecommand{\hslash}{%
  {%
   \vphantom{h}%
   \ooalign{\kern.05em\smash{\slashLikeH}\hidewidth\cr$h$\cr}%
   \kern.05em
  }%
}

\newcommand{\cls}{\ensuremath{\text{CL}_s}\xspace}
\newcommand{\clsb}{\ensuremath{\text{CL}_{s+b}}\xspace}
\newcommand{\clb}{\ensuremath{\text{CL}_b}\xspace}


==> tau/tau-header.tex <==
%
%
%
%
\newcommand{\hflavTauTag}{2023\xspace}

%
%
%
%
\newif\ifhevea\heveafalse
%

%
\makeatletter
\newenvironment*{fleqn}[1][\leftmargini minus\leftmargini]{\@fleqntrue
  \setlength\@mathmargin{#1}\ignorespaces
}{%
  \ignorespacesafterend
}
\makeatother

\ifhevea
  \renewcommand{\babar}{BaBar\xspace}
\else
  \makeatletter
  \providecommand{\cutname}[1]{}

  %
  \newenvironment{envsmall}%
  {\small}%
  {}

  %
  \newenvironment{ceqn}{\@fleqnfalse
    \@mathmargin\@centering \ignorespaces
  }{%
    \ignorespacesafterend
  }

  %
  \newenvironment{citenoleadsp}{\@fleqnfalse
    \let\cite@adjust\@empty
  }{%
    \ignorespacesafterend
  }

  %
  \newenvironment{ensuredisplaymath}
  {\(\displaystyle}
  {\)}
  \makeatother
\fi

%
%
%
\makeatletter

%

%
\def\dx@root{dx@root@}

%
\newcommand{\dxsetf}[1]{%
  \def\dx@fold{\dx@root-#1@}%
}
%
\dxsetf{}

%
\newcommand{\dxdef}[2]{%
  \@namedef{\dx@fold#1}{#2}%
}

%
\newcommand{\dxuse}[1]{%
  \ifcsname\dx@fold#1\endcsname
    \@nameuse{\dx@fold#1}%
  \else
    \@latex@error{Undefined macro \dx@fold#1}\@eha
  \fi
}

%
\newcommand{\dxusef}[2]{%
  \ifcsname\dx@root-#1@#2\endcsname
    \@nameuse{\dx@root-#1@#2}%
  \else
    \@latex@error{Undefined macro \dx@root-#1@#2}\@eha
  \fi
}

%

%

%
\newcommand{\dxQuantDef}[6]{%
  \dxdef{#1-gn}{\ensuremath{#2}}%
  \dxdef{#1-td}{\ensuremath{#3}}%
  \dxdef{#1-vu}{\ensuremath{#4}}%
  \dxdef{#1-v}{\ensuremath{#5}}%
  \dxdef{#1-u}{\ensuremath{#6}}%
}

%
\newcommand{\dxQuantLimitDef}[5]{%
  \dxdef{#1-gn}{\ensuremath{#2}}%
  \dxdef{#1-td}{\ensuremath{#3}}%
  \dxdef{#1-categ}{\ensuremath{#4}}%
  \dxdef{#1-ul}{\ensuremath{#5}}%
}

%
\newcommand{\dxMeasDef}[7]{%
  \dxdef{#1-quant}{\ensuremath{#2}}%
  \dxdef{#1-pdgref}{#3}%
  \dxdef{#1-vu}{\ensuremath{#4}}%
  \dxdef{#1-v}{\ensuremath{#5}}%
  \dxdef{#1-stat}{\ensuremath{#6}}%
  \dxdef{#1-syst}{\ensuremath{#7}}%
}

%
\newcommand{\dxConstrDef}[3]{%
  \dxdef{#1-left}{\ensuremath{#2}}%
  \dxdef{#1-right}{\ensuremath{#3}}%
}

%
\newcommand{\dxQuantLine}[3]{\ensuremath{\dxuse{#1-td}}&\ensuremath{#2}\\}

%
%
%
\newcommand{\dxQuantMeasLine}[1]{%
  \dxuse{#1-vu} & average &%
}

%
%
%
\newcommand{\dxLimitLine}[5]{%
  #1 & #2 & #3 & #4 & #5 \\
}
\newcommand{\dxLimitsMeasRow}[5]{%
  #1 & #2 & #3 & #4 & #5 \\
}
\newcommand{\dxCombExtraLine}[7]{%
  #1 & #2 & \cite{#3} & #4 & #5 & #6 & #7 \\
}
\newcommand{\dxLimitsMeasCombExtraRow}[7]{%
  \ensuremath{#2} &
  %
  \ensuremath{#4} &
  #5~\cite{#6}#7 &
}
\newcommand{\dxLimitsMeasCombExtraExtraRow}[4]{%
  #1 & \ensuremath{#2} & \ensuremath{#3} & #4
}
\newcommand{\dxLimitsMeasCombExtraExtraBrRow}[1]{%
  \multicolumn{4}{c}{\ensuremath{\BR = #1}}
}
\newcommand{\dxLimitsMeasCombExtraCombRow}[4]{%
  \ensuremath{#2} &
  %
  \ensuremath{#4} & Comb.
}
\newcommand{\dxLimitsMeasCombExtraLimitSep}{\\}
\newcommand{\dxLimitsMeasCombExtraCombSep}{\\}
\newcommand{\dxLimitsMeasCombExtraModeSep}{\\[1ex]}
%
\newcommand{\dxLimitsMeasCombExtraTypeSep}{\\}
\newcommand{\dxLimitsMeasCombExtraTypeHead}[1]{%
  \\[-1.5ex]
  \textbf{\ensuremath{#1} category} \\[0.5ex]
}

%

%
%
%
\ifhevea
  %
  \providecommand{\dxuse}{}
  \renewcommand{\dxuse}[1]{%
    \@nameuse{\dx@fold#1}%
  }

  %
  \providecommand{\dxusef}{}
  \renewcommand{\dxusef}[2]{%
    \@nameuse{\dx@root-#1@#2}%
  }

  %
  \providecommand{\dxLimitsMeasCombExtraTypeHead}{}
  \newcommand{\dxLimitsMeasCombExtraTypeHead}[1]{%
  \textbf{\ensuremath{#1} category} \\
  }
\fi

\makeatother

\ifhevea
  %
  %
  %
  \input{tau-defs}
  \input{avg-taubr-2023.tex}
  \dxsetf{uc}
  \input{avg-taubr-2023-uc.tex}
  \dxQuantDef{GammaUnitResid}{\BR_{\text{ur}}}{\BR(\tau^- \text{unitarity residual})}{0.0}{0.0}{\pm 0.0}
  \dxsetf{}
  \input{avg-taubr-2023-elab-vadirect.tex}
  \input{avg-taumass-2023.tex}
  \input{avg-taulife-2023.tex}
  \input{tau-lfv-data}
\else
  %
  %
  %
  \input{tau/tau-defs}
  \input{tau/avg-taubr-2023.tex}
  \dxsetf{uc}
  \input{tau/avg-taubr-2023-uc.tex}
  \dxQuantDef{GammaUnitResid}{\BR_{\text{ur}}}{\BR(\tau^- \text{unitarity residual})}{0.0}{0.0}{\pm 0.0}
  \dxsetf{}
  \input{tau/avg-taubr-2023-elab-vadirect.tex}
  \input{tau/avg-taumass-2023.tex}
  \input{tau/avg-taulife-2023.tex}
  \input{tau/tau-lfv-data}
\fi

%
%
%
\dxdef{tau_mass-gn}{\ensuremath{m_\mtau}}
\dxdef{tau_mass-td}{\text{\mtau mass [MeV]}}
\dxdef{tau_life-gn}{\ensuremath{\tau_\mtau}}
\dxdef{tau_life-td}{\text{\mtau lifetime [fs]}}


==> tau/tau-lfv-combs.tex <==
%
\subsection{%
\texorpdfstring{%
  Combination of upper limits on \mtau lepton-flavour-violating
  branching fractions}{%
  Combination of upper limits on tau lepton-flavour-violating branching
  fractions}%
}
\label{sec:tau:lfv-limits}
%
%
\cutname{lfv-combinations.html}

The Standard Model prediction for the \mtau lepton-flavour-violating
(LFV) branching fractions are of
order$10^{-54}$~\cite{Lee:1977tib,Petcov:1976ff}, which are too small to be measured experimentally.
Recently, the contributions due to finite neutrino masses for $\tau^- \to \ell_i^- \ell_j^+ \ell_a^- $ decays
(where $a~=~i~\mathrm{or}~j$, and $i$ may or may not be equal to $j$),
were re-scrutinized and also found to be in the range of $[10^{-56},10^{-54}]$~\cite{Hernandez-Tome:2018fbq,Blackstone:2019njl}.
However, these branching fractions are expected
to be of the order of $10^{-10}-10^{-9}$ in several new physics
scenarios~\cite{Ilakovac:1994kj,Raidal:2008jk,deGouvea:2013zba,Dorsner:2016wpm,Ardu:2022sbt},
which is just below the current experimental sensitivity. Several
searches have been performed to observe neutrino-less \mtau decays to
final states categorized as $\ell \gamma$, $\ell P^0$, $\ell V^0$, $\ell
S^0$, $\ell \ell \ell$, $\ell h h$, including decays that are also
baryon-number-violating (BNV). In
Table~\ref{tab:tau:lfv-limits-and-combs} and
Figure~\ref{fig:tau:lfv-limits-combs-plot}, we report the observed upper
limits on these branching fractions published by the $B$-factories
\babar and Belle and the LHC experiments. Weaker upper limits (mainly
from CLEO) have been omitted from
Table~\ref{tab:tau:lfv-limits-and-combs}, but are shown in
Figure~\ref{fig:tau:lfv-limits-combs-plot}, to document the historical
progress. For channels where multiple results of similar strengths are
available, we also report the combined upper limits, following the
prescription described below. No preliminary results are included in
this report.

We combine the reported upper limits by first averaging the central values
of the corresponding branching-fraction measurements to obtain the average branching fraction $\bar{\BR}$ and its uncertainty $\delta\bar{\BR}$,
\begin{align}
\bar{\BR} = \frac{\sum w_i \BR_i }{\sum w_i}\quad , \quad
\delta\bar{\BR} = \sqrt{\frac{1}{\sum w_i}}~,
\end{align}
where 
$\BR_i$ is the central value for the branching fraction of measurement $i$ and 
$w_i = 1 / \delta\BR_i^2$ is the inverse of square of its uncertainty.
We then compute the 90\%
confidence level (CL) upper limit as $\bar{\BR^{90}} = \bar{\BR} +
1.645\,\delta\bar{\BR}$, assuming a Gaussian uncertainty. The majority
of published limits do not have reported values for $\BR_i$ and $w_i$.
In such cases, we take the central value to be $\BR_i =
(N^i_{\text{obs}}-N^i_{\text{bkg}})/(N^i_\tau \varepsilon^i)$, where
$N^i_{\text{obs}}$ is the number of observed events, $N^i_{\text{bkg}}$ is
the number of expected background events, $N^i_\tau$ is the number of
$\tau$ decays in the data sample, and $\varepsilon^i$ is the signal
reconstruction efficiency in the signal region.
Additional information for central value of $\dxuse{Gamma283-td}$ are obtained from
the CMS~\cite{CMS:2023iqy} and LHCb~\cite{Aaij:2014azz} collaborations, respectively,
and are listed in Table~\ref{tab:tau:lfv-limits-and-combs} for future reference.

The uncertainty $\delta\BR_i$ is
computed assuming that the reported 90\% CL limit corresponds to
$\BR^{90}_i = \BR_i + 1.645\,\delta\BR_i$. 
Using this combination procedure, the resulting upper limit may be
weaker than the most stringent input limit, but always corresponds to a
more precise branching fraction, obtained by averaging multiple
measurements. Since there is negligible gain in combining limits of very
different strength, the combinations do not include the limits that are
more than 10 times larger than the strictest limit in the respective
channel. This excludes limits of the CLEO and ATLAS searches and the
LHCb searches for \mtau decays into proton and two muons. We report in
Table~\ref{tab:tau:lfv-limits-and-combs} and
Figure~\ref{fig:tau:lfv-limits-combs-plot} the observed upper limits
on the \mtau lepton-flavour-violating decays and their combinations.

\begin{center}
  \begin{longtable}{lrlrrrrr}
    \caption{Experimental upper limits on lepton flavour violating \mtau
      decays. The modes are grouped according to the properties of their
      final states. Modes with baryon number violation are labelled with
      ``BNV''. The combinations of upper limits are reported in the rows
      with label ``Comb.'' in the ``Experiment / Reference'' column.
      The measurements used to compute the
      combinations are tagged with an asterisk attached to their reference.
      Where available, additional information is reported about the number
      of \mtau decays used in the search, the efficiency of the selection, the
      expected background and the number of observed events,
      or the central value of branching fractions.
      \label{tab:tau:lfv-limits-and-combs}}%
    \\
    \toprule
    \multicolumn{1}{l}{\bfseries Decay mode}                                                                     &
    %
    \multicolumn{1}{c}{\bfseries \begin{tabular}{@{}c@{}}90\% CL\\Limit\end{tabular}}                            &
    \multicolumn{1}{l}{\bfseries Exp./Ref.}                                                                      &
    %
    \multicolumn{1}{c}{\bfseries \begin{tabular}{@{}c@{}}$N_{\tau}$\\($10^6$)\end{tabular}} &
    \multicolumn{1}{c}{\bfseries \begin{tabular}{@{}c@{}}$\varepsilon$\\(\%)\end{tabular}}                       &
    \multicolumn{1}{c}{\bfseries $N_{\text{bkg}}$}                                                               &
    \multicolumn{1}{c}{\bfseries $N_{\text{obs}}$}
    \\
    \midrule
    \endfirsthead
    \multicolumn{5}{c}{{\bfseries \tablename\ \thetable{} -- continued from previous page}}                        \\ \midrule
    \multicolumn{1}{l}{\bfseries Decay mode}                                                                     &
    %
    \multicolumn{1}{c}{\bfseries \begin{tabular}{@{}c@{}}90\% CL\\Limit\end{tabular}}                            &
    \multicolumn{1}{l}{\bfseries Exp./Ref.}                                                                      &
    %
    \multicolumn{1}{c}{\bfseries \begin{tabular}{@{}c@{}}$N_{\tau}$\\($10^6$)\end{tabular}} &
    \multicolumn{1}{c}{\bfseries \begin{tabular}{@{}c@{}}$\varepsilon$\\(\%)\end{tabular}}                       &
    \multicolumn{1}{c}{\bfseries $N_{\text{bkg}}$}                                                               &
    \multicolumn{1}{c}{\bfseries $N_{\text{obs}}$}
    \\
    \midrule
    \endhead
    \dxuse{LimitsMeasCombExtraTable}%
    \\
    %
    \bottomrule
  \end{longtable}
\end{center}


==> tau/tau-lfv-data.tex <==
\dxQuantLimitDef{Gamma256}{\BR_{256}}{\BR(\tau^- \to e^- \gamma)}{\ell\gamma}{2.6 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma257}{\BR_{257}}{\BR(\tau^- \to \mu^- \gamma)}{\ell\gamma}{2.7 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma258}{\BR_{258}}{\BR(\tau^- \to e^- \pi^0)}{\ell P^0}{6.4 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma259}{\BR_{259}}{\BR(\tau^- \to \mu^- \pi^0)}{\ell P^0}{8.1 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma260}{\BR_{260}}{\BR(\tau^- \to e^- K^0_S)}{\ell P^0}{2.0 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma261}{\BR_{261}}{\BR(\tau^- \to \mu^- K^0_S)}{\ell P^0}{1.8 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma262}{\BR_{262}}{\BR(\tau^- \to e^- \eta)}{\ell P^0}{7.4 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma263}{\BR_{263}}{\BR(\tau^- \to \mu^- \eta)}{\ell P^0}{6.1 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma272}{\BR_{272}}{\BR(\tau^- \to e^- \eta^\prime(958))}{\ell P^0}{1.3 \cdot 10^{-7}}
\dxQuantLimitDef{Gamma273}{\BR_{273}}{\BR(\tau^- \to \mu^- \eta^\prime(958))}{\ell P^0}{8.6 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma264}{\BR_{264}}{\BR(\tau^- \to e^- \rho^0)}{\ell V^0}{2.0 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma265}{\BR_{265}}{\BR(\tau^- \to \mu^- \rho^0)}{\ell V^0}{1.3 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma266}{\BR_{266}}{\BR(\tau^- \to e^- \omega)}{\ell V^0}{2.2 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma267}{\BR_{267}}{\BR(\tau^- \to \mu^- \omega)}{\ell V^0}{3.4 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma268}{\BR_{268}}{\BR(\tau^- \to e^- K^*(892))}{\ell V^0}{1.9 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma269}{\BR_{269}}{\BR(\tau^- \to \mu^- K^*(892))}{\ell V^0}{3.3 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma270}{\BR_{270}}{\BR(\tau^- \to e^- \bar{K}^*(892))}{\ell V^0}{1.5 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma271}{\BR_{271}}{\BR(\tau^- \to \mu^- \bar{K}^*(892))}{\ell V^0}{3.7 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma276}{\BR_{276}}{\BR(\tau^- \to e^- \phi)}{\ell V^0}{1.6 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma277}{\BR_{277}}{\BR(\tau^- \to \mu^- \phi)}{\ell V^0}{2.6 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma274}{\BR_{274}}{\BR(\tau^- \to e^- f_0(980))}{\ell S^0}{NA}
\dxQuantLimitDef{Gamma275}{\BR_{275}}{\BR(\tau^- \to \mu^- f_0(980))}{\ell S^0}{NA}
\dxQuantLimitDef{Gamma278}{\BR_{278}}{\BR(\tau^- \to e^- e^+ e^-)}{\ell\ell\ell}{1.9 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma279}{\BR_{279}}{\BR(\tau^- \to e^- \mu^+ \mu^-)}{\ell\ell\ell}{2.0 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma280}{\BR_{280}}{\BR(\tau^- \to \mu^- e^+ \mu^-)}{\ell\ell\ell}{1.4 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma281}{\BR_{281}}{\BR(\tau^- \to \mu^- e^+ e^-)}{\ell\ell\ell}{1.3 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma282}{\BR_{282}}{\BR(\tau^- \to e^- \mu^+ e^-)}{\ell\ell\ell}{1.1 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma283}{\BR_{283}}{\BR(\tau^- \to \mu^- \mu^+ \mu^-)}{\ell\ell\ell}{1.6 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma284}{\BR_{284}}{\BR(\tau^- \to e^- \pi^+ \pi^-)}{\ell hh}{2.1 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma285}{\BR_{285}}{\BR(\tau^- \to e^+ \pi^- \pi^-)}{\ell hh}{NA}
\dxQuantLimitDef{Gamma286}{\BR_{286}}{\BR(\tau^- \to \mu^- \pi^+  \pi^-)}{\ell hh}{NA}
\dxQuantLimitDef{Gamma287}{\BR_{287}}{\BR(\tau^- \to \mu^+ \pi^- \pi^-)}{\ell hh}{3.5 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma288}{\BR_{288}}{\BR(\tau^- \to e^- \pi^+ K^-)}{\ell hh}{3.8 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma289}{\BR_{289}}{\BR(\tau^- \to e^- K^+ \pi^-)}{\ell hh}{2.9 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma290}{\BR_{290}}{\BR(\tau^- \to e^+ \pi^- K^-)}{\ell hh}{3.1 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma291}{\BR_{291}}{\BR(\tau^- \to e^- K^0_S K^0_S)}{\ell hh}{NA}
\dxQuantLimitDef{Gamma292}{\BR_{292}}{\BR(\tau^- \to e^- K^+ K^-)}{\ell hh}{3.3 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma293}{\BR_{293}}{\BR(\tau^- \to e^+ K^- K^-)}{\ell hh}{3.2 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma294}{\BR_{294}}{\BR(\tau^- \to \mu^- \pi^+  K^-)}{\ell hh}{8.2 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma295}{\BR_{295}}{\BR(\tau^- \to \mu^- K^+  \pi^-)}{\ell hh}{4.6 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma296}{\BR_{296}}{\BR(\tau^- \to \mu^+ \pi^- K^-)}{\ell hh}{4.5 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma297}{\BR_{297}}{\BR(\tau^- \to \mu^- K^0_S  K^0_S)}{\ell hh}{NA}
\dxQuantLimitDef{Gamma298}{\BR_{298}}{\BR(\tau^- \to \mu^- K^+  K^-)}{\ell hh}{4.2 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma299}{\BR_{299}}{\BR(\tau^- \to \mu^+ K^- K^-)}{\ell hh}{NA}
\dxQuantLimitDef{Gamma311}{\BR_{311}}{\BR(\tau^- \to \pi^- \Lambda)}{\text{BNV}}{3.0 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma312}{\BR_{312}}{\BR(\tau^- \to \pi^- \bar{\Lambda})}{\text{BNV}}{3.8 \cdot 10^{-8}}
\dxQuantLimitDef{Gamma315}{\BR_{315}}{\BR(\tau^- \to \bar{p} e^+ e^-)}{\text{BNV}}{NA}
\dxQuantLimitDef{Gamma316}{\BR_{316}}{\BR(\tau^- \to p e^- e^-)}{\text{BNV}}{NA}
\dxQuantLimitDef{Gamma317}{\BR_{317}}{\BR(\tau^- \to \bar{p} e^+ \mu^-)}{\text{BNV}}{NA}
\dxQuantLimitDef{Gamma318}{\BR_{318}}{\BR(\tau^- \to \bar{p} e^- \mu^+)}{\text{BNV}}{NA}
\dxQuantLimitDef{Gamma319}{\BR_{319}}{\BR(\tau^- \to p \mu^- \mu^-)}{\text{BNV}}{NA}
\dxQuantLimitDef{Gamma320}{\BR_{320}}{\BR(\tau^- \to \bar{p} \mu^+ \mu^-)}{\text{BNV}}{NA}
\dxdef{LimitsMeasCombExtraTable}{%
\dxLimitsMeasCombExtraTypeHead{\ell\gamma}%
\dxLimitsMeasCombExtraRow{\BR_{256}}{\BR(\tau^- \to e^- \gamma)}{\ell\gamma}{3.3 \cdot 10^{-8}}{\babar}{Aubert:2009ag}{*}%
\dxLimitsMeasCombExtraExtraRow{963}{3.90 \pm 0.30}{1.60 \pm 0.40}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{5.6 \cdot 10^{-8}}{Belle}{Belle:2021ysv}{*}%
\dxLimitsMeasCombExtraExtraRow{1824}{2.90 \pm 0.19}{5.50 \pm 4.65}{5}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{2.6 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{257}}{\BR(\tau^- \to \mu^- \gamma)}{}{4.4 \cdot 10^{-8}}{\babar}{Aubert:2009ag}{*}%
\dxLimitsMeasCombExtraExtraRow{963}{6.10 \pm 0.50}{3.60 \pm 0.70}{2}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{4.2 \cdot 10^{-8}}{Belle}{Belle:2021ysv}{*}%
\dxLimitsMeasCombExtraExtraRow{1824}{3.70 \pm 0.21}{5.30 \pm 2.75}{5}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{2.7 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraTypeSep%
\dxLimitsMeasCombExtraTypeHead{\ell P^0}%
\dxLimitsMeasCombExtraRow{\BR_{258}}{\BR(\tau^- \to e^- \pi^0)}{\ell P^0}{1.3 \cdot 10^{-7}}{\babar}{Aubert:2006cz}{*}%
\dxLimitsMeasCombExtraExtraRow{623}{2.80 \pm 0.25}{0.17 \pm 0.04}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{8.0 \cdot 10^{-8}}{Belle}{Miyazaki:2007jp}{*}%
\dxLimitsMeasCombExtraExtraRow{737}{3.88 \pm 0.17}{0.20 \pm 0.20}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{6.4 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{259}}{\BR(\tau^- \to \mu^- \pi^0)}{}{1.1 \cdot 10^{-7}}{\babar}{Aubert:2006cz}{*}%
\dxLimitsMeasCombExtraExtraRow{623}{4.69 \pm 0.37}{1.33 \pm 0.15}{1}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{1.2 \cdot 10^{-7}}{Belle}{Miyazaki:2007jp}{*}%
\dxLimitsMeasCombExtraExtraRow{737}{4.48 \pm 0.20}{0.58 \pm 0.34}{1}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{8.1 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{260}}{\BR(\tau^- \to e^- K^0_S)}{}{3.3 \cdot 10^{-8}}{\babar}{Aubert:2009ys}{*}%
\dxLimitsMeasCombExtraExtraRow{862}{9.40 \pm 0.20}{1.00 \pm 0.40}{1}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{2.6 \cdot 10^{-8}}{Belle}{Miyazaki:2010qb}{*}%
\dxLimitsMeasCombExtraExtraRow{1234}{7.06 \pm 0.47}{0.18 \pm 0.18}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{2.0 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{261}}{\BR(\tau^- \to \mu^- K^0_S)}{}{4.0 \cdot 10^{-8}}{\babar}{Aubert:2009ys}{*}%
\dxLimitsMeasCombExtraExtraRow{862}{7.00 \pm 0.39}{5.30 \pm 2.20}{2}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{2.3 \cdot 10^{-8}}{Belle}{Miyazaki:2010qb}{*}%
\dxLimitsMeasCombExtraExtraRow{1234}{7.40 \pm 0.50}{0.35 \pm 0.21}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{1.8 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{262}}{\BR(\tau^- \to e^- \eta)}{}{1.6 \cdot 10^{-7}}{\babar}{Aubert:2006cz}{*}%
\dxLimitsMeasCombExtraExtraRow{623}{2.12 \pm 0.20}{0.22 \pm 0.05}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{9.2 \cdot 10^{-8}}{Belle}{Miyazaki:2007jp}{*}%
\dxLimitsMeasCombExtraExtraRow{737}{2.87 \pm 0.14}{0.78 \pm 0.59}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{7.4 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{263}}{\BR(\tau^- \to \mu^- \eta)}{}{1.5 \cdot 10^{-7}}{\babar}{Aubert:2006cz}{*}%
\dxLimitsMeasCombExtraExtraRow{623}{3.59 \pm 0.41}{0.75 \pm 0.08}{1}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{6.5 \cdot 10^{-8}}{Belle}{Miyazaki:2007jp}{*}%
\dxLimitsMeasCombExtraExtraRow{737}{4.08 \pm 0.20}{0.64 \pm 0.38}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{6.1 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{272}}{\BR(\tau^- \to e^- \eta^\prime(958))}{}{2.4 \cdot 10^{-7}}{\babar}{Aubert:2006cz}{*}%
\dxLimitsMeasCombExtraExtraRow{623}{1.53 \pm 0.16}{0.12 \pm 0.03}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{1.6 \cdot 10^{-7}}{Belle}{Miyazaki:2007jp}{*}%
\dxLimitsMeasCombExtraExtraRow{737}{2.15 \pm 0.11}{0.57 \pm 0.41}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{1.3 \cdot 10^{-7}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{273}}{\BR(\tau^- \to \mu^- \eta^\prime(958))}{}{1.4 \cdot 10^{-7}}{\babar}{Aubert:2006cz}{*}%
\dxLimitsMeasCombExtraExtraRow{623}{2.18 \pm 0.26}{0.49 \pm 0.04}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{1.3 \cdot 10^{-7}}{Belle}{Miyazaki:2007jp}{*}%
\dxLimitsMeasCombExtraExtraRow{737}{2.45 \pm 0.13}{0.46 \pm 0.33}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{8.6 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraTypeSep%
\dxLimitsMeasCombExtraTypeHead{\ell S^0}%
\dxLimitsMeasCombExtraRow{\BR_{274}}{\BR(\tau^- \to e^- f_0(980))}{\ell S^0}{6.8 \cdot 10^{-8}}{Belle}{Miyazaki:2008mw}{}%
\dxLimitsMeasCombExtraExtraRow{1233}{2.90 \pm 0.33}{0.10 \pm 0.07}{0}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{275}}{\BR(\tau^- \to \mu^- f_0(980))}{}{6.4 \cdot 10^{-8}}{Belle}{Miyazaki:2008mw}{}%
\dxLimitsMeasCombExtraExtraRow{1233}{3.01 \pm 0.33}{0.11 \pm 0.08}{0}%
\dxLimitsMeasCombExtraTypeSep%
\dxLimitsMeasCombExtraTypeHead{\ell V^0}%
\dxLimitsMeasCombExtraRow{\BR_{264}}{\BR(\tau^- \to e^- \rho^0)}{\ell V^0}{4.6 \cdot 10^{-8}}{\babar}{Aubert:2009ap}{*}%
\dxLimitsMeasCombExtraExtraRow{829}{7.31 \pm 0.18}{1.32 \pm 0.17}{1}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{2.2 \cdot 10^{-8}}{Belle}{Belle:2023ziz}{*}%
\dxLimitsMeasCombExtraExtraRow{1796}{8.49 \pm 0.37}{0.80 \pm 0.27}{1}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{2.0 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{265}}{\BR(\tau^- \to \mu^- \rho^0)}{}{2.6 \cdot 10^{-8}}{\babar}{Aubert:2009ap}{*}%
\dxLimitsMeasCombExtraExtraRow{829}{4.52 \pm 0.41}{2.04 \pm 0.19}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{1.7 \cdot 10^{-8}}{Belle}{Belle:2023ziz}{*}%
\dxLimitsMeasCombExtraExtraRow{1796}{7.78 \pm 0.36}{0.95 \pm 0.25}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{1.3 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{266}}{\BR(\tau^- \to e^- \omega)}{}{1.1 \cdot 10^{-7}}{\babar}{Aubert:2007kx}{*}%
\dxLimitsMeasCombExtraExtraRow{706}{2.61 \pm 0.11}{0.35 \pm 0.06}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{2.4 \cdot 10^{-8}}{Belle}{Belle:2023ziz}{*}%
\dxLimitsMeasCombExtraExtraRow{1796}{5.41 \pm 0.24}{0.74 \pm 0.43}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{2.2 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{267}}{\BR(\tau^- \to \mu^- \omega)}{}{1.0 \cdot 10^{-7}}{\babar}{Aubert:2007kx}{*}%
\dxLimitsMeasCombExtraExtraRow{706}{2.26 \pm 0.14}{0.73 \pm 0.03}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{3.9 \cdot 10^{-8}}{Belle}{Belle:2023ziz}{*}%
\dxLimitsMeasCombExtraExtraRow{1796}{3.27 \pm 0.16}{0.32 \pm 0.30}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{3.4 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{268}}{\BR(\tau^- \to e^- K^*(892))}{}{5.9 \cdot 10^{-8}}{\babar}{Aubert:2009ap}{*}%
\dxLimitsMeasCombExtraExtraRow{829}{8.00 \pm 0.19}{1.65 \pm 0.23}{2}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{1.9 \cdot 10^{-8}}{Belle}{Belle:2023ziz}{*}%
\dxLimitsMeasCombExtraExtraRow{1796}{6.94 \pm 0.28}{0.54 \pm 0.26}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{1.9 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{269}}{\BR(\tau^- \to \mu^- K^*(892))}{}{1.7 \cdot 10^{-7}}{\babar}{Aubert:2009ap}{*}%
\dxLimitsMeasCombExtraExtraRow{829}{4.57 \pm 0.36}{1.79 \pm 0.21}{4}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{2.9 \cdot 10^{-8}}{Belle}{Belle:2023ziz}{*}%
\dxLimitsMeasCombExtraExtraRow{1796}{4.52 \pm 0.19}{0.84 \pm 0.40}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{3.3 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{270}}{\BR(\tau^- \to e^- \bar{K}^*(892))}{}{4.6 \cdot 10^{-8}}{\babar}{Aubert:2009ap}{*}%
\dxLimitsMeasCombExtraExtraRow{829}{7.76 \pm 0.18}{2.76 \pm 0.28}{2}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{1.7 \cdot 10^{-8}}{Belle}{Belle:2023ziz}{*}%
\dxLimitsMeasCombExtraExtraRow{1796}{7.45 \pm 0.31}{0.25 \pm 0.11}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{1.5 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{271}}{\BR(\tau^- \to \mu^- \bar{K}^*(892))}{}{7.3 \cdot 10^{-8}}{\babar}{Aubert:2009ap}{*}%
\dxLimitsMeasCombExtraExtraRow{829}{4.11 \pm 0.32}{1.72 \pm 0.17}{1}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{4.3 \cdot 10^{-8}}{Belle}{Belle:2023ziz}{*}%
\dxLimitsMeasCombExtraExtraRow{1796}{4.58 \pm 0.20}{0.58 \pm 0.21}{1}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{3.7 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{276}}{\BR(\tau^- \to e^- \phi)}{}{3.1 \cdot 10^{-8}}{\babar}{Aubert:2009ap}{*}%
\dxLimitsMeasCombExtraExtraRow{829}{6.43 \pm 0.16}{0.68 \pm 0.12}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{2.0 \cdot 10^{-8}}{Belle}{Belle:2023ziz}{*}%
\dxLimitsMeasCombExtraExtraRow{1796}{6.45 \pm 0.29}{0.38 \pm 0.21}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{1.6 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{277}}{\BR(\tau^- \to \mu^- \phi)}{}{1.9 \cdot 10^{-7}}{\babar}{Aubert:2009ap}{*}%
\dxLimitsMeasCombExtraExtraRow{829}{5.18 \pm 0.27}{2.76 \pm 0.16}{6}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{2.3 \cdot 10^{-8}}{Belle}{Belle:2023ziz}{*}%
\dxLimitsMeasCombExtraExtraRow{1796}{5.59 \pm 0.27}{0.47 \pm 0.16}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{2.6 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraTypeSep%
\dxLimitsMeasCombExtraTypeHead{\ell\ell\ell}%
\dxLimitsMeasCombExtraRow{\BR_{278}}{\BR(\tau^- \to e^- e^+ e^-)}{\ell\ell\ell}{2.9 \cdot 10^{-8}}{\babar}{Lees:2010ez}{*}%
\dxLimitsMeasCombExtraExtraRow{860}{8.60 \pm 0.20}{0.12 \pm 0.02}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{2.7 \cdot 10^{-8}}{Belle}{Hayasaka:2010np}{*}%
\dxLimitsMeasCombExtraExtraRow{1437}{6.00 \pm 0.59}{0.21 \pm 0.15}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{1.9 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{279}}{\BR(\tau^- \to e^- \mu^+ \mu^-)}{}{3.2 \cdot 10^{-8}}{\babar}{Lees:2010ez}{*}%
\dxLimitsMeasCombExtraExtraRow{860}{6.40 \pm 0.40}{0.54 \pm 0.14}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{2.7 \cdot 10^{-8}}{Belle}{Hayasaka:2010np}{*}%
\dxLimitsMeasCombExtraExtraRow{1437}{6.10 \pm 0.58}{0.10 \pm 0.04}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{2.0 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{280}}{\BR(\tau^- \to \mu^- e^+ \mu^-)}{}{2.6 \cdot 10^{-8}}{\babar}{Lees:2010ez}{*}%
\dxLimitsMeasCombExtraExtraRow{860}{10.20 \pm 0.60}{0.03 \pm 0.02}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{1.7 \cdot 10^{-8}}{Belle}{Hayasaka:2010np}{*}%
\dxLimitsMeasCombExtraExtraRow{1437}{10.10 \pm 0.77}{0.02 \pm 0.02}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{1.4 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{281}}{\BR(\tau^- \to \mu^- e^+ e^-)}{}{2.2 \cdot 10^{-8}}{\babar}{Lees:2010ez}{*}%
\dxLimitsMeasCombExtraExtraRow{860}{8.80 \pm 0.50}{0.64 \pm 0.19}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{1.8 \cdot 10^{-8}}{Belle}{Hayasaka:2010np}{*}%
\dxLimitsMeasCombExtraExtraRow{1437}{9.30 \pm 0.73}{0.04 \pm 0.04}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{1.3 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{282}}{\BR(\tau^- \to e^- \mu^+ e^-)}{}{1.8 \cdot 10^{-8}}{\babar}{Lees:2010ez}{*}%
\dxLimitsMeasCombExtraExtraRow{860}{12.70 \pm 0.70}{0.34 \pm 0.12}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{1.5 \cdot 10^{-8}}{Belle}{Hayasaka:2010np}{*}%
\dxLimitsMeasCombExtraExtraRow{1437}{11.50 \pm 0.89}{0.01 \pm 0.01}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{1.1 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{283}}{\BR(\tau^- \to \mu^- \mu^+ \mu^-)}{}{3.8 \cdot 10^{-7}}{ATLAS}{Aad:2016wce}{}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{3.3 \cdot 10^{-8}}{\babar}{Lees:2010ez}{*}%
\dxLimitsMeasCombExtraExtraRow{860}{6.60 \pm 0.60}{0.44 \pm 0.17}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{2.1 \cdot 10^{-8}}{Belle}{Hayasaka:2010np}{*}%
\dxLimitsMeasCombExtraExtraRow{1437}{7.60 \pm 0.56}{0.13 \pm 0.20}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{1.9 \cdot 10^{-8}}{Belle\,II}{Belle-II:2024sce}{*}%
\dxLimitsMeasCombExtraExtraRow{777}{20.42 \pm 0.93}{0.70 \pm 0.56}{1}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{2.9 \cdot 10^{-8}}{CMS}{CMS:2023iqy}{*}%
\dxLimitsMeasCombExtraExtraBrRow{5.1 \cdot 10^{-9}}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{4.6 \cdot 10^{-8}}{LHCb}{Aaij:2014azz}{*}%
\dxLimitsMeasCombExtraExtraBrRow{2.3 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{1.6 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraTypeSep%
\dxLimitsMeasCombExtraTypeHead{\ell hh}%
\dxLimitsMeasCombExtraRow{\BR_{284}}{\BR(\tau^- \to e^- \pi^+ \pi^-)}{\ell hh}{1.2 \cdot 10^{-7}}{\babar}{Aubert:2005tp}{*}%
\dxLimitsMeasCombExtraExtraRow{407}{3.30 \pm 0.15}{0.81 \pm 0.13}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{2.3 \cdot 10^{-8}}{Belle}{Miyazaki:2012mx}{*}%
\dxLimitsMeasCombExtraExtraRow{1564}{5.45 \pm 0.31}{0.55 \pm 0.23}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{2.1 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{285}}{\BR(\tau^- \to e^+ \pi^- \pi^-)}{}{2.7 \cdot 10^{-7}}{\babar}{Aubert:2005tp}{}%
\dxLimitsMeasCombExtraExtraRow{407}{3.40 \pm 0.15}{0.41 \pm 0.10}{1}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{2.0 \cdot 10^{-8}}{Belle}{Miyazaki:2012mx}{}%
\dxLimitsMeasCombExtraExtraRow{1564}{6.56 \pm 0.36}{0.37 \pm 0.19}{0}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{286}}{\BR(\tau^- \to \mu^- \pi^+  \pi^-)}{}{2.9 \cdot 10^{-7}}{\babar}{Aubert:2005tp}{}%
\dxLimitsMeasCombExtraExtraRow{407}{3.40 \pm 0.19}{2.99 \pm 0.41}{3}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{2.1 \cdot 10^{-8}}{Belle}{Miyazaki:2012mx}{}%
\dxLimitsMeasCombExtraExtraRow{1564}{5.83 \pm 0.33}{0.63 \pm 0.23}{0}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{287}}{\BR(\tau^- \to \mu^+ \pi^- \pi^-)}{}{7.0 \cdot 10^{-8}}{\babar}{Aubert:2005tp}{*}%
\dxLimitsMeasCombExtraExtraRow{407}{3.30 \pm 0.18}{1.46 \pm 0.27}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{3.9 \cdot 10^{-8}}{Belle}{Miyazaki:2012mx}{*}%
\dxLimitsMeasCombExtraExtraRow{1564}{6.55 \pm 0.37}{0.33 \pm 0.16}{1}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{3.5 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{288}}{\BR(\tau^- \to e^- \pi^+ K^-)}{}{3.2 \cdot 10^{-7}}{\babar}{Aubert:2005tp}{*}%
\dxLimitsMeasCombExtraExtraRow{407}{3.10 \pm 0.13}{0.14 \pm 0.06}{1}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{3.7 \cdot 10^{-8}}{Belle}{Miyazaki:2012mx}{*}%
\dxLimitsMeasCombExtraExtraRow{1564}{3.97 \pm 0.25}{0.18 \pm 0.13}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{3.8 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{289}}{\BR(\tau^- \to e^- K^+ \pi^-)}{}{1.7 \cdot 10^{-7}}{\babar}{Aubert:2005tp}{*}%
\dxLimitsMeasCombExtraExtraRow{407}{3.08 \pm 0.13}{0.32 \pm 0.08}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{3.1 \cdot 10^{-8}}{Belle}{Miyazaki:2012mx}{*}%
\dxLimitsMeasCombExtraExtraRow{1564}{4.07 \pm 0.25}{0.55 \pm 0.31}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{2.9 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{290}}{\BR(\tau^- \to e^+ \pi^- K^-)}{}{1.8 \cdot 10^{-7}}{\babar}{Aubert:2005tp}{*}%
\dxLimitsMeasCombExtraExtraRow{407}{3.19 \pm 0.14}{0.16 \pm 0.06}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{3.2 \cdot 10^{-8}}{Belle}{Miyazaki:2012mx}{*}%
\dxLimitsMeasCombExtraExtraRow{1564}{4.00 \pm 0.25}{0.46 \pm 0.21}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{3.1 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{291}}{\BR(\tau^- \to e^- K^0_S K^0_S)}{}{7.1 \cdot 10^{-8}}{Belle}{Miyazaki:2010qb}{}%
\dxLimitsMeasCombExtraExtraRow{1234}{2.79 \pm 0.31}{0.07 \pm 0.07}{0}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{292}}{\BR(\tau^- \to e^- K^+ K^-)}{}{1.4 \cdot 10^{-7}}{\babar}{Aubert:2005tp}{*}%
\dxLimitsMeasCombExtraExtraRow{407}{3.77 \pm 0.16}{0.22 \pm 0.06}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{3.4 \cdot 10^{-8}}{Belle}{Miyazaki:2012mx}{*}%
\dxLimitsMeasCombExtraExtraRow{1564}{4.29 \pm 0.29}{0.17 \pm 0.10}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{3.3 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{293}}{\BR(\tau^- \to e^+ K^- K^-)}{}{1.5 \cdot 10^{-7}}{\babar}{Aubert:2005tp}{*}%
\dxLimitsMeasCombExtraExtraRow{407}{3.85 \pm 0.16}{0.04 \pm 0.04}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{3.3 \cdot 10^{-8}}{Belle}{Miyazaki:2012mx}{*}%
\dxLimitsMeasCombExtraExtraRow{1564}{4.64 \pm 0.30}{0.06 \pm 0.06}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{3.2 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{294}}{\BR(\tau^- \to \mu^- \pi^+  K^-)}{}{2.6 \cdot 10^{-7}}{\babar}{Aubert:2005tp}{*}%
\dxLimitsMeasCombExtraExtraRow{407}{2.87 \pm 0.16}{1.04 \pm 0.18}{1}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{8.6 \cdot 10^{-8}}{Belle}{Miyazaki:2012mx}{*}%
\dxLimitsMeasCombExtraExtraRow{1564}{2.72 \pm 0.17}{0.72 \pm 0.28}{1}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{8.2 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{295}}{\BR(\tau^- \to \mu^- K^+  \pi^-)}{}{3.2 \cdot 10^{-7}}{\babar}{Aubert:2005tp}{*}%
\dxLimitsMeasCombExtraExtraRow{407}{2.97 \pm 0.16}{1.67 \pm 0.29}{2}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{4.5 \cdot 10^{-8}}{Belle}{Miyazaki:2012mx}{*}%
\dxLimitsMeasCombExtraExtraRow{1564}{2.62 \pm 0.15}{0.64 \pm 0.23}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{4.6 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{296}}{\BR(\tau^- \to \mu^+ \pi^- K^-)}{}{2.2 \cdot 10^{-7}}{\babar}{Aubert:2005tp}{*}%
\dxLimitsMeasCombExtraExtraRow{407}{2.85 \pm 0.16}{1.54 \pm 0.25}{1}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{4.8 \cdot 10^{-8}}{Belle}{Miyazaki:2012mx}{*}%
\dxLimitsMeasCombExtraExtraRow{1564}{2.55 \pm 0.16}{0.56 \pm 0.21}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{4.5 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{297}}{\BR(\tau^- \to \mu^- K^0_S  K^0_S)}{}{8.0 \cdot 10^{-8}}{Belle}{Miyazaki:2010qb}{}%
\dxLimitsMeasCombExtraExtraRow{1234}{2.43 \pm 0.27}{0.12 \pm 0.08}{0}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{298}}{\BR(\tau^- \to \mu^- K^+  K^-)}{}{2.5 \cdot 10^{-7}}{\babar}{Aubert:2005tp}{*}%
\dxLimitsMeasCombExtraExtraRow{407}{2.16 \pm 0.12}{0.24 \pm 0.07}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{4.4 \cdot 10^{-8}}{Belle}{Miyazaki:2012mx}{*}%
\dxLimitsMeasCombExtraExtraRow{1564}{2.85 \pm 0.17}{0.51 \pm 0.19}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{4.2 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{299}}{\BR(\tau^- \to \mu^+ K^- K^-)}{}{4.8 \cdot 10^{-7}}{\babar}{Aubert:2005tp}{}%
\dxLimitsMeasCombExtraExtraRow{407}{2.06 \pm 0.11}{0.07 \pm 0.10}{1}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{4.7 \cdot 10^{-8}}{Belle}{Miyazaki:2012mx}{}%
\dxLimitsMeasCombExtraExtraRow{1564}{2.98 \pm 0.18}{0.25 \pm 0.13}{0}%
\dxLimitsMeasCombExtraTypeSep%
\dxLimitsMeasCombExtraTypeHead{\text{BNV}}%
\dxLimitsMeasCombExtraRow{\BR_{311}}{\BR(\tau^- \to \pi^- \Lambda)}{\text{BNV}}{7.2 \cdot 10^{-8}}{Belle}{Miyazaki:2005ng}{*}%
\dxLimitsMeasCombExtraExtraRow{283}{7.48 \pm 0.68}{1.70 \pm 0.80}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{4.7 \cdot 10^{-8}}{Belle\,II}{Belle-II:2024ynh}{*}%
\dxLimitsMeasCombExtraExtraRow{669}{9.50 \pm 0.26}{1.00 \pm 1.20}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{3.0 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{312}}{\BR(\tau^- \to \pi^- \bar{\Lambda})}{}{1.4 \cdot 10^{-7}}{Belle}{Miyazaki:2005ng}{*}%
\dxLimitsMeasCombExtraExtraRow{283}{7.54 \pm 0.69}{1.70 \pm 0.80}{1}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{4.3 \cdot 10^{-8}}{Belle\,II}{Belle-II:2024ynh}{*}%
\dxLimitsMeasCombExtraExtraRow{669}{9.90 \pm 0.28}{0.50 \pm 0.60}{0}%
\dxLimitsMeasCombExtraCombSep%
\dxLimitsMeasCombExtraCombRow{}{}{}{3.8 \cdot 10^{-8}}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{315}}{\BR(\tau^- \to \bar{p} e^+ e^-)}{}{3.0 \cdot 10^{-8}}{Belle}{Belle:2020lfn}{}%
\dxLimitsMeasCombExtraExtraRow{1682}{7.80 \pm 0.39}{0.50 \pm 0.35}{1}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{316}}{\BR(\tau^- \to p e^- e^-)}{}{3.0 \cdot 10^{-8}}{Belle}{Belle:2020lfn}{}%
\dxLimitsMeasCombExtraExtraRow{1682}{8.00 \pm 0.40}{0.23 \pm 0.07}{1}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{317}}{\BR(\tau^- \to \bar{p} e^+ \mu^-)}{}{2.0 \cdot 10^{-8}}{Belle}{Belle:2020lfn}{}%
\dxLimitsMeasCombExtraExtraRow{1682}{6.50 \pm 0.33}{0.22 \pm 0.06}{0}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{318}}{\BR(\tau^- \to \bar{p} e^- \mu^+)}{}{1.8 \cdot 10^{-8}}{Belle}{Belle:2020lfn}{}%
\dxLimitsMeasCombExtraExtraRow{1682}{6.90 \pm 0.34}{0.40 \pm 0.28}{0}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{319}}{\BR(\tau^- \to p \mu^- \mu^-)}{}{4.0 \cdot 10^{-8}}{Belle}{Belle:2020lfn}{}%
\dxLimitsMeasCombExtraExtraRow{1682}{4.60 \pm 0.23}{1.30 \pm 0.46}{1}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{4.4 \cdot 10^{-7}}{LHCb}{Aaij:2013fia}{}%
\dxLimitsMeasCombExtraModeSep%
\dxLimitsMeasCombExtraRow{\BR_{320}}{\BR(\tau^- \to \bar{p} \mu^+ \mu^-)}{}{1.8 \cdot 10^{-8}}{Belle}{Belle:2020lfn}{}%
\dxLimitsMeasCombExtraExtraRow{1682}{5.00 \pm 0.25}{1.14 \pm 0.43}{0}%
\dxLimitsMeasCombExtraLimitSep%
\dxLimitsMeasCombExtraRow{}{}{}{3.3 \cdot 10^{-7}}{LHCb}{Aaij:2013fia}{}%
}


==> tau/tau-lfv-limits-combs-plot.tex <==
%
%
\ifhevea
%
%
\fi

\begin{figure}[tb]
  \begin{center}
    \ifhevea
    \begin{tabular}{@{}cc@{}}
      \larger\bfseries\ahref{tau-lfv-limits.png}{full size PNG} &
      \larger\bfseries\ahref{tau-lfv-limits.pdf}{PDF format} \\
      \multicolumn{2}{c}{\ahref{tau-lfv-limits.png}{%
          \imgsrc[alt="Tau LFV limits combinations plot" height=340]{tau-lfv-limits-combs.png}}}
    \end{tabular}
    \else
%
     \includegraphics[angle=0,width=0.95\linewidth,clip]{figures/tau/tau-lfv-limits-combs.pdf}      
    \fi
    \caption{Tau lepton-flavour-violating branching fraction upper
      limits and combinations. In order to appreciate the physics reach
      improvement over time, the plot includes also the CLEO upper
      limits reported by PDG 2022~\cite{PDG_2022}.
      \label{fig:tau:lfv-limits-combs-plot}
    }
  \end{center}
\end{figure}


==> tau/tau-sections.tex <==
This section reports the averages of the \mtau
mass~(Section~\ref{sec:tau:mass}) and
lifetime~(Section~\ref{sec:tau:lifetime}), and a global fit of the
available measurements of the \mtau branching fractions
(Section~\ref{sec:tau:br-fit}). When the averaged measurements have
asymmetric uncertainties, they are symmetrized using the quadratic
average, i.e., the square root of the mean of the squares of the
positive and negative uncertainties.
\iffalse
  In this edition, we do not include the combinations of upper limits on
  \mtau lepton-flavour-violating branching fractions, which were
  published in previous editions, since it was not possible to update
  this contribution in due time.
\fi
The fit results are used in Section~\ref{sec:tau:leptonuniv} to test
the lepton-flavour universality of the charged-current weak interaction. A
``universality-improved''~\cite{Davier:2005xq} branching fraction
$\BR_e=\BR(\tau \to e \nu \bar{\nu})$ and the ratio between the hadronic
branching fraction and $\BR_e$ are obtained in
Section~\ref{sec:tau:be-univ-rtau}. The value of the Cabibbo-Kobayashi-Maskawa
(CKM) matrix element \Vus obtained from \mtau decays is given in
Section~\ref{sec:tau:vus}.
\iftrue
  Combinations of upper limits on
  lepton-flavour-violating \mtau branching fractions are computed in
  Section~\ref{sec:tau:lfv-limits}.
\fi
%
We use measurements reported through September 2023 and the following
ones that were made available at a later time:
\begin{itemize}
\item $\inlineFracParen{\dxuse{Gamma3by5-td}}$ by the Belle II experiment~\dxuse{\dxuse{Belle2.Gamma3by5.ADACHI.2024-pdgref}-cite},
\item $\dxuse{Gamma283-td}$ by the CMS experiment~\cite{CMS:2023iqy}, 
\item $\dxuse{Gamma283-td}$ by the Belle II experiment~\cite{Belle-II:2024sce}, 
\item ${\BR(\tau^- \to \pi^- \Lambda)}$ by the Belle II experiment~\cite{Belle-II:2024ynh}, and
\item ${\BR(\tau^- \to \pi^- \bar{\Lambda})}$ by the Belle II experiment~\cite{Belle-II:2024ynh}.
  
\end{itemize}

\subsection{\texorpdfstring{\mtau mass}{tau mass}}
\cutname{tau-mass-avg.html}
\label{sec:tau:mass}

A total of \dxuse{TauMassMeasNum} \mtau mass measurements are averaged. The fit
has $\chi^2/\text{d.o.f.} = \dxuse{TauMassChisq}/\dxuse{TauMassDof}$,
corresponding to a confidence level $\text{CL} = \dxuse{TauMassChisqProb}$.
We include recent measurements by Belle\,II~\dxuse{ADACHI 2023C-cite}
and KEDR~\dxuse{ANASHIN 2023A-cite}, which were not included in the 2022 edition and 2023 update of the Review of Particle Physics~\cite{PDG_2022}.
Table~\ref{tab:tau:mass} and
Figure~\ref{fig:tau:mass} report the experimental inputs and the calculated
average, which are also available
at~\cite{heavy_flavor_averaging_group_2024_13989054}.
%
%
%
\begin{table}[bp]
  \begin{center}
    \begin{envsmall}
      \setlength{\LTcapwidth}{0.85\linewidth}
      \renewcommand*{\arraystretch}{1.3}%
      \ifhevea
        \renewcommand{\bar}[1]{\textoverline{#1}}
      \else
        \begin{citenoleadsp}
          \fi
          \caption{%
            \mtau mass measurements and their average.\label{tab:tau:mass}}%
          \ifhevea
            \begin{center}
              \fi
              \begin{tabular}{llll}
                \toprule
                \multicolumn{1}{l}{\bfseries \mtau mass [MeV]} &
                \multicolumn{1}{l}{\bfseries Experiment}       &
                \multicolumn{1}{l}{\bfseries Reference}          \\
                \midrule
                \dxuse{TauMassQuantMeasTable}
                \\
                \midrule
                \dxuse{tau_mass-vu} & HFLAV average &
                \\
                \bottomrule
              \end{tabular}
              \ifhevea
            \end{center}
          \fi
          \ifhevea\else
        \end{citenoleadsp}
      \fi
    \end{envsmall}
  \end{center}
\end{table}
%
\begin{figure}[bp]
  \begin{center}
    \ifhevea
      \begin{tabular}{@{}cc@{}}
        \larger\bfseries\ahref{tau-mass.png}{PNG format} &
        \larger\bfseries\ahref{tau-mass.pdf}{PDF format}   \\
        \multicolumn{2}{c}{\ahref{tau-mass.png}{%
            \imgsrc[alt="Tau mass average"]{tau-mass.png}}}
      \end{tabular}
      \else
      {\fboxsep=2pt\fbox{%
          \includegraphics[width=0.50\linewidth,clip]{figures/tau/tau-mass.pdf}}}
    \fi
    \caption{\mtau mass measurements and their average.%
      \label{fig:tau:mass}%
    }
  \end{center}
\end{figure}

\subsection{\texorpdfstring{\mtau lifetime}{tau lifetime}}
\cutname{tau-lifetime-avg.html}
\label{sec:tau:lifetime}

A total of \dxuse{TauLifeMeasNum} \mtau lifetime measurements are averaged. All
are included in the 2022 edition and 2023 update of the Review of Particle
Physics~\cite{PDG_2022}. The fit has $\chi^2/\text{d.o.f.} =
  \dxuse{TauLifeChisq}/\dxuse{TauLifeDof}$, corresponding to a confidence level
$\text{CL} = \dxuse{TauLifeChisqProb}$. Table~\ref{tab:tau:lifetime} and
Figure~\ref{fig:tau:lifetime} report the experimental inputs and the calculated
average, which are also available
at~\cite{heavy_flavor_averaging_group_2024_13989054}.

%
%
%
\begin{table}[tbp]
  \begin{center}
    \begin{envsmall}
      \setlength{\LTcapwidth}{0.85\linewidth}
      \renewcommand*{\arraystretch}{1.3}%
      \ifhevea
        \renewcommand{\bar}[1]{\textoverline{#1}}
      \else
        \begin{citenoleadsp}
          \fi
          \caption{%
            \mtau lifetime measurements and their average.\label{tab:tau:lifetime}}%
          \ifhevea
            \begin{center}
              \fi
              \begin{tabular}{llll}
                \toprule
                \multicolumn{1}{l}{\bfseries \mtau lifetime [fs]} &
                \multicolumn{1}{l}{\bfseries Experiment}          &
                \multicolumn{1}{l}{\bfseries Reference}             \\
                \midrule
                \dxuse{TauLifeQuantMeasTable}
                \\
                \midrule
                \dxuse{tau_life-vu} & HFLAV average &
                \\
                \bottomrule
              \end{tabular}
              \ifhevea
            \end{center}
          \fi
          \ifhevea\else
        \end{citenoleadsp}
      \fi
    \end{envsmall}
  \end{center}
\end{table}
\begin{figure}[tbp]
  \begin{center}
    \ifhevea
      \begin{tabular}{@{}cc@{}}
        \larger\bfseries\ahref{tau-life.png}{PNG format} &
        \larger\bfseries\ahref{tau-life.pdf}{PDF format}   \\
        \multicolumn{2}{c}{\ahref{tau-life.png}{%
            \imgsrc[alt="Tau lifetime average"]{tau-life.png}}}
      \end{tabular}
      \else
      {\fboxsep=2pt\fbox{%
          \includegraphics[width=0.50\linewidth,clip]{figures/tau/tau-life.pdf}}}
    \fi
    \caption{\mtau lifetime measurements and their average.%
      \label{fig:tau:lifetime}%
    }
  \end{center}
\end{figure}

%
\subsection{Branching fraction fit}
\cutname{br-fit.html}
\label{sec:tau:br-fit}

A fit of the available experimental measurements is used to determine the \mtau
branching fractions.
\iffalse
  The \mtau branching fractions provide a test for theory predictions
  based on the Standard Model (SM) EW and QCD interactions and can be
  further elaborated to test the EW charged-current universality for
  leptons, and to determine the CKM matrix coefficient \Vus and the QCD
  coupling constant $\alpha_s$ at the \mtau mass.
\fi
All relevant published statistical
and systematic correlations among the measurements are used. In addition, for a
selection of measurements, particularly the most precise and the most recent
ones, the documentation on the systematic uncertainties' contributions is
examined to determine how they depend on parameters such as other \mtau
branching fractions or other external parameters, e.g., $\eta$ and $\omega$
meson branching fractions and the cross-section $\sigma(e^+e^- \to
  \tau^+\tau^-)$.
\ifx\tauStandalone\undefined
  We follow the procedures detailed
  in Section~\ref{sec:method:corrSysts} to
\else
  We use the standard HFLAV procedures~\cite{HFLAV:2022esi} to
\fi
adjust the measurements' values and
uncertainties to account for the updated values and uncertainties of the
external parameters, which are taken from the Review of Particle
Physics~\cite{PDG_2022}. The measurements' correlations are adjusted to account
for the dependence of different measurement on the same parameters.

Following a convention established in the Review of Particle Physics, \mtau
branching fractions are often labelled with the final state content of
$\pi^\pm$, $\pi^0$, $K^\pm$, $\gamma$, implicitly including decay chains that
involve intermediate particles, e.g., $K^0_S\to\pi^+\pi^-$, and $\eta$,
$\omega$, $\phi$ decays. When measurements exclude the contribution of some or
all the known intermediate particles, the branching fraction notation flags
this information by adding, e.g., ``ex.$K^0$''.

Each measurement is modeled with one fit parameter that is either a \mtau decay
branching fraction, labelled $\BR_{i}$, or a ratio of two \mtau decay branching
fractions, labelled $\BR_{i/j} = \BR_{i}/\BR_{j}$. Some branching fractions are
linear combinations of other branching fractions: for instance
$\dxuse{Gamma8-gn} = \dxuse{Gamma8-td}$ is the sum of $\dxuse{Gamma9-gn} =
  \dxuse{Gamma9-td}$ and $\dxuse{Gamma10-gn} = \dxuse{Gamma10-td}$, with the
symbol $h$ referring to a $\pi$ or a $K$. In some cases, constraints arise from
approximate relations that nevertheless hold within the present experimental
precision and are treated as exact. For instance, the constraint
$\dxuse{Gamma96-td} = \dxuse{Gamma167-td} \times \BR(\phi\to K^+K^-)$ is
justified according to the current experimental evidence. The constraint
equations depend on uncertain quantities, such as $\BR(\phi\to K^+K^-)$ in this
example. The uncertainties associated with these constraints are typically
smaller in relative value than the uncertainties on the \mtau branching
fractions. Therefore, we neglect all of them except for the poorly known
branching fraction $\dxuse{Gamma980-gn} = \dxuse{Gamma980-td}$, which is
modeled with a nuisance fit parameter, based on the value and uncertainty
estimated by the ALEPH collaboration~\dxuse{SCHAEL 05C-cite}. All the
constraints are listed in Section~\ref{sec:tau:constraints}.

The fit \chisq is \ifx\tauStandalone\undefined constructed following
  Eq.~(\ref{eq:averageEq}) \fi
\begin{align}
  \chisq =
  \sum_{ijkl}\left(m_i - M_{ik} q_k\right)
  \left(V^{-1}\right)_{ij}
  \left(m_j - M_{jl} q_l\right)
  +
  \sum_r \frac{(n_r - p_r)^2}{\sigma_{n_r}^2}
  ~,
\end{align}
where $m_i$ is a measurement result, $q_k$ is a fit
parameter, $V_{ij}$ is the covariance matrix that describes the measurements'
uncertainties and correlations, $M_{ik}$ is a model matrix that specifies
the linear combination of the fit parameters corresponding to the measurement $m_i$, $p_r$ is a nuisance fit
parameter, and $n_r$ and $\sigma_{n_r}$ are, respectively, the value and uncertainty that summarize the existing prior knowledge on $p_r$. In the current fit, the second sum includes just one nuisance fit parameter.

The \chisq is minimized varying all fit parameters while respecting all
constraints, using the technique of the Lagrange multipliers
\ifx\tauStandalone\undefined (see Sec.~\ref{sec:method})\else\fi.%

\label{ref:tau:kkk-unc-scale-factor}%
%
In performing the fit, a scale factor of 5.44 was applied to the published
uncertainties of the two severely inconsistent measurements of
\(\dxuse{Gamma96-gn} = \dxuse{Gamma96-td}\) by \babar and Belle. The
scale-factor value was chosen using the PDG procedure, \ie, it is such that
$\chi^2/\text{d.o.f.}=1$ when fitting just the two \(\dxuse{Gamma96-gn}\)
measurements.

%
\subsubsection{Changes with respect to the previous report}

The 2021 HFLAV report~\cite{HFLAV:2022esi} used the ALEPH 2006 estimate
of $\dxuse{Gamma805-gn} = \dxuse{Gamma805-td}$~\dxuse{SCHAEL 05C-cite}
and treated it as an experimental measurement, therefore
$\dxuse{Gamma805-gn} = \dxuse{Gamma805-td}$ was determined using
$\dxuse{Gamma980-gn} = \dxuse{Gamma980-td}$ and the values of
$\dxuse{Gamma62-gn} = \dxuse{Gamma62-td}$ and $\dxuse{Gamma20-gn} =
  \dxuse{Gamma20-td}$ as known at the time of the ALEPH 2006 publication.
In this edition, we use an estimate of \dxuse{Gamma980-gn} in a
constraint equation that defines \dxuse{Gamma805-gn}, and
\dxuse{Gamma980-gn} is optimized in the \mtau branching fraction fit as
nuisance fit parameter. With the current procedure, \dxuse{Gamma805-gn}
is determined using \dxuse{Gamma980-gn} and the fit values of
\dxuse{Gamma62-gn} and \dxuse{Gamma20-gn}. The fit returns
$\dxuse{Gamma805-gn} = \dxuse{Gamma805-vu}$, while the HFLAV 2021
report~\cite{HFLAV:2022esi} had $\dxuse{Gamma805-gn} = (0.40\pm
  0.20)\cdot10^{-3}$ (the ALEPH estimate~\cite{Schael:2005am}). The other
\mtau branching fractions averages are not affected by this modification
of the fit procedure.

We include in the \mtau branching fraction fit measurements the recently
published measurement of the ratio of the \mtau leptonic branching fractions:
\begin{align}
  \dxuse{Gamma3by5-td} = \dxuse{Belle2.Gamma3by5.ADACHI.2024-vu}
\end{align}
by the Belle~II
experiment~\dxuse{\dxuse{Belle2.Gamma3by5.ADACHI.2024-pdgref}-cite}.
Since this result is the most precise measurement from a single
experiment to date, the precision of the fitted leptonic branching
fractions is also improved.

We also report the results from a unitarity-constrained fit, along with
the results from the non-unitarity-constrained fit. The results from the
unitarity-constrained fit are required as inputs for tau-decay Monte
Carlo event generators, such as Tauola~\cite{Banerjee:2021rtn}, and were
not included in the previous reports.

The parameters used to update the measurements' systematic biases and the
parameters appearing in the constraint equations in
Section~\ref{sec:tau:constraints} have been updated to values reported in the Review of Particle Physics 2022 and 2023 update~\cite{PDG_2022}.

%
\subsubsection{Differences with respect to the PDG fit}
\label{sec:tau:diffpdg}

The \mtau branching fraction fit provided by HFLAV for the 2024 edition
of the Review of Particle Physics reports as in the past editions only
the unitarity-constrained fit results, and includes all the updates of
this report, except the recent Belle~II measurement of the ratio of the \mtau leptonic branching fractions, which was published later than the new literature publication deadline.

%
%

%
%
%
%
%
%

%
\subsubsection{Fit results}
\label{sec:tau:fit}

We use a total of \dxuse{TauBrMeasNum} \mtau branching fractions and ratios
measurements and \dxuse{TauBrMeasNumNuisance} nuisance fit parameter measurement to optimize \dxuse{TauBrQuantNum} fit parameters and \dxuse{TauBrQuantNumNuisance} nuisance fit parameter, while respecting
\dxuse{TauBrConstrNum} equality constraints.
%
When considering just the \mtau branching fractions, omitting the nuisance fit
parameter, the fit has $\chi^2/\text{d.o.f.} =
  \dxuse{TauBrChisq}/\dxuse{TauBrDof}$, corresponding to a confidence level
$\text{CL} = \dxuse{TauBrChisqProb}$.
%
The fitted parameters' values and uncertainties corresponding to \mtau
branching fractions measurements are listed in
Table~\ref{tab:tau:br-var-meas}, for both the universality-constrained fit and the unconstrained fit. The table also includes:
\begin{itemize}

  \item $\dxuse{Gamma110-gn} = \dxuse{Gamma110-td}$,
  the total measured branching fraction of \mtau decays
  to final states with net strangeness;

  \item $\dxuse{GammaAll-gn}$,
  the total branching fraction of the \mtau into any known
  final state according to measurements, defined by its constraint equation in Section~\ref{sec:tau:constraints};

  \item $\dxuse{GammaUnitResid-gn} = \dxuse{GammaUnitResid-right}$,
  the \mtau decay unitarity residual.

\end{itemize}
When no unitarity constraint is applied, we find that
\dxuse{GammaUnitResid-gn} is consistent with 0.
%
The nuisance fit parameter's value and uncertainty are listed in
Table~\ref{tab:tau:br-nuis-meas}.
%
All resulting fit parameters, their input measurements, and their
correlation matrix are available
at~\cite{heavy_flavor_averaging_group_2024_13989054}.
\iffalse
  Although the fit treats all fit parameters in the same way, for the
  purpose of presenting correlations we select a set of
  \dxuse{TauBrBaseQuantNum} ``basis fit parameters'' from which all
  remaining fit parameters can be calculated using the constraint
  equations listed in Section~\ref{sec:tau:constraints}. The correlation
  matrix between the basis fit parameters is listed in
  Section~\ref{sec:tau:fitcorr}.
\fi

%
%
%
{%
%
%
%
%
\renewcommand{\dxQuantMeasLine}[1]{%
  \dxuse{#1-vu} & average & \\
  \dxusef{uc}{#1-vu} & average with u.c. &%
}%
\begin{center}
  \begin{envsmall}
    \setlength{\LTcapwidth}{0.85\linewidth}
    \renewcommand*{\arraystretch}{1.3}%
    \ifhevea
      \renewcommand{\bar}[1]{\textoverline{#1}}
    \else
      \begin{citenoleadsp}
        \fi
        \begin{longtable}{llll}
          \caption{Fit averages and measurements of \mtau branching fractions and ratios of branching fractions.
            The label ``u.c.'' indicates the results from the unitarity-constrained fit.\label{tab:tau:br-var-meas}}%
          \\
          \toprule
          \multicolumn{1}{l}{\bfseries Fit parameter} &
          \multicolumn{1}{l}{\bfseries Experiment}    &
          \multicolumn{1}{l}{\bfseries Reference}                                                 \\
          \midrule
          \endfirsthead
          \multicolumn{4}{c}{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\ \midrule
          \multicolumn{1}{l}{\bfseries Fit parameter} &
          \multicolumn{1}{l}{\bfseries Experiment}    &
          \multicolumn{1}{l}{\bfseries Reference}                                                 \\
          \midrule
          \endhead
          \endfoot
          \endlastfoot
          \dxuse{TauBrVarMeasTable}                                                               \\
          \bottomrule
        \end{longtable}
        \ifhevea\else
      \end{citenoleadsp}
    \fi
  \end{envsmall}
\end{center}%
}

%
%
%
\begin{center}
  \begin{envsmall}
    \setlength{\LTcapwidth}{0.85\linewidth}
    \renewcommand*{\arraystretch}{1.3}%
    \ifhevea
      \renewcommand{\bar}[1]{\textoverline{#1}}
    \else
      \begin{citenoleadsp}
        \fi
        \begin{longtable}{llll}
          \caption{Nuisance fit parameter of the \mtau branching fractions fit.\label{tab:tau:br-nuis-meas}}%
          \\
          \toprule
          \multicolumn{1}{l}{\bfseries Nuisance fit parameter} &
          \multicolumn{1}{l}{\bfseries Experiment}             &
          \multicolumn{1}{l}{\bfseries Reference}                                                 \\
          \midrule
          \endfirsthead
          \multicolumn{4}{c}{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\ \midrule
          \multicolumn{1}{l}{\bfseries Nuisance fit parameter} &
          \multicolumn{1}{l}{\bfseries Experiment}             &
          \multicolumn{1}{l}{\bfseries Reference}                                                 \\
          \midrule
          \endhead
          \endfoot
          \endlastfoot
          \dxuse{TauBrNuisMeasTable}                                                              \\
          \bottomrule
        \end{longtable}
        \ifhevea\else
      \end{citenoleadsp}
    \fi
  \end{envsmall}
\end{center}

\iffalse
  \subsubsection{Correlation coefficients between the basis fit parameters' uncertainties}
  \label{sec:tau:fitcorr}

  Table~\ref{tab:tau:br-fit-corr} reports the correlation coefficients between
  basis fit parameters that were obtained from the \mtau branching fractions fit.

  %
  %
  %
  \begin{center}
    \begin{envsmall}
      \setlength{\LTcapwidth}{0.85\linewidth}
      \renewcommand*{\arraystretch}{1.3}%
      \ifhevea
        \renewcommand{\bar}[1]{\textoverline{#1}}%
      \else
        \begin{citenoleadsp}
          \fi
          \begin{longtable}{rrrrrrrrrrrrrrr}
            \caption{Correlations (in percent) between basis fit parameters.\label{tab:tau:br-fit-corr}}%
            \\
            \toprule
            \endfirsthead
            \multicolumn{15}{c}{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
            \midrule
            \endhead
            \endfoot
            \endlastfoot
            \dxuse{TauBrBaseQuantCorr}                                                               \\
            \bottomrule
          \end{longtable}
          \ifhevea\else
        \end{citenoleadsp}
      \fi
    \end{envsmall}
  \end{center}
\fi

%
\subsubsection{Equality constraints}
\label{sec:tau:constraints}

The constraints on the \mtau branching-fractions used in the fit are listed in
the following equations.

The equations involve fit parameters associated to \mtau branching fractions,
nuisance fit parameters, external parameters corresponding to non-\mtau
branching fractions (like $\BR_{K_S \to \pi^0\pi^0}$), probabilities
corresponding to squared moduli of amplitudes of quantum state mixtures, such
as $K^0$, $\bar{K}^0$, $K_S$, $K_L$. The probabilities are denoted with, \eg,
$\BR_{<K^0|K_S>} = |{<}K^0|K_S{>}|^2$. The values of all non-\mtau quantities
are taken from the PDG 2022 and 2023 update~\cite{PDG_2022} averages.

\begin{envsmall}
  \setlength\abovedisplayskip{0pt}
  \setlength\belowdisplayshortskip{0pt}
  \ifhevea\renewcommand{\bar}[1]{\textoverline{#1}}\fi
  %
  %
  %
  \dxuse{TauBrConstrEqs}
\end{envsmall}

%
\subsection{Tests of lepton universality}
\cutname{lepton-univ.html}
\label{sec:tau:leptonuniv}

Lepton universality tests probe the Standard-Model prediction that the weak
charged-current interaction has the same coupling for all lepton generations.
Beginning with our 2014 report~\cite{Amhis:2014hma}, the precision of such
tests was significantly improved thanks to the Belle \mtau lifetime
measurement~\cite{Belle:2013teo}. The most significant improvement of the \mtau branching
fraction fit results comes from the recent Belle~II measurement~\cite{Belle-II:2024vvr}.
We perform the universality tests by using
ratios of the partial widths of a heavier lepton $\lepth$ decaying to a lighter
lepton $\leptl$~\cite{Marciano:1988vm},
\begin{align}
  \Gamma(\lepth \to \nu_{\lepth} \leptl \nub_{\leptl} (\gamma)) =
  \frac{\BR(\lepth \to \nu_{\lepth} \leptl \nub_{\leptl})}{\tau_{\lepth}} =
  \frac {G_{\lepth} G_{\leptl} m^5_{\lepth}}{192 \pi^3}\, f\left(\frac {m^2_{\leptl}}{m^2_{\lepth}}\right)
  \radRatio^{\lepth\leptl}_W \radRatio^{\lepth}_\gamma~,
\end{align}
where
\begin{alignat}{3}
  G_{\leptl}                                            & = \frac {g^2_{\leptl}}{4 \sqrt{2} M^2_W}~,                                                 & \quad &   &
  f(x)                                                  & = 1 -8x +8x^3 -x^4 -12x^2 \text{ln}x~,                                                                   \\
  \radRatio^{\lepth\leptl}_W                            & = 1 + \frac {3}{5} \frac {m^2_{\lepth}}{M^2_W} + \frac {9}{5} \frac {m^2_{\leptl}}{M^2_W}~
  \cite{Pich:2013lsa, Ferroglia:2013dga, Fael:2013pja}, & \quad\quad                                                                                 &       &
  \radRatio^{\lepth}_\gamma                             & = 1+\frac {\alpha(m_{\lepth})}{2\pi} \left(\frac {25}{4}-\pi^2\right)~.
\end{alignat}
The equation holds at leading perturbative order (with some corrections being
computed at next-to-leading order) for branching fractions to final states that
include a soft photon, as detailed in the notation. The inclusion of soft
photons is not explicitly mentioned in the branching fractions notation used in
this chapter, but is implicitly assumed, since experimental
measurements do include soft photons. For most measurements of \mtau branching
fractions, soft photons are not experimentally reconstructed but accounted for
in the simulations used to estimate the experimental efficiency. We use
$\radRatio^\tau_\gamma=1-43.2\cdot 10^{-4}$,
$\radRatio^\mu_\gamma=1-42.4\cdot 10^{-4}$~\cite{Marciano:1988vm}
and take the averages for the \mtau mass, lifetime
and branching fractions from this report. We use the CODATA 2018 report~\cite{Tiesinga:2021myr} for the electron and muon masses, and PDG 2022 and 2023 update~\cite{PDG_2022} for the muon lifetime, the $\pi^\pm$ and $K^\pm$ meson masses and lifetimes, and the $W$ boson mass.

Using pure leptonic processes we obtain the coupling ratios
\begin{align}
  \left( \frac{g_\tau}{g_\mu} \right)_\tau = \dxuse{gtaubygmu_tau-vu}~,
  \\
  \left( \frac{g_\tau}{g_e} \right)_\tau  = \dxuse{gtaubyge_tau-vu}~,
  \\
  \left( \frac{g_\mu}{g_e} \right)_\tau  = \dxuse{gmubyge_tau-vu}~.
\end{align}

Under the assumption that the muon and electron charged weak couplings are equal, we average $\BR_e = \BR(\tau \to e \bar{\nu}_e \nu_\tau)$ and its prediction
from $\BR_\mu = \BR(\tau \to \mu\bar{\nu}_\mu\nu_\tau)$,
\begin{align}\label{eq:tau:Be_from_Bmu}
  \BR^{\BR_\mu}_e =
  \BR_\mu
  \frac{f(m_e^2/m_\tau^2)}{f(m_\mu^2/m_\tau^2)}
  \frac{R_W^{\tau e}}{R_W^{\tau \mu}}~,
\end{align}
to obtain $\BR^\prime_e$, a measurement of the \mtau electronic branching
fraction that summarizes the experimental information on the electron
and the muon couplings from the measurements of $B_e$ and $B_\mu$.
%
We test the universality of the couplings of the lighter
leptons with respect to the \mtau by comparing $\BR^\prime_e$ to the
predicted \mtau electronic branching fraction from the measurement of
the \mtau lifetime:
\begin{align}\label{eq:tau:Be_from_taulife}
  \BR^{\tau_\tau}_e =
  \BR(\mu \to e \bar{\nu}_e\nu_\mu) \frac{\tau_\tau}{\tau_\mu}
  \frac{m_\tau^5}{m_\mu^5}
  \frac{f(m_e^2/m_\tau^2)}{f(m_e^2/m_\mu^2)}
  \frac{R_W^{\tau e}}{R_W^{\mu e}}
  \frac{\radRatio^{\tau}_\gamma}{\radRatio^{\mu}_\gamma}~.
\end{align}
In Figure~\ref{fig:tau:lept-univ}, the plot shows the measured
$\BR^\prime_e$, the measured \mtau lifetime, and a band corresponding to
$\BR^{\tau_\tau}_e$ as function of the \mtau lifetime, whose
width depends primarily on the uncertainty on the \mtau mass,
which has been reduced thanks to the recent Belle
measurement~\dxuse{ADACHI 2023C-cite}.

\begin{figure}[tb]
  \begin{center}
    \ifhevea
      \begin{tabular}{@{}cc@{}}
        \larger\bfseries\ahref{tau-lept-univ-2023.png}{PNG format} &
        \larger\bfseries\ahref{tau-lept-univ-2023.pdf}{PDF format}   \\
        \multicolumn{2}{c}{\ahref{tau-lept-univ-2023.png}{%
            \imgsrc[alt="Vus summary plot"]{tau-lept-univ-2023.png}}}
      \end{tabular}
      \else
      {\fboxsep=2pt\fbox{%
          \includegraphics[width=0.50\linewidth,clip]{figures/tau/tau-lept-univ-2023.pdf}}}
    \fi
    \caption{%
      Test of the universality of the couplings of the lighter leptons $e$ and $\mu$, assumed to be the same, and of the \mtau lepton. The plot shows values and uncertainties of the \mtau lifetime and of $\BR^\prime_e$, a determination of the electronic \mtau branching fractions obtained from the direct measurements of the electronic and the muonic \mtau branching fractions. The contour delimits the 68\% CL region. The oblique band shows the Standard Model prediction of $\BR^\prime_e$ as a function of the \mtau lifetime, and its width is mainly determined by the uncertainty on the \mtau
      mass.\label{fig:tau:lept-univ}%
    }
  \end{center}
\end{figure}

An additional universality test is obtained using the measurements of
semileptonic branching fractions of pseudoscalar mesons,
using~\cite{Pich:2013lsa}:
\begin{align}
  \left( \frac{g_\tau}{g_\mu} \right)^2_h =
  \frac{\BR({\tau \to h \nu_\tau})}{\BR({h \to \mu \bar{\nu}_\mu})}
  \frac{2m_h m^2_{\mu}\tau_h}{(1 + \dRradTauhHmu)m^3_{\tau}\tau_{\tau}}
  \left( \frac{1-m^2_{\mu}/m^2_h}{1-m^2_h/m^2_{\tau}} \right)^2~,
\end{align}
where $h$ = $\pi$ or $K$. The radiative corrections $\dRradTaupiPimu$ and $\dRradTaukKmu$ have been recently updated with an improved estimation of
their uncertainties and their values are $(\dxuse{dRrad_tau_pi_by_pimu2-vu})\%$
and $(\dxuse{dRrad_tau_K_by_Kmu2-vu})\%$~\cite{Arroyo-Urena:2021nil}, respectively.
Using $\BR({\pi \to \mu \bar{\nu}_\mu})$ and $\BR({K \to \mu \bar{\nu}_\mu})$ from the Review of Particle Physics 2022 edition and 2023 update~\cite{PDG_2022}, we obtain:
\begin{align}
  \left( \frac{g_\tau}{g_\mu} \right)_\pi & = \dxuse{gtaubygmu_pi-vu}~,
                                          & \left( \frac{g_\tau}{g_\mu} \right)_K = \dxuse{gtaubygmu_K-vu}~.
\end{align}
The largest contribution to the uncertainties of these tests are the uncertainty
on $\dRradTaupiPimu$ for $({g_\tau}/{g_\mu})_\pi$ and the uncertainty on the
\mtau branching fraction for $({g_\tau}/{g_\mu})_K$. Similar tests can be
performed using measurements of decay modes with electrons, but are less
precise, since the meson decays to electrons are helicity suppressed and have
less precise experimental measurements. Averaging the three \(g_\tau/g_\mu\)
ratios we obtain
\begin{align}
  \left( \frac{g_\tau}{g_\mu} \right)_{\tau{+}\pi{+}K} & = \dxuse{gtaubygmu_fit-vu}~,
\end{align}
accounting for correlations and assuming that the $\dRradTaupiPimu$ and
$\dRradTaukKmu$ uncertainties are uncorrelated, as they are estimated to
be with good approximation~\cite{Arroyo-Urena:2021nil}.
Table~\ref{tab:tau:univ-fit-corr} reports the correlation coefficients for the
fitted coupling ratios.
\ifhevea\begin{table}\fi%
  \begin{center}
    \ifhevea
      \caption{Correlation coefficients (\%) of the coupling ratios.\label{tab:tau:univ-fit-corr}}%
    \else
      \begin{minipage}{\linewidth}
        \begin{center}
          \captionof{table}{Universality coupling ratios correlation coefficients (\%).}\label{tab:tau:univ-fit-corr}%
          \fi
          \begin{center}
            \renewcommand*{\arraystretch}{2}%
            \begin{tabular}{lcccc}
              \toprule
              \dxuse{g_ratios_corr}
              \\\bottomrule
            \end{tabular}
          \end{center}
          \ifhevea\else
        \end{center}
      \end{minipage}
    \fi
  \end{center}
  \ifhevea\end{table}\fi
\noindent
Since $(g_\tau/g_\mu)_\tau = (g_\tau/g_e)_\tau / (g_\mu/g_e)_\tau$,
the correlation matrix is expected to be positive semi-definite, with one eigenvalue equal to zero.
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
A numerical calculation of the eigenvalues returns the values
1.804, 1.329, 0.959, 0.907, $2.887\cdot10^{-15}$.
%
%

%
\subsection{\texorpdfstring{%
    Universality-improved values of $\BR(\tau \to e \bar{\nu}_e \nu_\tau)$ and $\Rhad$}{%
    Universality-improved B(tau -> e nu nu\_bar) and Rhad}}
\cutname{Be_univ_and_Rtau.html}
\label{sec:tau:be-univ-rtau}

Following Ref.~\cite{Davier:2005xq}, we compute the experimental value of
$\BR_e = \BR(\tau \to e \bar{\nu}_e \nu_\tau)$ assuming the Standard Model
lepton universality by averaging:
\begin{itemize}

  \item the $\BR_e$ fit value \dxuse{Gamma5-gn},

  \item
  the $\BR_e$ determination from the $\BR_\mu = \BR(\tau \to \mu \bar{\nu}_\mu
    \nu_\tau)$ fit value \dxuse{Gamma3-gn} assuming that $g_\mu/g_e = 1$ (Eq.~\ref{eq:tau:Be_from_Bmu}),

  \item
  the $\BR_e$ determination from the \mtau lifetime assuming that
  $g_\tau/g_\mu =1$ (Eq.~\ref{eq:tau:Be_from_taulife})~.

\end{itemize}
Accounting for correlations, we obtain
\begin{align}
  \BR_e^{\text{uni}} = (\dxuse{Be_univ-vu})\%.
\end{align}

We compute the sum of all {\em measured}
branching fractions to hadrons and the experimental value of the ratio
between the \mtau hadronic and electronic widths assuming the Standard Model
lepton universality:
\begin{align}
  \BR_{\text{had}}   & = (\dxuse{B_tau_had_fit-vu})\%~,
  \\
  \Rhad^{\text{uni}} & =
  \frac{\Gamma(\tau \to \text{hadrons}\, \nu_\tau)}{\Gamma^{\text{uni}}(\tau \to e \bar{\nu}_e \nu_\tau)} =
  \frac{\BR_{\text{had}}}{\BR_e^{\text{uni}}} =
  \dxuse{R_tau-vu}~.
\end{align}
%
An alternative definition of $\BR_{\text{had}}$ uses the unitarity of
the sum of all branching fractions, resulting in:
%
\begin{align}
  \BR_{\text{had}}^{\text{uni, lept}} & = 1 - \BR_e - \BR_\mu =
  (\dxuse{B_tau_had_uni-vu})\%~,
  \\
  \Rhad^{\text{uni, lept}}            & = \frac{1 - \BR_e - \BR_\mu}{\BR_e^{\text{uni}}} =
  \dxuse{R_tau_uni-vu}~.
\end{align}
%
A third definition of $\BR_{\text{had}}$ uses the unitarity of the sum of all
\mtau branching fractions, $1 = \BR_e + \BR_\mu + \BR_{\text{had}}$, the Standard
Model prediction of $\BR_\mu$ from $\BR_e$ in Eq.~\ref{eq:tau:Be_from_Bmu} and
$\BR_e^{\text{uni}}$ to define:
%
\begin{align}
  \BR_{\text{had}}^{\text{uni, SM}} & = 1 - \BR_e^{\text{uni}} -
  \BR_e^{\text{uni}} \cdot f(m^2_\mu/m^2_\tau)/f(m^2_e/m^2_\tau) =
  (\dxuse{B_tau_had_uni_SM-vu})\%~,
  \\
  \Rhad^{\text{uni, SM}}            & = \frac{1 - \BR_e^{\text{uni}} -
    \BR_e^{\text{uni}}\cdot f(m^2_\mu/m^2_\tau)/f(m^2_e/m^2_\tau)}{\BR_e^{\text{uni}}} =
  \dxuse{R_tau_uni_SM-vu}~.
\end{align}
%
Although $\BR_{\text{had}}^{\text{uni, lept}}$ and
$\BR_{\text{had}}^{\text{uni, SM}}$ are more precise than
$\BR_{\text{had}}^{\text{uni}}$, the precision of $\Rhad^{\text{uni, lept}}$
and $\Rhad^{\text{uni, SM}}$ is comparable to the one of
$\Rhad^{\text{uni}}$ because there are larger correlations between
$\BR_{\text{had}}^{\text{uni, lept}}$, $\BR_{\text{had}}^{\text{uni,
      SM}}$ and $\BR_e^{\text{uni}}$ than between $\BR_{\text{had}}$ and
$\BR_e^{\text{uni}}$.

%
\subsection{\texorpdfstring{Measurements of $\Vus$}{Vus measurement}}
\cutname{vus.html}
\label{sec:tau:vus}

The CKM matrix element magnitude \Vus is most precisely determined from kaon
decays~\cite{Antonelli:2010yf} (see Figure~\ref{fig:tau:vus-summary}), and its
precision is limited by the uncertainties of the lattice QCD estimates of the
meson form factor $f_+^{K\pi}(0)$ and decay-constant ratio
$f_{K\pm}/f_{\pi\pm}$.
%
%
%
%
%
%
The following sections report alternative determinations of \Vus based on the experimental measurements of the \mtau branching fractions.
%
%

%
\subsubsection{\texorpdfstring{\Vus from $\BR(\tau \to X_s\nu)$}{Vus from B(tau -> X\_s nu)}}
\label{sec:tau:vus:incl}

\Vus is computed using the inclusive \mtau branching fraction to strange hadronic final states as~\cite{Gamiz:2002nu,Gamiz:2004ar}
\begin{align}\label{eq:Vus-tau-incl}%
  \dxuse{VusTauIncl-OPE-1} & = \sqrt{\Rstrange/\left[\frac{\Rnonstrange}{\Vud^2} -  \deltaRtauSUtb\right]} = \dxuse{Vus_tau_Xs-vu}~,
\end{align}
where $\Rstrange = \BRstrange / \BR_e^{\text{uni}} =
  \dxuse{R_tau_s-vu}$, $\BRstrange = \dxuse{B_tau_s_fit-vu}$ is the
inclusive \mtau branching fraction to strange hadronic final states (see
also Table~\ref{tab:tau:vus}), $\Rnonstrange = \Rhad^{\text{uni}} - \Rstrange =
  \dxuse{R_tau_VA-vu}$, and $\Vud = \dxuse{Vud-vu}$ is taken from a recent
average of measurements of superallowed nuclear $\beta$ decays, neutron
decay measurements~\cite{Cirigliano:2022yyo}, and the correction
\deltaRtauSUtb accounts for the $SU(3)$-breaking effects due to the
difference between the strange, up and down quark masses. \deltaRtauSUtb
is determined using perturbative QCD and experimental low energy
scattering measurements~\cite{Gamiz:2006xx,Gamiz:2007qs,Maltman:2010hb}.
In this report, we compute $\deltaRtauSUtb = \dxuse{deltaR_su3break-vu}$
using Ref.~\cite{Gamiz:2006xx} and the $s$-quark mass $m_s =
  \dxuse{m_s-vu}\,\mev$~\cite{PDG_2022}. Ref.~\cite{Gamiz:2006xx}
estimates a \deltaRtauSUtb uncertainty that is intermediate with respect
to the other two assessments~\cite{Gamiz:2007qs,Maltman:2010hb}. The
uncertainty on \deltaRtauSUtb contributes a \dxuse{Vus_tau_Xs_unc_th_perc-v}\% systematic contribution on \dxuse{VusTauIncl-OPE-1}.
The above-mentioned
\deltaRtauSUtb calculations have been criticized for falling short in
dealing with the biases and uncertainties in the low-energy regime of
QCD~\cite{Hudspith:2017vew}. However, the community has not reached yet
a consensus on the matter. In order to obtain more reliable QCD
uncertainties, alternative procedures for computing \Vus using \mtau
decays have been proposed, which involve the \mtau spectral
functions~\cite{Hudspith:2017vew} and lattice QCD
methods~\cite{Boyle:2018dwv}.
Because of the complexity of these two last proposed
procedures, the effort that is required to use them to compute \Vus
using the current \hflavtau branching fractions exceeds the scope
of this report. Therefore, we just report the most recent
updates:
\begin{align}
  \dxuse{VusTauIncl-OPE-2}     & = 0.2219(22)\quad\cite{Maltman:2015xwa, Maltman:2019xeh} \\
  \dxuse{VusTauIncl-latt-disp} & = 0.2240(18)\quad\cite{Boyle:2018dwv, Maltman:2019xeh}
\end{align}
We also use a recently reported lattice QCD calculation of the inclusive
\mtau hadronic decay rate~\cite{ExtendedTwistedMass:2024myu} to compute an additional determination of \Vus,
\begin{align}\label{eq:Vus-tau-incl-latt-incl}%
  \dxuse{VusTauIncl-latt-incl} & =
  \sqrt{
    \left(\frac{\Vus^2}{\Rstrange}\right)_{\text{latt-incl}} 
    \cdot \Rstrange
  } = \dxuse{Vus_tau_Xs_latt_incl-vu}~,
\end{align}
where $(\Rstrange / \Vus^2)_{\text{latt-incl}} = 
  \dxuse{R_tau_us_by_Vus_sq-vu}$~\cite{ExtendedTwistedMass:2024myu}. It is
worth noting that all calculations of the \mtau inclusive decay
rate to hadrons are not presently including the long-distance
isospin-breaking corrections~\cite{ExtendedTwistedMass:2024myu}.

In several of the past determinations of \Vus, such as the 2009 HFLAV
report~\cite{Asner:2010qj}, the total hadronic branching fraction was
computed using unitarity as $\BRhad^{\text{uni}} = 1 - \BR_e -\BR_\mu$,
and $\BRnonstrange$ was obtained from $\BRhad^{\text{uni}} -
\BRstrange$. Here we rather use the direct experimental determination of
$\BRnonstrange$ for two reasons. First, both methods result in
comparable uncertainties on \Vus, since the better precision on
$\BRhad^{\text{uni}} = 1 - \BR_e -\BR_\mu$ with respect to $\BRhad$
equal to the sum of all \mtau hadronic branching fractions is offset by
increased correlations when considering $\Rhad^{\text{uni}} =
\BRhad/\BR_e^{\text{uni}}$ and similar expressions in the \Vus
calculation. Second, if there are unobserved \mtau hadronic decay modes,
they will affect \BRnonstrange and \BRstrange in a more asymmetric way
when using $\BRhad^{\text{uni}}$.

The values of \dxuse{VusTauIncl-OPE-1} and \dxuse{VusTauIncl-latt-incl}
are respectively $\dxuse{Vus_tau_Xs_mism_sigma_abs-vu}\sigma$ and $\dxuse{Vus_tau_Xs_latt_incl_mism_sigma_abs-vu}\sigma$ lower than the value
$\VusUni = \dxuse{Vus_uni-vu}$ predicted from the CKM unitarity relation
$(\VusUni)^2 = 1 - \Vud^2 - \Vub^2$, with
$\Vub = \dxuse{Vub-vu}$~\cite{PDG_2022}.
Using Eqs.~\ref{eq:Vus-tau-incl} and \ref{eq:Vus-tau-incl-latt-incl} we also compute
$\dxuse{VusTauInclbyVud-OPE-1} = \dxuse{Vus_by_Vud_tau_Xs-vu}$ and
$\dxuse{VusTauInclbyVud-latt-incl} = \dxuse{Vus_by_Vud_tau_Xs_latt_incl-vu}$.
\iffalse
  The 2018 \babar preliminary results improved the \Vus precision by
  about 10\% and reduced the discrepancy by about 6.5\%.
\fi

%
%
%
\begin{table}
  \begin{center}
    \renewcommand*{\arraystretch}{1.3}%
    \caption{A summary of the averaged \mtau branching fractions to strange final states.\label{tab:tau:vus}}%
    \ifhevea\renewcommand{\bar}[1]{\textoverline{#1}}\fi
    \begin{envsmall}
      \begin{center}
        \begin{tabular}{lc}
          \toprule
          \multicolumn{1}{l}{\bfseries Branching fraction} &
          \multicolumn{1}{c}{\bfseries HFLAV \hflavTauTag fit (\%)} \\
          \midrule
          \dxuse{TauBrStrangeVal}
          \\[-2.5ex]
          \dxuse{TauBrStrangeTotVal}
          \bottomrule
        \end{tabular}
      \end{center}
    \end{envsmall}
  \end{center}
\end{table}

%
%
%
\subsubsection{\texorpdfstring{%
    \Vus from $\BR(\tau \to K\nu) / \BR(\tau \to \pi\nu)$}{%
    Vus from B(tau -> K nu) / B(tau -> pi nu)}}
\label{sec:tau:vus:taukpi}
%
%

We also compute $\Vus/\Vud$ from the ratio of branching fractions
$\dxuse{Gamma10by9-gn} = \dxuse{Gamma10-td} / \dxuse{Gamma9-td} =
  \dxuse{Gamma10by9-vu}$ (Table \ref{tab:tau:br-var-meas}) using the
equation~\cite{Banerjee:2008hg}:
\begin{align}
  \frac{\dxuse{Gamma10-td}}{\dxuse{Gamma9-td}} & =
  \frac{f_{K\pm}^2 \Vus^2}{f_{\pi\pm}^2 \Vud^2}
  \frac{\left( m_\tau^2 - m_K^2 \right)^2}{\left( m_\tau^2 -  m_\pi^2 \right)^2}
  (1+\delta_{\tau K/\tau\pi})~,
\end{align}
where $\delta_{\tau K/\tau\pi} = (\dxuse{dRrad_tau_K_by_tau_pi-vu})\%$~\cite{Arroyo-Urena:2021nil} is the radiative correction for the ratio of partial widths $\Gamma(\tau\to K\nu_\tau [\gamma]) / \Gamma(\tau\to \pi\nu_\tau [\gamma])$.
Using the ratio of decay
constants $f_{K\pm}/f_{\pi\pm} = \dxuse{f_Kpm_by_f_pipm-vu}$ from the 2023 web update of the FLAG 2021
lattice QCD averages with $N_f=2{+}1{+}1$~\cite{Aoki:2021kgd,
  FLAG-2021-web-update-mar23, ExtendedTwistedMass:2021qui, Miller:2020xhy,
  Dowdall:2013rya, etm:2015lqcd, Bazavov:2017lyh}, we obtain $\Vus/\Vud = \dxuse{Vus_by_Vud_tau_K_by_tau_pi-vu}$.
By using the above-mentioned \Vud value, we compute $\VusTauKpi =
  \dxuse{Vus_tau_K_by_tau_pi-vu}$, which is
$\dxuse{Vus_tau_K_by_tau_pi_mism_sigma_abs-vu}\sigma$ below the CKM unitarity
prediction.

%
%
%
\subsubsection{\texorpdfstring{%
    \Vus from $\BR(\tau \to K\nu)$}{%
    Vus from B(tau -> K nu)}}
\label{sec:tau:vus:tauk}
%
We also determine \Vus from the branching fraction $\BFtautoknu$ using
\begin{align}
  \BR(\tau^- \to K^-\nu_\tau) =
  \frac{G^2_F}{16\pi\hslash} f^2_{K\pm} \Vus^2 \tau_{\tau}  m_{\tau}^3
  \left(1 - \frac{m_K^2}{m_\tau^2}\right)^2
  S_{\text{EW}}^{\tau h}
  (1+\delta_{\tau K})~.
\end{align}
We use $f_{K\pm} = \dxuse{f_Kpm-vu}\,\mev$ from the 2023 web update of the FLAG 2021 lattice
QCD averages with $N_f=2{+}1{+}1$~\cite{Aoki:2021kgd,
  FLAG-2021-web-update-mar23, ExtendedTwistedMass:2021qui,
  Dowdall:2013rya, Bazavov:2014wgs, etm:2015lqcd}.
The universal
short-distance electroweak correction for \mtau hadronic decays is
$S_{\text{EW}}^{\tau h} = S_{\text{EW}}^{R\tau h} \cdot
  S_{\text{EW}}^{\text{sub,lep}} = \dxuse{S_EW_tau_h-vu}$, where the radiative
correction for the tau spectral functions is
$S_{\text{EW}}^{R\tau h} = \dxuse{S_EW_R_tau_h-vu}$~\cite{Davier:2002dy,
  Pich:2013lsa, Davier:2023fpl} and the sub-leading universal short-distance correction for the
\mtau leptonic decays is $S_{EW}^{\text{sub,lep}} =
  \dxuse{S_EW_tau_sub_lep-v}$~\cite{Davier:2002dy}.
The long-distance radiative correction for $\BFtautoknu$ is
$\delta_{\tau K} = (\dxuse{dRrad_tau_K-vu})\%$~\cite{Arroyo-Urena:2021nil}.
The physical constants $G_F$ and $\hslash$ are taken from CODATA 2018~\cite{Tiesinga:2021myr}.
We obtain $\VusTauKnu = \dxuse{Vus_tau_K-vu}$,
which is $\dxuse{Vus_tau_K_mism_sigma_abs-vu}\sigma$ below
the CKM unitarity prediction.

%
%
%
\subsubsection{\texorpdfstring{Summary of \Vus from \mtau decays}{Summary of Vus from tau decays}}

\begin{figure}[tb]
  \begin{center}
    \ifhevea
      \begin{tabular}{@{}cc@{}}
        \larger\bfseries\ahref{vus-tau-hflav.png}{PNG format} &
        \larger\bfseries\ahref{vus-tau-hflav.pdf}{PDF format}   \\
        \multicolumn{2}{c}{\ahref{vus-tau-hflav.png}{%
            \imgsrc[alt="Vus summary plot"]{vus-tau-hflav.png}}}
      \end{tabular}
      \else
      {\fboxsep=2pt\fbox{%
          \includegraphics[width=0.50\linewidth,clip]{figures/tau/vus-tau-hflav.pdf}}}
    \fi
    \caption{\Vus determinations. The values of $\Vus_{K\ell3}$,
      $\Vus_{K\ell2}$ and the expected \Vus from the CKM matrix unitarity are taked from Ref.~\cite{Cirigliano:2022yyo}. The other reported \Vus values are documented in the text. When two uncertainties are reported, the first one accounts for the uncertainties of the \hflavtau fit results, and the second one accounts for the uncertainties of the theory and the other inputs that are used for the \Vus determinations.%
      \label{fig:tau:vus-summary}%
    }
  \end{center}
\end{figure}

We summarize the \Vus determinations that we updated using the present
\hflavtau averages by reporting the values, the discrepancy with
respect to the \Vus determination from CKM unitarity, and an
illustration of the measurement method:
\begin{alignat}{6}
  %
  \label{eq:VusTauUni}%
   & \VusUni                                                    &  & = \dxuse{Vus_uni-v}              &  & \pm \dxuse{Vus_uni-u}              & \quad & 0.0\sigma                                            & \quad
   & [\sqrt{1 - \Vud^2 - \Vub^2} \quad\text{(CKM unitarity)}]~,                                                                                                                                                      \\
  %
  \label{eq:VusTauKl3}%
   & \Vus_{K\ell3}                                              &  & = \dxuse{Vus_Kl3-v}              &  & \pm \dxuse{Vus_Kl3-u}              & \quad & \dxuse{Vus_Kl3_mism_sigma_abs-vu}\sigma              & \quad
   & [\BR_{K\ell3}~\cite{Cirigliano:2022yyo}]~,                                                                                                                                                                      \\
  \label{eq:VusTauKl2}%
   & \Vus_{K\ell2}                                              &  & = \dxuse{Vus_Kl2-v}              &  & \pm \dxuse{Vus_Kl2-u}              & \quad & \dxuse{Vus_Kl2_mism_sigma_abs-vu}\sigma              & \quad
   & [\BR_{K\ell2}~\cite{Cirigliano:2022yyo}]~,                                                                                                                                                                      \\
  %
  \label{eq:VusTauXs}%
   & \dxuse{VusTauIncl-OPE-1}                                   &  & = \dxuse{Vus_tau_Xs-v}           &  & \pm \dxuse{Vus_tau_Xs-u}           & \quad & \dxuse{Vus_tau_Xs_mism_sigma_abs-vu}\sigma           &
   & [\BR(\tau^- \to X_s^- \nut)]~,                                                                                                                                                                                  \\
  %
  \label{eq:VusTauXs_latt_incl}%
   & \dxuse{VusTauIncl-latt-incl}                               &  & = \dxuse{Vus_tau_Xs_latt_incl-v} &  & \pm \dxuse{Vus_tau_Xs_latt_incl-u} & \quad & \dxuse{Vus_tau_Xs_latt_incl_mism_sigma_abs-vu}\sigma &
   & [\BR(\tau^- \to X_s^- \nut)]~,                                                                                                                                                                                  \\
  %
  \label{eq:VusTauKpi}%
   & \VusTauKpi                                                 &  & = \dxuse{Vus_tau_K_by_tau_pi-v}  &  & \pm \dxuse{Vus_tau_K_by_tau_pi-u}  & \quad & \dxuse{Vus_tau_K_by_tau_pi_mism_sigma_abs-vu}\sigma  &
   & [\BR(\tauknu)/\BR(\taupinu)]~,                                                                                                                                                                                  \\
  %
  \label{eq:VusTauKnu}%
   & \VusTauKnu                                                 &  & = \dxuse{Vus_tau_K-v}            &  & \pm \dxuse{Vus_tau_K-u}            & \quad & \dxuse{Vus_tau_K_mism_sigma_abs-vu}\sigma            &
   & [\BR(\tauknu)]~.
\end{alignat}
%
Averaging the two \Vus determinations that rely on exclusive \mtau branching
fractions (Eqs.~\ref{eq:VusTauKpi}, \ref{eq:VusTauKnu}), we obtain:
\begin{alignat}{6}
   & \Vus_{\tau\text{ excl}}                                                 &  & = \dxuse{Vus_tau_excl-vu} & \quad & \dxuse{Vus_tau_excl_mism_sigma_abs-vu}\sigma \quad
   & [\text{average of \mtau exclusive measurements}]~.\label{eq:VusTauExcl}
\end{alignat}
%
Averaging the \mtau inclusive and exclusive \Vus determinations
(Eqs.~\ref{eq:VusTauXs}, \ref{eq:VusTauXs_latt_incl},
\ref{eq:VusTauKpi}, \ref{eq:VusTauKnu}), we obtain:
\begin{alignat}{6}
   & \Vus_\tau                                                        &  & = \dxuse{Vus_tau-vu} & \quad & \dxuse{Vus_tau_mism_sigma_abs-vu}\sigma \quad
   & [\text{average of 4 \Vus \mtau measurements}]~.\label{eq:VusTau}
\end{alignat}
In calculating the averages,
all correlations arising from using the \mtau branching fractions fit results and common external inputs are accounted for.
The systematic uncertainties of \dxuse{VusTauIncl-OPE-1} and \dxuse{VusTauIncl-latt-incl} have been assumed to be uncorrelated.
The correlation between $f_{K\pm}$ and
$f_{K\pm}/f_{\pi\pm}$ is conservatively set to 100\%.
For the purpose of estimating the correlations between $\delta_{\tau K}$,
$\delta_{\tau\pi}$ and $\delta_{\tau K/\tau\pi}$, we use the
information~\cite{Arroyo-Urena:2021nil} that the uncertainties on $\delta
  _{\tau K}$ and $\delta_{\tau\pi}$ are uncorrelated to a good approximation,
and that $\delta_{\tau K/\tau\pi} = \delta_{\tau K} - \delta_{\tau\pi}$.

All \Vus determinations based on measured \mtau branching fractions are lower
than both the kaon and the CKM-unitarity determinations. This is correlated
with the fact that the direct measurements of the three largest \mtau branching
fractions to kaons [$\dxuse{Gamma10-td}$, $\dxuse{Gamma16-td}$ and
    $\dxuse{Gamma35-td}$] yield lower values than their SM predictions based on the
branching fractions of leptonic kaon decays~\cite{Pich:2013lsa, Jamin:2008qg,
  Antonelli:2013usa}.

Figure~\ref{fig:tau:vus-summary} reports our \Vus determinations using
the present \hflavtau averages, two additional \Vus determinations
using partially different \mtau measurements
inputs~\cite{Maltman:2015xwa, Boyle:2018dwv, Maltman:2019xeh}, two
determinations based on kaon data~\cite{Cirigliano:2022yyo}, and the
\Vus value obtained from \Vud using the CKM-matrix
unitarity~\cite{Cirigliano:2022yyo}.


==> tau/tau_all_common.tex <==
%

%
%
%

%
%
%

\ifhevea\else
\makeatletter
\let\citeSaveTau\cite
\let\bfseriesSaveTau\bfseries
\let\LT@makecaptionSaveTau\LT@makecaption
\makeatother

%
\renewcommand{\cite}[1]{\ifmmode\text{\citeSaveTau{#1}}\else\citeSaveTau{#1}\fi}

%
\makeatletter
\DeclareRobustCommand\bfseries{%
  \not@math@alphabet\bfseries\mathbf
  \fontseries\bfdefault\selectfont\boldmath}
\DeclareRobustCommand*{\bm}[1]{%
    \mathchoice{\bmbox{\displaystyle}{#1}}%
               {\bmbox{\textstyle}{#1}}%
               {\bmbox{\scriptstyle}{#1}}%
               {\bmbox{\scriptscriptstyle}{#1}}}
\DeclareRobustCommand*{\bmbox}[2]{\mbox{\bfseries$#1 #2$}}
\makeatother

%
\makeatletter
\def\LT@makecaption#1#2#3{%
  \LT@mcol\LT@cols c{\hbox to\z@{\hss\parbox[t]\LTcapwidth{%
    \sbox\@tempboxa{\normalsize#1{#2: }#3}%
    \ifdim\wd\@tempboxa>\hsize
      \normalsize#1{#2: }#3%
    \else
      \hbox to\hsize{\hfil\box\@tempboxa\hfil}%
    \fi
    \endgraf\vskip\baselineskip}%
  \hss}}}
\makeatother

\begin{fleqn}
\fi
%
%
%
\ifhevea
\input{tau-sections}
\input{tau-lfv-combs}
%
%
\input{tau-lfv-limits-combs-plot}
\else
\input{tau/tau-sections}
\input{tau/tau-lfv-combs}
%
%
\input{tau/tau-lfv-limits-combs-plot}
\fi
%
%
%
\ifhevea\else
\end{fleqn}

\makeatletter
\let\cite\citeSaveTau
\let\bfseries\bfseriesSaveTau
\let\LT@makecaption\LT@makecaptionSaveTau
\makeatother
\fi

